Undirected $(1+\varepsilon)$-Shortest Paths via Minor-Aggregates: Near-Optimal Deterministic Parallel & Distributed Algorithms

This paper presents near-optimal deterministic parallel and distributed algorithms for computing $(1+\varepsilon)$-approximate single-source shortest paths in any undirected weighted graph. On a high level, we deterministically reduce this and other shortest-path problems to $\tilde{O}(1)$ Minor-Aggregations. A Minor-Aggregation computes an aggregate (e.g., max or sum) of node-values for every connected component of some subgraph. Our reduction immediately implies: Optimal deterministic parallel (PRAM) algorithms with $\tilde{O}(1)$ depth and near-linear work. Universally-optimal deterministic distributed (CONGEST) algorithms, whenever deterministic Minor-Aggregate algorithms exist. For example, an optimal $\tilde{O}(HopDiameter(G))$-round deterministic CONGEST algorithm for excluded-minor networks. Several novel tools developed for the above results are interesting in their own right: A local iterative approach for reducing shortest path computations "up to distance $D$" to computing low-diameter decompositions "up to distance $\frac{D}{2}$". Compared to the recursive vertex-reduction approach of [Li20], our approach is simpler, suitable for distributed algorithms, and eliminates many derandomization barriers. A simple graph-based $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing based on low-diameter decompositions that can be evaluated in near-linear work. The previous such routing [ZGY+20] was $n^{o(1)}$-competitive and required $n^{o(1)}$ more work. A deterministic algorithm to round any fractional single-source transshipment flow into an integral tree solution. The first distributed algorithms for computing Eulerian orientations.

==> Deterministic_SSSP/TS-and-Boosting.tex <==


\section{Transshipment Boosting via Multiplicative Weights}\label{sec:boosting}

 % theorem 1.5
% Theorem 1.5. (Distributed oblivious routing evaluation). Let G = (V, E) be a weighted graph with weights in [1, n O(1) ]. There exists an exp(O(log n · log log n) 3/4 )-approximate ` 1 -oblivious routing R such that we can perform the following computations in exp(O(log n · log log n) 3/4 ) rounds of Minor-Aggregation. Given any distributedly stored node vector d ∈ R n and edge vector c ∈ R n , we can evaluate and distributedly store Rd ∈ R m and R T c ∈ R n


  % Let $R$ be an $\alpha$-approximate $\ell_1$-oblivious routing with respect to a transshipment instance on a weighted graph $G$. Suppose we can compute matrix-vector products with $R$ and $R^T$ in $M$ Minor-Aggregation rounds. Then we can compute and distributedly store a flow $f \in \R^m$ and a \emph{vector of potentials} $\phi$ in $\tilde{O}(\alpha^2\eps^{-2}M)$ rounds such that
  % \begin{enumerate}
  % \item $\norm{Wf}_1 \trleq (1+\eps)d^{\top} \phi \leq (1+\eps) \norm{d}_{\opt}$;
  % \item $\norm{Bf - d}_{\opt} \leq \eps \norm{d}_{\opt}$;
  % \item $\norm{W^{-1} B^T \phi}_\infty \le 1$.
  % \end{enumerate}


\begin{lemma}
\label{lem:transshipment_primal_dual}
Let $R \in \R^{V \times \vec{E}}$ be an $\alpha$-approximate $\ell_1$-oblivious routing on a weighted graph $H = (V, E)$ with weight vector $\ell \in \R^E$, let $b \in \R^V$ be a demand vector with $\sum_{v \in V} b_v = 0$, and let $0 < \eps < 1/2$. Suppose we can compute matrix-vector products with $R$ and $R^T$ in $M$ \aggregate rounds. Then, in $\eps^{-2}\poly(\alpha, M, \log n)$ \aggregate rounds, we can compute a flow $f \in \R^{\vec{E}}$ that satisfies the demand $b$, and a vector of potentials $\phi$ such that $\ell(f) \le (1+\eps)b^T\phi$.
\end{lemma}
\begin{proof}
  Lemma 6.1 of \cite{goranci2022universally} proves there exist a $\tilde{O}(\alpha^2 \eps^{-2} M)$ \aggregate round algorithm that computes a flow $f' \in \R^{\vec{E}}$ and potentials $\phi' \in \R^{V}$ satisfying (1) $\ell(f') \le (1 + \eps) b^T \phi \le (1 + \eps) \norm{b}_\opt$ , and (2) flow $f'$ satisfies a potentially different demand $b'$ with the guarantee $\norm{b - b'}_\opt \le \eps \norm{b}_\opt$ (i.e., that one can near-optimally route the difference). This nearly matches our required guarantees with the exception that we require our final flow $f$ to perfectly satisfy the guarantees.

  For future reference, we show that $\norm{b}_\opt \le (1 + 5 \eps) b^T \phi$. First, there exists a flow $f_2^*$ that satisfies $b'$ of $\ell(f_2^*) \le \norm{b'}_\opt \le \eps \norm{b}_\opt$. Since $f' + f_2^*$ satisfies $b$, we have that $\norm{b}_\opt \le \ell(f') + \ell(f_2^*) \le (1 + \eps) b^T \phi + \eps \norm{b}_\opt$. Therefore, $(1 - \eps) \norm{b}_\opt \le (1 + \eps) b^T \phi$, or $\norm{b}_\opt \le (1 + 5 \eps) b^T \phi$.

  To fix $f$, we can simply call the above procedure with an enhanced guarantee of $\eps' := \eps / \alpha$, guaranteeing $\norm{b - b'}_\opt \le \frac{\eps}{\alpha} \norm{b}_\opt$. Then, utilizing the $\alpha$-competitive oblivious routing $R$, we compute $f'' := R(b - b')$ which satisfies $\ell(f'') \le \alpha \norm{b - b'}_\opt \le \alpha \frac{\eps}{\alpha} \norm{b}_\opt = \eps \norm{b}_\opt$. Therefore, the flow $f' + f''$ (perfectly) satisfies $(b - b') + b' = b$ and has cost $\ell(f' + f'') \le \ell(f') + \ell(f'') \le (1 + \eps)b^T \phi + \eps \norm{b}_\opt \le (1 + \eps)b^T \phi + \eps (1 + 5 \eps) b^T \phi \le (1 + 5 \eps) b^T \phi$. Reducing $\eps$ by a factor of $5$ gives the final result.
\end{proof}


\begin{restatable}[Boosting + Rounding]{theorem}{boosting}
\label{theorem:boosting_rounding}
Let $R$ be an $\alpha$-approximate $\ell_1$-oblivious routing on a weighted graph $H$ and $s \in V(H)$ be arbitrary. For a given $\eps \in (0,1]$, one can compute:
\begin{itemize}
  \item A potential $\phi$ with $\phi(s) = 0$. 
  \item A tree $T$ rooted at $s$ such that for each $v \in V(H)$ we have that $\dist_T(v) \le (1 + \eps) \phi(v)$.    
  \end{itemize}
  The computation runs in $\tilde{O}(\poly(\alpha)\eps^{-2})$ \aggregate rounds in $H$, together with $\tilde{O}(\poly(\alpha)\eps^{-2})$ many computations of matrix-vector products with $R$ and $R^T$ and $\poly(\log n)$ oracle calls to $\oRound_{\eps / 2}$.
\end{restatable}
  The main ideas of the solution to this task were mostly presented as the Algorithm SSSPTree of \cite{haeuplerLi2018sssp}. We adapt the ideas from this and describe them here for completeness.
\begin{proof}

%  Initially, let $b \in \R^V$ be a demand with $b(s) \gets -(n-1)$ and $b(v) \gets 1$ for all $v \neq s$. 

First we present a procedure with $k = O(\log n)$ phases that in each phase constructs a tree-potential pair $\phi_i, T_i$ by invoking \cref{lem:transshipment_primal_dual}. 
During this procedure, we maintain a set of \emph{unhappy} nodes $V_i$. 
At the beginning, $V_i = V \setminus \{s\}$. 
A node $v \in V_i$ becomes happy in a phase $i$ if $d_{T_i}(s, v) \le (1+\eps)\phi_i(v)$. 
Let us moreover define $\zeta_i = \sum_{v \in V_i} \dist(s, v)$. 

We now describe the procedure in a greater detail and prove that $\zeta_i$ decreases by a constant factor every phase, hence after $ k = O(\log n)$ phases $\zeta_k  = 0$ and every node is happy. 
In each phase, we invoke \cref{lem:transshipment_primal_dual} with our $\ell_1$-oblivious routing $R$ and a demand $b(s) = -|V_i|$ and $b(v) = 1$ for all $v \in V_i$. 
 \Cref{lem:transshipment_primal_dual} returns a flow $f_i$ and a potential $\phi_i$ with $\ell(f_i) \le (1 + \frac{\eps}{10}) b^T \phi_i$; suppose that (by translation) $\phi_i(s) = 0$. 
 Using the rounding oracle $\oRound_{G, \eps/2}$ we round $f$ to a tree $T$ satisfying $\sum_{v, b(v) \neq 0} b(v) \dist_{T_i}(s, v) \le (1 + \frac{\eps}{2}) \ell(f_i)$. 
    Hence, have
  \begin{align}
  \label{eq:sss}
    \sum_{v \in V_i} \dist_{T_i}(s, v) 
    \le \left( 1 + \frac{\eps}{2}\right) \ell(f) 
    \le \left( 1 + \frac{\eps}{2} \right) \left( 1 + \frac{\eps}{10} \right) b^T \phi_i 
    \le \left( 1 + \frac{2}{3} \eps \right) \sum_{v \in V_i} \phi_i(v).  
  \end{align}
 
 %Note that the distances in $T$ are good on average, but not individually good. We use the following procedure to correct this issue.
Let $U_i \subseteq V_i$ be the set of nodes $v$ that become happy in phase $i$, that is, $v \in U_i$ if  $\dist_{T_i}(s, v) \le (1+\eps)\phi_i(v)$. 
  We can compute the root-to-$v$ distances in $T_i$ with the ancestor sum operation (\Cref{lemma:ancestor-subtree-sum}) in $\tilde{O}(1)$ \aggregate rounds. 
  Therefore, we can check for each node $v \in V_i$ whether $v \in U_i$ or not and define $V_{i+1} = V_i \setminus U_i$. 

  Since $\phi_i$ is a potential, we have $ \sum_{v\in U_i} \phi_i(v) \le \sum_{v \in U_i} \dist_{T_i}(s, v) $ and by definition $(1+\eps)\sum_{v\in V_i \setminus U_i} \phi_i(v) \le \sum_{v \in V_i \setminus U_i} \dist_{T_i}(s, v)$. 
  Together with above inequality we get
  \begin{align*}
      \sum_{v \in U_i} \phi_i(v) + \left( 1 +\eps \right)\sum_{v \in V_i \setminus U_i} \phi_i(v) \le \left( 1 + 2\eps/3 \right) \sum_{v \in V_i} \phi_i(v),
  \end{align*}
  hence
  \begin{align*}
   \eps \sum_{v \in V_i \setminus U_i} \phi_i(v) \le 2\eps/3 \sum_{v \in V_i} \phi_i(v) 
  \end{align*}
  or
  \begin{align}
  \label{eq:psss}
   \sum_{v \in U_i} \phi_i(v) \ge \sum_{v \in V_i} \phi_i(v)/3.  
  \end{align}
  
    Hence, we have 
    \begin{align*}
        \zeta_{i} - \zeta_{i+1}
        &= \sum_{v \in U_i} \dist(s, v)
        \ge \sum_{v \in U_i} \phi_i(v) && \text{$\phi_i$ is a potential} \\
        &\ge \sum_{v \in V_i} \phi_i(v)/3 &&  \text{Eq. \cref{eq:psss}}\\
        &\ge \sum_{v \in V_i} \dist_{T_i}(s, v)/4 &&  \text{Eq. \cref{eq:sss}}\\
        &\ge  \sum_{v \in V_i} \dist(s, v)/4
        = \zeta_i / 4 
    \end{align*}
  
Hence, after $k = O(\log n)$ phases $\zeta_k = 0$ and every node is happy. 

 Next, we use potentials $\phi_1, \ldots, \phi_k$ and trees $T_1, \ldots, T_k$ to construct a common potential $\phi$ and tree $T$ that we output. 
 First, we construct a common potential $\phi \in \R^V$ by $\phi(v) = \max_{i=1}^k \phi_i(v)$. 
 Note that $\phi$ is potential by \cref{fact:potential_min_max} and if $v$ got happy in the $i$-th phase, we have $d_{T_i}(s, v) \le (1+\eps)\phi(v)$. 

Second, we construct a common tree $T$ by letting each node maintain its $T$-\emph{parent} and a \emph{distance label} which is an upper bound on the distance to the root in $T$. First, direct all trees $T_i$ from the root to the leafs using \Cref{lemma:ancestor-subtree-sum}. 
Then, set $T := T_1$ (by copying the parent pointers) and initialize the distance label of $v$ with $\dist_{T_i}(s, v)$. Then, we process $T_2, T_3, \ldots, T_k$ one-by-one. Each node $v$ considers whether the distance label of the $T_i$-parent plus the weight of the $T_i$-parent-edge is smaller than the current distance label. If yes, its sets its parent pointer to its $T_i$-parent and updates the distance label. After processing all $T_i$, the parent pointers characterize the tree $T$. Furthermore, it is easy to show that the distance label for a node $v$ is upper bounded by $\min_{i=1}^k \dist_{T_i}(s, v)$, hence every node $v$ satisfies $\dist_{T}(s, v) \le (1+\eps)\phi(v)$. 
\end{proof}


==> Deterministic_SSSP/abstract.tex <==
\begin{abstract}
\noindent This paper presents near-optimal deterministic parallel and distributed algorithms for computing $(1+\eps)$-approximate single-source shortest paths in any undirected weighted graph.
\medskip

\noindent On a high level, we deterministically reduce this and other shortest-path problems to $\tO(1)$ \footnote{We use $\tO$-notation to suppress polylogarthmic factors in the number of nodes $n$, e.g., $\tO(m) = m \log^{O(1)} n$. We use the term near-linear to mean $\tO(m)$.} Minor-Aggregations. 
A Minor-Aggregation computes an aggregate (e.g., max or sum) of node-values for every connected component of some subgraph.

\medskip


\noindent Our reduction immediately implies:
\begin{itemize}
    \item Optimal deterministic parallel (\pram) algorithms with $\tO(1)$ depth and near-linear work.
    \item Universally-optimal deterministic distributed (\congest) algorithms, whenever deterministic Minor-Aggregate algorithms exist. For example, an optimal $\tO(\hopDiameter{G})$-round deterministic \congest algorithm for excluded-minor networks.
\end{itemize}

\medskip

\noindent Several novel tools developed for the above results are interesting in their own right:

\begin{itemize}
    \item A local iterative approach for reducing shortest path computations ``up to distance $D$'' to computing low-diameter decompositions  ``up to distance $\frac{D}{2}$''. Compared to the recursive vertex-reduction approach of \cite{Li20}, our approach is simpler, suitable for distributed algorithms, and eliminates many derandomization barriers.
    \item A simple graph-based $\tO(1)$-competitive $\ell_1$-oblivious routing based on low-diameter decompositions that can be evaluated in near-linear work. The previous such routing~\cite{goranci2022universally} was $n^{o(1)}$-competitive and required $n^{o(1)}$ more work.   

    \item A deterministic algorithm to round any fractional single-source transshipment flow into an integral tree solution. 

    \item The first distributed algorithms for computing Eulerian orientations. 
\end{itemize}

\smallskip


\end{abstract}






==> Deterministic_SSSP/algorithm-main.tex <==

\section{SSSP via Minor-Aggregations: A Local Iterative Reduction Cycle}
\label{sec:localiterative}



In \cref{sec:intro} and \cref{fig:main}, we gave an idealized and informal description of our algorithm.
The real set of reductions our algorithm is built on is not quite the perfect cycle from \cref{fig:main}, but instead it looks like \cref{fig:oracles}. 
In \cref{sec:key_definitions}, we give a formal definition for each part of this new ``cycle'' and explain how the parts of the new cycle correspond to parts in the old cycle. 
Once we have defined each part of the new cycle, each arrow in \cref{fig:oracles} corresponds to a formal statement.
These formal statements can be found in \cref{sec:implications_cycle}, along with informal explanations how the statements can be proven. \\
Finally, \cref{sec:main_theorems} contains statements of our main theorems together with simple proof sketches.
The formal proofs for all the results stated in \cref{sec:implications_cycle} and \cref{sec:main_theorems} can be found in \cref{sec:missingProofs}.


\begin{figure}[ht]
    \centering
    \includegraphics[width = \textwidth]{fig/oracles.eps}
    \caption{The figure illustrates a single iteration of our local iterative reduction cycle. At the beginning of the cycle, the algorithm has already computed a distance structure for every scale $D_j$ with $D_j < D_i$. After completion of the cycle, the algorithm has computed a distance structure for scale $D_i$, under the assumption that it has access to the rounding oracle $\oRound$ (or the \euler oracle $\oEuler$). \cref{lem:cycleone} states this result formally.
    Moreover, each arrow in the cycle corresponds to a formal statement of the following form: Given $A$ (and $B$), then one can efficiently (in $\tilde{O}(1)$ \aggregate rounds) compute $C$. }
    \label{fig:oracles}
\end{figure}

\subsection{Key Definitions and Oracles}
\label{sec:key_definitions}

The definition of the oblivious routing oracle $\oObliv_{D_i}$ relies on the definition of the graph $G_{S,D}$ and the definition of distance scales.

We start with the definition of the graph $G_{S,D}$.

\begin{definition}[Graph $G_{S,D}$]
Let $S \subseteq V$ and $D \in [\poly(n)]$. We construct the graph $G_{S,D}=(V \cup \{\vD,\sstar\}, E \cup \{\{\vD,u\} \mid u \in V\} \cup \{\{\sstar,u\} \mid u \in S\})$ by adding two additional nodes $\vD$ and $\sstar$ to $G$. The node $\vD$ is connected to each node in $V$ and the node $\sstar$ is connected to all the nodes in $S$, with all the new edges having a weight of $D$. Moreover, we denote with $G_S$ the unweighted graph one obtains by discarding the edge weights in the weighted graph $G_{S,D}$.
\end{definition}

Informally speaking, $G_{S,D}$ preserves distance information only up to distance $2D$. More formally, any shortest path between two nodes in $G$ remains a shortest path in $G_{S,D}$ if this path is of length at most $2D$. Shortest paths in $G$ longer than $2D$, on the other hand, are not preserved in $G_{S,D}$, since any two nodes in $G_{S,D}$ have a shortest path of length $2D$ via $\vD$.
Moreover, consider a shortest path tree from vertex $\sstar$ up to distance $2D$. If one removes $\sstar$ and $\vD$ from this tree, then the resulting forest is a shortest path forest in $G$ from set $S$ up to distance $D$. 

We next give the definition of distance scales, along with defining global parameters which are used throughout the paper.
\begin{definition}[Distance Scales]\label{def:distance_scales}
We set $\valSNC = \log^7(n)$, $\beta = 8\valSNC$ and $D_i = \beta^i$. 


A distance scale is a value contained in the set $\{D_i \colon i \in \mathbb{N}, D_i \leq n^2 \max_{e \in E} \ell(e)\}$.
In particular, if we denote with $i_{max}$ the largest integer $i$ for which $D_{i}$ is a distance scale, then $D_{i_{max}} \geq \diam(G)$.
\end{definition}

We are finally ready to formally define oracle $\oObliv_{D_i}$, the $\ell_1$-Oblivious Routing Oracle for scale $D_i$. It corresponds to computing an ``$\ell_1$-oblivious routing up to distance $D_i$'' in \cref{fig:main}.

\begin{restatable}[$\ell_1$-Oblivious Routing Oracle for scale $D_i$ --- $\oObliv_{D_i}$]{definition}{oblivousroutingoracle}
\label{def:oracle_oblivousrouting}
The $\ell_1$-Oblivious Routing Oracle for scale $D_i$, $\oObliv_{D_i}$, takes as input a set $S \subseteq V$ as well as a demand $b$ and a flow $f$ for $G_{S,D_i}$. It outputs $R_S b$ and $R_S^T f$ for a fixed $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing $R_S$ for $G_{S,D_i}$.
\end{restatable}

Next, we give the formal definition of the forest oracle $\oDist_{\eps,D}$.


\begin{restatable}[$(1+\eps)$-Approximate Forest for distance $D$ rooted at $S$ / Forest Oracle --- $\oDist_{\eps,D}$]{definition}{distanceoracle}\label{def:oracle_dist}
The forest oracle $\oDist_{\eps,D}$ takes as input a node set $S \subseteq V$.
The output is a $(1+\eps)$-approximate forest for distance $D$ rooted at $S$, which is a forest $F$ rooted at $S$ such that the following holds.
\begin{enumerate}
    \item For every $u \in V(G)$ with $\dist_G(S,u) \le D$ we have $u \in V(F)$.
    \item For every $u \in V(F)$, $\dist_F(S,u) \le (1+\eps)D$. 
\end{enumerate}
\end{restatable}

For a given distance scale $D_i$, having access to $\oDist_{\frac{1}{\log^3(n)},D}$ for every $D \in \left[ \frac{D_i}{\valSNC}, D_i\right]$ corresponds to ``$(1+\eps)$ set-shortest path up to distance $D_i$'' in \cref{fig:main}.


The notion of ``$(1+\eps)$ transshipment up to distance $D$'' in \cref{fig:main} does not have a direct correspondence in \cref{fig:oracles}.
However, the potential oracle $\oPot_{D_i}$ outputs a potential capturing a certain version of (dual) transshipment potentials. 
%We don't make this notion precise. \todo{V: rephrase}
The oracle $\oPot_{D_i}$ is defined as follows:

\begin{definition}[Potential for scale $D_i$ with respect to set $S$ / Potential Oracle --- $\oPot_{D_i}$] \label{def:potential}
The potential oracle $\oPot_{D_i}$ takes as input a node set $S \subseteq V$.
The output is a potential $\phi_{S, D_i} \in \R^{V(G_{S, D_i})}$ for scale $D_i$ with respect to $S$.
A potential for scale $D_i$ with respect to a set $S \subseteq V$ is a non-negative potential $\phi_{S,D_i}$ (satisfying the conditions given in \Cref{sec:preliminaries}) such that:
\begin{enumerate}
    \item $\forall v \in S:\ \phi_{S,D_i}(v) = 0$ and
    \item $\dist_G(v,S) \geq \frac{D_i}{\valSNC}$ implies $\phi_{S,D_i}(v) \geq 0.5\frac{D_i}{\valSNC}$.
\end{enumerate} 
\end{definition}


We next give the definition of a distance structure for scale $D_i$.
\begin{definition}[Distance Structure for scale $D_i$]
\label{def:distance_structure}
A distance-structure for scale $D_i$
consists of a sparse neighborhood cover with covering radius $\frac{D_i}{\valSNC}$. Moreover, each cluster $C$ in one of the clusterings comes with 
\begin{enumerate}
    \item a tree $T_C$ of diameter at most $D_i$ which spans $C$ and is rooted at some node $v_C \in C$. We refer to $v_C$ as the cluster center.
    \item A potential for scale $D_i$ with respect to $V \setminus C$ (known to nodes in $C$). \alert{we never defined what potentials with respect to a subset means.. also, with respect to which weighted graph is this? (I suppose $G_{D_i}$ or something.. but this is important to say?}
\end{enumerate}
\end{definition}

\alert{also, I think that the dist structure potentials are quite hard to parse for non-authors of this paper .. we should explain that this potentials with respect to the outside of the cluster actually means we want to know the distance to the boundary, but we are happy with an approximate distance that satisfies the potential smoothness properties or whatever.}

In \cref{fig:main}, ``distance structures up to distance $D$'' correspond to having a distance structure for every scale $D_j$ with $D_j \leq D$.

In \cref{sec:intro} we outlined the problem of rounding a transshipment flow, and that rounding can be deterministically reduced to solving $\tilde{O}(1)$ \euler problems. 
We now define the oracles for the two problems.

The rounding oracle is defined as follows. \alert{in sec 5 we actually give an implementation for a perfect $\eps = 0$ rounding oracle .. Christoph explained that this is to future-proof the proof as someone might come up with a (distributed) rounding faster algorithm in the future. However, without any explanation here this is extremely confusing (at least to me). Can we please add a explanation why we state it in this form.}

\begin{restatable}[Rounding Oracle --- $\oRound_{\eps}$]{definition}{roundingoracle}
\label{def:oracle_rounding}
The Rounding Oracle $\oRound_{\eps}$ takes as input a weighted graph $H$ with length function $\ell_H$ and a flow $f$ on $H$. The weighted graph $H$ needs to be a subgraph of some graph $H'$ that one can obtain from $G$ by adding up to $\tilde{O}(1)$ virtual nodes and adding edges of arbitrary nonnegative length incident to the virtual nodes. The flow $f$ needs to satisfy the following condition. Let $b$ be the demand that $f$ routes. Then, $b(v) \geq 0$ for all $v \in V(H)$ except for some $s \in V(H)$ called the source. 
The output is a rooted tree $T$ with root $s$ spanning all vertices of $H$ with non-zero demand such that $\sum_{v:b(v) \neq 0}b(v)\dist_T(s,v) \le (1+\eps')\ell_H(f)$ with $\eps' = \min \left( \eps,\frac{1}{20\log^3(n)\valSNC} \right)$. 
\end{restatable} 

Note that $\oRound_{\eps}$ takes as input a weighted graph that can have more vertices than $G$. This allows us to use $\oRound_{\eps}$ to round a transshipment flow defined on the graph $G_{S,D}$. 
Moreover, we sometimes just write $\oRound$, without a precision parameter $\eps$, which we define as $\oRound = \oRound_1 = \oRound_{\frac{1}{20\log^3(n)\valSNC}}$.

The \euler oracle is defined next. 

\begin{restatable}[\euler Oracle --- $\oEuler$]{definition}{euleroracle}
\label{def:oracle_euler}
The \euler oracle $\oEuler$ takes as input a Eulerian graph $H$. The graph $H$ has to be a subgraph of some graph $H'$ that one can obtain from $G$ by adding up to $\tilde{O}(1)$ virtual nodes and adding any edges incident to the virtual nodes.
The output is an orientation of the edges of $H$ such that the in-degree of every node is equal to its out-degree.
\end{restatable}







\subsection{Formal Statements Corresponding to \cref{fig:oracles}}
\label{sec:implications_cycle}

For the sake of this section, we say that we can solve a problem or compute a structure \emph{efficiently} if there exists a \aggregate algorithm for the task that runs in $\tilde{O}(1)$ rounds. 

In this subsection, we give one formal statement for each arrow in \cref{fig:oracles}, as promised at the beginning of \cref{sec:localiterative}.
Before that, we state a result which captures the main essence of our local iterative reduction cycle. 

\begin{restatable}[Main Lemma]{lemma}{cycleone}
\label{lem:cycleone}
Assume a distance structure for every scale $D_j$ smaller than scale $D_i$ and oracle $\oRound$ are given. A distance structure for scale $D_i$ can be efficiently computed.
\end{restatable}

\cref{lem:cycleone} is a simple corollary of the next four lemmas. The formal proof can be found in \cref{sec:missingProofs}.



\begin{restatable}{lemma}{cycletwo}
\label{lem:cycletwo}
Assume a distance structure for every scale $D_j$ smaller than scale $D_i$ is given. Then, $\oObliv_{D_i}$ can be efficiently computed. 
\end{restatable}
\cref{lem:cycletwo} follows from a simple adaption of our $\tO(1)$-competitive $\ell_1$-oblivious routing construction, explained in \cref{sec:l1-oblivious-routing}.

\begin{restatable}{lemma}{cyclethree}
\label{lem:cyclethree}
Assume oracle $\oRound$ and $\oObliv_{D_i}$ are given. Then, $\oPot_{D_i}$ and $\oDist_{\frac{1}{\log^3(n)},D}$ can be efficiently computed for every $D \in \left[ \frac{D_i}{\valSNC},D_i \right]$.
\end{restatable}
\cref{lem:cyclethree} follows mainly from previous work. More precisely, having access to a $\tO(1)$-competitive $\ell_1$-oblivious routing in $G_{S,D_i}$, we can compute the following two objects via boosting and rounding \cite{She17, BKKL17, Li20, goranci2022universally}. First, a $(1+\eps)$-SSSP-tree in $G_{S,D_i}$ rooted at $\sstar$. Second, an individually good $(1+\eps)$-approximate potential in $G_{S,D_i}$ for the single-source transshipment demand with source $\sstar$. 
For completeness, we give a summary of these steps in the proof of \cref{theorem:boosting_rounding}.

If one looks at what the aforementioned tree and potential in $G_{S,D_i}$ correspond to in the graph $G$, then one can relatively straightforwardly transform them to obtain a $\left(1+\frac{1}{\log^3 n}\right)$-approximate forest for $D$ rooted at $S$ and a potential for scale $D_i$ with respect to $S$, assuming $\eps = \frac{1}{\poly(\log n)}$ is sufficiently small.
The details of this transformation can be found in the proof of \cref{lem:cyclethree} in \cref{sec:missingProofs}.


\begin{restatable}{lemma}{cyclefour}
\label{lem:cyclefour}
Assume oracle $\oDist_{\frac{1}{\log^3(n)},D}$ is given for every $D \in \left[ \frac{D_i}{\valSNC},D_i \right]$. Then, a sparse neighborhood cover with covering radius $\frac{D_i}{\valSNC}$ together with a rooted spanning tree $T_C$ of diameter at most $D_i$ for every cluster $C$ in the cover can be computed efficiently.
\end{restatable}

\cref{lem:cyclefour} directly follows from \cite[Theorem C.4]{elkin2022decompositions}, which is proven by adapting the algorithms of \cite{rozhon_ghaffari2019decomposition,chang_ghaffari2021strong_diameter} for the closely-related network decomposition problem. 

%As a last step we want to use $\oPot$ and $\oDist$ to compute a distance structure for the next scale. For this we first use $\oDist$ to compute a sparse neighborhood cover and then use $\oPot$ and $\oDist$ to compute the distance information for each cluster, i.e., the tree and the potential. These two steps are formally given next:



\begin{restatable}{lemma}{cyclefive}
\label{lem:cyclefive}
Assume we are given an oracle $\oPot_{D_i}$ and a sparse neighborhood cover with covering radius $\frac{D_i}{\valSNC}$ together with a rooted spanning tree $T_C$ of diameter at most $D_i$ for every cluster $C$ in the cover. 
Then, a distance structure for scale $D_i$ can be computed efficiently.
\end{restatable}

Given a sparse neighborhood cover together with a tree for each cluster, it only remains to compute the potential for scale $D_i$ with respect to $V \setminus C$ for each cluster $C$ in the sparse neighborhood cover. 
One can compute the potentials for all the clusters in a given clustering $\fC$ simultaneously. The simplest approach for computing these potentials is to compute a single potential for scale $D_i$ with respect to all the nodes that are neighboring one of the clusters in $\fC$. This approach works as long as there does not exist a node that is both clustered and neighboring a different cluster. Even though this can indeed happen, there is a simple solution that solves this problem. The details can be found in the proof of \cref{lem:cyclefive} in \cref{sec:missingProofs}. 

\alert{this lemma is never proven, what is proven is a (differently stated and more precise) Theorem 5.1.. we should probably replace this lemma with that theorem.}
\begin{restatable}{lemma}{cycleeuler}
\label{lem:cycleeuler}
Assume the oracle $\oEuler$ is given. Then, $\oRound$ can be efficiently computed. 
\end{restatable}
The main ideas to prove this lemma were already discussed in the introduction.
The details can be found in \cref{sec:rounding}.

\subsection{Main Theorems}
\label{sec:main_theorems}

In this part, we state the main theorems of this paper. 

First of all, a simple induction proof on top of \cref{lem:cycleone} leads to the following result.

\begin{restatable}{lemma}{cyclesix}
\label{lem:cyclesix}
Assume oracle $\oRound$ is given. Then, a distance structure for every scale $D_i$ can be efficiently computed.
\end{restatable}

Note that for $i = 1$, \cref{lem:cycleone} states that given access to $\oRound$, one can efficiently compute a distance structure for scale $D_1$.
The complete induction proof can be found in \cref{sec:missingProofs}.


Given access to a distance structure for every scale $D_i$, the theorem below follows directly from our $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing scheme described in \cref{sec:l1-oblivious-routing}.

\begin{restatable}[Distance Structures give $\ell_1$-Oblivious Routing]{theorem}{cycleseven}
\label{theorem:cycleseven}
Assume a distance structure for every scale $D_i$ is given. Then, there exists a $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing $R$ for $G$ for which $R$ and $R^T$ can be efficiently evaluated.
\end{restatable}




As discussed in \Cref{sec:intro}, $\ell_1$-oblivious routing and rounding is sufficient to solve the $(1+\eps)$-SSSP tree and the $(1+\eps)$-transshipment problems~\cite{She17, BKKL17,Li20,goranci2022universally}.

\begin{restatable}[$\ell_1$-Oblivious Routing gives SSSP and transshipment]{theorem}{cycleeight}
\label{theorem:cycleeight}
Assume oracle $\oRound_{\eps/2}$ is given for some $\eps \in (0,1]$ and that there exists an efficient algorithm to evaluate $R$ and $R^T$ for some $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing $R$ for $G$. Then, the $(1+\eps)$-transshipment problem and the $(1+\eps)$-SSSP-tree problem in $G$ can be solved in $\tilde{O}(1/\eps^2)$ \aggregate rounds. 
\end{restatable}


Combining \cref{lem:cyclesix}, \cref{theorem:cycleseven} and \cref{theorem:cycleeight} results in the following theorem.

\begin{restatable}{theorem}{cyclenine}
\label{theorem:cyclenine}
Assume oracle $\oRound_{\eps/2}$ is given for some $\eps \in (0,1]$. The $(1+\eps)$-transshipment problem and the $(1+\eps)$-SSSP-tree problem in $G$ can be solved in $\tilde{O}(1/\eps^2)$ \aggregate rounds.
\end{restatable}

The theorem above together with the fact that $\oRound$ can be efficiently implemented given $\oEuler$ implies the following result.

\begin{restatable}{theorem}{cycleten}
\label{theorem:cycleten}
Assume oracle $\oEuler$ is given and let $\eps \in (0,1]$. The $(1+\eps)$-transshipment problem and the $(1+\eps)$-SSSP-tree problem in $G$ can be solved in $\tilde{O}(1/\eps^2)$ \aggregate rounds.
\end{restatable}

The \euler problem can be solved with near-linear work and polylogarithmic depth \cite{atallah_vishkin1984euler_pram}. Together with the theorem above and the fact that each $\aggregate$ round can be simulated with near-linear work and polylogarithmic depth, we obtain our main parallel result.

\mainparallel*

Moreover, our \congest algorithms for the \euler problem developed in \cref{sec:euler} together with general simulation results for the \congest model developed in prior work (see \cref{thm:compilation_pa_congest}), we obtain our main result in the \congest model.

\maindistributed*

We finish this section by stating the conditional results on universally-optimal SSSP and transshipment algorithms one can obtain from this work:


\begin{theorem} \label{lem:universalOptreduction1}
Suppose there exists a deterministic algorithm for partwise aggregation that runs in $\shortcutQuality{G} \cdot n^{o(1)}$ \congest rounds, then there exist deterministic $(1+\eps)$-SSSP and $(1+\eps)$-transshipment algorithms with a round complexity of $\shortcutQuality{G}) \cdot n^{o(1)}$, which is universally-optimal up to a $n^{o(1)}$-factor. 
\end{theorem}

We get even stronger conditional results if more efficient \congest algorithms for computing cycle covers as defined in \cite{parter_yogev2019cycle_decomp_near_linear,parter_yogev2019cycle_covers_minor_closed} are given. 

\begin{theorem}\label{lem:universalOptreduction2}
Suppose there exists a deterministic algorithm for partwise aggregation that runs in $\tO(\shortcutQuality{G})$ \congest rounds and a $(\tO(1),\tO(1))$ cycle cover algorithm for $\tO(1)$-diameter graphs which runs in $\tO(1)$ \congest rounds. Then, there exist deterministic $(1+\eps)$-SSSP and $(1+\eps)$-transshipment algorithms with a round complexity of $\tO(\shortcutQuality{G})$, which is universally-optimal up to polylogarithmic factors. 
\end{theorem}

While the polylogarithmically tight algorithmic results assumed in \Cref{lem:universalOptreduction2} seem out of reach of current techniques, our conditional results show that the problem-specific part towards universally optimal shortest path algorithms, even deterministic ones, are essentially fully understood through the techniques of this paper. 

\Cref{lem:universalOptreduction2} and \Cref{lem:universalOptreduction1} follow from \Cref{thm:main_distributed} in \cref{sec:missingProofs} which shows that to get the near-optimal round complexity of $\tO_{\eps}(\shortcutQuality{G})$ in \cref{thm:main_distributed}, it suffices to solve efficiently the Partwise-Aggregation problem (see \cref{sec:computational-models}) and implement efficiently the oracle $\oEuler$ which can be done by an efficient solution of the cycle cover problem (see \cref{sec:euler}). 




%\begin{remark}[Universally Optimal Algorithm?]
%We remark that the proof of \cref{thm:main_distributed} in \cref{sec:missingProofs} implies that to get the near-optimal round complexity of $\tO_{\eps}(\shortcutQuality{G})$ in \cref{thm:main_distributed}, it suffices to solve efficiently the Partwise-Aggregation problem (see \cref{sec:computational-models}) and implement efficiently the oracle $\oEuler$ which can be done by an efficient solution of the cycle cover problem (see \cref{sec:euler}). 
%\end{remark}






% Local Variables:
% TeX-master: "main"
% End:


==> Deterministic_SSSP/euler.tex <==
\section{Distributed Algorithms for the Eulerian-Orientation Problem}
\label{sec:euler}

In this section, we show how to construct the \euler oracle $\oEuler$. 
Instead of talking about oracles, we talk about solving the \euler problem, in which we are asked to orient each edge such that each node has the same indegree and outdegree. 
The main result of the section is the following theorem. 

\begin{restatable}{theorem}{thmeuler}
\label{thm:euler_dist}
There are deterministic algorithms for the \euler problem (that is, implementing the oracle $\oEuler$) with the following round complexities. 
\begin{enumerate}
    \item $\tO(\hopDiameter{G})$ \congest rounds if $G$ comes from a fixed minor-free family. 
    \item $n^{o(1)}$ \congestPA rounds. 
    \item $\tO(\sqrt{n} + \hopDiameter{G})$ \congest rounds. 
\end{enumerate}
\end{restatable}


There is a simple deterministic parallel algorithm for the \euler problem with near-linear work and polylogarithmic depth \cite{atallah_vishkin1984euler_pram}. 
The algorithm starts by pairing up all edges at every node of $H$. This splits $E(H)$ into a set of closed walks. In the following $O(\log |E(H)|)$ rounds, edges of the same closed walk are collected and the whole walk is consistently oriented. 
This ensures the equal indegree and outdegree at each node of $H$. 

\begin{theorem}[\cite{atallah_vishkin1984euler_pram}]
\label{thm:euler_pram}
There is a deterministic $O(\log n)$ depth and $O(m \log n)$ work algorithm for the \euler problem on CRCW \pram.  
\end{theorem}

However, to the best of our knowledge there are no non-trivial distributed algorithms known for the Eulerian-Orientation problem. 
Here we provide a fast distributed algorithms using the Low Congestion Cycle Covers of \cite{parter_yogev2019cycle_covers_minor_closed,parter_yogev2019cycle_decomp_near_linear,hitron_parter2021adversarial_compilers}. 
First, we prove several preparatory lemmas in \cref{sec:eulerTechnical} and postpone the proof of \cref{thm:euler_dist} in \cref{sec:eulerMain}. 



\subsection{Technical Preparations}
\label{sec:eulerTechnical}

First, we prepare several necessary tools. We start by proving that if we contract degree two nodes in a graph, in the contracted graph we can simulate \congestPA rounds. 

\begin{lemma}
\label{lem:simulation_contraction}
Let $G$ be a graph and $G'$ be a graph we get by contracting every node of degree $2$ in $G$. 
Then we can simulate one \congestPA round in $G'$ in $O(1)$ \congestPA rounds in $G$. 

Moreover, if each edge $e \in E(G')$ is arbitrarily oriented, we can consistently orient the whole path in $G$ contracting to $e$ in that direction in $O(\log n)$ \congestPA rounds. 
\end{lemma}
\begin{proof}
To simulate one \congest round in $G'$, we first use one \congest round in $G$ to send the message along edges that remain the same in $G$ and $G'$. 
Moreover, for each path $u_1, u_2, \dots, u_k$ in $G$ that contracts to an edge $e$ in $G'$, we let $u_1$ send the message meant to $u_k$ to its neighbor $u_2$. 
The path $u_2, u_3, \dots, u_{k-1}$ is node-disjoint from all other contracted paths, hence the message to $u_k$ can be sent to $u_{k-1}$ with one call to the partwise aggregation oracle. In one final \congest round the message is delivered to $u_k$. 

The simulation of the partwise aggregation oracle in $G'$ is implemented analogously: each edge in $G'$ connecting two nodes of the same part is expanded to a full path. The new set of parts of $G$ is still node-disjoint. We then use the partwise aggregation oracle of $G$

The final claim is proven by building a tree of constant degree and radius $O(\log n)$ on top of each path, in $O(\log n)$ \congestPA rounds. 
The tree is then used to propagate an information about the orientation of the path to all nodes, in $O(\log n)$ \congestPA rounds. We omit details as they are standard and essentially the same as in the proof of \cref{euler:lem:sqrt}. 
\end{proof}

\paragraph{Dealing with virtual nodes}
Next, we discuss how to handle virtual nodes. See \cref{subsec:minor_aggregation} for the definitions related to virtual nodes. In what follows, we assume that the input graph $G$ may contain $\tO(1)$ virtual nodes and show how one can reduce this case to the case without any virtual nodes. 






\begin{lemma}[Variant of Lemma 4.3.2 in \cite{peleg2000distributed}]
\label{euler:lem:matching}
Let $T \subseteq G$ be a rooted tree of $G$ and $S$ a set of \emph{marked} nodes. 
Then, in $\tO(1)$ \congestPA rounds, we can output a set of paths $P= \{p_1, p_2, \dots, p_{\lfloor S/2 \rfloor}\}$ such that
\begin{enumerate}
    \item Each path $p \in P$ satisfies $p \subseteq T$. 
    \item All nodes of $S$, except of possibly one, are endpoints of exactly one $p \in P$. 
    \item Any two $p_1, p_2 \in P$ are edge-disjoint. 
    \item We can implement partwise aggregation on $P$ in $O(1)$ \congestPA rounds of $G$. 
\end{enumerate}

%Then, in $O(\hopDiameter{G})$ \congest rounds, we can output a matching $M = \{ \{s_1, t_1\}, \dots, \{s_{\lfloor S/2 \rfloor}, t_{\lfloor S/2 \rfloor}\} \}$, where for each $1 \le i \le \lfloor S/2 \rfloor$, $s_i, t_i \in S$. 

%Moreover, for each $\{s_i, t_i\}$, we return a subpath $P_i$ of $T$  with the following property. 
%Let $u_i$ be the node of $P_i$ closest to the root $r$ of $T$ and we write $P_i = P_i^1 \circ \{u_i\} \circ P_i^2$, that is, we write $P_i$ as a concatenation of a path from $s_i$ to a node below $u_i$, next a trivial path $\{u_i\}$, and a path from a node below $u_i$ to $t_i$. 
%Then, all sets $\{P_1^1, P_1^2, P_2^1, P_2^2, \dots, P_{\lfloor S/2 \rfloor}^1, P_{\lfloor S/2 \rfloor}^2\}$ are node-disjoint. 
\end{lemma}
\begin{proof}
We first describe how we build the set $P$ of paths. 
For each $u \in V(T)$, let $x_u = 1$ if $u\in S$ and $x_u = 0$ otherwise. We use \cref{lemma:ancestor-subtree-sum} to compute $s_u = \sum_{v \in T_u} x_v$ for every $u$, where $T_u$ is the subtree of $u$ in $T$. 
If $s_u$ is odd, $u$ will be connected in a path with its parent $\parent(u)$ (unless $u$ is the root) and sends this information to $\parent(u)$. Next, each node $u$ collects messages from all its children nodes to know which of them will be in the same path as $u$. The node $u$ arbitrarily pairs up these proposals into paths (for each such created path, $u$ is the node in it closest to the root). 
By construction, there is a leftover, unpaired, proposal if and only if $u$ itself proposed and $u \not\in S$ (unless $u$ is a root). 
In this case, the leftover unpaired child of $u$ is combined with $u$ in the same path. 
Otherwise, if $u\in S$ and children of $u$ are paired up, $u$ is the endpoint of a new path that continues to $\parent(u)$. 
This local algorithm defines the set of paths $P$. 
The only reason why $P$ not necessarily satisfies properties 1,2,3 from the lemma statement is that if $|S|$ is odd, $P$ contains an additional path from a vertex in $S$ to the root of $T$. Next, we describe how to implement any  partwise aggregation  on $P$ and this allows us to remove this additional path from $P$ so that it satisfies all three desired properties.  

To prove property 4, let $p_i \in P$ be any path and let us write $p_i = r_i, \dots, s_i^-, s_i, s_i^+, \dots, t_i$, where $s_i$ is the node on $p_i$ closest to the root of $T$. 
Consider any two paths $P_i,P_j$ and let $v \in P_i \cap P_j$. We know that the edge from $v$ to its parent can be present in at most one of the paths $P_i,P_j$ as they are edge-disjoint, hence $v \in \{s_i, s_j\}$. That is, if two paths $P_i, P_j$ intersect in a node, the node is the ``top'' node of one of them. 
Hence, to implement a  partwise aggregation on $P$, we compute the operation on the parts $\{\{r_i, \dots, s_i^-\}, \{s_i^+, \dots, t_i\}\}_{1 \le i \le {\lfloor S/2 \rfloor}}$ that are node-disjoint and use additional $O(1)$ \congest rounds to extend the operation to the set of full paths. 
\end{proof}

\begin{proposition}
\label{euler:prop:get_rid_of_virtual_edges}
Given an input $H$ to the \euler problem with $k = \tO(1)$ virtual nodes, there is a deterministic distributed algorithm that orients some subgraph $I \subseteq H$ such that 
\begin{enumerate}
    \item All edges incident to virtual nodes are in $I$. 
    \item Each node has the same indegree and outdegree in $I$. In particular, the residual graph $H \setminus I$ is still Eulerian. 
\end{enumerate}
The algorithm needs $\tO(1)$ \congestPA rounds. 
\end{proposition}

First, we sketch how to prove the above proposition if there is just one virtual node. 
We then proceed with the more difficult (but still routine) proof for multiple virtual nodes. 

To prove \cref{euler:prop:get_rid_of_virtual_edges} with $k = 1$, we start by finding any spanning forest $F$ of $H$ in $\tO(1)$ \congestPA rounds using the distributed MST algorithm \cite{kutten1998fast}. 
Next, we use \cref{euler:lem:matching} with $S$ being the neighborhood of the virtual node $u$. As the size of the neighbourhood of $u$ in any component of $F$ is even, we pair all of its nodes. 
Note that each constructed path closes a cycle together with the two appropriate virtual edges to $u$. We can use the fact that we can aggregate information on these paths (property 4 in \cref{euler:lem:matching}) to consistently orient the graph $I$ formed by these cycles, which proves the proposition in case $k = 1$. 
We now continue with the proof for $k = \tO(1)$. 

\begin{proof}
The first part of the algorithm consists of $k$ steps. 
During the $i$-th step we orient some of the virtual edges incident to $u_i$ as well as some non-virtual edges. We maintain a residual graph $H_i$ of not yet oriented edges at the beginning of the $i$-th phase. 

More precisely, at the beginning of the $i$-th phase we compute a spanning forest of $H_i[V(G)]$ (that is, we consider only the graph of non-virtual nodes and edges of $H_i$) by an MST algorithm. Next, in each connected component of $H_i[V(G)]$ we use, in parallel,  \cref{euler:lem:matching} to match nodes neighboring with $u_i$. At most one node is unmatched in each connected component of $H_i$. 
Each path $p$ in the set of matching paths closes a cycle together with the two virtual edges connecting the endpoints of $p$ with $u_i$. We can orient this cycle consistently in $\tO(1)$ \congestPA rounds using property (4) in \cref{euler:lem:matching}. This leaves us with a new residual graph $H_{i+1}$ such that $H_{i+1}[V(G)]$ has possibly more connected components but it still retains the property that each connected component of $H_{i+1}[V(G)]$ is incident to at most one edge from $u_i$. 
Hence, after $k$ phases, we are left with a residual graph $H' = H_{k+1}$ such that each connected component of $H'[V(G)]$ contains at most $k$ edges to virtual nodes. Moreover, the number of these incident virtual edges is even. 

In the second part of the algorithm, we use \cref{euler:lem:matching} on the spanning forest of $H'[V(G)]$ again, but this time every node incident to $\{u_1, \dots, u_k\}$ is in the set $S$. The lemma yields a set of edge-disjoint paths such that each path $p$ between two nodes $s$ and $t$, incident to $u_i$ and $u_j$, respectively, connects $u_i$ with $u_j$). 
For each such path, we replace the two virtual edges $\{u_i,s\}, \{u_j, t\}$ with a new virtual edge $\{u_i,u_j\}$, to create a new graph $H''$. After the replacement, there are no connections between the virtual and nonvirtual nodes, hence $H''$ satisfies that $H''[\{u_1, \dots, u_k\}]$ is an Eulerian graph. 
All nodes of $G$ now learn the graph $H''[\{u_1, \dots, u_k\}]$ in $O(k^2) = \tO(1)$ \congestPA rounds and all nodes of $G$ compute internally the same Eulerian orientation of it. 
Finally, we will uncontract each contracted edge $(u_i, u_j)$ of $H''[\{u_1, \dots, u_k\}]$ into the original path and orient the respective path $(u_i, s), p, (t, u_j)$ in the same direction as how the edge $(u_i, u_j)$ was oriented. 
More concretely, for every multi-edge $\{u_i, u_j\} \in E(H''[\{u_1\dots, u_k\}])$, we know two numbers $a_{ij}$ and $b_{ij}$ such that $a_{ij}$ paths contracted to an edge $\{u_i, u_j\}$ need to be oriented from $u_i$ to $u_j$ and $b_{ij}$ paths need to be oriented from $u_j$ to $u_i$. If each path $p$ retains a unique identifier, using binary search, in $\tO(1)$ \congestPA rounds we can decide that $a_{ij}$ paths connecting $u_i$ and $u_j$ with lower identifiers will be oriented from $u_i$ to $u_j$, and the rest in the opposite direction. 
Hence, in $\tO(1)$ \congestPA rounds, we can extend the Eulerian orientation of $H''[\{u_1, \dots, u_k\}]$ to an Eulerian orientation of a subgraph of $H'$ that contains all virtual edges, as needed. 
\end{proof}


\begin{comment}
\begin{lemma}
\label{lem:simulation_virtual}
Let $G$ be a graph and $H$ an Eulerian graph which is, up to a set of $k = \tO(1)$ virtual nodes $u_1, u_2, \dots, u_k$ a subgraph of $G$. 
Then, in $\tO(1)$ \aggregate rounds we can construct an Eulerian multigraph $H'$ which is a subset of $G$, up to multiplicities and up to a set of virtual edges $e_1, \dots, e_\ell$ such that
\begin{enumerate}
        \item One \congest or one \aggregate round on $G \cup H'$ can be implemented in one \congest plus $\tO(1)$ \aggregate rounds on $G$. 
        \item A solution of \euler with $H'$ can be lifted to a solution of \euler on $H$ in additional $\tO(1)$ \aggregate rounds on $G$. 
\end{enumerate}
\end{lemma}
\begin{proof}
For each virtual node $u$ we do the following. 
Let $T$ be the BFS tree in $G$ from some arbitrary non-virtual root node $r$. We use \cref{lem:matching_peleg} with the set $S$ being the set of nodes neighboring to $u$. 
Next, for each pair of nodes $s_i, t_i$, we add a virtual edge $\{s_i, t_i\}$ to $H$ instead of the two virtual edges $\{s_i, u\}, \{t_i, u\}$. 
We do the same for every virtual node. 
Each virtual node retains at most one edge connecting it to non-virtual nodes. 
We broadcast the set of all such edges to all the nodes in $O(\hopDiameter{G})$ rounds. 
Then, internally, each node computes a consistent orientation of a maximal set of cycles consisting of only virtual nodes. The remaining edges incident with virtual nodes form $\tO(1)$ paths that are then contracted to additional virtual edges. 
This process defines a graph $H'$ such that $V(H')$ contains no virtual nodes. 
Moreover, a solution to \euler on $H'$ can be lifted to a solution on $H$ in $\tO(\hopDiameter{G})$ additional \congest rounds. 

We start by proving item (1) from the statement. 
To implement one \congest round on $G \cup H'$, each virtual edge $\{s,t\}$ is replaced by the appropriate path $P = P^1 \circ \{u\} \circ P^2$. 
A message from $s$ to $t$ is sent in $2$ \aggregate and $2$ \congest rounds as follows: first $s$ sends it to the other endpoint of $P^1$, then it is passed to $u$ that passes it to the endpoint of $P^2$ that sends it to $t$. Since for given virtual node $u$ all appropriate paths $P$ are node-disjoint by \cref{lem:matching_peleg}, we can implement all sending along all virtual edges of $H'$ in $\tO(1)$ \congest plus \aggregate rounds, as needed. 

Additionally, one \aggregate round on $G \cup H'$ can be implemented in $\tO(1)$ \aggregate rounds on $G$, since for each virtual edge inside some connected component $C$, we can put its appropriate path in $T$ to $C$. Then, if we started with node-disjoint components $C_1, \dots, C_k$, after the replacement of each virtual edge by a path we have that each node is in $\tO(1)$ different components by item (3). 
\end{proof}
\end{comment}

\begin{comment}

\begin{definition}[Subdivided graph $\tG$]
Let $\tG$ be a graph such that $V(\tG) = \{ (u,e) | u \in e\}$. That is, the nodes of $\tG$ are the \emph{half-edges} in $G$. 
For each $e = \{u,v\} \in E(G)$, $\tG$ contains an edge between $(u,e)$ and $(v,e)$ and for every node $u \in V(G)$ such that $u$ is contained in edges $e_1, e_2, \dots, e_{\deg(u)}$, for every $1\le i < j \le \deg(u)$, $\tG$ contains an edge between $(u,e_i)$ and $(u,e_j)$. 
\end{definition}
Note that one round of communication in $\tG$ can be implemented in one communication round in $G$: each node $u \in V(G)$ will take care of all nodes $(u,e) \in V(\tG)$. 
Also, $\hopDiameter{G}(\tG) = O(\hopDiameter{G}(G))$. 
\end{comment}


\paragraph{Weaker Result} We now give an algorithm for the \euler problem with weaker than desired propeties. It will be used in the proof of \cref{thm:euler_dist}. 

\begin{lemma}
\label{euler:lem:sqrt}
There is a distributed algorithm that solves the \euler problem in $\tilde{O}(\sqrt{|E(G)|} + \hopDiameter{G})$ rounds. 
\end{lemma}
\begin{proof}
We assume the input Eulerian graph $H$ does not contain any virtual nodes, as we can deal with them using \cref{euler:prop:get_rid_of_virtual_edges} and \cref{thm:compilation_pa_congest} in $\tO(\sqrt{n} + \hopDiameter{G})$ \congest rounds. 
%First we deal with virtual nodes $u_1, u_2, \dots, u_k$, analogously to \cref{lem:simulation_virtual}. For each virtual node $u_i$, we find a collection $\fP_i$ of edge-disjoint paths of total length at most $n-1$, each of length at most $\hopDiameter{G}$, that pairs up non-virtual nodes incident to $u_i$. 
%We add all edges from $\fP_i, 1 \le i \le k$ to the graph $H$ and forget virtual nodes and edges incident to it. This creates a multigraph $H$ which is, up to multiplicities of edges which are bounded by $\tO(1)$, a subgraph of $G$. We will now solve the \euler problem in $H$, with the additional restriction that for each path $p \in \fP_i$, all of its edges need to be oriented consistently in one of two possible directions. Then it is easy to see how to extend the solution to a solution in $H$ in additional $\tO(\hopDiameter{G})$ \congest rounds. 

Each node $u$ arbitrarily pairs up the edges of $H$ incident to it -- note that their number is even. 
Starting in any edge, the pairing defines a closed walk containing the edge. We will next orient each such walk consistently, which solves the \euler problem. 

To orient the walks, each one first elects a leader in $O(\log n)$ steps as follows. At first, we interpret each edge as a path of length $1$. 
Next, we concatenate these paths using our pairing into progressively longer paths, until all paths of the walk are glued together. 
In particular, consider the incidence graph of our paths, induced by our edge pairing, which is always a set of disjoint cycles. 
In each step we use Linial's deterministic algorithm to compute a $(3, 4)$-ruling set \cite{linial92LOCAL}. 
That means we mark some of the paths such that the marked paths are of distance at least $3$ in the incidence graph, while every path is of distance at most $4$ to a marked path. Next, each unmarked path is joined with the closest marked path, to form a longer path. 
There are always at least $3$ and at most $5$ paths forming a longer path, unless the whole walk is connected in this step. 
Hence, in $O(\log n)$ steps, all paths are connected. Each step needs $O(\log^* n)$ \congest rounds of communication in the incidence graph. To simulate one round in the incidence graph, we need to implement sending messages in parallel from one endpoint of a path to the other endpoint. To do that, each path remembers its length. If it is at most $\sqrt{|E(H)|}$, then it sends the message from its endpoint to the other one along its edges. If it is more than $\sqrt{|E(H)|}$, it broadcasts the message to the whole graph using the edges of $G$. 
As there are at most $\sqrt{|E(H)|}$ such paths, it is a standard fact that, with correct implementation, in $O(\hopDiameter{H} + \sqrt{|E(H)|})$ rounds all broadcasts finish. 
Hence, in $\tO(\hopDiameter{H} + \sqrt{|E(H)|}) = \tO(\hopDiameter{G} + \sqrt{|E(G)|})$ rounds each walk can elect a leader. The leader chooses an arbitrary orientation and, similarly to the election, this orientation is messaged to smaller and smaller paths, until after additional $O(\log n)$ steps, each implemented in $\tO(\hopDiameter{G} +\sqrt{|E(G)|})$ rounds, each edge knows it. 

\begin{comment}
In particular, for each walk $e_1, e_2, \dots, e_k$, with $e_i = \{u_i, v_i\}$ and $v_i = u_{i+1}$ for each $1\le i \le k-1$, we consider the corresponding cycle $(e_1, u_1), (e_1, v_1), (e_2, u_2), (e_2, v_2), \dots, (e_k, u_k), (e_k, v_k)$ in $\tG$. Node that since the original walks are edge-disjoint, the cycles in $\tG$ are node-disjoint. 
Hence, in $O(1)$-aggregation round the nodes in the cycle $C$ can elect a leader and compute the number of nodes in $C$. 
After that, in additional $O(\log n)$ \aggregate rounds, we can gradually split $C$ into exponentially smaller node-disjoint paths, such that in step $i$ we have $O(2^i)$ paths of length $O(n/2^i)$. 
At the beginning, we arbitrarily choose one of the two possible orientation of the $C$ and whenever a path $p$ is split into two paths $p_1, p_2$, $p$ tells the border nodes of $p_1, p_2$ how their edges should be oriented. This way we orient consistently all edges of each $C$ in parallel, in $O(\log n)$ \aggregate rounds on $\tG$.  
We can use the trivial shortcuts on $\tG$ to implement this algorithm in $\tO(\sqrt{|V(\tG)|} + D_{\tG}) = \tO(\sqrt{m} + \hopDiameter{G})$ \congest rounds in $G$. 
\end{comment}

\end{proof}

\begin{remark}
The above result seems to imply that the \euler problem can be solved in $\tO(1)$ part-wise aggregations. 
However, in each step, the parts where aggregation happens are only edge-disjoint and not node-disjoint. 
\end{remark}



\paragraph{Cycle Covers}

The concept of cycle covers was introduced in the line of work \cite{parter_yogev2019cycle_covers_minor_closed,parter_yogev2019cycle_decomp_near_linear,hitron_parter2021adversarial_compilers,hitron2021broadcast} for the unrelated reason of making distributed computations more resilient to edge-faults introduced by a Byzantine adversary. 

\begin{definition}[$(d, c)$-cycle cover]
A $(d,c)$ cycle cover of $G$ is a collection of cycles $\fC = \{C_1, \dots, C_k\}$ in $G$ such that
\begin{enumerate}
    \item Each non-bridge edge of $G$ is in at least one $C \in \fC$ and at most $c$ different cycles. 
    \item Each cycle $C$ contains at most $d$ edges. 
\end{enumerate}
\end{definition}


\begin{lemma}[A variant of Theorem 11 in \cite{parter_yogev2019cycle_decomp_near_linear}, see also Fact 12 and Observation 13 in \cite{hitron_parter2021adversarial_compilers}]
\label{lem:general_cycle_cover}
For every graph $G$ and $0 < \eps < 1$ there is a deterministic \congest algorithm that computes a $(d,c)$ cycle cover $\fC$ with $d = 2^{O(1/\eps)}\hopDiameter{G}$ and $c = O(n^\eps)$ within $O (2^{O(1/\eps)} \cdot n^{O(\eps)} \cdot \hopDiameter{G})$ rounds.  
\end{lemma}
\begin{proof}
In \cite{parter_yogev2019cycle_decomp_near_linear}, the authors prove above theorem, but use a randomized algorithm. % with a better round complexity $\tilde{O} (2^{1/\eps} \cdot n^{\eps} \cdot \hopDiameter{G})$. 
Their algorithm uses randomness in two places. First, it uses a randomized routing through a set of paths with maximum dilation $d$ and total congestion of any edge bounded by $c$ in $\tO(c+d)$ \congest rounds. However, we can use a simple deterministic $\tO(cd)$ routing instead. 
Second, their algorithm uses a randomized Luby's algorithm \cite{luby86,alon86lubys_algorithm} to compute an MIS in a certain graph $\hat{G}$ in $O(\log n)$ rounds, where each round of communication in $\hat{G}$ can be implemented in $O(cd)$ rounds. Instead of Luby's algorithm, we can use the deterministic MIS algorithm from \cite{censor2017derandomizing,ghaffari_grunau_rozhon2020improved_network_decomposition} that works in $\tO(1)$ \congest rounds. 
\end{proof}


\paragraph{Excluded Minor Graph Families}
We will use the following results on the forbidden minor graph families. 

\begin{lemma}[Theorem 3 in \cite{parter_yogev2019cycle_covers_minor_closed}]
\label{lem:minor_closed_cycle_covers}
For every minor-closed, 2-connected graph $G$, in $\tilde{O}(\hopDiameter{G})$ rounds of the \congest model, one can construct an $(\tilde{O}(\hopDiameter{G}), \tilde{O}(1))$ cycle cover $\fC$ in $\tO(\hopDiameter{G})$ rounds.  
%For every minor-closed graph $G$, in $\tilde{O}(\hopDiameter{G})$ deterministic rounds of the \congest model, one can construct an $(\tilde{O}(OPT(G)), \tilde{O}(1))$ cycle cover $\fC$ in $\tO(OPT(G))$ \congest rounds. 
%Here, $OPT(G) = max_{e \in E(G)} min_{\text{cycle } C, e \in C} |C|$. 
\end{lemma}

\begin{comment}
\begin{corollary}
\end{corollary}
\begin{proof}
Consider any edge $e = \{u,v\} \in E(G)$ and start BFS from the set $\{u,v\}$. After at most $\hopDiameter{G}$ rounds this BFS covers the whole graph $G$ and constructs two BFS trees $T_u$ and $T_v$ rooted at $u$ and $v$, respectively. Due to 2-connectivity of $G$, there is an edge $f$ connecting the two trees and this edge closes a cycle containing $e$ of size $O(\hopDiameter{G})$. 
\end{proof}
\end{comment}

\subsection{The Eulerian Orientation Algorithm}
\label{sec:eulerMain}

Finally, we are ready to prove \cref{thm:euler_dist}. 

\begin{proof}
Let $H$ be the input Eulerian graph and assume there are no virtual nodes, as we can deal with them with \cref{euler:prop:get_rid_of_virtual_edges,thm:compilation_pa_congest}. 

We start with item (1), the proofs of other items will be similar. 
We will construct the Eulerian orientation in $t = \tO(1)$ steps. 
In the $i$-th step, we are given a residual Eulerian subgraph $H_i \subseteq H$ containing edges left to orient. 
We find a collection of edge-disjoint cycles $\fC$ containing at least $O(|E(H_i)| / \poly\log n)$ edges of $H_i$ in $\tO(\hopDiameter{G})$ \congest rounds and orient them consistently. %, such that the maximum size of each cycle is $s = \tO(\hopDiameter{G})$. 
%In the next $s$ \congest rounds, we consistently orient edges in each cycle in $\fC$ and 
Next, we discard oriented edges from $H_i$, creating a new residual Eulerian graph $H_{i+1}$ used in the next iteration. If $t = \tO(1)$ is chosen large enough, after $t$ rounds we have $|E(H_t)| = 0$ and we are done. 
It remains to describe how we find the set of edge-disjoint cycles $\fC$ which we do next.  


    We will work in a graph $H'_i$ that we get from $H_i$ by contracting all degree $2$ nodes and discarding isolated nodes. 
    When we work later with $H'_i$, we use \cref{lem:simulation_contraction} to reduce operations on $H'_i$ to operations on $H_i$ and \cref{thm:compilation_pa_congest} to reduce partwise aggregations on $H_i$ to $\tO(\hopDiameter{G})$ \congest operations on $H_i$. 
    Note that every node in $H'_i$ has degree at least $4$, as $H'_i$ is Eulerian and does not contain nodes of degree $0$ or $2$. 
    Hence, we have 
    \begin{align}
    \label{euler:eq:EV}
     |E(H'_i)| \ge 4|V(H'_i)|/2 = 2|V(H'_i)|.    
    \end{align}

    Next, we describe the algorithm. 
\begin{enumerate}
\newcommand{\bH}{\overline{H}}
\newcommand{\bC}{\overline{C}}
    \item Let $\bH_i$ be the graph that we get from $H'_i$ by subdividing each edge $e \in E(H'_i)$. That is, $V(\bH_i) = V(H'_i) \cup E(H'_i)$ and for $v \in V(H'_i), e \in E(H'_i)$ we have $\{v,e\} \in E(\bH_i)$ if $v \in e$.  
    We run the clustering algorithm for separated strong-diameter network decomposition from \cite{elkin2022decompositions} on $\bH_i$. 
    The algorithm discards at most $|E(\bH_i)|/10 = (|V(H'_i)| + |E(H'_i)|) / 10 $ nodes such that the undiscarded nodes form connected clusters $\bC_1, \bC_2, \dots, \bC_q$, each of strong radius $O(\log^2 n)$. 
    Moreover, for any two different clusters $\bC_i, \bC_j$ we have $d_{\bH_i}(\bC_i, \bC_j) \ge 3$. 
    The algorithm needs $\tO(1)$ \congest rounds of $\bH_i$, hence can be implemented in $\tO(1)$ \congest rounds of $H'_i$. 
    After building the clustering in $\bH_i$, for each $\bC \subseteq V(\bH_i)$ we define a cluster $C \subseteq V(H'_i)$ as follows: 
    For each node $e = \{u,v\} \in \bC \cap E(H'_i)$ we put both $u$ and $v$ to $C$. 
    This new clustering of nodes in $H'_i$ still consists of disjoint clusters due to the property $d_{\bH_i}(\bC_i, \bC_j) \ge 3$. Moreover, all clusters still have strong radius $O(\log^2 n)$ and the number of unclustered edges in $H'_i$ remains bounded by $(|V(H'_i)| + |E(H'_i)|) / 10$.   
    
    \item Each cluster runs the algorithm from \cref{lem:minor_closed_cycle_covers} to obtain its cycle cover $\fC$ such that each non-bridge edge is covered by $c = \tO(1)$ cycles of $\fC$ and each cycle of $\fC$ has size $d = \tO(D) = \tO(1)$. Note that total number of all bridges over all clusters is bounded by $|V(H'_i)|$. 
    \item Next, we implement the deterministic MIS algorithm of \cite{censor2017derandomizing} of round complexity $\tO(1)$ in the conflict graph of found cycles. In the conflict graph, each cycle $C \in \fC$ is connected with cycles of $\fC$ that share an edge with $C$. 
    One \congest round in the conflict graph can be implemented in $O(cd) = \tO(1)$ \congest rounds in $H'_i$, hence the overall round complexity of this step is $\tO(1)$ rounds in $H'_i$. 
    The found MIS is the set of cycles $\fC$ that we output. 
    

    \item Finally, we consistently orient the edges in the MIS in additional $d = \tO(1)$ \congest steps on $H'_i$. 
\end{enumerate}
    
    The whole algorithm uses $\tO(1)$ \congestPA steps in $H'_i$, hence using \cref{lem:simulation_contraction,thm:compilation_pa_congest}, we can make above steps run in $\tO(\hopDiameter{G})$ \congest rounds in $G$. 
    
    It remains to argue that the above algorithm orients at least $O(|E(H'_i)| / \poly\log(n))$ of $H'_i$. 
    The number of cycles in the conflict graph is at least the number of clustered non-bridge edges of $H'_i$, which is at least 
    \begin{align*}
     &|E(H'_i)| - (|V(H'_i)| + |E(H'_i)|) / 10 - |V(H')| \\
     & \ge \frac{9}{10} |E(H'_i)| - \frac{11}{10}|V(H'_i)|
     \ge |E(H'_i)| / 10. && \text{Equation \ref{euler:eq:EV}}
    \end{align*}

    On the other hand, the degree of each cycle $C$ in the conflict graph can be bounded by $cd = \tO(1)$, since each of $d$ edges of $C$ can intersect $c$ different cycles. 
    Hence, there are at least $|E(H'_i)| / (3cd)$ cycles in the MIS that cover at least $|E(H'_i)| / (3cd) = O(|E(H'_i)| / \poly\log(n))$ edges of $H'_i$ and the proof of item (1) is finished. 


To prove item (2), we simply use \cref{lem:general_cycle_cover} with $\eps = 1/\sqrt{\log n}$ instead of \cref{lem:minor_closed_cycle_covers}.
In each step we cover at least $|E(H'_i)|/2^{O(\sqrt{\log n})}$ edges and we set the number of steps $t$ to be of order $2^{O(\sqrt{\log n})} = n^{o(1)}$. 

To prove item (3), we adapt the above procedure so that by repeatedly orienting cycles, we orient all edges except at most $2n$ of them, in $n^{O(\eps)}$ \congest rounds for any constant $\eps > 0$. 
Then, we consider the $2n$ remaining edges forming a residual Eulerian subgraph and use \cref{euler:lem:sqrt} to orient them in $\tO(\sqrt{n} + \hopDiameter{G})$ time. It remains to adapt the above procedure to orient all but at most $2n$ edges in $n^{O(\eps)}$ rounds. 

We choose a sufficiently small constant $\eps  > 0$ and run the above procedure with the number of steps set to $t = n^{O(\eps)}$. Alternatively, we finish once the number of edges in $H_i$ drops below $2n$. 
During the procedure, we do not contract the degree $2$ nodes and instead of \cref{lem:minor_closed_cycle_covers} we use \cref{lem:general_cycle_cover} with our parameter $\eps$. 
An analysis analogous to the one above shows that, since we always have $|E(H_i)| \ge 2n$ (cf. Equation \ref{euler:eq:EV}), in each step of the process we orient at least $O(|E(H_i)| / n^{O(\eps)})$ edges. Hence, $t = n^{O(\eps)}$ steps are enough to finish. 
Moreover, one step can be implemented in $n^{O(\eps)}$ \congest rounds, without any need of partwise aggregations, implying the round complexity of $n^{O(\eps)} \cdot n^{O(\eps)} = n^{O(\eps)}$, which is less than $O(\sqrt{n})$ for small enough $\eps$, as needed. 
\end{proof}

% Local Variables:
% TeX-master: "main"
% End:

\begin{remark}
We believe, but do not prove, that any (randomized) algorithm for the  \euler problem on all graphs has to have round complexity $\tilde{\Omega}(\sqrt{n})$ for a graph of radius $\hopDiameter{G} = O(\log n)$. This can be seen by the following construction of the input graph $H$ and the network graph $G \supseteq H$. Let $H = \sqrt{n}C_{\sqrt{n}}$, that is, $H$ consists of $\sqrt{n}$ cycles $C_1, C_2,  \dots C_{\sqrt{n}}$, each of length $\sqrt{n}$. 
Let $V_0, V_1, \dots, V_{\sqrt{n}/2}$ be a partition of $V(H)$ defined as follows. $V_0$ is an arbitrary set of $\sqrt{n}$ nodes such that it contains exactly one node from each cycle $C_i$. 
Next, for $i > 0$ we define  $V_i$  as the set of nodes of distance $i$ from $V_0$. 
The network graph $G \supseteq H$ moreover contains the following additional nodes and edges. First, we build a binary tree on top of each $V_i$ (that is, $V_i$ are the leaves of the tree) and then an additional binary tree on top of the roots of these trees. This defines $G$. 
The graph $G$ contains $O(n)$ nodes and its diameter is $O(\log n)$. On the other hand, we believe one can mimic the well-known lower bound of \cite{sarma2012distributed} to prove that $\tilde{\Omega}({\sqrt{n}})$ rounds are needed to orient all cycles consistently.  
\end{remark}

==> Deterministic_SSSP/introduction.tex <==
\section{Introduction}\label{sec:intro}

This paper gives essentially near-optimal\footnote{We refer to optimality up to polylogarithmic factors as \emph{near-optimality}, while \emph{almost-optimality} refers to optimality up to subpolynomial, i.e., $n^{o(1)}$, factors.} deterministic parallel algorithms for various $(1+\eps)$-approximate shortest-path-type problems in undirected weighted graphs. These problems include computing $(1+\eps)$-approximate shortest paths or shortest path trees from a single source (shortened to $(1+\eps)$-SSSP) and $(1 + \eps)$-approximate minimum transshipment (shortened to $(1+\eps)$-transshipment). Our algorithms run in polylogarithmic time and require near-linear work. This is optimal up to polylogarithmic factors. All prior parallel deterministic algorithms with polylogarithmic depth for $(1+\eps)$-SSSP required $n^{\Theta(1)}$ more work and, to our knowledge, no sub-quadratic work NC algorithm was known for $(1+\eps)$-transshipment. We also give deterministic distributed algorithms for the above problems, including the first non-trivial distributed deterministic $(1+\eps)$-transshipment algorithm. 

Computing a single-source shortest path is one of the most fundamental problems in combinatorial optimization. Already in 1956, Dijkstra \cite{dijkstra1959dijkstra} gave a simple deterministic $O(m \log n)$ time algorithm for computing an exact single-source shortest path tree in any directed graph. Parallel and distributed algorithms on the other hand have been subject of over three decades of extensive research \cite{ullman1991high,cohen1994polylog,klein1997randomized,spencer1997time,galil1997all,alon1997exponent,zwick1998all,shi1999time,Nan14,EN16,henzinger2016almost,BKKL17,Elk17,elkin2017linearsize,FN18,GL18,haeuplerLi2018sssp,elkin2019hopsets,EN19,henzinger2019deterministic,LPP19,CM20,elkinMatar2021detPRAMSSSP,goranci2022universally} with much remaining unknown. Much recent research has focused on $(1+\eps)$-approximate shortest paths in undirected graphs, the problem solved in this paper. We provide a detailed summary of this prior work next and describe related work on SSSP algorithms in other computational models or on other related problems, including all-pair-shortest-path and SSSP in directed graphs, in \Cref{sec:morerelatedwork}. We focus on randomized and deterministic parallel algorithms with polylogarithmic depth, i.e., RNC and NC algorithms. 

\paragraph{Parallel Algorithm.}
The \pram model of parallel computation was introduced in 1979. After a decade of intense study, Karp and Ramachandran noted in their influential 1989 survey on parallel algorithms~\cite{karp1989survey} that the ``transitive closure bottleneck'' for shortest-path-type problem required work ``far in excess of the time required to solve the problem sequentially''. Indeed, these algorithms build on matrix multiplication or on transitive closure routines and require $O(n^{3})$ work. A line of work \cite{ullman1991high,klein1997randomized,spencer1997time,cohen1997using,shi1999time} provided algorithms with different work-time trade-offs but without much improvement on the cubic work bound for fast parallel algorithms. 


% \begin{comment}
% Previous:

% Indeed, all algorithms build on matrix multiplication or transitive closure routines with $O(n^{3})$ work\alert{not sure what this sentence is supposed to say}. 
% Algorithms by  [UY91, KS97, Spe97, SS99] gave randomized algorithms with different processor-time tradeoffs but without much improvement on the cubic work bound for fast parallel algorithms. [Coh97] gave a deterministic algorithm with similar tradedoffs. [GM97, AGM97, Zwi98] gave algorithm with work equal to $\tO(m^{\omega})$, where $\omega < 2.37\ldots$ is the fast matrix multiplication exponent~\cite{}. 
% \end{comment}





In a major breakthrough, Cohen~\cite{cohen1994polylog} gave a randomized $(1 + \eps)$-SSSP algorithm based on hopsets with $\tO_\rho(1)$ time and $O(m^{1+\rho})$ work for any constant $\rho > 0$. Algorithms with slightly improved time-work tradoffs were given~\cite{elkin2017linearsize,elkin2019hopsets} but these algorithms still required a polynomial $m^{\rho}$ factor more work than Dijkstra's algorithm to parallelize shortest path computations to polylogarithmic parallel time. 
%On the other hand, using modern methods from continuous optimization \cite{She13,BKKL17,She17b}, recent algorithms 

This remained the state-of-the-art until 2020 when methods from continuous optimization developed by Sherman~\cite{She13,She17b} enabled further progress on shortest-path type problems. In particular, Sherman gave an $m \cdot n^{o(1)}$ sequential algorithm for the $(1+\eps)$-approximate minimum transshipment problem. \emph{Transshipment}, also known as uncapacitated min-cost flow, Wasserstein distance, or optimal transport, is the other major problem solved in this paper. The input to the transshipment problem on some weighted graph $G$ consists of a \emph{demand} $b$ which specifies for each node a positive or negative demand value with these values summing up to zero. The goal is to find a flow of minimum cost which sends flow from nodes with surplus to nodes with positive demands. Here the cost of routing a unit of flow over an edge is proportional to the weight/length of the edge. For example, an optimal transshipment flow for a demand with $b(s)=-1$ and $b(t)=1$ is simply a unit flow from $s$ to $t$ which decomposes into a distribution over shortest $(s,t)$-paths. We remark that transshipment is in many ways a powerful generalization of shortest-path problems, including computing SSSP (trees), with the exception that extracting trees or paths from a continuous transshipment flow often remains a hard problem itself which requires highly nontrivial rounding algorithms. While having an innocent feel to them, such rounding steps have a history of being inherently randomized and being algorithmic bottlenecks for shortest-path problems on several occasions. 

Sherman's almost-linear time transshipment algorithm did not imply anything new for SSSP at first, but it inspired two independent approaches by \cite{Li20} and Andoni, Stein, and Zhong \cite{AndoniSZ20} that led to near-optimal randomized parallel shortest path algorithms with polylogarithmic time and near-linear work. In particular, Li~\cite{Li20} improved several parts of Sherman's algorithm and combined it with the vertex-reduction framework that Peng~\cite{Pen16} had introduced to give the first near-linear time algorithm for $(1+\eps)$-maximum-flow. \cite{Li20} also adopts a randomized rounding algorithm of \cite{BKKL17} based on random walks to extract approximate shortest-path trees from transshipment flows. Overall, this results in randomized PRAM algorithms for both $(1+\eps)$-transshipment and $(1+\eps)$-SSSP with polylogarithmic time and near-linear work.
%We give a more detailed description of this in \alert{???}\Cref{???}.
Concurrently, Andoni, Stein, and Zhong \cite{AndoniSZ20} achieved the same result for $(1+\eps)$-transshipment by combining Sherman's framework with ideas from hop-sets. They also provide a randomized rounding based on random walks algorithm that can extract an $s$-$t$ shortest path. Later, this rounding was extended in Zhong's thesis~\cite{zhong2021new} to extract the full $(1+\eps)$-SSSP tree. 

It is remarkable that all parallel $(1+\eps)$-SSSP algorithms described above (with the exception of the super-quadratic work algorithms before Cohen's 25 year old breakthrough) crucially rely on randomization for efficiency. Indeed, the only modern deterministic parallel $(1+\eps)$-SSSP algorithm is a very recent derandomization of Cohen's algorithm by Elkin and Matar~\cite{elkinMatar2021detPRAMSSSP}. This algorithm suffers from the familiar $O(m^{1+\rho})$ work bound for a polylogarithmic time parallel algorithm. For the $(1+\eps)$-transshipment problem even less is known. Indeed we are not aware of any efficient deterministic parallel algorithm before this work and would expect that much larger polynomial work bounds would be required to achieve a deterministic algorithm with polylogarithmic parallel time.

In this paper, we give deterministic parallel algorithms for both the $(1 + \eps)$-SSSP and the $(1+\eps)$-transshipment problem in undirected weighted graphs. Both algorithms only require near-linear work and run in polylogarithmic time. This solves these two and various other shortest-path-type problems optimally, up to polylogarithmic factors. 

\begin{restatable}[Deterministic Parallel SSSP and Transshipment]{theorem}{mainparallel}
\label{thm:main_parallel}
There is a deterministic parallel algorithm that, given an undirected graph with nonnegative weights, computes a $(1+\eps)$-approximate single-source shortest path tree or a $(1+\eps)$-approximation to minimum transshipment in $\tO(m \cdot \eps^{-2})$ work and $\tO(1)$ time in the \pram model for any $\eps \in (0,1]$.
\end{restatable}

\paragraph{Distributed Algorithm.}
We also give new distributed $(1+\eps)$-SSSP and $(1+\eps)$-transshipment algorithms in the standard \congest model of distributed computing. 
For distributed algorithms a lower bound of $\Omega(\sqrt{n} + \Dhop)$ rounds is known for worst-case topologies~\cite{elkin2006unconditional,sarma2012distributed}, where $\Dhop$ is the unweighted (i.e., hop) diameter of the network. We refer to this as the \emph{existential lower bound} since it depends on the parameterization by $(n, \Dhop)$, as opposed to the later-discussed \emph{universal lower bound} which does not.

In his 2004 survey on distributed approximation, Elkin~\cite{elkin2004distributed} pointed to the distributed complexity of shortest paths approximations as one of two fundamental and wide-open problems in the area---as no non-trivial algorithms complementing the above lower bounds were known.

Since then, the $(1+\eps)$-SSSP problem is one of the most studiedonly give a brief summary here: Lenzen and Patt-Shamir gave an $\tO(n^{1/2 + \eps} + \Dhop)$-round $O(1 + \frac{\log 1/\eps}{\eps})$-SSSP algorithm \cite{lenzen2013fast} and a $(1+o(1))$-approximation in $\tO(n^{1/2}\cdot \Dhop^{1/4}+\Dhop)$ rounds was given by Nanongkai \cite{Nan14}. 
Building on Sherman's transshipment framework mentioned before, \cite{BKKL17} gave a randomized $\tO(\eps^{-3} \cdot (\sqrt n + \Dhop))$ algorithm.
The first algorithm improving over the $\Omega({\sqrt{n}})$ barrier was given in \cite{haeuplerLi2018sssp} with a running time of $\shortcutQuality{G} \cdot n^{o(1)}$ albeit with a bad $n^{o(1)}$-approximation. 
This was recently improved by \cite{goranci2022universally} to a $(1+\eps)$-approximation with the same round complexity. 
Using \cite{ghaffari_haeupler2021shortcuts_in_minor_closed}, this gives a $(1+\eps)$-approximation algorithm with round complexity $\Dhop \cdot n^{o(1)}$ for any excluded minor topology (e.g., planar graphs). 
All the above algorithms are randomized: The only deterministic distributed algorithm is the $(1 + o(1))$-SSSP algorithm of \cite{henzinger2019deterministic} with a $(n^{1/2+o(1)} + \Dhop^{1+o(1)})$ running time. For $(1+\eps)$-transshipment, the only known sublinear distributed algorithm is the randomized $\shortcutQuality{G} \cdot n^{o(1)}$-round algorithm of \cite{goranci2022universally}. No non-trivial  deterministic distributed $(1+\eps)$-transshipment algorithm (with sub-linear round complexity) was known prior to this work.

The distributed results of this paper include deterministic distributed algorithms for $(1+\eps)$-SSSP, its generalization $(1+\eps)$-\setssp (in which we are looking for distances from a subset of nodes), and  $(1+\eps)$-transshipment. Our results improve over the previous best running times of deterministic distributed algorithms for each of the above problems, both in the worst-case and for any excluded minor graph. Both the round and the message complexities (in $KT_0$, see \cite{peleg2000distributed} for the definition) of our algorithms are (existentially) optimal, up to $\poly\log n$ factors, in all cases. 
%The algorithm solves the more general version of the problem where the source of the shortest path computation is an arbitrary set of nodes. 

%as well as a universally optimal distributed algorithm if the topology is known. (this is actually not easily doable because we need fast deterministic routing, too. Technically one can achieve this using deterministic semi-oblivious routing but the local computations would be exponential time if one would want them to be deterministic. LOL

\begin{restatable}[Deterministic Distributed SSSP and Transshipment]{theorem}{maindistributed}
\label{thm:main_distributed}
There is a deterministic \congest algorithms that, given an undirected graph with non-negative weights, compute a $(1+\eps)$-approximate \setssp forest or a $(1+\eps)$-transshipment solution for any $\eps \in (0,1]$. Our algorithms have an optimal message complexity of $\tO (m) \cdot  \eps^{-2}$ and are guaranteed to terminate in at most 
\begin{enumerate}
    \item within at most $\tO(\sqrt{n} + \Dhop) \cdot \eps^{-2}$ rounds and
    \item within at most $\tO(\Dhop) \cdot  \eps^{-2}$ rounds if $G$ does not contain any $\tO(1)$-dense minor.
\end{enumerate}
%Here, $\Dhop$ is the hop diameter of $G$. 
\end{restatable}

%Our results are the first deterministic $(1+\eps)$-SSSP for excluded minor graphs and even improve the randomized complexity for these graphs. In terms of worst-case complexity, we improve the running time of the best deterministic algorithm of \cite{Nan14} to near-optimal, matching the time of the fastest randomized algorithm of \cite{BKKL17}.

\underline{Universal optimality.} Recently, the pervasive $\tilde{\Omega}(\Dhop + \sqrt{n})$ distributed lower bounds have been extended to a near-tight universal lower bound~\cite{haeupler2021universally} which shows that most optimization problems including all problems studied in this paper require $\tilde{\Omega}(\shortcutQuality{G})$ rounds on any communication graph $G$. Here $\shortcutQuality{G}$ is a natural graph parameter (we refer the interested reader to \cite{haeupler2021universally} for a formal definition). For experts interested in universally-optimal distributed algorithms we remark that the results of this paper imply strong conditional results. We state these results for the interested reader in \Cref{sec:main_theorems}. 



%In summary, this is the first deterministic distributed algorithm for excluded minor graph and simultaneously improves the running time to optimal up to polylog n factors compared to the best randomized algorithm. In terms of worst-case complexity this improved the running time of the best det algorithm of Nan to near optimal, matching the time of the near-optimal randomized algorithm of becker.



\subsection{Technical Overview}

\begin{figure}
    \centering
    \includegraphics[width = \textwidth]{fig/main.eps}
    \caption{This figure summarizes our approach with our contributions marked in red. It is known that a $\tO(1)$-competitive solution to $\ell_1$-oblivious routing can be boosted to a $(1+\eps)$-approximate transshipment which can then be rounded to yield a $(1+\eps)$-approximate SSSP tree. We close the circle of reductions by constructing certain distance structures from the approximate SSSP tree. Think of those distance structures as a family of clusterings on different scales, storing some additional distance information. One of our main technical contributions is the efficient construction of a $\tO(1)$-approximate oblivious routing from the distance structures, which closes the loop. \\
    This loop of reductions itself is not very useful as the complexity of the problems does not decrease. 
    We break this loop by our \emph{distance reduction} framework by showing one can construct distance structures ``up to distance $D$'' using distance structures ``up to distance $D /\poly\log n$. 
    %, we construct $\ell_1$-oblivious routing up to the larger distance $D$, which enables us to construct (in order) approximate transshipment, SSSP tree, and finally distance structures up to distance $D$. 
    %The notion of ``up to distance $D$'' is formalized by adding the virtual \emph{cheating node} connecting to all other nodes via an edge of length $D$. 
    After $O(\log n)$ iterations, we build up the desired solution to any of the four problems, in particular to approximate transshipment and set-SSSP. }
    \label{fig:main}
\end{figure}


While the results for SSSP and transshipment are important, the main impact of this paper will likely be the new tools and algorithmic ideas developed in this paper. We expect these ideas to be applicable beyond shortest path problems. Next, we give a brief summary of the most relevant parts and ideas of prior work which are needed to understand our work and put in proper context. We then give an informal high-level overview of our new algorithm and some of the new tools developed for it. A readable and more precise technical proof overview is given in \Cref{sec:localiterative}.

\subsubsection{Background and Prior Work}

{\bfseries Transshipment Boosting, $\ell_1$-Oblivious Routing, and Transshipment Flow Rounding} \\
All modern SSSP-algorithms, including ours, compute shortest paths via the transshipment problem (see text before \Cref{thm:main_parallel} for a definition). The key idea in this approach of Sherman~\cite{She13, She17b} is that even a rather bad $\alpha$-approximation algorithm for (dual) transshipment can be \emph{boosted} to a $(1+\eps)$-approximation. This is achieved via the multiplicative weights method (or equivalently: gradient descent) and requires only $\poly(\alpha, \eps^{-1}, \log n)$ invocations of the $\alpha$-approximation algorithm~\cite{She17b,BKKL17,zuzic2021simple}. A particularly convenient way of obtaining such a boostable $\alpha$-approximation is to design a linear matrix $R$ which maps any node-demand $b$ to an $\alpha$-approximate transshipment flow for $b$. Such a matrix is called an $\ell_1$-oblivious routing because linearity forces each node to route its demand obliviously, i.e., without knowledge of the demand on other nodes. As mentioned before, in order to obtain an actual $(1+\eps)$-SSSP tree from a transshipment flow most algorithms~\cite{Li20} are using an approach of \cite{becker2019low} which produces a $(1+\eps)$-SSSP tree after $O(\log n)$ adaptive applications of some rounding algorithm. All parts of this reduction except for the rounding algorithm are deterministic.

Putting all these pieces together proves that all one needs to obtain an efficient (deterministic) algorithm for both the  $(1+\eps)$-transshipment and the $(1+\eps)$-SSSP problem is a $\tO(1)$-competitive $\ell_1$-oblivious routing that can be evaluated efficiently and a (deterministic) rounding algorithm. Our algorithm uses these steps in a black-box fashion except that we need to replace the randomized rounding algorithm by a new deterministic transshipment flow rounding procedure. 

%our SSSP algorithm 

%The works that are most closely related to the algorithm presented here are the works of \cite{Li20,goranci2022universally}, which in turn build on multiplicative-weight boosting, pre-conditioning with $\ell_1$-routing, the vertex-reduction framework of Peng~\cite{Pen16}, and the Minor-Aggregations framework. We give a brief overview over the relevant parts of these prior works, some of which our algorithm utilizes in a black-box manner.

%{\bfseries SSSP via Transshipment, Multiplicative-Weight Boosting of Transshipment}\\
%Like all modern SSSP algorithms, we use the framework of Sherman~\cite{She13, She17b} which proceeds by reducing the problem to transshipment.
% This calls for solving a generalized continuous version of shortest paths---the transshipment problem (also called uncapacitated min-cost flow, Wasserstein distance, or optimal transport). The input to the problem is a weighted graph $G$ and a so-called \emph{demand vector} $b : V(G) \to \R$ satisfying $\sum_{v \in V(G)} b(v) = 0$. The goal is to find a flow of minimum cost that satisfies the demand $b$ (i.e., the inflow minus outflow at $v$ should equal $b(v)$).
%Transshipment clearly generalizes the $s$-$t$ shortest path problem since the min-cost solution satisfying the demand $b = \mathbb{1}_s - \mathbb{1}_t$ is the $s$-$t$ shortest path. Albeit more involved, transshipment also generalizes SSSP if one is given a rounding procedure which transforms the fractional flow to an integral one supported on a tree.

%The key feature exploited in all modern SSSP approaches is that an $\alpha$-approximation algorithm for (dual) transshipment can be \emph{boosted} to a $1+\eps$ approximation. This is achieved via gradient descent or, equivalently, the multiplicative weights method, using only $\poly(\alpha, \eps^{-1}, \log n)$ invocations of the $\alpha$-approximation algorithm~\cite{She17b,BKKL17,zuzic2021simple}. A particularly convenient way of obtaining an $\alpha$-approximate dual solution is to design a linear $\ell_1$-oblivious $\alpha$-competitive routing, described below. 


%In summary, it is sufficient to design any $\tO(1)$-competitive $\ell_1$-oblivious routing to near-optimally solve $(1+\eps)$-approximate transshipment, which can then be rounded to a solution for $(1+\eps)$-SSSP.

%{\bfseries Graph Based $\ell_1$-oblivious routing}\\
%Given a weighted graph $G$, the $\ell_1$-oblivious routing $R$ is a linear map (matrix) which maps a demand $b : V(G) \to \R$ to a flow $f := R b$ which is an approximately-optimal solution to the corresponding transshipment problem (satisfying demand $b$ on $G$). The routing has the adjective \emph{oblivious} since its linearity forces each node $v$ to route $v$'s demand without knowledge of the demand on other nodes. The goal in this paper is to design a deterministic routing that achieves a $\tO(1)$ approximation for all demands, while still allowing efficient evaluations.


%Othisne natural candidate for an $\ell_1$-oblivious routing would be to sample a probabilistic tree embedding of $G$ with $O(\log n)$-distance distortion and let each node route its demand to the root. This is a valid linear map and can be evaluated fast. Moreover, it is easy to see that the cost of the resulting flow is $O(\log n)$-competitive \emph{in expectation} with the optimal transshipment solution.

% The approximation is furthermore $O(\log n)$ in expectation if the demand is chosen independently from the randomness used to construct the map, which is provably best possible.

%Unfortunately, such a guarantee in expectation is not enough for the MW-boosting framework, as a valid $\alpha$-competitive routing needs to be competitive \emph{for all} demands. To boost the guarantee from an expected guarantee to a worst-case (for all) guarantee one can sample multiple linear maps as above and define $R$ to be the average. This can result in the desired deterministic approximation guarantee but only if linearly many samples are taken, leading to a quadratic time for construction and evaluation. There has thus been a consensus that such an approach cannot be made to work. 

\begin{comment}
All previous parallel approaches to construct a high-quality oblivious routing relied on first computing an $\ell_1$-embedding, which is a mapping from the nodes of a graph to vectors in $\ell_1$ such that the distances are approximately preserved, and then performing the routing in the (significantly simpler) $\ell_1$-space. This includes the approaches of Sherman~\cite{She17b}, Li~\cite{Li20}, Andoni, Stein, and Zhong~\cite{AndoniSZ20}, etc.
\end{comment}

% The drawback of this scheme is that the known $\ell_1$-embeddings are inherently randomized and that the routing and flow obtained are in the auxiliary (virtual) $\ell_1$-space. It is not clear how to obtain a flow in $G$ from this. Fortunately, merely a vector whose $\ell_1$-norm approximates the optimal transshipment flow cost is needed for the boosting framework.

%Instead, the $\ell_1$-oblivious routings of , are based on first computing an $\ell_1$-embedding and then performing an $\ell_1$-oblivious routing in this $\ell_1$-space, which is much easier. 

\begin{comment}
A very recent paper~\cite{goranci2022universally} showed that a simple graph-based $n^{o(1)}$-competitive $\ell_1$-oblivious routing could be directly defined on the network $G$ by using only a simple randomized graph decomposition primitive called \emph{low-diameter decomposition}. Unfortunately, many barriers prevent this approach from achieving a polylog-competitive routing even if one does not require deterministic algorithms. This paper builds upon their approach and develops the necessary tools and ideas to both yield polylog-competitiveness and deterministic guarantees of the routing.
\end{comment}

% $n^{o(1)}$ many low-diameter decompositions of exponentially increasing radii. Luckily, low-diameter decompositions (of super-low, $n^{o(1)}$, quality) can be computed in $n^{o(1)}$ minor aggregation steps using the algorithm of Haeupler and Li \cite{HL18}, which is basically following the simple pioneering approach of Alon et al.~\cite{alon1995graph}. The advantages of the approach of \cite{goranci2022universally} are that they work well with the \aggregate framework, that the routing matrix is simple, and directly maps to a flow in $G$ (rather than an auxiliary space). Unfortunately, this approach is fundamentally unable to achieve a $n^{o(1)}$-competitive routing even before attempting derandomization, even if one is given an oracle which constructs (optimal) $O(\log n)$-quality low-diameter decompositions. We develop many new tools in this paper in order to achieve this goal.


{\bfseries Vertex Reduction Framework}\\
Unfortunately, it is clear that $\ell_1$-oblivious routing cannot be done without having some approximate shortest path information. This chicken and egg problem is resolved via a clever vertex-reduction framework of Li~\cite{Li20}.  % first introduced by Peng~\cite{Pen16} for solving max-flow, i.e., the $\ell_\infty$ analog of SSSP / transshipment, and adapted to the transshipment setting by Li~\cite{Li20}. 
The vertex-reduction framework relies on a cyclic sequence of efficient problem reductions. For transshipment~\cite{Li20}, these problems are SSSP, transshipment, $\ell_1$-oblivious routing, and $\ell_1$-embedding. Specifically:
\begin{itemize}
\item To solve $(1+\eps)$-SSSP on $G$, it is sufficient to solve $(1+\eps)$-transshipment on $G$, 
\item for which it is sufficient to construct $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing on $G$ (via boosting),
\item for which it is sufficient to construct an $\tilde{O}(1)$-distortion $\ell_1$-embedding on $G$,
\item for which it is sufficient to solve $O(\log^2 n)$ instances of $\tilde{O}(1)$-SSSP on a sequence of graphs $G'_1, G'_2, \ldots, G'_{O(\log^2 n)}$, which are resolved recursively.
\end{itemize}
As stated, this simply reduced $(1+\eps)$-SSSP on $G$ to multiple $\tilde{O}(1)$-SSSP on graphs that are slightly larger than $G$, which isn't particularly helpful on its own. The key idea to transform this ``branching cycle'' into a branching spiral that terminates (fast) is to add a step into the cycle which applies ultrasparsification on $G'_i$, which is an operation that transforms a graph with $n$ nodes to a smaller graph with $\frac{n}{\gamma}$ nodes such that distances in the smaller graph $\tilde{O}(\gamma)$-approximate distances in the larger graph. Applying this step, we can reduce $(1 + \eps)$-SSSP on a graph with $n$ nodes to $O(\log^2 n)$ instances of $\tilde{O}(1)$-SSSPs on smaller graphs with $O\left(\frac{n}{\log^{100} n}\right)$ nodes. It is easy to see that the total size of all recursive calls falls exponentially on each subsequent level, hence the total parallel runtime is $\tilde{O}(1)$ and the total work $\tilde{O}(m)$ (since a single sequence of reductions requires $\tilde{O}(m)$ work).

%The issues with this approach is that (1) there are currently no known deterministic constructions of $\ell_1$-embeddings, and (2) the oblivious routing in the $\ell_1$-space is inherently hard to convert to a small number of minor aggregations (see below), leading to algorithms that are not appropriate for the distributed setting. \alert{mention somewher that this is performed on different graphs}

% Several of these reductions are losing polylogarithmic factors in approximation, but these turn into polylogarithmic increases in running time thanks to boosting. The key idea to transform this branching cycle into a branching spiral that terminates (fast) is to add a step into the cycle which applies ultrasparsification followed by vertex-sparsification. The two sparsification procedures used in this step replace the $n$-node graph $G$ by a graph $H$ with a $\frac{n}{\gamma}$ nodes for any polylogarithmic $\gamma$ while still approximating $G$ up to polylogarithmic factors. \todo{What does approximating mean in that context?}The loss in approximation is again removed with the boosting step. While a single SSSP on $G$ now still generates some $\beta = O(log^2 n)$ recursive SSSP calls, these SSSP calls are on \emph{on smaller graphs} with $\frac{n}{\gamma}$ nodes.

% The overall time complexity for these recursive calls satisfies the recurrence relation $T(n) = \beta T(n/\gamma) + \tO(n)$ which is easily seen to resolve to $T(n)=\tO(n)$ when $\gamma$ is chosen to be at least a constant factor larger than $\beta$.

% Figure 1 gives a slightly rearranged description of the algorithm of Li:

% $(1+eps)$-SSSP on G    



\iffalse

{\bfseries Vertex Reduction Framework}\\
The main problem with reducing $(1+\eps)$-SSSP to $\ell_1$-oblivious routing is that some non-trivial shortest path information is clearly necessary to route a flow $\tO(1)$-competitively. \cite{Li20} resolves this chicken and egg problem via the vertex-reduction framework of Peng~\cite{Pen16}. First a cyclic sequence of efficient problem reductions is established and then the cyclicity is broken up by introducing an ultra-sparsification and vertex reduction step. Overall one SSSP call on $G$ is reduced to $\tO(1)$ SSSP calls on smaller graphs $G_1, G_2, \ldots$ whose sizes sum up to at most $|G|/2$. Each $G_1$ is essentially a minor of $G$.


Starting with an SSSP algorithm Li produces uses $\tO(1)$ recursive calls to this SSSP algorithm to compute Bourgain's randomized $\tilde{O}(1)$-distortion $\ell_1$-embedding he then uses an ultra sparsification step to 

on $G$

Starting with the above mentioned reductions from SSSP via transshipment to $\ell_1$-oblivious routing Li add the following steps
\begin{itemize}
\item $\ell_1$-oblivious routing is reduced to 


To solve $(1+\eps)$-SSSP on $G$, it is sufficient to solve $(1+\eps)$-transshipment on $G$, 
\item for which it is sufficient to construct $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing on $G$ (via boosting),
\item for which it is sufficient to construct an $\tilde{O}(1)$-distortion $\ell_1$-embedding on $G$,
\item for which it is sufficient to solve $O(\log^2 n)$ instances of $\tilde{O}(1)$-SSSP on a sequence of graphs $G'_1, G'_2, \ldots, G'_{O(\log^2 n)}$, which are resolved recursively.
\end{itemize}


shows how to reduce t

, G'_{O(\log^2 n)}$

result in 



. For transshipment~\cite{Li20}, these problems are SSSP, transshipment, $\ell_1$-oblivious routing, and $\ell_1$-embedding. Specifically:
\begin{itemize}
\item To solve $(1+\eps)$-SSSP on $G$, it is sufficient to solve $(1+\eps)$-transshipment on $G$, 
\item for which it is sufficient to construct $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing on $G$ (via boosting),
\item for which it is sufficient to construct an $\tilde{O}(1)$-distortion $\ell_1$-embedding on $G$,
\item for which it is sufficient to solve $O(\log^2 n)$ instances of $\tilde{O}(1)$-SSSP on a sequence of graphs $G'_1, G'_2, \ldots, G'_{O(\log^2 n)}$, which are resolved recursively.
\end{itemize}


This chicken and egg problem is resolved via a clever vertex-reduction framework of Li~\cite{Li20}.

it is pretty clear 


\begin{comment}
All previous parallel approaches to construct a high-quality oblivious routing relied on first computing an $\ell_1$-embedding, which is a mapping from the nodes of a graph to vectors in $\ell_1$ such that the distances are approximately preserved, and then performing the routing in the (significantly simpler) $\ell_1$-space. This includes the approaches of Sherman~\cite{She17b}, Li~\cite{Li20}, Andoni, Stein, and Zhong~\cite{AndoniSZ20}, etc.
\end{comment}

t induces 


Unfortunately, it is clear that $\ell_1$-oblivious routing cannot be done without having some approximate shortest path information. This chicken and egg problem is resolved via a clever vertex-reduction framework of Li~\cite{Li20}.  % first introduced by Peng~\cite{Pen16} for solving max-flow, i.e., the $\ell_\infty$ analog of SSSP / transshipment, and adapted to the transshipment setting by Li~\cite{Li20}. 
The vertex-reduction framework relies on a cyclic sequence of efficient problem reductions. For transshipment~\cite{Li20}, these problems are SSSP, transshipment, $\ell_1$-oblivious routing, and $\ell_1$-embedding. Specifically:
\begin{itemize}
\item To solve $(1+\eps)$-SSSP on $G$, it is sufficient to solve $(1+\eps)$-transshipment on $G$, 
\item for which it is sufficient to construct $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing on $G$ (via boosting),
\item for which it is sufficient to construct an $\tilde{O}(1)$-distortion $\ell_1$-embedding on $G$,
\item for which it is sufficient to solve $O(\log^2 n)$ instances of $\tilde{O}(1)$-SSSP on a sequence of graphs $G'_1, G'_2, \ldots, G'_{O(\log^2 n)}$, which are resolved recursively.
\end{itemize}
As stated, this simply reduced $(1+\eps)$-SSSP on $G$ to multiple $\tilde{O}(1)$-SSSP on graphs that are slightly larger than $G$, which isn't particularly helpful on its own. The key idea to transform this ``branching cycle'' into a branching spiral that terminates (fast) is to add a step into the cycle which applies ultrasparsification on $G'_i$, which is an operation that transforms a graph with $n$ nodes to a smaller graph with $\frac{n}{\gamma}$ nodes such that distances in the smaller graph $\tilde{O}(\gamma)$-approximate distances in the larger graph. Applying this step, we can reduce $(1 + \eps)$-SSSP on a graph with $n$ nodes to $O(\log^2 n)$ instances of $\tilde{O}(1)$-SSSPs on smaller graphs with $O\left(\frac{n}{\log^{100} n}\right)$ nodes. It is easy to see that the total size of all recursive calls falls exponentially on each subsequent level, hence the total parallel runtime is $\tilde{O}(1)$ and the total work $\tilde{O}(m)$ (since a single sequence of reductions requires $\tilde{O}(m)$ work).

%The issues with this approach is that (1) there are currently no known deterministic constructions of $\ell_1$-embeddings, and (2) the oblivious routing in the $\ell_1$-space is inherently hard to convert to a small number of minor aggregations (see below), leading to algorithms that are not appropriate for the distributed setting. \alert{mention somewher that this is performed on different graphs}

% Several of these reductions are losing polylogarithmic factors in approximation, but these turn into polylogarithmic increases in running time thanks to boosting. The key idea to transform this branching cycle into a branching spiral that terminates (fast) is to add a step into the cycle which applies ultrasparsification followed by vertex-sparsification. The two sparsification procedures used in this step replace the $n$-node graph $G$ by a graph $H$ with a $\frac{n}{\gamma}$ nodes for any polylogarithmic $\gamma$ while still approximating $G$ up to polylogarithmic factors. \todo{What does approximating mean in that context?}The loss in approximation is again removed with the boosting step. While a single SSSP on $G$ now still generates some $\beta = O(log^2 n)$ recursive SSSP calls, these SSSP calls are on \emph{on smaller graphs} with $\frac{n}{\gamma}$ nodes.

% The overall time complexity for these recursive calls satisfies the recurrence relation $T(n) = \beta T(n/\gamma) + \tO(n)$ which is easily seen to resolve to $T(n)=\tO(n)$ when $\gamma$ is chosen to be at least a constant factor larger than $\beta$.

% Figure 1 gives a slightly rearranged description of the algorithm of Li:

% $(1+eps)$-SSSP on G    

% can be computed via log n calls to TS+randomized rounding which can all be answered using a single $\ell_1$-oblivious routing matrix of in G  (this is the boosting framework)

% $O(log^6 n)$-competitive $\ell_1$-oblivious routing matrix of G    

% using the two sparsification procedures the problem of finding an $\ell_1$-oblivious routing matrix of G can be reduced to finding an $\ell_1$-oblivious routing matrix for a graph H with $O(\frac{n}{100 log^2 n})$ nodes.

% $O(log^2 n)$-approx $\ell_1$-oblivious routing matrix of H

% Li showed that an $\ell_1$-oblivious routing can be computed using an $O(log^? n)$-distortion $\ell_1$-embedding of $H$. Such an $\ell_1$-embedding can be computed using Bourgains embedding which requires $\beta = O(log^2 n)$ calls to S-set-source shortest paths on $H$ for different vertext sets $S_1,S_2,\ldots,S_\beta$. These can be computed via single-source shortest path computations on the $\beta$ different graphs $H_i$ for $i \in [\beta]$, where $H_i$ is the graph $H$ plus one extra node $s$ connected to all nodes in $S_i$ via a short or zero length edges. 

% (1+eps)-SSSP on $H_1,H_2,\ldots,H_{\beta}$ with at most $\frac{n}{\gamma}$ nodes each
\fi

{\bfseries Minor Aggregates and the Low-Congestion Shortcuts Framework}\\
The low-congestion shortcuts framework was originally intended for designing simple and efficient \emph{distributed} graph algorithms and was developed over a long sequence of works~\cite{GH16,haeupler2016low,haeupler2016near,haeupler2018round,haeupler2018minor,ghaffari_haeupler2021shortcuts_in_minor_closed,haeupler2021universally,kogan2021low,ghaffari2021hop,GHR21}. However, this paper argues that the framework provides a natural language even for developing fast parallel algorithms. Indeed, we present our parallel SSSP algorithm using the framework and our hope is that this choice simplifies the exposition, even before considering the benefits of immediately obtaining distributed results.

We describe our algorithms in the recently introduced \aggregate model~\cite{goranci2022universally, ghaffari2021universally}, which offers an intuitive interface to the recent advancements in the low-congestion shortcut framework. In the \aggregate model, one can (1) contract edges, thereby operating a minor, (2) each (super)node in the contracted graph can compute an aggregate (e.g., min, max, sum) of surrounding neighbors, and (3) add $\tilde{O}(1)$ arbitrarily-connected virtual nodes over the course of the algorithm. The goal is to design $\tO(1)$-round algorithms in this model. Such a \aggregate algorithm can be compiled to a near-optimal algorithm in both the parallel and distributed settings.

% Note that computing a partwise aggregate is basically same as computing a node-wise aggregate in the minor in which each part is contracted. Any algorithm that uses some $k$ rounds of contractions and node-aggregation on the resulting minors thus directly translates into an algorithm with $\tilde{O}(k)$ partwise aggregations on $G$ (the different interfaces or partwise and minor aggregations account for the $\tilde{O}(1)$ overhead). Our goal is to design $\poly\log n$-round \aggregate algorithms, which immediately yield polylog-depth and near-linear-work parallel algorithms, and universally-optimal distributed algorithms. \Cref{sec:minoraggregatemodel} summarizes this model which we use throughout this paper.


\subsubsection{Our New Tools}

%Our first two tools are interesting beyond the problem of derandomization and we introduce them in a probabilistic language which is more intuitive. \alert{?!?!}

{\bfseries Near-Optimal Graph-Based $\ell_1$-oblivious routing}\\
The first key contribution of this paper is a new construction of graph-based $\ell_1$-oblivious routing with drastically improved guarantees from the so-called sparse neighborhood covers. A sparse neighborhood cover of distance scale $D$ is a collection of $O(\log n)$ clusterings (partitioning of the node set into disjoint \emph{clusters}) such that (1) each cluster has diameter at most $D$, and (2) each ball in $G$ of radius $D / (\log^{C} n)$ is fully contained in at least one cluster (for some fixed constant $C > 0$). Specifically, given sparse neighborhood covers for all $O(\log n)$ exponentially-increasing distance scales $\beta, \beta^2, \beta^3, \dots, \poly(n)$ for some $\beta = \tO(1)$ along with some extra distance information, we construct an $\tO(1)$-competitive $\ell_1$-oblivious routing. 
The algorithm greatly differs from all prior approaches, as all of them had inherent barriers preventing them from achieving deterministic near-optimality, which we describe below.

\underline{Derandomization issues:} Efficient constructions of an $\ell_1$-oblivious routing either use an $\ell_1$-embedding or so-called low-diameter decompositions; this is a clustering problem whose deterministic version is also known as a sparse neighborhood cover. 
Sparse neighborhood covers were introduced in the seminal work of \cite{awerbuch1990sparse} and applied with great success for many problems, including approximate shortest paths and other distance based problems \cite{cohen98pairwise_covers,bartal2021RamseyEmbeddings}. 

Since an efficient deterministic $\ell_1$-embedding is not known, we need a deterministic construction of sparse neighborhood covers.  
%The low-diameter decomposition, known to be efficiently constructable from approximate distances in the randomized world \cite{becker2019low}, is a probability distribution. 
Luckily, many of the ideas required to derandomize the computation of sparse neighborhood covers were developed very recently by a sequence of papers that derandomized the closely related network decomposition problem which is, essentially, an unweighted version of the sparse cover problem~\cite{rozhon_ghaffari2019decomposition,ghaffari_grunau_rozhon2020improved_network_decomposition,chang_ghaffari2021strong_diameter}.
In \cite{elkin2022decompositions}, these unweighted results were extended to an algorithm constructing sparse neighborhood cover for weighted graphs and this is the result that we use to solve the shortest path problem here. 
% It can be shown that all prior approaches based on low-diameter decompositions or sparse neighborhood covers are inherently unable to be polylog competitive. To this end, we crucially use several key ideas that depart from all prior constructions.

% \underline{Idea 1: Remembering where the flows came from.} Oblivious routing intuitively works by judiciously intermixing the demand, until eventually, all demand is routed to some single node (note that sending a negative demand along a directed edge corresponds to sending a positive demand over the reversed edge). This is a valid solution to the transshipment problem, albeit its competitiveness depends on the intermixing strategy. 
% However, all prior approaches have the property that flows/demands that are ever joined will not again split apart, but will be treated equally. 
% We, on the other hand, treat the flows differently based on their origin node, making the flows splittable even after being aggregated. This idea, along with the next one, allows us to convert the multiplicative losses to additive ones, helping us achieve polylog-competitive routing.

% \underline{Idea 2: Reduce the outflow of nodes close to the boundary.} All prior approaches work by choosing a clustering (from the sparse neighborhood cover or low-diameter decomposition) and then for each cluster $C \subseteq V(G)$ in the clustering they send all demand from $v \in C$ to the cluster center. On average, this operation both reduces the dispersion of the demand (we want the demand to be accumulated in a single node), and has an acceptable cost. However, in worst case, if a pair of close-together nodes $u, v$ are separated into different clusters (a low-probability event), the operation yields an unacceptably high cost for this pair. 
% Prior approaches address this issue by averaging the operation over a large number independently sampled clusters. On the other hand, we observe that if such a worst-case event happens, both nodes $u, v$ are extremely close to the cluster boundary. In motivates the following: a node close to the boundary only sends a small fraction of its demand to the cluster center.

% A quantitative version of these two ideas allow us to convert a sparse neighborhood cover for all distance scales to a $(\poly\log n)$-competitive oblivious routing matrix $R$ that can be efficiently evaluated using only minor-aggregations.


% Unfortunately, inherent barriers prevent low-diameter decomposition/sparse neighborhood cover-based approaches from achieving polylog-competitiveness 


%for all $O(\log n)$ exponentially-increasing distance scales. A sparse neighborhood cover of some distance scale $D$ is simply a .

%We develop this polylog-competitive $\ell_1$-oblivious routing by using (near-optimal) polylog-quality low-diameter decompositions (LDDs). A $\tilde{O}(1)$-quality low-diameter decomposition is a randomized partitioning of the nodes of $V$ into so-called \emph{clusters} of a specified radius $r$ such that two nodes $u, v$ are in different clusters with probability at most $\tilde{O}(1) \frac{\dist(u, v)}{r}$. Notably, we use a ``deterministic version'' of LDDs, namely sparse neighborhood covers; we mostly consider randomized approaches in this introductory discussion due to its relative simplicity. A randomized version of an LDD-based approach was considered in \cite{goranci2022universally}, but achieved only a $n^{o(1)}$-competitive routing. Moreover, many inherent barriers prevent an LDD-based approach from achieving polylog-competitiveness and we develop several new ideas described below to overcome them.

%For the purposes of this section, we pretend we have access to an oracle constructing polylog-quality LDDs (or sparse neighborhood covers). Note that this is also an important open problem which we solve concurrently using our local reduction framework described later.

%\underline{Idea 1: Remembering where the flows came from.}

%Oblivious routings generally work by taking a demand $b : V(G) \to R$ and judiciously intermixing it until, eventually, all demand is routed to some single node. This is a valid solution to the transshipment problem, albeit its competitiveness depends on the intermixing strategy. Note that sending a negative demand along a directed edge corresponds to sending a positive demand over the reversed edge.

% All current approaches to oblivious routing had the property that once two demand (i.e., flows) were merged in a single node during the intermixing, from this point on they were always routed together. Such strategies make the routing and the analysis simple: each intermixing step only depends on the demand vector given to it at the start, hence can be analyzed independently of other steps. For example, \cite{Li20} does a $\ell_1$-embedding based approach using $O(\log n)$ steps of intermixing, each blowing up the optimum by a multiplicative $(1 + 1 / \log n)$, yielding a polylog-competitive routing (in each step the current optimum is added to the solution). Similarly, \cite{goranci2022universally} does a LDD-based approach with $(\log n)^{1/4}$ steps of intermixing, each losing a $2^{\sqrt{\log n}}$ factor, hence yielding a $2^{(\log n)^{3/4}} = n^{o(1)}$-competitive routing. Unfortunately, all approaches that use LDDs and lose a polylog factor in each step (this is optimal) require at least $O(\frac{\log n}{\log \log n})$ steps, yielding only an (unusable) polynomially-competitive routing. This is a inherent barrier preventing LDDs-based approaches from being polylog-competitive.

% We overcome this barrier by remembering the origin of each flow. In other words, instead of simply remembering that, after an intermixing step, there is $b'_u$ flow at a node $u$, we remember that there is $b'_u(v)$ flow at $u$ that originated at node $v$. Therefore, each flow is treated differently based on its origin, making the flows splittable even after being aggregated at the same node. This idea, along with the next one, allows us to convert the multiplicative polylog-losses to additive ones, hence achieve a polylog-competitive routing.

% \underline{Idea 2: Reduce the outflow of nodes close to the boundary.}
% Consider the following natural intermixing step. Sample an LDD of (large) radius $r$, and send the entire demand of each node $v$ to the center of its cluster in the LDD. Let us examine how the demand $b := \mathbb{1}_u - \mathbb{1}_v$ supported on two nodes $u$ and $v$ at distance $\dist_G(u, v) = 1$ gets intermixed. If $u, v$ are in the same cluster, their demand gets merged and the new transshipment cost is $0$. On the other hand, if they end up in different clusters, the new transshipment cost grows by at most $+2r$, but this happens (by LDD properties) only with probability $\tilde{O}(1) \cdot \frac{1}{r}$. Therefore, in expectation the new transshipment cost grows by an (acceptable) polylog factor. However, in worst-case the cost grows by an (unacceptable) multiplicative $O(r)$, requiring the algorithm to average over $\tilde{O}(r)$ different LDDs until the blowup becomes acceptable. The key idea in the approach of is to gradually increase the radius \cite{goranci2022universally} by a $n^{o(1)}$ factor until a single cluster consumes the entire graph and the demand is consolidated in a single node. This gradual increase enables one to average only over $n^{o(1)}$ different LDD samples and achieve a worst-case guarantee, even when the radius is $\Omega(n)$.

% We, on the other hand, choose an approach that does not include a large number of repetitions to achieve worst-case guarantees. First, we note that if two very-close nodes $u$ and $v$ are not in the same cluster, then they are extremely close to the boundaries of their respective clusters. Our key idea is that nodes that are close to the boundary only send a small portion of their flow to the center of the LDD cluster. This allows us to repeat the LDD sampling until every node is far-away from the boundary in at least one sample, hence we repeat the sampling only $O(\log n)$ times.

% We now consider the intermixing strategy associated with a single LDD sample of radius $r$. Formally, let $b(u)$ the distance of $u$ to the boundary of $u$'s LDD cluster. The node $u$ will only send approximately $b(u) / r$ amount of flow to the center of the cluster (up to a polylog constant of proportionality which we ignore here). Therefore, since $\dist_G(u, v) = 1$, we know the difference in the flows sent by $u$ and $v$ to the some $r$-distant cluster center is at most $|b(u) - b(v)|/r \le 1/r$ (this is the amount we have to pay for), yielding a cost of at most $\tilde{O}(1)$ per LDD sample independent of the LDD radius. Of course, this only describes the routing in the first step. Later, as the radius of the LDD clusters increase, the flow that originated at $u$ (called $u$-associated flow) is already intermixed in various nodes, we generalize the strategy in the following way. Each node $w$ sends approximately $b(u) / r$-fraction of its incoming $u$-associated flow (from $w$) to the center of the LDD cluster \emph{containing the origin $u$} (note: $w$ is not considered here). Note that this idea crucially requires us to remember where the flow comes from. Again, it is easy to show that the cost per LDD is $\tilde{O}(1)$. After the LDD radius is exponentially increased for a logarithmic number of steps, the LDDs start consuming the entire graph and the entire demand is consolidated at a polylogarithmic cost, achieving a polylog-competitive routing (at least for $u, v$ at distance $1$, but also generally).

% \underline{Algorithmic remark.} 
% In addition to being extremely simple this new $\ell_1$-oblivious routing is also routing directly on the graph G and thus provides a linear $n \times m$ map $R$ which directly maps any node-demand to a $\tO(1)$-approximate transshipment flow in $G$. Moreover, the evaluations of this routing map $R$ can trivially be evaluated in near-linear time because it can be written as a product $R = A \times B$ of two sparse matrices $A$ and $B$. Here, $A$ maps each node to $\tO(1)$ paths and $B$ map each path to its edges, where each edge is used by at most $\tO(1)$ paths. These two sparse mappings can furthermore be directly read off in near-linear time if the $O(\log^2 n)$ LDDs and (approximate) distances of nodes to the LDD boundary are given.



% \alert{OLD}

% The first key contribution of this paper is a new graph-based $\ell_1$-oblivious routing with drastically improved guarantees. One way to look at this routing is following the idea of using probabilistic tree embeddings. For example, sampling $O(log n)$ hierarchical LDDs for each diameter $D_i = log^{2i} n$ with $i \in [\log n/2]$ one obtains $O(log^2 n)$ many Bartal-style probabilitstic tree embedding which are $O(log^3 n)$ approximate in expectation. Our $\ell_1$-oblivious routing can be seen as letting each node send its demand to the root of each of these $O(log^2 n)$ trees. Of course the well-known problem is that in each embedding every edge has a small probability of $\tO(1/n)$ that it is stretched by up to a factor of $n$ by a random embedding. However, for this a node has to be very close to the boundary of an LDD, indeed much closer than one should expect it to be for a random LDD. Furthermore, a node can immediately see in which of the tree embeddings such a potentially bad event happened. Lastly, since the probability for this is small most of the embeddings will be fine for every node. Intuitively speaking each node would like to only send demand in trees that are good for some chosen cut-off for goodness but this would result different nodes sending in different subset of trees. Instead our routing can be seen as defining a notion of goodness and simply sending in each tree demand proportional to its goodness. Our analysis shows that the closer any pair of nodes are the more related their goodness score is and that any loss in approximation of flows sent between them that are cause by differing goodness scores are proportional to the cost of the flow and thus do not decrease the approximation guarantee of the oblivious routing. On the other hand, this reweighting guarantees that any flow that is routed in an embedding between pairs that are highly overstretched is inversely proportional to this stretch due to a small goodness score and thus does not contributed much to the overall cost. 

% In addition to being extremely simple this new $\ell_1$-oblivious routing is also routing directly on the graph G and thus provides a linear $n \times m$ map $R$ which directly maps any node-demand to a $\tO(1)$-approximate transshipment flow in $G$. Moreover the evaluations of this routing map $R$ can trivially be evaluated in near-linear time because it can be written as a product $R = A \times B$ of two sparse matrices $A$ and $B$. Here, $A$ maps each node to $\tO(1)$ paths and $B$ map each path to its edges, where each edge is used by at most $\tO(1)$ paths. These two sparse mappings can furthermore be directly read of in near-linear time if the $O(log^2 n)$ LDDs and distances of nodes to the LDD boundary to compute the goodness scores are given.

% \textbf{Routing scheme.}

% \begin{itemize}

% \item For simplicity of exposition, we define a set of ``trivial clusters'' $\calS_0 := \bigcup_{v \in V(G\cheat_D)} \mathrm{TrivialCluster}(v)$, which contain exactly one node $v$ as its only member and its center (the padding is empty). Furthermore, let $c$ be the cheating node of $G\cheat_D$, and define $\calS_{L+1}$ to be a single cluster containing the entire $G\cheat_D$ in its core, with the cheating node as its center (and no padding). Note that the radius of this cluster is at most $D \le R_{L+1}$. This allows us to define $\calS := \bigcup_{\ell=0}^{L+1} \calS_\ell$ to be the set of clusters in our (extended) sparse neighborhood cover.
  
% \item We now describe a linear routing scheme on $G\cheat_D$ by describing the (unit) flow each node sends. A node $v$ sends a unit flow which we denote via $f(v) \in \mathbb{R}^{\vec{E}}$ and refer to it as the $v$-associated flow. The cheating node $c \in V(G\cheat_D)$ simply uses the trivial flow $f(c) = \vec{0}$, i.e., that leaves all of the demand in itself. For (non-cheating) nodes $v$, we specify $f(v)$ by specifying the amount of flow $f_{i, j}(v)$ that travels from the center of cluster $C_i \in \calS$ to another cluster center $C_j \in \calS$. Given $f_{i, j}(v)$ for all $C_i, C_j \in \calS$, we can convert the representation to $f(v)$ by choosing (an oriented) path $\Path_{i, j}$ between the centers (the path we specify later) and increasing the flow along each edge on the path by $f_{i, j}(v)$. Note that $\Path_{i, j}$ does not depend on $v$ (i.e., it is consistently chosen among different nodes).

%   \alert{did I handle the cheating node properly?}

% \item Consider a (non-cheating) node $v \in V(G)$. On a high-level, the $v$-associated flow first routes from $v$ (i.e., from $\calS_0$) to the centers of clusters $C \in \calS_1$ (i.e., on the first level), then to the centers of clusters $C \in \calS_2$ (on the second level), and so on until the centers of clusters $C \in \calS_\ell$. Finally, all available flow is routed from the centers of cluster in $\calS_\ell$ to the cheating node (i.e., the only cluster on level $L+1$).
  
% \item We now formally specify the $v$-associated flow. First, for each $\ell \in \{1, \ldots, L+1\}$, each cluster $C_i \in \calS_\ell$ that contains $v \in C_i$ computes a value $p_i(v)$ defined as the distance from $v$ to the closest node outside of $C_i$, divided by the radius of $C_i$. Furthermore, we define $w_\ell(v)$ as the sum of $p_i(v)$ over all clusters in $\calS_\ell$.
% \begin{align*}
%   p_i(v) :=   & \min\left( 1, \frac{\dist_G(v, V(G) \setminus C_i)}{R_\ell} \right) \\
%   w_\ell(v) := & \sum_{C_i \in \calS_\ell} p_i(v)
% \end{align*}

% The clusters $C_i$ that do not contain $v$ have $p_i(v) := 0$. In particular (this follows from the formula, but we make explicit for concreteness), on level $\ell=0$ we define $p_i(v) = 1$ when $C_i \in \calS_0$ is the trivial cluster containing $v$ and $p_i(v) = 0$ otherwise (hence $w_0(v) = 1$). On level $\ell = L+1$, we define $p_i(v) = 1$ if $C_i$ is the cluster containing all of $G\cheat_D$ (hence $w_{L+1}(v) = 1$).

% \item We now define $f_{ij}(v)$ to be the amount of flow we route from center of $C_i$ to the center of $C_j$ ($i, j$ range over the set of all clusters in the sparse neighborhood). Only flow from the previous level $\calS_{\ell}$ enters the next level $\calS_{\ell+1}$, hence $f_{ij} = 0$ unless $C_i \in \calS_\ell$ and $C_j \in \calS_{\ell+1}$. For each $\ell \in \{1, \ldots, L-1\}$ and each cluster $C_i \in \calS_\ell$, we split the flow entering the center of $C_i$ (from $\calS_{\ell-1}$) proportionally with respect to $p_j(v)$ and route the corresponding proportion to $C_j \in \calS_{\ell+1}$ (on the next level).
% \end{itemize}
 

{\bfseries Distance-reduction framework: Iterative and Locality-Friendly}\\
As we explained earlier, our new $\ell_1$-oblivious routing construction reduces the SSSP problem in $G$ to computing sparse neighborhood covers along with some extra distance information.
% Moreover, due to the reduction of outflow of nodes close to the boundary, each node is required to know (an approximate) distance to the boundary of its cluster.
Clearly, this requires our SSSP computation to compute some distance information, leading again to a chicken and egg problem. Unfortunately, directly applying the vertex-reduction framework is not compatible with our desire to obtain fast minor-aggregation (or distributed) algorithms. In particular, at the lowest level of the recursion, the vertex-reduction framework generates a polynomial number of constant-size SSSP problems, each of which essentially corresponds to a minor of $G$. While these problems can each be solved in constant time in the parallel setting, the fact that these minors can be arbitrarily overlapping and each correspond to large diameter subsets in $G$ means that polynomially many instead of the desired polylogarithmic number of minor aggregations are necessary.

This paper therefore designs a novel, completely different, and more locality-friendly complexity-reduction framework: \emph{distance reduction}. On a high-level, we show that obtaining ``sparse neighborhood covers up to distance scale $D$'' can be reduced to several ``shortest path computations up to distance $D$'' which are computable from ``sparse neighborhood covers up to distance $D/\poly\log n$'' (see \cref{fig:main}). 
This iterative and local nature of our distance-reduction framework directly translates into a small overall number of minor aggregations; this is in stark contrast to the inherently recursive vertex-reduction framework (which recurses on different graphs, requiring a recursive approach).
As a nice little extra, combining our distance-reduction framework with the new $\ell_1$-embedding makes for an algorithm that is (in our not exactly unbiased opinion) a good bit simpler than the previous algorithms of \cite{Li20,AndoniSZ20}. 
We note that this framework is more reminiscent of older approaches to hopset constructions~\cite{cohen1994polylog, EN16}. In these approaches, hopsets over longer paths which use at most $\ell / 2$ edges are used to bootstrap the construction of hopsets over paths using at most $\ell$ edges.

%Specifically, it removes not just the two sparsification procedures used for the vertex-reduction itself but also gets rid of other steps in the vertex-reduction framework that seem hard\todo{are they? the clustering approach to bourgain embedding needs distance only up to scale D} to derandomize, including Bourgain's $\ell_1$-embedding.

A key definition to formalize what exactly the ``up to distance $D$'' in our distance-reduction framework means is the following. We attach a virtual, so-called, \emph{cheating node} and connect it to all other nodes with an edge of length $D$. This new graph naturally preserves distance information ``up to distance $D$'' and the complexity of computing distances increases as $D$ increases.

%The formal definition of ``shortest path structures up to distance $D$'' in our framework can be found in \Cref{sec:bla} and corresponds to a family of $O(\log n)$ representative LDDs for each scale up to $D$ together with distance information for each node about their distance to the boundary to its cluster in each of the LDDs. This is exactly what is needed for our $\ell_1$-oblivious routings and we show that such a distance structure is sufficient to compute SSSP soluations in $G_{D,S}$ for any set $S$. 

% Figure 2 gives a summary of our iterative local complexity-reduction framework:

% A representative set of $O(log n)$  LDDs and their boundary distances in G for distance $D$

% can be computed using polylog n SSSP problems in $G_{D,S_i}$ for different sets $S_i$

% (1+eps)-SSSP on $G_{D,S}$ for polylogarithmically many $S$

% can be computed via log n calls to TS and a rounding procedure. Each TS problem on some $G_{D,S}$ can be answered using an $\ell_1$-oblivious routing matrix of for $G_{D,S}$  (this is the boosting framework)

% $O(log^6 n)$-approx $\ell_1$-oblivious routing matrix for graphs $G_{D,S}$ for polylogarithmically many $S$ 

% we show that a distance structure for distance $D/log^2 n$, i.e., sets of LDDs for distances in $G$ up to distance $D/log^2 n$ are sufficient to generate the $\ell_1$-oblivious routing matrix for $G_{D,S}$ for any $S$. 

% representative set of $O(log n)$  LDDs and their boundary distances in G for any distance $D_i = 2^{i}$ for integer $i$ with $D_i \leq D/2$


{\bfseries Derandomization: Deterministic Transshipment Flow Rounding via Eulerian Tours}\\
All previous transshipment approaches crucially use randomization. The most significant challenge we had to overcome in making our results deterministic stem from the following issue: The only problem that remains to be derandomized in this paper is \emph{rounding} a (fractional) transshipment solution to (a flow supported on) a tree, a crucial step in the distance-reduction framework. We prove the following theorem (only the parallel version is stated for simplicity). 

%The above two tools give a randomized reduction of the $(1+\eps)$-SSSP problem to polylogarithmically many minor aggregates. It remains to give a derandomization. Fortunately, our new framework has eliminated the $\ell_1$-embedding and the two sparsification steps. 
%We also do not need to develop any new ideas for computing sparse neighborhood covers deterministically but can use generalizations of the recent algorithms \cite{rozhon_ghaffari2019decomposition,ghaffari_grunau_rozhon2020improved_network_decomposition,chang_ghaffari2021strong_diameter} developed for unweighted graphs.% \todo{drop blurry ball growing citation somewhere \cite{becker2019low}}
%to weighted graph clusterings~\footnote{In this paper we only require a particularly simple variant of the clusterings given in \cite{} except that one needs some additional care to only use shortest paths computations in $G$ without any changes to its structure to preserve the iterative nature of our reduction framework. This is a special requirement which is not very natural outside the context of this paper and not easily addressed by the powerful general clustering method for weighted graphs given in \cite{}. For sake of clarity and completeness we therefore make this paper self-contained and provide the simplified clustering algorithm used in this paper in Appendix bla}. 

\begin{theorem}\label{thm:eulerrounding-intro}
There is a deterministic parallel algorithm which takes as an input any fractional transshipment flow $f$ satisfying some single-source transshipment demand $b$ in the graph $G$ and in near-linear work and polylogarithmic time outputs a flow $f'$ of equal or smaller cost which is supported on some tree in $G$.
\end{theorem}

While such a flow rounding seems an unlikely bottleneck for a deterministic SSSP algorithm, we remark that even for randomized algorithms a lot of complexity has come from this rounding step in the algorithms of \cite{Li20, AndoniSZ20, BKKL17}---all these approaches are based on random walks and are inherently randomized.

%Moreover, in the recent paper by Andoni, Stein, and Zhong~\cite{AndoniSZ20}, the lack of such a rounding procedure is the only reason why only $s$-$t$ shortest paths can be computed and not SSSP trees. However, this extension was later provided in Zhong's thesis~\cite{zhong2021new}.

Note that if the fractional flow $f$ is acyclic (has no \emph{directed} cycles), then there is a trivial randomized rounding which simply samples one outgoing edge for each node in $G$ through which flow is routed, choosing the probability of each edge proportional to the outflow in $f$. It is easy to see that retaining the edges that are in the connected component of the source truthfully samples a tree-supported flow from $f$. The complexity comes in once $f$ is not acyclic as the sampled edges can now create many connected components. This requires finding the cycles in these components, contracting the edges and again running a randomized out-edge sampling on the remaining graph. 

Deterministically none of the above works. Indeed, we are not aware of any simple(r) way of deterministically obtaining a tree-supported flow even if $f$ is acyclic. Our rounding procedure can be seen as a generalization of an algorithm of Cohen's rounding~\cite{cohen1995approximateMaxFlow}, which can be used to round any fractional transshipment flow to an integral flow by scaling flow values to only leave integral and half-integral flow values and then finding an Eulerian tour covering all half-integral edges. Pushing one half-unit of flow in the cheaper direction of this Eulerian tour makes all flow values fully integral and allows the scaling to be reduced. At the end of this procedure, all flow values are integral but this does not guarantee that the flow is supported on a tree. To eliminate any non-tree like parts of the flow we show how to keep the algorithm running and find further Eulerian tours until the flow becomes tree-supported. 

{\bfseries A Distributed Eulerian Tour Algorithm}\\
The problem of computing Eulerian Tours can be stated as follows. Given an undirected graph with all degrees even, direct the edges in such a way that the out-degree of every node equals the in-degree. Note that we do not require connectedness. While computing Eulerian tours is a well-known parallel primitive which can be efficiently computed in near-linear work and polylogarithmic time \cite{atallah_vishkin1984euler_pram}, there are, to our knowledge, no distributed algorithms known for this problem. 

Therefore, to also give \emph{distributed} SSSP algorithms in this paper we need to design efficient distributed Eulerian-tour algorithms that can then be used in the Eulerian-tour-based rounding procedure of \Cref{thm:eulerrounding-intro}.  We build the first algorithm computing such an Eulerian tour orientation by using algorithms from \cite{parter_yogev2019cycle_covers_minor_closed,parter_yogev2019cycle_decomp_near_linear} for low-congestion cycle covers. Interestingly, these low-congestion cycle covers were only developed for the completely unrelated purpose of making distributed computation resilient to Byzantine faults introduced by an adversary in a recent line of work \cite{parter_yogev2019cycle_covers_minor_closed,parter_yogev2019cycle_decomp_near_linear,hitron_parter2021adversarial_compilers,hitron2021broadcast}. 

\begin{theorem}[Informal]\label{thm:euler-intro}
There is a deterministic \congest algorithm which, given any Eulerian subgraph $H$ of the network $G$ as an input, computes an Eulerian tour orientation in $\tO(\sqrt{n} + \Dhop)$ rounds or $\tO(\Dhop)$ rounds if $G$ is an excluded-minor graph. %Here, $\Dhop$ is the hop diameter of $G$. % using sublinear number of \congest rounds and minor aggregates. 
%There also exists a deterministic \congest algorithm which computes an Eulerian tour orientation of any Eulearian subgraph of an $n$-node graph $G$ with hop diameter $D$ in $\tO(\sqrt{n} + D)$ rounds or $\tO(D)$ rounds if $G$ is an exluded-minor graph. 
\end{theorem}

The most general and fully formal statements of all results proven in this paper are given in \Cref{sec:main_theorems}.

% Local Variables:
% TeX-master: "main"
% End:



==> Deterministic_SSSP/l1-Oblivious_Routing.tex <==
\section{$\ell_1$-Oblivious Routing with $\tilde{O}(1)$ Competitiveness and Evaluation Time via Sparse Neighborhood Covers}\label{sec:l1-oblivious-routing}

In this section, we prove our main result, an efficient $\ell_1$-oblivious routing in the distributed setting. We first give an overview of the new ideas required to overcome the barriers present in all previously known approaches, and then present a formal construction and proofs in \Cref{sec:routing-formal}.

\subsection{An Overview of New Ideas}\label{sec:routing-overview}

The first key contribution of this paper is a new graph-based $\ell_1$-oblivious routing with drastically improved guarantees. In order to simplify the discussion, in this overview we will explain the ideas from a randomized (low-diameter decomposition) perspective, rather than a deterministic (sparse neighborhood covers) one.

We develop this polylog-competitive $\ell_1$-oblivious routing by using (near-optimal) polylog-quality low-diameter decompositions (LDDs). A $\tilde{O}(1)$-quality low-diameter decomposition is a randomized partitioning of the nodes of $V$ into so-called \emph{clusters} of a specified radius $r$ such that two nodes $u, v$ are in different clusters with probability at most $\tilde{O}(1) \frac{\dist(u, v)}{r}$. Notably, we use a ``deterministic version'' of LDDs, namely sparse neighborhood covers; we mostly consider randomized approaches in this introductory discussion due to its relative simplicity. A randomized version of an LDD-based approach was considered in \cite{goranci2022universally}, but achieved only a $n^{o(1)}$-competitive routing. Moreover, many inherent barriers prevent an LDD-based approach from achieving polylog-competitiveness and we develop several new ideas described below to overcome them.

For the purposes of this section, we pretend we have access to an oracle constructing polylog-quality LDDs (or sparse neighborhood covers). Note that this is also an important open problem which we solve concurrently using our locality-friendly reduction framework from \cref{sec:localiterative}.

\underline{Idea 1: Remembering where the flows came from.}

Oblivious routings generally work by taking a demand $b : V(G) \to R$ and judiciously intermixing it until, eventually, all demand is routed to some single node. This is a valid solution to the transshipment problem, albeit its competitiveness depends on the intermixing strategy. Note that sending a negative demand along a directed edge corresponds to sending a positive demand over the reversed edge.

All current approaches to oblivious routing had the property that once two demand (i.e., flows) were merged in a single node during the intermixing, from this point on they were always routed together. Such strategies make the routing and the analysis simple: each intermixing step only depends on the demand vector given to it at the start, hence can be analyzed independently of other steps. For example, \cite{Li20} does a $\ell_1$-embedding based approach using $O(\log n)$ steps of intermixing, each blowing up the optimum by a multiplicative $(1 + 1 / \log n)$, yielding a polylog-competitive routing (in each step the current optimum is added to the solution). Similarly, \cite{goranci2022universally} does a LDD-based approach with $(\log n)^{1/4}$ steps of intermixing, each losing a $2^{\sqrt{\log n}}$ factor, hence yielding a $2^{(\log n)^{3/4}} = n^{o(1)}$-competitive routing. Unfortunately, all approaches that use LDDs and lose a polylog factor in each step (this is optimal) require at least $O(\frac{\log n}{\log \log n})$ steps, yielding only an (unusable) polynomially-competitive routing. This is a inherent barrier preventing LDDs-based approaches from being polylog-competitive.

We overcome this barrier by remembering the origin of each flow. In other words, instead of simply remembering that, after an intermixing step, there is $b'_u$ flow at a node $u$, we remember that there is $b'_u(v)$ flow at $u$ that originated at node $v$. Therefore, each flow is treated differently based on its origin, making the flows splittable even after being aggregated at the same node. This idea, along with the next one, allows us to convert the multiplicative polylog-losses to additive ones, hence achieve a polylog-competitive routing.

\underline{Idea 2: Reduce the outflow of nodes close to the boundary.}
Consider the following natural intermixing step. Sample an LDD of (large) radius $r$, and send the entire demand of each node $v$ to the center of its cluster in the LDD. Let us examine how the demand $b := \mathbb{1}_u - \mathbb{1}_v$ supported on two nodes $u$ and $v$ at distance $\dist_G(u, v) = 1$ gets intermixed. If $u, v$ are in the same cluster, their demand gets merged and the new transshipment cost is $0$. On the other hand, if they end up in different clusters, the new transshipment cost grows by at most $+2r$, but this happens (by LDD properties) only with probability $\tilde{O}(1) \cdot \frac{1}{r}$. Therefore, in expectation the new transshipment cost grows by an (acceptable) polylog factor. However, in worst-case the cost grows by an (unacceptable) multiplicative $O(r)$, requiring the algorithm to average over $\tilde{O}(r)$ different LDDs until the blowup becomes acceptable. The key idea in the approach of \cite{goranci2022universally} is to gradually increase the radius by an $n^{o(1)}$ factor until a single cluster consumes the entire graph and the demand is consolidated in a single node. This gradual increase enables one to average only over $n^{o(1)}$ different LDD samples and achieve a worst-case guarantee, even when the radius is $\Omega(n)$.

We, on the other hand, choose an approach that does not include a large number of repetitions to achieve worst-case guarantees. First, we note that if two very-close nodes $u$ and $v$ are not in the same cluster, then they are extremely close to the boundaries of their respective clusters. Our key idea is that nodes that are close to the boundary only send a small portion of their flow to the center of the LDD cluster. This allows us to repeat the LDD sampling until every node is far-away from the boundary in at least one sample, hence we repeat the sampling only $O(\log n)$ times.

We now consider the intermixing strategy associated with a single LDD sample of radius $r$. Formally, let $d(u)$ the distance of $u$ to the boundary of $u$'s LDD cluster. The node $u$ will only send approximately $d(u) / r$ amount of flow to the center of the cluster (up to a polylog constant of proportionality which we ignore here). Therefore, since $\dist_G(u, v) = 1$, we know the difference in the flows sent by $u$ and $v$ to the some $r$-distant cluster center is at most $|d(u) - d(v)|/r \le 1/r$ (this is the amount we have to pay for), yielding a cost of at most $\tilde{O}(1)$ per LDD sample independent of the LDD radius. Of course, this only describes the routing in the first step. Later, as the radius of the LDD clusters increase, the flow that originated at $u$ (called $u$-associated flow) is already intermixed in various nodes, we generalize the strategy in the following way. Each node $w$ sends approximately $d(u) / r$-fraction of its incoming $u$-associated flow (from $w$) to the center of the LDD cluster \emph{containing the origin $u$} (note: $w$ is not considered here). Note that this idea crucially requires us to remember where the flow comes from. Again, it is easy to show that the cost per LDD is $\tilde{O}(1)$. After the LDD radius is exponentially increased for a logarithmic number of steps, the LDDs start consuming the entire graph and the entire demand is consolidated at a polylogarithmic cost, achieving a polylog-competitive routing (at least for $u, v$ at distance $1$, but also generally).

\underline{Algorithmic remark.} 
In addition to being extremely simple this new $\ell_1$-oblivious routing is also routing directly on the graph G and thus provides a linear $n \times m$ map $R$ which directly maps any node-demand to a $\tO(1)$-approximate transshipment flow in $G$. Moreover, the evaluations of this routing map $R$ can trivially be evaluated in near-linear time because it can be written as a product $R = A \times B$ of two sparse matrices $A$ and $B$. Here, $A$ maps each node to $\tO(1)$ paths and $B$ map each path to its edges, where each edge is used by at most $\tO(1)$ paths. These two sparse mappings can furthermore be directly read off in near-linear time if the $O(\log^2 n)$ LDDs and (approximate) distances of nodes to the LDD boundary are given.

\subsection{Formal Construction of the Routing}\label{sec:routing-formal}




\begin{theorem}
\label{thm:oblivious_routing}
Let $G$ be a weighted graph. Assume a distance-structure for every scale $D_j, j < i$ is given.
Then, for a given set $S \subseteq V(G)$, there exists a $\textup{poly}(\log n)$-competitive $\ell_1$-oblivious routing $R$ for $G_{S,D_i}$ such that we can compute matrix-vector products with $R$ and $R^T$ in $\textup{poly}(\log n)$ \aggregate rounds in $G$. \\
Moreover, if $\beta^{i-1}/\valSNC$ is greater than the diameter of $G$, then there exists a $\textup{poly}(\log n)$-competitive $\ell_1$-oblivious routing $R$ for $G$ such that we can compute matrix-vector products with $R$ and $R^T$ in $\textup{poly}(\log n)$ \aggregate rounds in $G$.
\end{theorem}


\textbf{Extending the sparse covers to $G_{S,D_i}$.} For each $j<i$, consider the sparse neighborhood cover of $G$ from the distance-structure for distance $D_j$. Recall from \Cref{def:distance_structure} that it has covering radius $D_j/\valSNC$. Extend it to a sparse neighborhood cover of $G_{S,D_i}$ by letting $v_{D_i}$ and $s^*$ each be a singleton component, and name the new sparse neighborhood cover $\mathcal S_j$. We now claim that it still has covering radius $D_j/\valSNC$, this time on $G_{S,D_i}$. Since $D_j/\valSNC<D_i$, and since $v_{D_i}$ and $s^*$ have distance at least $D_i$ to all other nodes, the ball around any node $v\in V$ does not contain $v_{D_i}$ or $s^*$, so it is still fully contained in some cluster. The balls around $v_{D_i}$ and $s^*$ are simply the singleton sets $\{v_{D_i}\}$ and $\{s^*\}$, respectively, so they are also covered by their respective singleton clusters. It follows that the new sparse neighborhood cover has covering radius $D_i\ge D_i/\valSNC$. As for the potentials, we simply define $\tilde d_{\{v_{D_i}\}}(v_{D_i})=D_i$ and $\tilde d_{\{s^*\}}(s^*)=D_i$ for the clusters $\{v_{D_i}\}$ and $\{s^*\}$, respectively. These clearly satisfy \Cref{def:potential}.

Let $\mathcal S_i$ be the sparse neighborhood cover consisting of the entire graph $G_{S,D_i}$ as a single cluster $V'$, which has radius $2 D_i$ when centered at $v_{D_i}$. Let spanning tree of the cluster be the star centered at $v_{D_i}$ with leaves $V$, with $s^*$ attached to an arbitrary leaf node. We can trivially define $\tilde d_{V'}(v)=D_i$ for all $v\in V'$, which satisfies \Cref{def:potential} (where property~(1) is vacuously satisfied since there are no nodes outside the cluster).

\textbf{Notation.} For each clustering $\mathcal C$ in some sparse neighborhood cover $\mathcal S_j$, let $\tilde d_C$ be the corresponding distance label. For each cluster $C$ in some clustering, let $r_C$ be the cluster center, and let $T_C$ be the cluster spanning tree rooted at $r_C$ of radius at most $\alpha D_j$. Let $\gamma:=O(\log n)$ be an upper bound on the number of clusters in each clustering as guaranteed by Definition~\ref{def:distance_structure}. Furthermore, to avoid clutter, define $V':=V\cup\{v_{D_i},s^*\}$ as the vertices of $G_{S,D_i}$.

For each node $v\in V'$, integer $j<i$, and cluster $C$ containing $v$ that is in some clustering $\mathcal C\in\mathcal S_j$, define the value $p_{C}(v):=\max\{0,\tilde d_C(v)/D_j-0.25/\valSNC\}$, and for each $j<i$, define $w_j(v):=\sum_{C\in\mathcal C\in\mathcal S_j}p_{C}(v)$. 

\begin{lemma}\label{lem:w-lower-bound}
For all $j<i$, we have $w_\ell(v)\ge0.25/\valSNC$.
\end{lemma}
\begin{proof}
Since $\mathcal S_j$ is a sparse neighborhood cover of quality $\valSNC$, there exists a clustering $\mathcal C\in\mathcal S_j$ such that the ball around $v$ of radius $D_j/\valSNC$ is contained inside some cluster $C$ in $\mathcal C$. Equivalently, the distance of $v$ to a node outside $C$ is more than $D_j/\valSNC$. By property~(ii) of the definition of $\tilde d_C(v)$ (see Definition~\ref{def:distance_structure}), we have $\tilde d_C(v)\ge0.5D_j/\valSNC$. It follows that $w_j(v)\ge p_{C}(v)\ge\tilde d_C(v)/D_j-0.25/\valSNC\ge0.5/\valSNC-0.25/\valSNC=0.25/\valSNC$.
\end{proof}

We now describe the oblivious routing flow ``associated'' with each node $v\in V'$; the overall oblivious routing is simply the sum of the flows on each node $v$ multiplied by the demand at $v$.

The $v$-associated flow sends, for each $j<i$, and clusters $C\in\mathcal C\in\mathcal S_j$ and $C'\in \mathcal C'\in\mathcal S_{j+1}$ both containing $v$, a flow from the center $r_C$ to the center $r_{C'}$, and the amount of flow is $f_{C,C'}(v):=(p_{C}(v)/w_j(v))\cdot(p_{C'}(v)/w_{j+1}(v))$. (We do not yet specify the path from $r_C$ to $r_{C'}$ along which the flow is sent.) Over a single level $j$, the flow can be viewed as a ``product flow'' among all clusters $C$ in $\mathcal S_j$ and $C'$ in $\mathcal S_{j+1}$ containing $v$, weighted proportionally to $p_{C}(v)$ and $p_{C'}(v)$, respectively.

\begin{figure}
    \centering
    \includegraphics[width = .6\textwidth]{fig/routing.eps}
    \caption{Example of the first two levels of the oblivious routing under construction. The node $v$ is deep enough in two clusters $C_1, C_2$ in the sparse neighborhood cover $\mathcal{S}_1$ to send flow to their centers $r_{C_1}, r_{C_2}$. 
    There are two clusters $C'_1, C'_2$ in the cover $\mathcal{S}_2$ where $v$ is deep enough to send flow to their centers. The flow is sent from $r_{C_1}$ and $r_{C_2}$ and the amount of flow sent follows the product distribution $f_{C, C'}(v) \propto p_C(v) p_{C'}(v)$. Note that by \cref{obs:C-inside} we have $C_1 \cup C_2 \subseteq C'_1 \cap C'_2$. }
    \label{fig:routing}
\end{figure}

\begin{claim}\label{obs:flow-conservation}
For each $v\in V'\setminus\{v_{D_i}\}$, the $v$-associated flow sends $1$ unit of net flow out of $v$, $1$ unit of net flow into the virtual node $v_{D_i}$, and zero net flow into/out of any other node. The $v_{D_i}$-associated flow has zero net flow into/out of every node.
\end{claim}
\begin{proof}
Fix any node $v\in V'$. Since $\sum_{C\in\mathcal C\in\mathcal S_j}p_{C}(v)/w_j(v)=1$ for all $j$, it is easy to see that each node $v$ receives exactly $p_{C}(v)/w_j(v)$ total flow from level $j-1$ and sends exactly $p_{C}(v)/w_j(v)$ total flow to level $j+1$, which is a net flow of zero. This also means that for $j=1$, the node $v$ sends $1$ unit of flow out. Finally, since $\mathcal S_i$ has a single cluster with center $v_{D_i}$, all flow eventually coalesces at node $v_{D_i}$. This means that if $v\ne v_{D_i}$, then the flow sends $1$ unit out of $v$ and $1$ unit into $v_{D_i}$, and if $v=v_{D_i}$, then the two units of flow cancel, and the net flow is zero on every node.
\end{proof}

\begin{claim}\label{obs:C-inside}
We have $f_{C,C'}(v)\ne0$ only if $C\subseteq C'$.
\end{claim}
\begin{proof}
The claim is vacuous for $j=i-1$ since $\mathcal S_i$ has a single cluster of all the nodes, so assume that $j<i-1$. If $f_{C,C'}(v)\ne0$ then in particular, $p_{C'}(v)=\max\{0,\tilde d_{C'}(v)/D_{j+1}-0.25/\valSNC\}>0$, which implies that $\tilde d_{C'}(v)\ge 0.25D_{j+1}/\valSNC$. Since $\tilde d_{C'}$ is a potential with respect to $V'\setminus C'$, by properties~(1)~and~(2) of Definition~\ref{def:potential}, we have $\dist_G(v,V'\setminus C')\ge\tilde d_{C'}(v)\ge0.25D_{j+1}/\valSNC$. In other words, $v$ has distance at least $0.25D_{j+1}/\valSNC$ to the outside of cluster $C'$. Since $\valSNC\le\beta/8$ by construction, this distance is at least $2D_{j+1}/\beta=2D_j$. Since $C$ is a cluster of radius at most $D_j$, node $v$ has distance at most $2D_j$ to all of $C$, and it follows that $C\subseteq C'$. 
\end{proof}

The following lemma is key to bounding the competitive ratio of the oblivious routing algorithm.
\begin{lemma}\label{lem:flow-uv-diff}
Fix two nodes $u,v\in V'$. For every $j<i$ and two clusters $C\in\mathcal C\in\mathcal S_j$ and $C'\in\mathcal C'\in\mathcal S_{j+1}$, we have $|f_{C,C'}(u)-f_{C,C'}(v)|\le O(\gamma \valSNC d_G(u,v)/D_j)$.
\end{lemma}
\begin{proof}
Consider some $j<i$ and clusters $C\in\mathcal C\in\mathcal S_j$ and $C'\in \mathcal C'\in\mathcal S_{j+1}$.
To avoid clutter, let $d:=\dist_G(u,v)$ and $\delta:=\dist_G(u,v)/D_j$.
 The claim is trivial if $\delta\ge1/(\gamma \valSNC)$ since $f_{C,C'}(u),f_{C,C'}(v)\in[0,1]$ by construction. For the rest of the proof, assume that $\delta\le1/(\gamma \valSNC)$. It suffices to prove $f_{C,C'}(u)-f_{C,C'}(v)\le O(\gamma \valSNC d_G(u,v)/D_j)$ without the absolute value, since we can swap $u$ and $v$ to obtain the other direction.

By property~2(ii) of Definition~\ref{def:distance_structure}, both $|\tilde d_C(u)-\tilde d_C(v)|$ and $|\tilde d_{C'}(u)-\tilde d_{C'}(v)|$ are at most $d$, so both $|p_{C}(u)-p_{C}(v)|$ and $|p_{C'}(u)-p_{C'}(v)|$ are at most $d/D_j=\delta$. Since $w_j(v)=\sum_{C''\in\mathcal C''\in\mathcal S_j}p_{C''}(v)$ is the sum of at most $\gamma$ many terms, we have $|w_j(u)-w_j(v)|\le\gamma\delta$. Similarly, $|w_{j+1}(u)-w_{j+1}(v)| \le \gamma d/D_{j+1} \le \gamma d/D_j= \gamma\delta$. Therefore,
\begin{align*}
&f_{C,C'}(u)-f_{C,C'}(v)
\\&= \frac{p_{C}(v)}{w_j(v)}\cdot\frac{p_{C'}(v)}{w_{j+1}(v)} - \frac{p_{C}(u)}{w_j(u)}\cdot\frac{p_{C'}(u)}{w_{j+1}(u)}
\\&= \frac{p_{C}(v)p_{C'}(v)w_j(u)w_{j+1}(u) - p_{C}(u)p_{C'}(u)w_j(v)w_{j+1}(v)}{w_j(v)w_{j+1}(v)w_j(u)w_{j+1}(u)}
\\&\le \frac{p_{C}(v)p_{C'}(v)(w_j(v)+\gamma \delta)(w_{j+1}(v)+\gamma\delta) - (p_{C}(v)-\delta)(p_{C'}(v)-\delta)w_j(v)w_{j+1}(v)}{w_j(v)w_{j+1}(v)w_j(u)w_{j+1}(u)}
%\\&\le \frac{p_{C}(v)p_{C'}(v)(w_j(v)w_{j+1}(v)+\gamma\delta(w_j(v)+w_{j+1}(v))+(\gamma\delta)^2) - (p_{C}(v)-\delta)(p_{C'}(v)-\delta)w_j(v)w_{j+1}(v)}{w_j(v)w_{j+1}(v)w_j(u)w_{j+1}(u)}
.
\end{align*}
Expanding out the numerator and canceling out the $p_{C}(v)p_{C'}(v)w_j(v)w_{j+1}(v)$ terms, we obtain
\begin{align*}
&p_{C}(v)p_{C'}(v)(w_j(v)w_{j+1}(v)+\gamma\delta w_j(v)+\gamma\delta w_{j+1}(v)+(\gamma\delta)^2) 
\\&\quad-(p_{C}(v)p_{C'}(v)-\delta p_C(v)-\delta p_{C'}(v)+\delta^2)w_j(v)w_{j+1}(v) 
\\={}&  p_{C}(v)p_{C'}(v)(\gamma\delta w_j(v)+\gamma\delta w_{j+1}(v)+(\gamma\delta)^2) + (\delta p_C(v)+\delta p_{C'}(v)-\delta^2)w_j(v)w_{j+1}(v).
\end{align*}
Using that $p_{C}(v)\le w_j(v)$ and $p_{C'}(v)\le w_{j+1}(v)$, and ignoring the last $-\delta^2$ term, this is at most
\begin{align*}
&w_j(v)w_{j+1}(v)(\gamma\delta w_j(v)+\gamma\delta w_{j+1}(v)+(\gamma\delta)^2) + (\delta w_j(v)+\delta w_{j+1}(v))w_j(v)w_{j+1}(v) 
\\={}& w_j(v)w_{j+1}(v)((\gamma+1)\delta w_j(v)+(\gamma+1)\delta w_{j+1}(v)+(\gamma\delta)^2)
\end{align*}
Dividing by the denominator $w_j(v)w_{j+1}(v)w_j(u)w_{j+1}(u)$ and then using $|w_j(u)-w_j(v)|\le\gamma\delta$ and $|w_{j+1}(u)-w_{j+1}(v)|\le\gamma\delta$, we upper bound $f_{C,C'}(u)-f_{C,C'}(v)$ by
\begin{align*}
&\frac{(\gamma+1)\delta w_j(v)+(\gamma+1)\delta w_{j+1}(v)+(\gamma\delta)^2}{w_j(u)w_{j+1}(u)}
\\\le{}& \frac{(\gamma+1)\delta (w_j(u)+\gamma\delta)+(\gamma+1)\delta(w_{j+1}(u)+\gamma\delta)+(\gamma\delta)^2}{w_j(u)w_{j+1}(u)} \\\le{}& \frac{(\gamma+1)\delta w_j(u)+(\gamma+1)\delta w_{j+1}(u)+O(\gamma\delta)^2}{w_j(u)w_{j+1}(u)}
\\={}&\frac{(\gamma+1)\delta}{w_{j+1}(u)} + \frac{(\gamma+1)\delta}{w_j(u)} + \frac{O(\gamma\delta)^2}{w_j(u)w_{j+1}(u)}
.\end{align*}
Finally, using that $w_j(u),w_j(v)\ge0.25/\valSNC$ from \Cref{lem:w-lower-bound}, this is at most $O(\gamma \valSNC\delta+(\gamma \valSNC\delta)^2)$. Since $\delta\le1/(\gamma \valSNC)$, the linear term dominates, and we obtain the desired $f_{C,C'}(u)-f_{C,C'}(v)\le O(\gamma \valSNC\delta)$.
\end{proof}

\begin{lemma}\label{lem:competitive-ratio-final}
Assume that $\valSNC\le\beta/8$.
For any demand vector $b:\mathbb R^{V'}$ for the graph $G_{S,D_i}$, the summation
\begin{align*}
    \sum_{j<i}\sum_{\substack{C\in\mathcal C\in\mathcal S_j,\\C'\in\mathcal C'\in\mathcal S_{j+1}}}\bigg| \sum_{v\in V'}b(v)f_{C,C'}(v) \bigg|\cdot D_j
\end{align*}  is at most $i\gamma^3\valSNC$ times the optimal cost of a transshipment flow on $G_{S,D_i}$ satisfying demand $b$. 
\end{lemma}
\begin{proof}
Decompose the optimal transshipment flow into a collection $\mathcal P$ of paths. Fix a path with endpoints $u,v$ of flow value $F$, which contributes cost $F\cdot d_G(u,v)$ to the transshipment solution. For any $j<i$, there are at most $\gamma^2$ pairs $(\mathcal C,\mathcal C')$ with $\mathcal C\in\mathcal S_j$ and $\mathcal C'\in\mathcal S_{j+1}$, and for each $(\mathcal C,\mathcal C')$, there are at most two pairs $(C,C')$ with $C\in\mathcal C$ and $C'\in\mathcal C'$ for which either $f_{C,C'}(u)$ or $f_{C,C'}(v)$ is nonzero: these are the pairs $C,C'$ that either both contain $u$ or both contain $v$. So the total summation of $F\cdot |f_{C,C'}(u)-f_{C,C'}(v)|\cdot D_j$ from level $j$ is $O(\gamma^3\valSNC d_G(u,v))\cdot F$ by \Cref{lem:flow-uv-diff}. There are $i-1$ levels for a total of $O(i\gamma^3\valSNC d_G(u,v))\cdot F$, which we charge to the cost $F\cdot d_G(u,v)$ in the transshipment solution. It follows that $\sum_{u,v,F}\sum_{C,C'}F\cdot|f_{C,C'}(u)-f_{C,C'}(v)|\cdot D_j$ is at most $O(i\gamma^3\valSNC d_G(u,v))$ times the transshipment cost, so it remains to relate this summation to the desired $\sum_{C,C'}|\sum_{v\in V}b(v)f_{C,C'}(v)|\cdot D_j$.

 Summing over all paths in $\mathcal P$, we obtain 
\begin{align}
\sum_{u,v,F}\sum_{C,C'}F\cdot|f_{C,C'}(u)-f_{C,C'}(v)|\cdot D_j &\ge \sum_{C,C'}\left| \sum_{u,v,F}F\cdot(f_{C,C'}(u)-f_{C,C'}(v)) \right|\cdot D_j.\label{eq:comp-ratio}
\end{align}
Since the paths in $\mathcal P$ together form a transshipment solution that satisfies demand $b$, the sum of $F\cdot(\mathbbm1_u-\mathbbm1_v)$ over all paths in $\mathcal P$ (with endpoints $u,v$ and flow $F$) is exactly the demand vector $b$. That is, $\sum_{u,v,F}F\cdot(\mathbbm1_u-\mathbbm1_v)=b$ as vectors. Multiplying each vector coordinate $v$ by $f_{C,C'}(v)$ for any $C,C'$ and then summing over all coordinates, we obtain $\sum_{u,v,F}F\cdot(f_{C,C'}(u)-f_{C,C'}(v)) =\sum_{v\in V'}b(v)f_{C,C'}(v)$. It follows that the right-hand side of (\ref{eq:comp-ratio}) is exactly our desired expression $\sum_{C,C'}\left|\sum_{v\in V}b(v)f_{C,C'}(v)\right|\cdot D_j$, and we are done.
\end{proof}

In the next corollary, we replace $D_j$ in the summation with $D_{j+1}$, which is needed for our final analysis, and we also add an additional restriction $C\subseteq C'$.
\begin{corollary}\label{cor:competitive-ratio}
Assume that $\valSNC\le\beta/8$.
For any demand vector $b:V'\to\mathbb R$ for the graph $G_{S,D_i}$, the summation
\begin{align*}
    \sum_{j<i}\sum_{\substack{C\in\mathcal C\in\mathcal S_j,\\C'\in\mathcal C'\in\mathcal S_{j+1}\\{C\subseteq C'}}}\bigg| \sum_{v\in V'}b(v)f_{C,C'}(v) \bigg|\cdot D_{{j+1}}
\end{align*} 

at most $O(i\gamma^3\valSNC \beta)$ times the optimal cost of a transshipment flow on $G_{S,D_i}$ satisfying demand $b$.
\end{corollary}
\begin{proof}
We invoke \Cref{obs:C-inside}, which allows us to eliminate the restriction $C\subseteq C'$, since all other pairs $(C,C')$ satisfy $f_{(C,C')}(v)=0$ for all $v$.
The statement follows from \Cref{lem:competitive-ratio} and the fact that $D_{j+1}= D_j\cdot \beta$.
\end{proof}

We now define our oblivious routing matrix $R$. It is the product of two matrices $A\times B$, where $A\in\mathbb R^{\vec{E}\times P}$ and $B\in\mathbb R^{P\times(V')}$ where $P$ is the set of all pairs of clusters $C,C'\subseteq V'$ such that (1)~$C\subseteq C'$, and (2)~there exists $j<i$ such that $C$ is a cluster in some clustering $\mathcal C\in\mathcal S_j$ and $C'$ is a cluster in some clustering $\mathcal C'\in\mathcal S_{j+1}$.

We construct $B\in\mathbb R^{P\times V'}$ as $B_{(C,C'),v}=f_{(C,C')}(v)$ if clusters $C,C'$ both contain $v$, and $0$ otherwise. For $A\in\mathbb R^{\vec{E}\times P}$, consider two clusters $C,C'$. Since $C\subseteq C'$, we have in particular the center $r_C$ is in $C'$. Take the path from $r_C$ to $r_{C'}$ in the spanning tree $T_{C'}$ of $C'$. For each edge $(u,v)$ on the path, assign entry $A_{(u,v),(C,C')}=1$ if the path travels in the direction $u$ to $v$, and $-1$ otherwise. All other entries on column $(C,C')$ get assigned $0$.

\begin{lemma}\label{lem:competitive-ratio}
Assume that $\valSNC\le\beta/8$.
For any demand vector $b:\mathbb R^{V'}$ for the graph $G_{S,D_i}$, let $\textsf{\textup{opt}}(b)$ be the optimal cost of a transshipment flow on $G_{S,D_i}$ satisfying demand $b$. Then, $\textsf{\textup{opt}}(b)\le\left\lVert ABb\right\rVert_1\le i\gamma^3\valSNC \beta\textsf{\textup{opt}}(b)$.
\end{lemma}
\begin{proof}
We begin with the first inequality. Observe that by construction, for each $v\in V$ and $\mathbbm 1_v$ as the indicator vector of $v$, the vector $AB\mathbbm 1_v$ is the final flow distribution on nodes $V'$ of the $v$-associated flow. By \Cref{obs:flow-conservation}, this flow distribution is $\mathbbm 1_{v_{D_i}}$, i.e., all flow eventually ends up at $v_{D_i}$. Since $\sum_{v\in V'}b(v)=0$, the sum of the flows $AB\mathbbm 1_v$ over all $v\in V'$ routes all demands successfully. In other words, $AB\mathbbm 1_v$ is a valid transshipment flow on $G_{S,D_i}$ satisfying demand $b$, so its cost $\left\lVert ABb\right\rVert_1$ is at least $\textsf{opt}(b)$.

We now prove the second inequality. By construction of $B$, entry $(C,C')$ of $Bb$ is exactly $\sum_vb(v)f_{(C,C')}(v)$. Next, for the indicator vector $\mathbbm 1_{(C,C')}$, by construction of $A$, we have $\left\lVert A\mathbbm 1_{(C,C')}\right\rVert_1$ is exactly the length of the path from $r_C$ to $r_{C'}$ in the spanning tree $T_{C'}$ of $C'$, which is at most $\alpha D_j$ for the level $j$ whose $\mathcal S_j$ contains cluster $C'$. It follows that
\begin{align*}
\left\lVert ABb\right\rVert_1 &= \left\lVert A\times\sum_{(C,C')}\left(\sum_{v\in V}b(v)f_{C,C'}(v)\right)\mathbbm 1_{(C,C')}\right\rVert_1 
\\&\le \sum_{(C,C')}\left|\sum_{v\in V}b(v)f_{C,C'}(v)\right|\left\lVert A\mathbbm 1_{(C,C')}\right\rVert_1
\\&\le \sum_{\substack{(C,C')\\C'\in\mathcal C'\in\mathcal S_j}}\left|\sum_{v\in V}b(v)f_{C,C'}(v)\right|\alpha D_j.
\end{align*}
By \Cref{cor:competitive-ratio}, this is at most $\alpha\cdot O(i\gamma^3\valSNC \beta)\cdot\textsf{opt}(b)$.
\end{proof}

Finally, we discuss distributed implementations of multiplying by $R$ and $R^T$ for $R=AB$.

\begin{lemma}\label{lem:distributed-oblivious}
Suppose each node $v\in V$ knows $\tilde d_C(v)$ for all clusterings $C$ containing $v$. For any vector $b\in\mathbb R^V$ where each node $v$ knows $b(v)$, we can compute $Rb$ in $\textup{poly}(\gamma\log n)$ \aggregate rounds (on network $G$) so that each entry $(u,v)$ of $Rb$ is known by both $u$ and $v$. Also, for any vector $c\in\mathbb R^{\vec{E}}$ where each entry $c_{(u,v)}$ is known by $u$\ and $v$, we can compute $R^Tc$ in $\textup{poly}(\gamma\log n)$ \aggregate rounds (on network $G$) so that each node $v\in V$ learns entry $v$ of $R^Tc$.
\end{lemma}
\begin{proof}
We work on network $G_{S,D_i}$ instead, which can be simulated on network $G$ with a constant-factor blowup by \Cref{thm:simulating-virtual-nodes}.

To multiply $Rb$ for vector $b\in\mathbb R^V$, we first multiply $Bb$ as follows. For each $j<i$ and clusters $C\in\mathcal C\in\mathcal S_j$ and $C'\in\mathcal C'\in\mathcal S_{j+1}$ containing $v$, the node $v$ locally computes $f_{(C,C')}(v)$ using $\tilde d_C(v)$ and $\tilde d_{C'}(v)$. Then, for each level $j<i$ and each clustering $\mathcal C\in\mathcal S_j$, we perform a minor aggregation on each cluster $C\in\mathcal C$ to compute the sum $\sum_{v\in C}b(v)f_{(C,C')}(v)$ for all $C'$ (where $f_{(C,C')}(v)=0$ if $v\notin C'$). Here, we crucially use the fact that we only consider clusters $C'$ with $C\subseteq C'$, which is at most $\gamma$ many since there is at most one such cluster $C'$ in each clustering of $\mathcal S_{j+1}$. As a result of the aggregation, for each pair $(C,C')$, the center $r_C$ of $C$ knows entry $(C,C')$ in $Bb$. Finally, to compute $A(Bb)$, perform the following separately for each $j<i$ and each clustering $\mathcal C'\in\mathcal S_{j+1}$: for each cluster $C'\in\mathcal C'$ in parallel, take the spanning tree $T_{C'}$ rooted at $r_{C'}$ and for each $(C,C')$, initialize at node $r_C\in C'$ the value of entry $(C,C')$ in $Bb$, which is known by $r_C$. Call \Cref{lemma:ancestor-subtree-sum} to obtain all subtree sums, and for each node $v\in C'\setminus\{r_{C'}\}$ with parent $u$, the subtree sum at $v$ is exactly the contribution of the paths in cluster $C'$ to the total flow along edge $(u,v)$, possibly negated depending on the orientation of edge ($u,v)$. Each entry $(u,v)$ of $A(Bb)$ then becomes the sum of all such contributions over all $C'$ whose spanning tree $T_{C'}$ contains edge $(u,v)$,  This concludes multiplication by $R$.

To multiply $R^Tc$ for $c\in\mathbb R^{\vec{E}}$, we first multiply $A^Tc$ as follows. Perform the following separately for each $j<i$ and each clustering $\mathcal C'\in\mathcal S_{j+1}$: for each cluster $C'\in\mathcal C'$ in parallel, take the spanning tree $T_{C'}$ rooted at $r_{C'}$ and for each edge $(u,v)$ in $T_{C'}$, initialize the value of entry $(u,v)$ in $c$. Then, in $\textup{poly}(\log n)$ \aggregate rounds, we can compute, for each node $v\in C'$, the sum of all entries on the path from $r_{C'}$ to $v$ in $T_{C'}$ (\Cref{lemma:ancestor-subtree-sum}). In particular, for each pair $(C,C')$, this sum is entry $(C,C')$ of $A^Tc$, which node $r_C$ now knows. Finally, to compute $B^T(A^Tc)$, each cluster $C$ broadcasts entry $(C,C')$ of $A^Tc$ to all its nodes, which is again at most $\gamma$ many since we only consider clusters with $C\subseteq C'$. Each node $v$ can then locally compute $f_{(C,C')}(v)$ to learn its entry in $B^T(A^Tc)$.
\end{proof}

%We claim the bound $|P|\le(i-1)\gamma^2n$. For each $j<i$, there are at most $\gamma^2$ pairs $(\mathcal C,\mathcal C')$ with $\mathcal C\in\mathcal S_j$ and $\mathcal C'\in\mathcal S_{j+1}$, and for a given node $v\in V$, at most one cluster $C\in\mathcal C$ and $C'\in\mathcal C'$ can contain $v$, so at most $(i-1)\gamma^2$ many pairs of clusters $(C,C')\in P$ both contain $v$. Summing over all $v\in V$ gives the desired bound on $|P|$.

Together, \Cref{lem:competitive-ratio-final,lem:distributed-oblivious} conclude the first part of \Cref{thm:oblivious_routing}. 

For the last statement of the theorem, if $D_{i-1}/\valSNC$ is larger than the diameter of $G$, then we modify the sparse neighborhood covers as follows. For each $j<i$, remove the singleton clusters $\{v_{D_i}\}$ and $\{s^*\}$ from each clustering in $\mathcal S_j$ (and remove their potentials $\tilde d_{\{v_{D_i}\}}(v_{D_i})$ and $\tilde d_{\{s^*\}}(s^*)$). For the single clustering $V'$ in $\mathcal S_i$, replace it with a single cluster $V$ with an arbitrary spanning tree $T$ of $G$ with diameter at most $D_{i-1}$, which we show how to find later. Once again, we trivially define $\tilde d_V(v)=D_i$ for all $v\in V$. We construct the oblivious routing and matrices $A,B$ in the same way. By the same arguments, this is a $\poly(\log n)$-competitive $\ell_1$-oblivious routing matrix for $G$.

We now discuss how to compute the spanning tree $T$ of $G$ with diameter at most $D_{i-1}$. Since $\mathcal S_{i-1}$ is a sparse cover of covering radius $D_{i-1}/\valSNC$, there exists a clustering in $\mathcal S_{i-1}$ such that the ball of radius $D_{i-1}/\valSNC$ around any $v\in V$ is contained in some cluster $C$. Since $\beta^{i-1}/\valSNC$ is greater than the diameter of $G$, this cluster $C$ must contain all the vertices $V$. Therefore, the spanning tree $T_C$ of diameter at most $D_{i-1}$ is our desired spanning tree of $G$.

%The algorithm is iterative and takes $\gamma \valSNC\beta$ iterations, and maintains a tree $T$ of $G$ that eventually spans all vertices $V$ after all iterations. Initially, $T$ is the empty tree on a single arbitrary vertex $v_0\in V$. On each iteration, we select a clustering $\mathcal C$ of sparse neighborhood cover $\mathcal S_{i-1}$ and for each cluster $C$ with at least one vertex $v$ in $T$, we root the corresponding spanning tree $T_C$ of $C$ at $v$ and add to $T$ all edges in the rooted tree $T_C$ whose child endpoint was not a vertex in $T$. At the end of this iteration, $T$ is still a tree, and it contains all vertices in clusters $C$ that contained at least one vertex in $T$.

%Since each spanning tree $T_C$ has diameter at most $D_{i-1}$, the radius of $T_C$ (centered at $v_0$) grows additively by at most $D_{i-1}$ on each iteration, so over all $\gamma \valSNC\beta$ iterations, the final tree $T$ has radius at most $\gamma \valSNC\beta \cdot D_{i-1} = \gamma \valSNC D_i$, as promised. It remains to show that $T$ does in fact span $V$, which will depend on our choice of clustering $\mathcal C$ on each iteration, which we specify next.

%Over the $\gamma \valSNC\beta$ iterations, we select the clusterings $\mathcal C\in\mathcal S$ in a round-robin fashion: we order the clusterings arbitrarily as $\mathcal C_0,\ldots,\mathcal C_{\gamma-1}$ and on iteration $i$, we select clustering $C_{i\bmod\gamma}$. We show by induction on $k$ that at the end of the first $k\gamma$ iterations, all vertices of distance at most $k D_{i-1}/\valSNC$ from $v_0$ are spanned by $T$. After $\gamma \valSNC\beta$ iterations, this covers all vertices of distance at most $D_i$, which is all of $V$ since $D_i$ is greater than the diameter of $G$ by assumption.

%The claim is trivial for $k=0$, so assume that $k>0$. Let $v\in V$ be a vertex of distance at most $k D_{i-1}/\valSNC$ from $v_0$ not yet covered. Select a vertex $u$ with $\dist_G(u,v_0)\le(k-1) D_{i-1}/\valSNC$ and $\dist_G(v_0,v)\le D_{i-1}/\valSNC$, which by induction is spanned after $(k-1)\gamma$. Since $\mathcal S_{i-1}$ is a sparse cover of covering radius $D_{i-1}/\valSNC$, there exists a cluster $C$ in some clustering such that the ball of radius $D_{i-1}/\valSNC$ around $u$ is contained in $C$. In particular, $v\in C$. Since the round-robin algorithm visits cluster $C$ once on iterations $(k-1)\gamma+1$ through $k\gamma$, all vertices in $C$ are spanned by iteration $k\gamma$, which includes $v$, completing the induction.

%\alert{(Goran) .. not completely sure can we claim that the same routing works for G since the routing in $G_{S, bla}$ eventually aggregates everything in cheating node $v_{D_i}$ and this node does not exist in $G$. So if I understand everything correctly, when you talk about G you need to aggregate in some other node. This might be trivial, but it's probably wrong without talking how to adapt it. Jason: that's true... Seems like a lot of work to make the oblivious routing work without the cheating node, since I'd have to specify a spanning tree of diameter $D_i$ to use instead of the cheating node, and this isn't given to me. And our application doesn't need it since we just need the value of the routing. Could this part of the theorem statement just be removed? \color{blue} (Goran): I talked to Christoph, and he suggests doing the following. If you have a sparse cover where the distance scale is larger than the diameter of G, then at least one cluster preserves the entire graph, and you get the spanning tree along with it. Does that help? If you still feel it's a bit tediuos to prove it with this, we can probably removing it on the other end, but that will also take some work. (Jason): I wrote it up, wasn't too bad. Biggest part was just showing that I can construct the spanning tree since I'm given clusterings at smaller scales.}

This concludes our distributed $\ell_1$-oblivious routing algorithm. 

\paragraph{Remark.}

% Sparse matrices are particularly nice because vector-matrix products can trivially be computed in sparsity work and polylog n depths in \pram (once the matrix is computed). Unfortunately even for a path graph all known constructions (including our) do not yield a sparse $V \times E$ $l_1$-oblivious routing matrix. However as the next remark shows we easily can write our routing matrix $R$ as a product of two sparse $\tilde{O}(n) \times \tilde{O}(n)$ matrices. Vertex-matrix products for such a matrix product are similarly easy to evaluate. 

% Note that $|\mathcal P|=\tO(n)$ and that $B$ is a $n \times \tilde{O}(n)$ matrix with $\tilde{O}(n)$ non-zero entries. Indeed, $B_{(C,C'),v}\ne0$ only when $v\in C\cap C'$, and there are at most $O(\log^2n)$ clusters $C$ containing $v$, since there are $O(\log^2n)$ total clusterings $\mathcal C$ and each has at most one cluster containing $v$. On the other hand, the matrix $A$ as defined is not sparse since its construction is based on subtree sums, which are not sparse for unbalanced trees (like a path). 

% We remark that we can slightly modify the construction so that the oblivious routing matrix $R$ can indeed be written as a product of two \emph{\emph{sparse}} matrices. This gives an alternative, easy way to multiply vectors by $R$ and $R^T$ in near-linear time without resorting to subtree sums in the proof of \Cref{lem:distributed-oblivious}. (Since we do not require it for our distributed algorithm, we do not discuss how to construct the matrices in a distributed setting.)

% The additional idea is to represent subtree sums concisely by the standard trick of computing a DFS traversal of the spanning tree $T_{C'}$ and then building a segment tree on top of the linear ordering of nodes. Recall from the proof of \Cref{lem:distributed-oblivious} that to multiply matrices $A$ and $Bb$, we take, for each cluster $C'$, the spanning tree $T_{C'}$ rooted at $r_{C'}$, and for each relevant cluster $C$, we initialize at node $r_C\in C'$ the value of entry $(C,C')$ in $Bb$. For each edge $(u,v)$ in $T_{C'}$, the contribution of cluster $C'$ to entry $(u,v)$ in the product $A\times Bb$ then becomes a subtree sum on this tree. We can represent all subtree sums concisely as follows: take a DFS traversal of $T_{C'}$ so that each subtree consists of consecutive nodes in the traversal order, and build a segment tree on top of the linear ordering of $C'$, which is a collection of $O(|C'|\log|C'|)$ segments such that (1)~each subtree of $T_{C'}$ consists of consecutive nodes in the linear ordering, (2)~each set of consecutive nodes in the ordering is a disjoint union of $O(\log|C'|)$ of these segments, and (3)~each node appears in $O(\log|C'|)$ many segments. Now, instead of taking matrix $B$ in the matrix product of $R$, we instead build a matrix $B'$ whose rows represent these segments (over all clusters $C'$). Namely, for a given cluster $C'$, for each segment of nodes $Q\subseteq C'$, we add a row of $B'$ whose value is the sum of all rows $(C,C')$ of $B$ satisfying $r_C\in Q$. This gives us $O(|C'|\log|C'|)$ new rows for cluster $C'$. To bound the sparsity of these rows, note that each nonzero entry in some $(C,C')$ can only make $O(\log|C'|)$ entries nonzero in the new rows, since only $O(\log|C'|)$ many segments can contain node $r_C$. It follows that the number of nonzero entries of the $O(|C'|\log|C'|)$ new rows is at most $O(\log|C'|)$ times the number of nonzero entries of entries $(C,C')$ in $B$. Since $B$ has $\tO(m)$ entries, it follows that $B'$ does as well.

% We now construct matrix $A'$ to sum up the segments accordingly. Namely, for a row $(u,v)$ and cluster $C'$, instead of assigning value $\pm1$ at columns $(C,C')$ whose node $r_C$ is in the subtree, we instead assign $\pm1$ to the segments comprising this subtree. This is at most $O(\log|C'|)$ nonzero entries for each $(C,C')$, and there are $O(\log n)$ clusters $C'$ containing edge $(u,v)$ on each of the $i$ levels, so each row $(u,v)$ has at most $\poly(\log n)$ nonzero entries. Thus, $A'$ has $\tO(m)$ nonzero entries.



% \alert{End here. Below is a sketch of the same argument, except Bernhard uses heavy-light decomposition, which I feel is more complicated than my subtree-sum approach.}
Sparse matrices are particularly nice because vector-matrix products can trivially be computed in sparsity work and polylog n depths in \pram (once the matrix is computed). Unfortunately even for a path graph there cannot exist a sparse $\vec{E} \times V$ $l_1$-oblivious routing matrix.\footnote{Here is a simple argument that the oblivious routing matrix $R$ must have $\Omega(n^2)$ nonzero entries. Let the vertices of the path be $v_1,\ldots,v_n$ in that order, and assume for simplicity that $n$ is even. For each $i$ from $1$ to $n/2$, consider the demand $\mathbb{1}_{v_i} - \mathbb{1}_{v_{i+n/2}}$. Clearly, the optimal routing routes $1$ flow along each edge from $v_i$ to $v_{i+n/2}$, but note that \emph{any} feasible routing must route nonzero flow along those edges. This means that $R(\mathbb{1}_{v_i} - \mathbb{1}_{v_{i+n/2}})$ has $\Omega(n)$ nonzero entries, which implies that columns $v_i$ and $v_{i+n/2}$ in $R$ together have $\Omega(n)$ nonzero entries. Summed over all $i$, this is $\Omega(n^2)$ nonzero entries in $R$.} However as the next remark shows we easily can write our routing matrix $R$ as a product of two sparse $\tilde{O}(n) \times \tilde{O}(n)$ matrices. Vertex-matrix products for such a matrix product are similarly easy to evaluate. 

Note that $|P|=O(n\log^2 n)$ and that $B$ is a $\tilde{O}(n) \times n$ with $\tilde{O}(n)$ non-zero entries - at most $O(\log^2 n)$ per node. Indeed each node has its demand routed through only $O(\log^2 n)$ clusters-centers, namely the ones it is contained in, which is at most one for each of the $O(\log^2 n)$ clusterings. The matrix $A$ as defined above is not sparse as most paths between cluster centers can be $O(n)$ long. However we can decompose these paths in such a way that $A$ can be written as a product of two sparse matrices. For this note that for the paths from smaller clusters to larger clusters all come from the spanning tree $T_C$ of this clustering. Decompose this spanning tree into a set of polylog n many paths by first doing a heavy-light decomposition of the tree and then taking each of the resulting paths and for every power of two $2^j$ cutting it into segments by cutting the path at any node which is a multiple of $2^j$ (starting from any end). For a clustering do this for all spanning trees of all clusters simultaneously. This results in $O(n \log n)$ paths per clustering and $O(n \log^3 n)$ paths overall. Call the set of these paths $P'$. Note that any path between the cluster centers of two clusters $C,C'$ with $C \subset C'$ along the spanning tree $T_{C'}$ can be written as a concatenation of $O(\log n)$ paths from $P'$. Moreover each edge is used by at most $O(\log^3 n)$ paths in $P'$ since it is a union of $O(\log^2 n)$ disjoint set of paths and there are at most $O(\log n)$ intervals per paths that contain an edge $e$. Overall, we can write the matrix $A$ as a product of a sparse $\vec{E} \times P'$ matrix $A_1$ with $O(\log^2 n)$ one entries per edge (indeed there is only a $m' = O(n \log^2 n)$ size subset of edges, namely the union of the spanning trees for each clustering, which are used by the routing at all, all other edges never carry any flow) and a $P' \times P$ matrix $A_2$ which assigns each cluster center pair to at most $O(\log n)$ paths in $P'$. This writes $R=A_1 A_2 B$ as the product of three sparse matrices. Moreover, since every node is mapped to at most $O(\log^3 n)$ cluster pairs by $B$ and each cluster pair is mapped to at most $O(\log n)$ paths from $P'$ the matrix-product of $A_2 B$ is sparse and assigns each node to $O(\log^4 n)$ paths in $P'$. In total this writes $R$ as a product of a $m' \times O(n \log^3 n)$ matrix with is $O(\log^2 n)$-row sparse and a $O(n \log^3 n) \times n$ matrix which is $O(\log^4 n)$-column sparse. Given the distance structures and their trees the heavy-light decomposition can be computed in $\tilde{O}(1)$ \aggregate rounds \Cref{lemma:ancestor-subtree-sum} and therefore also in PRAM.


%%% OLD STUFF
\iffalse

\oblivious*
\todo{Please change the language so that it fits the theorem above}
\textbf{Setting.} Let $G$ be the underlying graph and let $D > 0$. We are given sparse neighborhood covers $\calS_1, \calS_2, \ldots, \calS_L$ of $G$ where $\calS_\ell$ has radius $R_\ell := R^\ell$ for some $R := O(\log^5 n)$, quality $\valSNC := O(\log^4 n)$, and are each composed of $\gamma = \tilde{O}(1)$ clusterings. The number of levels $L = \tilde{O}(1)$ is such that $R_{L+1} \ge D$. We define the \textbf{cheating graph} $G\cheat_D$ as $G$ adjoined with an special \textbf{cheating node} $c$ that is connected to each node $v \in V(G)$ with a distance of $D$.

\textbf{Assumptions (to be removed).}
\begin{itemize}
\item We assume exact distances and exact computation of $p_i$'s.
\item We don't discuss algorithmic issues.
\end{itemize}


\textbf{Routing scheme.}

\begin{itemize}

\item For simplicity of exposition, we define a set of ``trivial clusters'' $\calS_0 := \bigcup_{v \in V(G\cheat_D)} \mathrm{TrivialCluster}(v)$, which contain exactly one node $v$ as its only member and its center (the padding is empty). Furthermore, let $c$ be the cheating node of $G\cheat_D$, and define $\calS_{L+1}$ to be a single cluster containing the entire $G\cheat_D$ in its core, with the cheating node as its center (and no padding). Note that the radius of this cluster is at most $D \le R_{L+1}$. This allows us to define $\calS := \bigcup_{\ell=0}^{L+1} \calS_\ell$ to be the set of clusters in our (extended) sparse neighborhood cover.
  
\item We now describe a linear routing scheme on $G\cheat_D$ by describing the (unit) flow each node sends. A node $v$ sends a unit flow which we denote via $f(v) \in \mathbb{R}^{\vec{E}}$ and refer to it as the $v$-associated flow. The cheating node $c \in V(G\cheat_D)$ simply uses the trivial flow $f(c) = \vec{0}$, i.e., that leaves all of the demand in itself. For (non-cheating) nodes $v$, we specify $f(v)$ by specifying the amount of flow $f_{i, j}(v)$ that travels from the center of cluster $C_i \in \calS$ to another cluster center $C_j \in \calS$. Given $f_{i, j}(v)$ for all $C_i, C_j \in \calS$, we can convert the representation to $f(v)$ by choosing (an oriented) path $\Path_{i, j}$ between the centers (the path we specify later) and increasing the flow along each edge on the path by $f_{i, j}(v)$. Note that $\Path_{i, j}$ does not depend on $v$ (i.e., it is consistently chosen among different nodes).

  \alert{did I handle the cheating node properly?}

\item Consider a (non-cheating) node $v \in V(G)$. On a high-level, the $v$-associated flow first routes from $v$ (i.e., from $\calS_0$) to the centers of clusters $C \in \calS_1$ (i.e., on the first level), then to the centers of clusters $C \in \calS_2$ (on the second level), and so on until the centers of clusters $C \in \calS_\ell$. Finally, all available flow is routed from the centers of cluster in $\calS_\ell$ to the cheating node (i.e., the only cluster on level $L+1$).
  
\item We now formally specify the $v$-associated flow. First, for each $\ell \in \{1, \ldots, L+1\}$, each cluster $C_i \in \calS_\ell$ that contains $v \in C_i$ computes a value $p_i(v)$ defined as the distance from $v$ to the closest node outside of $C_i$, divided by the radius of $C_i$. Furthermore, we define $w_\ell(v)$ as the sum of $p_i(v)$ over all clusters in $\calS_\ell$.
\begin{align*}
  p_i(v) :=   & \min\left( 1, \frac{\dist_G(v, V(G) \setminus C_i)}{R_\ell} \right) \\
  w_\ell(v) := & \sum_{C_i \in \calS_\ell} p_i(v)
\end{align*}

The clusters $C_i$ that do not contain $v$ have $p_i(v) := 0$. In particular (this follows from the formula, but we make explicit for concreteness), on level $\ell=0$ we define $p_i(v) = 1$ when $C_i \in \calS_0$ is the trivial cluster containing $v$ and $p_i(v) = 0$ otherwise (hence $w_0(v) = 1$). On level $\ell = L+1$, we define $p_i(v) = 1$ if $C_i$ is the cluster containing all of $G\cheat_D$ (hence $w_{L+1}(v) = 1$).

\item We now define $f_{ij}(v)$ to be the amount of flow we route from center of $C_i$ to the center of $C_j$ ($i, j$ range over the set of all clusters in the sparse neighborhood). Only flow from the previous level $\calS_{\ell}$ enters the next level $\calS_{\ell+1}$, hence $f_{ij} = 0$ unless $C_i \in \calS_\ell$ and $C_j \in \calS_{\ell+1}$. For each $\ell \in \{1, \ldots, L-1\}$ and each cluster $C_i \in \calS_\ell$, we split the flow entering the center of $C_i$ (from $\calS_{\ell-1}$) proportionally with respect to $p_j(v)$ and route the corresponding proportion to $C_j \in \calS_{\ell+1}$ (on the next level).

\begin{lemma}\label{lemma:flow-entering-cluster}
  The total amount of $v$-associated flow entering (the center of) $C_i \in \calS_\ell$ is $\frac{p_i(v)}{w_\ell(v)}$, for all $\ell$ (i.e., $\ell \in \{0, \ldots, L+1\}$).
\end{lemma}
\begin{proof}
  Let $C_x \in \calS_{\ell-1}$ be a cluster on the previous level. From $C_x$ to $C_i$ we route a flow proportional to $p_i(v)$, hence we route a $\frac{p_i(v)}{w_{\ell}}$-fraction of $C_x$'s flow due to $w_\ell(v)$ be the normalizing factor (i.e., $\sum_{C_i \in \calS_{\ell}} \frac{p_i(v)}{w_{\ell}} = 1$). Note that this fraction does not depend on $x$, hence we route the same fraction of flow for each $C_x \in \calS_{\ell-1}$. Since the total amount of flow entering all (centers of) clusters on the previous level is $1$, we conclude that the amount of flow entering (the center of) $C_i$ is $\frac{p_i(v)}{w_{\ell}}$. Finally, we note that for $\ell = L+1$ and cheating node $c$, by definition the entire unit flow enters $c$. This agrees with the formula since $p_c(v) = w_{L+1}(v) = 1$, hence $1 = \frac{p_c(v)}{w_{L+1}(v)}$.
\end{proof}

\alert{CHECK IF EVERYTHING FITS WITHIN OUT EXTENDED DEFINITION OF CLUSTERS AND WHATNOT .. from this point on!}

\begin{lemma}
  The total amount of $v$-associated flow routed between (the center of) $C_i \in \calS_\ell$ and (the center of) $C_j \in \calS_{\ell+1}$ is $f_{ij}(v) = \frac{p_i(v)}{w_\ell(v)} \cdot \frac{p_j(v)}{w_{\ell+1}(v)}$, for all $\ell$ (i.e., $\ell \in \{1, \ldots, L\}$).
\end{lemma}
\begin{proof}
  We know that from $C_i$ to $C_j$ we route a flow proportional to $p_j(v)$, hence we route a $\frac{p_j(v)}{w_{\ell+1}}$-fraction of $C_i$'s flow since $\sum_{C_j \in \calS_{\ell+1}} \frac{p_j(v)}{w_{\ell+1}} = 1$. Combining it with the amount of flow entering $C_i \in \calS_\ell$ being $\frac{p_i(v)}{w_\ell(v)}$ (\Cref{lemma:flow-entering-cluster}), we get that $f_{ij}(v) = \frac{p_i(v)}{w_\ell(v)} \cdot \frac{p_j(v)}{w_{\ell+1}(v)}$, as needed.
\end{proof}

Finally, we specify the paths $\Path_{i, j}$ along which we route the flow between the centers $c_i$ of $C_i \in \calS_{\ell}$ and center $c_j$ of $C_j \in \calS_{\ell+1}$ (for all $\ell \in \{0, \ldots, L\}$). Assuming that $f_{i, j}(v) > 0$ (otherwise we need not specify the paths), We simply define $\Path_{i, j}$ to be an arbitrary path between $c_i$ and $c_j$ of length (distance) at most $\tilde{O}(R_\ell)$. This must exist since if $f_{i, j}(v) > 0$ we have that the core of both $C_i$ and $C_j$ contains $v$, hence their radii bounds tell us that $\dist_G(c_i, c_j) \le \dist_G(c_i, v) + \dist_G(v, c_j) \le R_\ell + R_{\ell+1} \le 2 \cdot R \cdot R_\ell = \tilde{O}(R_\ell)$.

\textbf{Misc calculations.}


\begin{lemma}\label{lemma:magnitude-properties-p-w}
  We have that for all $\ell$ (i.e., $\ell \in \{0, \ldots, L+1\}$:
  \begin{align*}
    %p_i(v) \le 1 \text{ \alert{is this even true?}}\\
    w_\ell(v) \ge 1/\valSNC \\
    %w_\ell(v) \le \gamma \text{ \alert{is this even true?}} \\
  \end{align*}
\end{lemma}
\begin{proof}
  For $\ell = 0$ or $\ell = L+1$ the claim is immediate from the definition. Otherwise, since $\calS_\ell$ is a sparse neighborhood cover of radius $R_\ell$ and quality $\valSNC$, the ball around $v$ of radius $R_\ell / \valSNC$ is contained in the core of some cluster $C_i \in \calS_{\ell}$. Therefore, $w_\ell(v) \ge p_i(v) = \dist_G(v, V(G) \setminus C_i) / R_\ell \ge (R_\ell / \valSNC) / (R_\ell) \ge 1/\valSNC$.
\end{proof}

\begin{lemma}
  Fix two nodes $u, v$ and let $d := \dist_G(u, v)$. For every $\ell$ (i.e., $\ell \in \{0, \ldots, L+1\}$) and each cluster $i \in \calS_\ell$ we have that:
  \begin{align} 
    p_i(u) - p_i(v) \le \frac{d}{R_\ell} \\
    | \{ i : p_i(v) \neq 0 \} | \le \gamma \label{eq:p-support-size} \\
    w_\ell(u) - w_\ell(v) \le 2 \gamma \cdot \frac{d}{R_\ell} = \tilde{O}(\frac{d}{R_\ell}) \\
    w_\ell(u) \le w_\ell(v) \cdot ( 1 + 2 \gamma \valSNC \frac{d}{R_\ell} ) = w_\ell(v) \cdot (1 + \tilde{O}(\frac{d}{R_\ell}) )
  \end{align}
\end{lemma}
\begin{proof}
  \begin{itemize}
  \item By triangle inequality, we have that: $p_i(u) \le \frac{\dist_G(u, V(G) \setminus C_i)}{R_\ell} \le \frac{\dist_G(u, v) + \dist_G(v, V(G) \setminus C_i)}{R_\ell} \le \frac{d}{R_\ell} + p_i(v)$.

  \item The support size $| \{ i : p_i(v) \neq 0 \} | \le \gamma$ since in each clustering only one cluster can contain $v$, and only that cluster (within the clustering) can have $p_i(v) \neq 0$.

  \item Due to the support size, we have that $w_\ell(v) - w_\ell(u) \le \sum_{C_i \in \calS_\ell} p_i(v) - p_i(v) \le 2 \gamma \frac{d}{R_\ell}$ as the difference is $0$ whenever $p_i(v) = p_i(u) = 0$.

  \item $w_\ell(u) = w_\ell(v) \cdot \frac{w_\ell(u)}{w_\ell(v)} \le w_\ell(v) \cdot \frac{w_\ell(v) + 2 \gamma d/R_\ell}{w_\ell(v)} \le w_\ell(v) \cdot (1 + 2 \gamma \valSNC \frac{d}{R_\ell}) = (1 + \tilde{O}(\frac{d}{R_\ell})) \cdot w_\ell(v)$ ... in the last inequality we used $w_\ell(v) \ge 1/\valSNC$ from \Cref{lemma:magnitude-properties-p-w}.
  \end{itemize}
\end{proof}


\begin{lemma}
  Fix two nodes $u, v$ and let $d := \dist_G(u, v)$. For every $\ell$ (i.e., $\ell \in \{0, \ldots, L\}$) and each two clusters $i \in S_\ell, j \in S_{\ell+1}$ we have that:
  \begin{align}
    R_\ell \cdot [ f_{i, j}(u) - f_{i, j}(v) ] \le \tilde{O}(d) ???
  \end{align}
\end{lemma}
\begin{proof}
  First, we note that the claim is trivial if $d \ge R_\ell$ since $0 \le f_{i, j} \le 1$, giving us that $| R_\ell \cdot [ f_{i,j}(u) - f_{i, j}(v) | \le 2 d = O(d)$. In the following, we assume that $d \le R_\ell$. To simplify calculations, we replace $\delta := d/R_\ell$ (note that $\delta \le 1$).
  \begin{align*}      
    f_{i,j}(u) - f_{i, j}(v) & = \frac{p_i(v)}{w_\ell(v)} \cdot \frac{p_j(v)}{ w_{\ell+1}(v) } - \frac{p_i(u)}{w_\ell(u)} \cdot \frac{p_j(u)}{w_{\ell+1}(u)} \\
                             & = ( w_{\ell}(u) w_{\ell+1}(u) )^{-1} \cdot \left[ [1 + \tilde{O}(\delta)]^2 \cdot p_i(v) p_j(v) - p_i(u) p_j(u) \right] \\
                             & \le \valSNC^2 \cdot \left[ [1 + \tilde{O}(\delta)] \cdot p_i(v) p_j(v) - p_i(u) p_j(u) \right]
  \end{align*}
  \begin{align*}
    (1 + \tilde{O}(\delta)) p_i(v) p_j(v) - p_i(u) p_j(v) & \le (1 + \tilde{O}(\delta)) (p_i(u) + \delta) (p_j(u) + \delta) - p_i(u) p_j(v) \\
                                                          & = \tilde{O}(\delta) p_i(u) p_j(u) + \tilde{O}(\delta) + \tilde{O}(\delta)^2 \\
                                                          & \le \tilde{O}(\delta)
  \end{align*}
  Combining, we get that $f_{i,j}(u) - f_{i, j}(v) \le \valSNC^2 \cdot \tilde{O}(\delta) = \tilde{O}(d / R_\ell)$. Finally, we have that $R_\ell \cdot [ f_{i, j}(u) - f_{i, j}(v) ] \le R_\ell \cdot \tilde{O}(d / R_\ell) = \tilde{O}(d)$, as required.

\end{proof}

\end{itemize}


\textbf{Cost analysis.}

\begin{lemma}
  It is sufficient to prove it for every pair of nodes $u, v$ that they are $\alpha$-approximate. \alert{write this out}
\end{lemma}
\begin{proof}
  BLA
\end{proof}


Fix two nodes $u, v$ and let $d := \dist_G(u, v)$. Let $w_G(\Path_{i, j})$ be the length of $\Path_{i, j}$. Calculation of the total cost between $u, v$:
\begin{align*}
  \sum_{C_i, C_j \in \calS} w_G(\Path_{i, j}) \cdot | f_{i, j}(v) - f_{i, j}(u) | & \le \sum_{\ell=0}^{L} \sum_{C_i \in \calS_\ell} \sum_{C_j \in \calS_{\ell+1}} w_G(\Path_{i, j}) \cdot | f_{i, j}(v) - f_{i, j}(u) | \\
                                                                                  & \le \sum_{\ell=0}^{L} \sum_{C_i \in \calS_\ell} \sum_{C_j \in \calS_{\ell+1}} \tilde{O}(R_\ell) \cdot | f_{i, j}(v) - f_{i, j}(u) | \\
                                                                                  & \le \sum_{\ell=0}^{L} \sum_{C_i \in \calS_\ell} \sum_{C_j \in \calS_{\ell+1}} \1{f_{i, j}(u) \neq 0 \lor f_{i, j}(v) \neq 0} \cdot \tilde{O}(d)  \\
                                                                                  & \le (L+1) \cdot 2\gamma \tilde{O}(d) = \tilde{O}(d) \\
\end{align*}


%%% END OLD STUFF
\fi


% Local Variables:
% TeX-master: "main"
% End:





==> Deterministic_SSSP/minor-aggregation-model.tex <==
\section{Computational Models: Minor-Aggregation, \congest, \pram}\label{sec:computational-models}

In this section we give a description of various models we use throughout this paper.

\subsection{\congest model}

First, we define the standard distributed model of computation called \congest. Any algorithm defined in the \aggregate model efficiently compiles down to \congest.

\begin{definition}[\congest]
  We are given an undirected graph $G = (V, E)$ called the ``communication network''. The vertices of $G$ are called nodes and they are independent computational units (i.e., have their own processor and private memory). Communication between nodes occurs in synchronous rounds. In each round, each pair of nodes adjacent in $G$ exchange $O(\log n)$ bits. Nodes perform arbitrary local computation between rounds. Initially, nodes wake up at the same time and only know their unique $O(\log n)$-bit ID.
\end{definition}

\subsection{Partwise Aggregation, Low-Congestion Shortcut Framework, and the \congestPA model}
We start by giving some background on partwise aggregation (PA) and the low-congestion shortcut framework before defining the \congestPA model.

\textbf{Partwise aggregation (PA)} is a high-level primitive that frequently arises while designing distributed (and parallel) algorithms. A partwise aggregation task is specified by giving each node a \emph{private value}, choosing a simple aggregation function such as min, max, or sum, and specifying a collection of connected and node-disjoint subsets $P_1, P_2, \ldots \subseteq V$. To solve partwise aggregation, all nodes $v$ are required to output the aggregate of all private values of the nodes in $v$'s part. Note that PA is immediately solvable in parallel using near-linear work and polylogarithmic depth. 

While extremely simple, the utility of PA stems from the fact that many important graph problems (e.g., MST, SSSP, min-cut, etc.) can be reduced to a small (polylogarithmic or $n^{o(1)}$) number of partwise aggregation instances. Therefore, any reduction to $\poly\log n$ many PA instances directly gives near-optimal parallel algorithms.

\textbf{The low-congestion shortcuts framework} was first introduced in \cite{GH16} and developed over a long sequence of works~\cite{GH16,haeupler2016low,haeupler2016near,haeupler2018round,haeupler2018minor,ghaffari_haeupler2021shortcuts_in_minor_closed,haeupler2021universally,kogan2021low,ghaffari2021hop,GHR21}. %that recently culminated in the design of universally-optimal distributed algorithms.
The framework defines a natural graph parameter called $\shortcutQuality{G}$ which assigns a number to each undirected and unweighted graph $G$. The framework then shows that shortcut quality is \emph{THE} parameter that characterizes the distributed complexity for a large class of seemingly unrelated graph problems. In particular: any distributed \congest algorithm for MST, (approximate) min-cuts, connectivity, max-flow, partwise aggregation~\cite{haeupler2021universally}, and SDD or Laplacian system solving~\cite{forster2020minor,anagnostides2021accelerated} requires \emph{at least} $\shortcutQuality{G}$ rounds on a network $G$ (up to polylogarithmic factors), even if only a non-trivial approximation is required and randomization is allowed. In more details, on a fixed graph $G$ the adversary can always force any correct algorithm to require $\tilde{\Omega}(\shortcutQuality{G})$ rounds if the adversary is allowed to choose the input (e.g., edge weights).
%We remark that this lower bound holds when 

On the other hand, the framework complements the above lower bound with an efficient distributed implementation of partwise aggregation. The ultimate goal would be to show that PA can be solved in (deterministic) $\tilde{O}(\shortcutQuality{G})$ \congest rounds, which would be near-optimal and would yield unconditional universally near-optimal algorithms for all of the above problems. However, we currently only achieve such a result under some conditions about the graph topology $G$. For example, such a result can be achieved in excluded-minor graphs where \cite{haeupler2016low} and \cite{haeupler2018minor} show that PA can be solved in $\tilde{O}(\shortcutQuality{G}) = \tilde{O}(\hopDiameter{G})$ rounds. Moreover, very recent work on hop-bounded oblivious routings and hop-bounded expander decomposition~\cite{ghaffari2021hop,GHR21} shows that PA can be solved in randomized $n^{o(1)}$ \congest rounds whenever $\shortcutQuality{G} \le n^{o(1)}$.

With the knowledge that PA can be efficiently implemented, we define the \congestPA  model which is simply \congest with access to a PA oracle.
\begin{definition}[\congestPA model]
  The \congestPA model naturally extends the \congest model. However, in each round we can choose to either perform a standard \congest round, or we can call the PA oracle. For the latter, each node chooses a private input at the start and learns the partwise aggregate at the end of the round.
\end{definition}

Per the above discussion, we can implement the PA oracle with the following constraints.
\begin{theorem}\label{thm:congestpa-simulation}
  A $\tau$-round \congestPA algorithm can be simulated in $\tilde{O}(\tau \cdot \tau_{PA})$ rounds of \congest, where $\tau_{PA}$ is the number of rounds in which one can solve any partwise aggregation instance on $G$. The following bounds have been proven for $\tau_{PA}$:
  \begin{itemize}
  \item For all graphs $G$, there is a deterministic algorithm with $\tau_{PA} \le \tilde{O}(\hopDiameter{G} + \sqrt{n})$.~\cite{GH16}
  \item If $G$ is minor-free, there is a deterministic algorithm with $\tau_{PA} \le \tilde{O}(\hopDiameter{G})$ (the hidden constants depend on the family).~\cite{ghaffari_haeupler2021shortcuts_in_minor_closed}
  \item If the nodes of $G$ know the topology in advance, there is a randomized algorithm with $\tau_{PA} \le \tilde{O}(\shortcutQuality{G})$.~\cite{haeupler2021universally}
  \item If $\shortcutQuality{G} \le n^{o(1)}$, there is a randomized algorithm with $\tau_{PA} \le n^{o(1)}$.~\cite{GHR21}
  \end{itemize}
\end{theorem}

\subsection{Minor-Aggregation Model}
\label{subsec:minor_aggregation}

In this section we define the \aggregate model, defined in \cite{goranci2022universally} and \cite{ghaffari2021universally}, an expressive model which provides an easy-to-use interface to the most recent advancements in the low-congestion framework. Specifically, the \aggregate model leverages partwise aggregation to implement fast aggregation operations on minors of the communication network $G$. The connection between minor aggregations and partwise aggregations is straightforward: computing a partwise aggregate is basically the same as computing a node-wise aggregate in the minor in which each part is contracted.

We first define a notion of aggregations and then formally specify the Distributed \aggregate model.

\begin{definition}[Aggregation operator]
  An aggregation operator $\bigoplus$ takes two $B$-bit inputs $m_1, m_2$ for some $B = \tilde{O}(1)$, and combines them into a new $B$-bit output $m_1 \bigoplus m_2$. Furthermore, given $k$ inputs $m_1, \ldots, m_k$, their $\bigoplus$-aggregate $\bigoplus_{i=1}^k m_i$ is the result from arbitrarily aggregating some two inputs until a single one remains.
\end{definition}

Note that for a commutative and associative operator (e.g., sum or max), the value $\bigoplus_{i=1}^n m_i$ is unique.
However, we gain flexibility by allowing for arbitrary operators where the output might depend on the execution sequence. 

\begin{definition}[Distributed Minor-Aggregation model]\label{def:aggregation-congest}
  We are given an undirected graph $G = (V, E)$. Both nodes and edges are separate computational units (i.e., have their own processor and private memory). Communication occurs in synchronous rounds and nodes/edges perform $\tilde{O}(1)$-work local computation between rounds. Initially, nodes wake up at the same time and only know their unique $\tilde{O}(1)$-bit ID, while edges know the IDs of their endpoints. Each round consists of the following three steps (in that order).
  \begin{itemize}    
  \item \textbf{Contraction step.} Each edge $e$ chooses a value $c_e = \{\bot, \top\}$. This defines a new \emph{minor network} $G' = (V', E')$ constructed as $G' = G / \{ e : c_e = \top \}$, i.e., by contracting all edges with $c_e = \top$ and self-loops removed. Vertices $V'$ of $G'$ are called supernodes, and we identify supernodes with the subset of nodes $V$ it consists of, i.e., if $s \in V'$ then $s \subseteq V$.

  \item \textbf{Consensus step.} Each individual node $v \in V$ chooses a $\tilde{O}(1)$-bit value $x_v$. For each supernode $s \in V'$ we define $y_s := \bigoplus_{v \in s} x_v$, where $\bigoplus$ is some predefined aggregation operator. All nodes $v \in s$ learn $y_s$.

  \item \textbf{Aggregation step.} Each edge $e \in E'$ connecting supernodes $a \in V'$ and $b \in V'$ learns $y_a$ and $y_b$, and chooses two $\tilde{O}(1)$-bit values $z_{e, a}, z_{e, b}$ (i.e., one value for each endpoint). Finally, (every node of) each super $s \in V'$ learns the aggregate of its incident edges in $E'$, i.e., $\bigotimes_{e \in \text{incidentEdges(s)}} z_{e, s}$ where $\bigotimes$ is some predefined aggregation operator.
  \end{itemize}
\end{definition}

\textbf{Distributed storage and inputs.} Our \aggregate algorithm operates on objects that are \emph{``distributedly'' stored}, meaning that each processor has its own part of the object in private memory. Specifically, we store a \emph{node vector} $x \in \R^V$ by storing $x_v$ in node $v$. Similarly, edge vectors $x \in \R^{E}, x \in \R^{\vec{E}}, x\in \R^{\overleftrightarrow{E}}$ are distributed over edges. Subgraphs $H \subseteq G$ are specified by distributedly storing the characteristic vectors $\mathbb{1}_{V(H)} \in \R^{E(G)}$ and $\mathbb{1}_{E(H)} \in \R^{E(G)}$. Initially, the problem-specific input is assumed to be distributedly stored. For transshipment and SSSP, we assume the lengths (edge vector) and demands (node vector) are stored. At termination, the output is required to be distributedly stored.

\textbf{Minors.} Algorithms designed in this model can take advantage of several high-level primitives typically unavailable in other distributed models (due to the power of being able to solve PA). Notably, any algorithm can be run on any minor in a black-box manner. For example, this allows extremely simple descriptions of contraction-based algorithms such as Boruvka's MST algorithm.

\begin{corollary}\label{corollary:computation-on-minors}
  Any $\tau$-round \aggregate algorithm on a minor $G' = G / F$ of $G = (V, E)$ can be simulated via a $\tau$-round \aggregate algorithm on $G$. Initially, each edge $e \in E$ needs to know whether $e \in F$ or not. Upon termination, each node in $G$ learns all the information that the supernode it was contained in learned.
\end{corollary}

\textbf{Node-disjoint scheduling.} It is immediate, but useful to note, that we can can simultaneously run algorithms on node-disjoint subsets.
\begin{corollary}\label{lemma:node-disjoint-scheduling}
  Let $G$ be an undirected graph. Given any $\tau$-round \aggregate algorithms $A_1, \ldots, A_k$ running on node-disjoint and connected subgraphs (of $G$) $H_1, H_2, \ldots, H_k$, we can run $A_1, \ldots, A_k$ simultaneously within a $\tau$-round \aggregate algorithm $A$ that runs on $G$.
\end{corollary}

\textbf{Ancestor and subtree sums.} The following operation, proven in \cite{ghaffari2021universally}, is often useful.
\begin{lemma}[Ancestor and subtree sums]\label{lemma:ancestor-subtree-sum}
  Let $F$ be a forest (each edge $e$ knows whether $e \in E(F)$ or not) and suppose that each connected component has a unique root (each node knows whether it is the root). Suppose each node $v$ has an $\tilde{O}(1)$-bit private input $x_v$. There is a deterministic $\tilde{O}(1)$-round Minor-Aggregation algorithm that computes for each node $v$ the values values $p_v := \bigoplus_{\ell \in A(v)} x_w$ and $s_v := \bigoplus_{\ell \in D(v)} x_w$, where $A(v)$ and $D(v)$ are the set of ancestors and descendants of $v$ of $F$ with respect to the root, where $\bigoplus$ is some pre-defined aggregation operator.
\end{lemma}

\textbf{Simulation in \congest and \pram.} It is immediately clear that any \aggregate algorithm can be turned into a fast \pram algorithm. However, the power of the \aggregate framework comes from the possibility of compiling it to an efficient distributed (i.e., \congest) algorithm, assuming the partwise aggregation oracle can be solved efficiently---which is provided by the low-congestion shortcut framework (under some conditions). This is formalized in the following theorem.

\begin{theorem}\label{thm:compilation_pa_congest}
  Let $A$ be any (deterministic) $\tau$-round \aggregate algorithm on $G$ with $n := |V(G)|$ and $m := |E(G)|$. In \pram, we can deterministically simulate $A$ with $\tilde{O}(m \cdot \tau)$ work and $\tilde{O}(\tau)$ depth. Furthermore, in the distributed setting, we can simulate $A$ in $\tilde{O}(\tau)$ \congestPA rounds.
\end{theorem}
\begin{proof}
  The \pram part of the theorem is immediate. The randomized \congestPA simulation is proven in \cite{goranci2022universally}, albeit without explicitly defining the \congestPA model. The deterministic \congestPA simulation is proven in \cite{ghaffari2021universally}, albeit also without explicitly defining the \congestPA model.
\end{proof}


\subsection{Virtual Nodes in the \aggregate Model}

Another useful high-level primitive is adding $\tilde{O}(1)$ arbitrarily-connected virtual nodes to the communication network $G$ and running an arbitrary \aggregate algorithm in a black-box manner on the new graph while only incurring a $\tilde{O}(1)$ slowdown. Note that such an operation is completely inadmissible in other models of distributed computing like \congest~\cite{peleg2000distributed} where nodes are allowed to send/receive arbitrary (i.e., non-aggregate) information to/from each one of their neighbors separately, as this would allow efficiently communicating the entire network topology to a single node and solving the problem locally. On the other hand, virtual-node addition can be efficiently simulated in the \aggregate model due to the ``aggregate''-nature of communication. For example, we use this operation to connect a ``supersource'' node, enabling us to use our standard SSSP algorithm to implement a set-source-$S$ shortest path.

Given a graph $G$, we can construct a \emph{virtual graph} by repeatedly adding a \emph{virtual node} and connecting it to an arbitrary set of neighbors. This is formalized in the following definition.
\begin{definition}
  A virtual graph $G\virt$ extending a connected graph $G = (V, E)$, is a graph whose node set can be partitioned into $V$ and a set of so-called \emph{virtual nodes} $V\virt$, i.e., $V(G\virt) = V \sqcup V\virt$. Furthermore, the edge set $E(G\virt)$ can be partitioned into $E$ and a set of so-called \emph{virtual edges} $E\virt$ with the property that every virtual edge is adjacent to at least one virtual node. We say $G\virt$ has at most $\beta$ virtual nodes if $|V\virt| \le \beta$.
\end{definition}

\textbf{Distributed storage of virtual graphs.} In order to ``construct'' a virtual graph, one needs to be able to distributedly store it; unfortunately, this requires specifying some low-level storage details. A virtual graph $G\virt$ is distributedly stored in $G$ in the following way. A virtual edge connecting a non-virtual $u$ and a virtual $v$ is only stored in $u$ (other nodes do not need to know about its existence). A virtual edge between two virtual nodes is required to be known by all nodes. All nodes know about all virtual nodes.

% \begin{definition}[Virtual node addition]\label{def:virtual-node-addition}
%   Adding a virtual node to a graph $G = (V, E)$ corresponds to changing $G$ into $G\virt = (V \cup \{\mathrm{virt}\}, E \cup \bigcup_{v \in \Gamma\virt} \{ \mathrm{virt}, v\})$, where $\mathrm{virt}$ is a new ``virtual'' node, and $\Gamma\virt \subseteq V$ are the set of neighbors of $\mathrm{virt}$. Edges adjacent to virtual nodes are called ``virtual edges''.
% \end{definition}

\textbf{Simulations on virtual graphs.} We can add $\beta$ many virtual (arbitrarily interconnected) nodes to any graph $G$ and still simulate any Minor-Aggregation algorithm on the virtual graph with a $O(\beta + 1)$ blowup in the number of rounds. We say a node/edge $a$ simulates a virtual node/edge $v$ if $a$'s private memory contains all data of $v$'s private memory in the virtual graph (i.e., $a$ knows what $v$ is outputting in each round, and learns everything $v$ receives). The following simulation result formalizes this (proven in \cite{ghaffari2021universally}).
\begin{theorem}\label{thm:simulating-virtual-nodes}
  Suppose $A\virt$ is a $\tau$-round Minor-Aggregation algorithm on a virtual graph $G\virt(\beta)$ that extends $G$ and has at most $\beta$ virtual nodes. Any such $A\virt$ can be simulated in $G$ with a $\tau \cdot O(\beta + 1)$-round Minor-Aggregation algorithm.
  Upon termination, each non-virtual node $v \in V(G)$ learns all information learned by $v$ and all virtual nodes in $A\virt$.

  Each virtual node is simulated by all (non-virtual) nodes. Similarly, the virtual edges connecting two virtual nodes are simulated by all nodes, while the edges connecting a virtual and a non-virtual node are simulated by the non-virtual node.
\end{theorem}

Suppose we are given a \aggregate algorithm on a graph with virtual nodes. We can simulate the algorithm in \congest by first applying \Cref{thm:simulating-virtual-nodes}, thereby obtaining a (non-virtual) \aggregate algorithm. Then, we can use the general simulation results \Cref{thm:compilation_pa_congest,thm:oracleSimulation} to obtain a \congest algorithm.

\subsection{Oracles in the \congest and Minor-Aggregation Model}

An oracle is a black-box function that takes a certain input (on the original graph) and produces a specified output. A \aggregate/\congest algorithm with access to an oracle can, in each round, choose to perform a regular \aggregate/\congest round, or to make a single oracle call (i.e., multiple oracle calls per round are forbidden). For example, \congestPA is simply the \congest model with access to the PA oracle. 
The reason why oracles are useful are results like the following fact that follows from \cref{thm:compilation_pa_congest}. 

\begin{fact}[Oracle simulation]
  \label{thm:oracleSimulation}
  Suppose $A$ is a $\tau$-round \aggregate algorithm with access to oracles $\fO^1, \ldots, \fO^k$. The following simulation results hold:
  \begin{enumerate}
  \item Suppose each oracle $\fO^i$ call can be simulated in \pram in at most $\tau_{work}$ work and $\tau_{time}$ time. Then $A$ can be simulated with a \pram algorithm in total work $\tilde{O}(\tau \cdot (\tau_{work} + m))$ and total time $\tilde{O}(\tau \cdot (\tau_{time} + 1))$.

  \item Suppose each oracle $\fO^i$ call can be simulated in \congestPA in at most $\tau_{oracle}$ rounds. Then $A$ can be simulated with a \congestPA algorithm in at most $\tilde{O}(\tau \cdot (\tau_{oracle} + 1))$ rounds.
  
  \item Suppose each oracle $\fO^i$ call can be simulated in \congest in at most $\tau_{oracle}$ rounds. Then $A$ can be simulated with a \congest algorithm in at most $\tilde{O}(\tau \cdot (\tau_{oracle} + \sqrt{n} + \hopDiameter{G} ))$ rounds. 
  
    \item Suppose each oracle $\fO^i$ call can be simulated in \congest in at most $\tau_{oracle}$ rounds on a fixed minor-free family. 
    Then $A$ can be simulated with a \congest algorithm in at most $\tilde{O}(\tau \cdot (\tau_{oracle} + \hopDiameter{G} ))$ rounds. 
  \end{enumerate}
\end{fact}


\begin{comment}
For the distributed setting, we can combine the fact above with the \congestPA simulation result (\Cref{thm:congestpa-simulation}) to obtain the following result.
\begin{corollary}\label{corollary:minor-oracle-to-congest}
  Suppose $A$ is a $\tau$-round \aggregate algorithm with access to oracles $\fO^1, \ldots, \fO^k$ that can all be implemented in at most $\tau_{oracle}$ \congestPA rounds. Then $A$ can be simulated in $\tilde{O}(\tau \cdot \tau_{PA})$ \congest rounds, where the bounds from \Cref{thm:congestpa-simulation} apply. In particular, on excluded-minor graphs, $A$ can be simulated in $\tilde{O}(\tau \cdot \hopDiameter{G})$ \congest rounds.
\end{corollary}
\end{comment}
% Local Variables:
% TeX-master: "main"
% End:



==> Deterministic_SSSP/missingproofsgeneralresults.tex <==
\section{Missing Proofs of \cref{sec:localiterative}}
\label{sec:missingProofs}
\cycleone*

\begin{proof}
Combining \cref{lem:cycletwo} and \cref{lem:cyclethree} implies that $\oPot_{D_i}$ and $\oDist_{\eps,D}$ can be efficiently computed for every $D \in \left[\frac{D_i}{\valSNC},D_i \right]$ and every $\eps = \frac{1}{\tilde{O}(1)}$.
Being able to efficiently compute $\oDist_{\eps,D}$ for every $D \in \left[\frac{D_i}{\valSNC},D_i\right]$ and every $\eps = \frac{1}{\tilde{O}(1)}$  together with \cref{lem:cyclefour} implies that we can efficiently compute a sparse neighborhood cover with covering radius $\frac{D_i}{\valSNC}$ together with a rooted spanning tree $T_C$ of diameter at most $D_i$ for every cluster $C$ in the cover.
Moreover, once we have computed such a sparse neighborhood cover, \cref{lem:cyclefive} together with the fact that we can efficiently compute $\oPot_{D_i}$ implies that we can efficiently compute a distance structure for the scale $D_i$, as desired.
\end{proof}

\cycletwo*

\begin{proof}
Directly follows from the first part of \cref{thm:oblivious_routing}.
\end{proof}


\cyclethree*

\begin{proof}

Consider an arbitrary $D \in \left[\frac{D_i}{\valSNC},D_i \right]$ and $S  \subseteq V$. 
We show how to answer both $\oDist_{\frac{1}{\log^3(n)},D}(S)$ and $\oPot_{D_i}(S)$.

In case $S = \emptyset$, we can answer $\oDist_{\frac{1}{\log^3(n)},D}(S)$ by returning an empty forest and $\oPot_{D_i}(S)$ by setting $\phi_{S,D_i}(v) = D_i$ for every $v \in V$.
Hence, it remains to consider the case $S \neq \emptyset$.


When $S$ is the first input given to $\oObliv_{D_i}$, then $\oObliv_{D_i}$ implements matrix-vector products with some fixed matrix. We denote this matrix by $R_S$.
%For a moment, assume that our actual input graph is $G_{S,D_i}$ instead of $G$.
We invoke \cref{theorem:boosting_rounding} with $R = R_S$, $H = G_{S,D_i}$, $\eps = \frac{1}{10\log^3(n)\valSNC}$ and $s = \sstar$ to get an algorithm running in $\tilde{O}(1)$ \aggregate rounds when given access to the rounding oracle $\oRound_{\eps/2} = \oRound$ and an oracle which performs matrix-vector products with $R_S$ and $R_S^T$.

The output of the algorithm consists of two parts.
First, a potential $\phi$ for $G_{S,D_i}$ with $\phi(\sstar) = 0$. \\
Second, a tree $T \subseteq G_{S,D_i}$ rooted at $\sstar$ such that for each $v \in V(G_{S,D_i})$ we have $\dist_T(\sstar, v) \leq (1+\eps) \phi(v)$.

We can efficiently simulate this algorithm in $G$, viewing $G_{S,D_i}$ as a virtual graph with two virtual nodes that extend $G$.
Indeed, \cref{thm:simulating-virtual-nodes} implies that each \aggregate round in $G_{S,D_i}$ can be simulated with $O(1)$ \aggregate rounds in $G$. Moreover, we can use the oracle $\oObliv_{D_i}$ to compute the $\tilde{O}(1)$ matrix-vector products with $R_S$ and $R_S^T$. Finally, we can directly simulate the oracle $\oRound$ for the virtual graph $G_{S,D_i}$ with the oracle $\oRound$ for the actual graph $G$, as the set of valid input graphs for both oracles are the same.

Next, we show that $T$ can be used to efficiently answer $\oDist_{\frac{1}{\log^3(n)},D}(S)$ and $\phi$ can be used to efficiently answer $\oPot_{D_i}(S)$.

\paragraph{Implementing the Forest Oracle}

We answer $\oDist_{\frac{1}{\log^3(n)},D}(S)$ by returning the rooted forest $F$ with 

\begin{enumerate}
    \item $V(F) = \{v \in V \colon \dist_T(\sstar, v) \leq (1+\eps)(D_i + D)\}$,
    \item each node $v \in V(F) \cap S$ is a root in $F$, and
    \item each node $v \in V(F) \setminus S$ has the same parent in $F$ and $T$.
\end{enumerate}

Note that $F$ is only well-defined if for each node $v \in V(F) \setminus S$, the parent of $v$ in $T$, which we denote by $p_v$, is actually a vertex in $F$.
We first verify that $p_v \in V$, which is equivalent to $p_v \notin \{\sstar, v_D\}$. Clearly, $p_v \neq s^*$, as there is no edge in $G_{S,D_i}$ between $s^*$ and a node in $V \setminus S$.
For the sake of contradiction, assume that $p_v = v_D$. Then, 
\begin{align*}\dist_T(\sstar,v) = \dist_T(\sstar, v_D) + \dist_T(v_D,v) \geq 2D_i + D_i> (1+\eps)(D_i + D),
\end{align*}
which is a contradiction with $\dist_T(\sstar,v) \leq (1+\eps)(D_i + D)$, which follows from $v \in V(F)$.
Hence, $p_v \in V$ and as $\dist_G(\sstar,p_v) \leq \dist_G(\sstar,v)\leq (1+\eps)(D_i + D)$, we can conclude that $p_v \in V(F)$.

Next, we show that each node $v \in V$ with $\dist_G(S,v) \leq D$ is contained in $V(F)$. 
This is indeed the case as 
\begin{align*}\dist_T(\sstar,v) \leq (1+\eps)\dist_{G_{S,D_i}}(\sstar,v) \leq (1+\eps)(D_i + D).
\end{align*}

In particular, each node in $S$ is contained in $V(F)$ and therefore $F$ is a forest rooted at $S$. 
It therefore remains to verify that for each node $v \in V(F)$, $\dist_F(S,v) \leq (1+\frac{1}{\log^3(n)})D$.
To that end, consider the unique path between $\sstar$ and $v$ in the tree $T$. This path contains at least one vertex in $S$. Let $s$ be the last vertex in $S$ on that path. From the previous discussion, it follows that $\dist_F(s,v) = \dist_T(s,v)$, as the unique path between $s$ and $v$ in $T$ is fully  contained in $F$. We therefore have,

\begin{align*}
    &\dist_F(S,v) \leq \dist_T(s,v) \leq \dist_T(\sstar,v) - D_i \\
    &\leq (1+\eps)(D_i + D) - D_i\leq D + 2\eps D_i\leq \left( 1+\frac{1}{\log^3(n)} \right) D,
\end{align*}

where the last inequality follows from $D \geq \frac{D_i}{\valSNC}$ and $\eps \leq \frac{1}{2\log^3(n)\valSNC}$.




\paragraph{Implementing the Potential Oracle}
We answer $\oPot_{D_i}(S)$ by setting for each $v \in V$
$$\phi_{S,D_i}(v) = \max(\phi(v) - D_i,0).$$

As $\phi_{S,D_i}$ can be written as a maximum of two potentials, $\phi_{S,D_i}$ is a valid (non-negative) potential according to \cref{fact:potential_min_max}. It therefore remains to verify the two conditions stated in \cref{def:potential}. We first verify the first condition. Consider am arbitrary vertex $v \in S$. We have

\begin{align*}\phi(v) \leq \phi(\sstar) + |\phi(v) - \phi(\sstar)| \leq 0 + \ell_{G_{S,D_i}}(s^*,v) \le D_i
\end{align*}

and therefore $\phi_{S,D_i}(v) = 0$.



To verify the second condition, consider an arbitrary $v \in V$ with $\dist_G(v,S) \geq \frac{D_i}{\valSNC}$. We have



\begin{align*}\phi_{S,D_i}(v) \geq \phi(v) - D_i \geq \frac{\dist_T(\sstar, v)}{1+\eps} - D_i \geq \frac{D_i + \dist_G(v,S)}{1+\eps} - D_i \geq \frac{D_i/\valSNC - \eps D_i}{1+\eps} \geq 0.5\frac{D_i}{\valSNC},
\end{align*}


where the last equality follows from $\eps \leq \frac{1}{10 \valSNC}$. 
\end{proof}



\cyclefour*

\begin{proof}
Directly follows from \cref{thm:sparse_cover} with $D = D_i$.
\end{proof}

\cyclefive*

\begin{proof}
Given the sparse neighborhood cover together with the trees, the only missing piece for the distance structure for the scale $D_i$ is a potential for the scale $D_i$ with respect to $V \setminus C$ for every cluster $C$ in one of the clusterings (which only needs to be known to the nodes inside $C$).

Let $\fC$ be one of the clusterings in the sparse neighborhood cover.  
We show how to simultaneously compute for each cluster $C \in \fC$ a potential for scale $D_i$. 

For each node $v$, let $id(v)$ denote the unique $O(\log n)$-bit identifier of $v$.
We assign each cluster $C \in \fC$ an identifier by concatenating the identifier of its cluster center $id(v_C)$ with the bit-wise negation of $id(v_C)$.
We call the resulting $b$-bit identifier $id(C)$.
For $j \in [b]$, we say that a cluster is active in round $j$ if the $j$-th bit of its identifier is $1$.
Note that for two distinct clusters $C_1,C_2 \in \fC$, there exists at least one round in which $C_1$ is active and $C_2$ is inactive.
We denote with $V_{active,j} \subseteq V$ the set of vertices that are contained in a cluster that is active in round $j$.
In round $j$, we use oracle $\oPot_{D_i}$ with input $V \setminus V_{active,j}$ to compute a potential $\phi_j$ for scale $D_i$ with respect to $V \setminus V_{active,j}$.

For each cluster $C \in \fC$ and $v \in V$, we set $\phi_{V \setminus C, D_i}(v) = \min_{\text{$j \colon$ $C$ is active in round $j$}} \phi_j(v)$.

We show that $\phi_{V \setminus C,D_i}$ is a potential for scale $D_i$ with respect to $V \setminus C$.

First, $\phi_{V \setminus C, D_i}$ is the minimum of non-negative potentials and therefore a non-negative potential itself according to \cref{fact:potential_min_max}.
It therefore remains to verify that $\phi_{V \setminus C, D_i}$ satisfies the two conditions of \cref{def:potential}. To verify the first condition, consider an arbitrary $v \in V \setminus C$. We have to show that $\phi_{V \setminus C, D_i}(v) = 0$. There exists some round $j$ in which $C$ is active and $v$ is not contained in an active cluster. For this $j$, $\phi_j(v) = 0$ and therefore $\phi_{V \setminus C, D_i}(v) = 0$, as desired.


It remains to check the second condition. To that end, consider an arbitrary $v \in V$ with $\dist_G(v,V \setminus C) \geq \frac{D_i}{\valSNC}$.
We need to show that this implies $\phi_{V \setminus C,D_i}(v) \geq 0.5\frac{D_i}{\valSNC}$.
Consider an arbitrary round $j$ in which $C$ is active.
As $\dist_G(v,V \setminus C) \geq \frac{D_i}{\valSNC}$, we have $\dist_G(v,V \setminus V_{active,j}) \geq \frac{D_i}{\valSNC}$ which in turn implies $\phi_j(v) \geq 0.5\frac{D_i}{\valSNC}$.
Hence, $\phi_{V \setminus C,D_i}(v) \geq 0.5\frac{D_i}{\valSNC}$.

The result now follows by iterating over all of the $O(\log n)$ clusterings in the sparse neighborhood cover.
\end{proof}

\cycleeuler*
\begin{proof}
Directly follows from \cref{thm:rounding}. 
\end{proof}


\cyclesix*

\begin{proof}
We prove by induction on $i$ that a distance structure for every scale $D_j$ with $j \leq i$ can be computed in $i \cdot \tilde{O}(1)$ \aggregate rounds.
The base case $i = 1$ directly follows from \cref{lem:cycleone}.
Now, consider an arbitrary $i > 1$ (such that $D_i$ is a scale) and assume that the claim above holds for $i-1$. Hence, we can compute a distance structure for every scale $D_j$ with $j \leq i - 1$ in $(i-1)\tilde{O}(1)$ \aggregate rounds.
Now, applying \cref{lem:cycleone} with the scale $D_i$ implies that in $\tilde{O}(1)$ additional \aggregate rounds we can compute a distance structure for the scale $D_i$, which finishes the induction step.
This finishes the proof, as there are only $O(\log n)$ different scales.
\end{proof}


\cycleseven*

\begin{proof}
Directly follows from the second part of \cref{thm:oblivious_routing}.
\end{proof}

\cycleeight*

\begin{proof}
First, \cref{lem:transshipment_primal_dual} implies that the $(1+\eps)$-transshipment problem can be solved in $\tO(1/\eps^2)$ \aggregate rounds.
Second, the tree returned by the algorithm of \cref{theorem:boosting_rounding} is a $(1+\eps)$-SSSP-tree and the algorithm runs in $\tO(1/\eps^2)$ \aggregate rounds, as each of the $\tilde{O}(1)$ matrix-vector products with $R$ and $R^T$ can be computed in $\tO(1)$ \aggregate rounds.
\end{proof} 

\cyclenine*

\begin{proof}
\cref{lem:cyclesix} states that a distance structure for every scale $D_i$ can be efficiently computed (as $\oRound$ can be implemented with $\oRound_{\eps/2}$).
Together with \cref{theorem:cycleseven}, this implies that there exists an $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing $R$ for $G$ for which $R$ and $R^T$ can be efficiently evaluated.
Combining this with \cref{theorem:cycleeight}, we can conclude that the $(1+\eps)$-transshipment problem and the $(1+\eps)$-SSSP-tree problem in $G$ can be efficiently solved.
\end{proof}

\cycleten*

\begin{proof}
Directly follows from \cref{theorem:cyclenine} together with \cref{lem:cycleeuler}. 
\end{proof}

\mainparallel*

\begin{proof}
\cref{thm:euler_pram} states that there exists a \pram algorithm with near-linear work and $\tO(1)$ depth that implements $\oEuler$. The result now follows by \cref{theorem:cycleten}. 
\end{proof}

\maindistributed*

\begin{proof}
\cref{thm:euler_dist} states that the oracle $\oEuler$ can be implemented with the desired round complexity. The result for the single source shortest path then follows from \cref{theorem:cycleten,thm:oracleSimulation}. 
To extend it to the shortest forest from the set $S$ problem, we add a virtual node $s$ to our graph and connect it to nodes of $S$ via edges of weight $0$ (technically, we do not allow zero weights, but we can choose the weight to be negligible to all other weights). Then, we use the fact that, by definition, the oracle $\oEuler$ supports virtual nodes and, by \cref{thm:simulating-virtual-nodes} we can simulate virtual nodes in the \aggregate model. 
\end{proof}


==> Deterministic_SSSP/preamble.tex <==
\usepackage{fullpage}
\usepackage{parskip}

\usepackage{amsthm,amsmath,amssymb,booktabs,xcolor,graphicx}
\usepackage{thm-restate}
\usepackage{bbm}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{appendix}
\usepackage{enumerate}
\usepackage{mathbbol}
\usepackage[numbers]{natbib}
\usepackage{comment}
\usepackage[shortlabels]{enumitem}

\usepackage[margin=1in]{geometry}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

%\usepackage[textsize=small,backgroundcolor=orange!20]{todonotes}
\usepackage[disable]{todonotes}
\usepackage[hidelinks]{hyperref}
\usepackage{url}
\usepackage{etoolbox}
\usepackage{appendix}
\usepackage{xspace}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
% \usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage[labelfont=bf]{caption}
\usepackage[noabbrev,capitalize]{cleveref}
\crefname{equation}{}{} %remove ``Equation''    
\newcommand{\creflastconjunction}{, and\nobreakspace} %Oxford comma
\AtBeginEnvironment{appendices}{\crefalias{section}{appendix}} %appendices

\usepackage[color,final]{showkeys} %add in 'final' into parameter to remove showkeys
\renewcommand\showkeyslabelformat[1]{\scalebox{.8}{\normalfont\footnotesize\ttfamily#1}\hspace{-.5em}}
% showkeys font
\colorlet{refkey}{orange!20}
\colorlet{labelkey}{blue!30}

% ------   Theorem Styles -------
\numberwithin{equation}{section}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{algo}[theorem]{Algorithm}
\crefname{claim}{Claim}{Claims}

\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem*{question*}{Question}
\newtheorem{fact}[theorem]{Fact}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{question}[theorem]{Question}
\newtheorem*{definition*}{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{setup}[theorem]{Setup}
\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\newtheorem*{notation}{Notation}
\newcommand{\assign}{\leftarrow}

%\newcommand{\alert}[1]{{\color{orange}#1}}
\newcommand{\alert}[1]{}
\renewcommand{\tilde}{\widetilde}

% ----- Delimiters ----
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\snorm}[1]{\lVert#1\rVert}
\newcommand{\ang}[1]{\left\langle #1 \right\rangle}
\newcommand{\sang}[1]{\langle #1 \rangle}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\sqb}[1]{\left[ #1 \right]}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\setcond}[2]{\left\{ #1 \;\middle\vert\; #2 \right\}}
\newcommand{\cond}[2]{\left( #1 \;\middle\vert\; #2 \right)}
\newcommand{\sqcond}[2]{\left[ #1 \;\middle\vert\; #2 \right]}
\newcommand{\one}{\mathbbm{1}}
\newcommand{\otilde}{\widetilde{O}}
\newcommand{\poly}{\mathrm{poly}}

\newcommand{\fC}{\mathcal{C}}
\newcommand{\mb}{\mathbb}
\newcommand{\potential}{\phi}
\newcommand{\mbf}{\mathbf}
\newcommand{\mbm}{\mathbbm}
\newcommand{\mc}{\mathcal}
\newcommand{\mf}{\mathfrak}
\newcommand{\mr}{\mathrm}
\newcommand{\ol}{\overline}
\newcommand{\on}{\operatorname}
\newcommand{\wh}{\widehat}
\newcommand{\wt}{\widetilde}
\newcommand{\edit}[1]{{\color{red}#1}}
\renewcommand{\l}{\langle}
\renewcommand{\r}{\rangle}
\newcommand{\RFin}[1]{2^{\mb{RP}^#1}_{\on{fin}}}
\newcommand{\g}{\nabla}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\argmin}{\mathrm{argmin}}
\newcommand{\eps}{\varepsilon}
\newcommand{\etal}{\textit{et~al.}}
\newcommand{\Tr}{\mathrm{Tr}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\ls}{\lesssim}
\newcommand{\pe}{\preceq}
\newcommand{\se}{\succeq}
\newcommand{\op}{\mathrm{op}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calS}{\mathcal{S}}
%\newcommand{\dist}{\mathrm{dist}}
\newcommand{\diam}{\textrm{diam}}
\newcommand{\parent}{\textrm{par}}
\renewcommand{\d}{d}
\newcommand{\Dpad}{D_\textrm{pad}}
\newcommand{\fO}{\mathcal{O}}
\newcommand{\setssp}{set-source shortest path\xspace}
\newcommand{\tO}{\tilde{O}}
\newcommand{\tG}{\tilde{G}}
\newcommand{\fP}{\mathcal{P}}
\newcommand{\polylog}{\mathrm{polylog\ }}
\newcommand{\btodo}[1]{{\bfseries ToDo: #1}\\}
\newcommand{\congest}{\ensuremath{\mathsf{CONGEST}}\xspace}
\newcommand{\congestPA}{\ensuremath{\mathsf{CONGEST}^{PA}}\xspace}
\newcommand{\aggregate}{\ensuremath{\mathsf{Minor}}\text{-}\ensuremath{\mathsf{Aggregation}}\xspace}
\newcommand{\pram}{\ensuremath{\mathsf{PRAM}}\xspace}
\newcommand{\euler}{\ensuremath{\textsc{Eulerian-}\textsc{Orientation}}\xspace}
\newcommand{\1}[1]{\mathbb{1}[#1]}
\newcommand{\cheat}{\ensuremath{^{\mathrm{cheat}}}\xspace}
\newcommand{\Path}{\mathrm{Path}}

\newcommand{\oEuler}{\fO^{Euler}}
\newcommand{\oRound}{\fO^{Round}}
\newcommand{\oDist}{\fO^{Forest}}
\newcommand{\oForest}{\fO^{Forest}}
\newcommand{\oPot}{\fO^{Pot}}
\newcommand{\oObliv}{\fO^{Obliv}}

\newcommand{\Dhop}{\hopDiameter{G}}
\newcommand{\sstar}{s^*}
\newcommand{\vD}{v_D}
\newcommand{\Lref}[1]{{\text{L\ref{#1}}}}
\newcommand{\Tref}[1]{{\text{T\ref{#1}}}}
\newcommand{\Pref}[1]{{\text{P\ref{#1}}}}
\newcommand{\Coref}[1]{{\text{C\ref{#1}}}}

\newcommand{\defeq}{\stackrel{\mathrm{\scriptscriptstyle def}}{=}}
\newcommand{\opt}{\mathrm{OPT}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\cost}{{\mathrm{cost}}}
\newcommand{\shortcutQuality}[1]{\mathrm{Shortcut}\-\mathrm{Quality}(#1)}
\newcommand{\hopDiameter}[1]{\mathrm{Hop}\-\mathrm{Diam}(#1)}
\newcommand{\diameter}{\mathrm{HopDiameter}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\virt}{\ensuremath{_{\mathrm{virt}}}\xspace}

\newcommand{\bnote}[1]{{\bfseries B: #1}}
\newcommand{\todob}[1]{}   %these are markers for my todo list

\newcommand{\core}{\mathrm{core}}
\newcommand{\pad}{\mathrm{pad}}
\newcommand{\Vrem}{V_\textrm{remaining}}
\newcommand{\Valive}{V_\textrm{alive}}
\newcommand{\Vdead}{V_\textrm{dead}}
\newcommand{\Vactive}{V_{\text{active}}}
\newcommand{\PA}{\ensuremath{^{\mathrm{PA}}}\xspace}

\newcommand{\valSNC}{\tau}

\newcommand{\minorplusvirtual}{\textrm{Class}}


% Local Variables:
% TeX-master: "main"
% End:



==> Deterministic_SSSP/preliminaries.tex <==

\section{Preliminaries and Terminology}\label{sec:preliminaries}

In this section, we first review some basic terminology related to graphs, clusterings, shortest paths and (transhipment) flows. Afterwards, we describe the computational models we use in this paper.

\paragraph{Graphs.} 
For a graph $G$ we use $V(G), E(G)$ to denote its node set and edge set, respectively. The set of neighbors of a node $v$ is denoted with $\Gamma_G(v) \subseteq V$.
An eulerian graph is a graph with $|\Gamma_G(v)|$ being even for every $v \in V(G)$.
It is often convenient to direct $E$ consistently. For simplicity and without loss of generality, we assume that $V = \{v_1, v_2, \ldots, v_{n}\}$ and define $\vec{E} = \{ (v_i,v_j) \mid (v_i, v_j) \in E, i < j\}$. We identify $E$ and $\vec{E}$ by the obvious bijection. We chose this orientation for simplicity and concreteness: arbitrarily changing the orientations does not influence the results (if done consistently). We also introduce the notation $\overleftrightarrow{E}$ which includes each edge of $\{u, v\} \in E$ in both directions: $(u, v) \in \overleftrightarrow{E}$ and $(v, u) \in \overleftrightarrow{E}$. 


A weighted graph $G$ is an undirected graph, together with a function $\ell_G : E \rightarrow \{1, \ldots, n^{O(1)}\}$ that assigns a polynomially-bounded non-negative weight to each edge in $E$. We sometimes use just $\ell$ if $G$ is clear from context. This weight function induces a distance function $\dist_G(u, v)$ on $G$. For two sets of nodes $A,B \subseteq V(G)$ we define $\dist_G(U,W) = \min_{u \in U, w \in W} \dist_G(u, w)$ and sometimes write $\dist_G(U, w)$ for $\dist_G(U, \{w\})$. 
A ball $B_G(u, r)$ of radius $r$ around a node $u$ is a set of nodes $v$ such that $\dist_G(u, v) \le r$. The diameter of a weighted graph $G$ is defineed as $\diam(G) = \max_{u,v} \dist_G(u,v)$ and its hop diameter $\hopDiameter{G}$ is the longest unweighted shortest path (i.e., in terms of hops and not weight). 

\paragraph{Clusters and Clusterings.}
A \emph{cluster} $C$ is a set of nodes $C \subseteq V(G)$. 
A \emph{clustering} $\fC$ is a collection of disjoint clusters.
Finally, a \emph{sparse neighborhood cover} of a graph $G$ with \emph{covering radius} $R$ is a collection of $\gamma := O(\log n)$ \footnote{Sometimes we use $\log(\cdot)$ outside the $O$-notation, in which case it stands for $\log_2(\cdot)$. \alert{is this even used anywhere?} } clusterings $\fC_1, \dots, \fC_\gamma$ such that for each node $v \in V(G)$ there exists some $i \in \{1,\ldots,\gamma\}$ and some $C \in \fC_i$ with $B(v, R) \subseteq C$. 


%\paragraph{Smooth Functions}

%We say that a function $\phi: V(G) \rightarrow [n^{O(1)}]$ is \emph{smooth} if it satisfies that for any two nodes $u, v$ we have $\phi(u) - \phi(v) \le \dist_G(u, v)$. Equivalently, we can require that for any edge $\{u, v\}$ we have $\phi(u) - \phi(v) \le \ell(\{u,v\})$. 

%\begin{fact}
%\label{fact:smoothMinMaxSum}
%Let $\phi_1, \phi_2, \dots, \phi_k$ be smooth.  
%Then $\sum_{i = 1}^k \phi_i/k,\, \min_{i = 1}^k \phi_i,\, \max_{i  = 1}^k \phi_i$ is smooth. 
%\end{fact}

\paragraph{Flows, Transshipment, and SSSP.}
Given a graph $G=(V,E)$, a flow is either a function $f:\overleftrightarrow{E}\to\mathbb R_{\ge0}$ (that is identified with a vector $\R_{\ge 0}^{\overleftrightarrow{R}}$ by the obvious identification), or a function $f : \vec{E} \to \R$ (identified with $\R^{\vec{E}}$). We often use one or the other flow notation for convenience. Given $f \in \overleftrightarrow{E}$, we can covert it to $f' \in \vec{E}$ by letting $(f')_{(u, v)} := f(u, v) - f(v, u)$ and, similarly, in the other direction $f_{(u, v)} := \1{(u, v) \in \vec{E}} f'_{(u, v)} - \1{(v, u) \in \vec{E}} f'_{(v, u)}$. A \emph{demand} $b$ is simply a function $b : V \to \mathbb{R}$ (or equivalently $\R^V$) satisfying $\sum_{v \in V} b_v = 0$. We say a flow $f \in \R^{\overleftrightarrow{E}}$ \emph{satisfies} a demand $b \in \R^V$ if for all $v \in V$, we have $\sum_{u:(u,v)\in\overleftrightarrow{E}}(f(u,v)-f(v,u))=b(v)$. Given edge weights $\ell \in \R^{E}$, the \emph{transshipment cost} of the flow is $\ell(f) := \sum_{(u,v)\in\overleftrightarrow E}\ell(\{u,v\})f(u,v)$.

Furthermore, we say that a function $\phi: V(G) \rightarrow \mathbb{R}$ (a vector in $\mathbb{R}^{V(G)}$) is a \emph{potential} if $|\phi(u) - \phi(v)| \le \dist_G(u, v)$ for all $u,v \in V$. Equivalently, we can require that for every edge $\{u, v\}$ we have $|\phi(u) - \phi(v)| \le \ell(\{u,v\})$. We note the following useful fact about potentials.
\begin{fact}
\label{fact:potential_min_max}
If $\phi_1, \phi_2, \ldots, \phi_k$ are potentials, then $\phi_{min}$ and $\phi_{max}$ are also potentials. Here, $\phi_{min}(v) = \min_{i \in [k]} \phi_i(v)$ and
$\phi_{max}(v) = \max_{i \in [k]} \phi_i(v)$ for all $v\in V$.
\end{fact}

This now allows us to formally define (approximate) transshipment and SSSP.
\begin{definition}[Transshipment]
  Given a (connected) graph $G = (V, E)$ with lengths $\ell \in \R^E$ and a demand $b \in \R^V$, the transshipment problem asks us to find (1) a flow $f \in \R^{\vec{E}}$, and (2) a potential $\potential \in \R^V$ that minimize/maximize their respective program in the following primal-dual formulation:
  \begin{align*} % \label{eq:transshipmentLP}
    \min~ \ell(f) : \text{$f$ is a flow satisfying $b$}, && \max~ b^{\top} \potential : \text{$\potential$ is a potential}. %\label{eq:transshipmentDualLP}
  \end{align*}
  For $\alpha \ge 1$, a solution $(f, \potential)$ is $\alpha$-approximate if both $f$ and $\potential$ are feasible ($f$ satisfies $b$, $\potential$ is a potential), and $\ell(f) \le \alpha \cdot b^{\top} \potential$. Note that a $1$-approximate solution is optimal.
\end{definition}
\begin{definition}[SSSP and \setssp] 
  Suppose we are given a (connected) graph $G = (V, E)$ with lengths $\ell \in \R^E$. Given a \emph{set-source} $S \subseteq V$, the $\alpha$-approximate \setssp problem asks us to compute a forest $F$ spanning $G$ such that $\dist_F(S, u) \le \alpha \cdot \dist_G(S, u)$ for each node $v \in V$. The problem is called $\alpha$-approximate SSSP when $S = \{ s \}$. The singleton node $s \in S$ is called the \emph{source}.
\end{definition}

% A \emph{demand} is a $b \in \R^{V}$. We say a demand is \emph{proper} if $\one^T b=0$. A \emph{flow} is a vector $f \in \R^{\vec{E}}$. A flow $f$ \emph{routes} demand $b$ if $Bf = b$. It is easy to see only proper demands are routed by flows. The cost $\ell(f)$ of a flow $f$ is $\norm{Lf}_1$.
% %
% For a weighted graph $G$ and a given proper demand $b$ the \emph{transshipment problem} asks to find a flow $f_d^*$ of minimum cost among flows that route $b$. When the underlying graph is clear from the context, we let $\norm{b}_\opt := \ell(f_d^*)$ denote the cost of the optimal flow for routing demand $b$. For any $\alpha \geq 1$, we say a flow $f$ is $\alpha$-\emph{approximate} if $\ell(f) \leq \alpha \cdot \norm{b}_\opt$ (such a flow does not necessarily need to route $b$).
% %
% n the vector $\phi \in \R^{V}$ are generally referred to as vertex \emph{potentials}.
 
% \todo{merge with description below}

\paragraph{$\ell_1$-Oblivious Routing.}
Let $G = (V, E)$ be a fixed graph with weights $\ell \in \R_{\ge 0}^{E}$. For a demand $b \in \R^V$ with $\sum_{v \in V} b_v = 0$ we define $\norm{b}_\opt := \ell(f_b^*)$ to be the cost of the minimum-cost flow that satisfies the demand $b$. Then, the $\ell_1$-oblivious routing is defined as follows.

%For any $k$ and $\alpha > 1$, Sherman~\cite{She17b} defined an $\alpha$-approximate (linear) $\ell_1$-preconditioner for a weighted graph $G$ as a $k \times n$ matrix $P$, such that, for any proper demand $d$ it holds that $$\norm{d}_\opt \le \norm{P d}_1 \le \alpha \norm{d}_\opt.$$ Any such $\alpha$-preconditioner which can be computed in $T$ rounds can be used to give a $\tilde{O}(\eps^{-2} \alpha^2 T)$ algorithm for transshipment~\cite{She17}. We are constructing a strictly stronger object that is required to output a flow that routes any demand with $\alpha$-approximate cost.

\begin{definition}[$\ell_1$-oblivious routing]
  For a graph $G=(V,E)$, a matrix $R \in \R^{\vec{E} \times V}$ is called a (linear) $\ell_1$-oblivious routing if for any demand $b \in \R^V$ with $\sum_{v \in V} b_v = 0$ the flow $f := R b \in \R^{\vec{E}}$ satisfies the demand $b$. Furthermore, an $\ell_1$-oblivious routing $R$ is $\alpha$-competitive if for all demands $b \in \R^V$ with $\sum_{v \in V} b_v = 0$ we have that the cost of the flow $f_{R,b}:=Rb$ is at most $\alpha \norm{b}_\opt$, i.e., $\ell(f_{R,b}) \leq \alpha \cdot \norm{b}_\opt$.
\end{definition}



% \iffalse
% We still don't know what the right way and definition to talk about smoth distances. We thus won't use any such terminology here and simply stick to the standard language of approximate shortest path trees and transshipment potentials.

% \subsection{Smooth Distance Function}

% For a given subset $S \subseteq V$ of \emph{source nodes} we say a function $\dist_S : V\times V \rightarrow [n^{O(1)}]$ is a valid distance (upper bound) function if $\dist_S(s)=0$ for every node $s \in S$ and if for every node $u \in V$ it holds that $\dist_S(u) \geq d_G(S,u)$. \alert{(G) what is dist(s) .. it's a 2-ary function?}
% Throughout the paper we assume (for now) that there is a single source, i.e., $|S|=1$, but all results and notions straightforwardly carry over to larger $S$.  \alert{(G) so the definitions don't carry over or are we talking about the general problem of solving SSSP? why not just write out the definitions?} 
% We also usually assume that $s$ is always the designated source node and in that case largely omit $S = \{s\}$ from subscripts of $\dist$.

% \begin{definition}[strongly-approximate $\alpha$-approximate SSSP distance]
% A valid distance function $\dist$ for a graph $G$ and source node $s$ is strongly $\alpha$-approximate for some $\alpha \geq 1$ if $$\forall u,v: \ \ |\dist(u) - \dist(v)| \leq \alpha \cdot d_G(u,v).$$
% \end{definition}
% \begin{definition}[(perfectly) tree-like distance functions]
% Let $\dist$ be a valid distance on $G$. We say $\dist$ is tree-like if $$\forall u \neq s: \ \exists v \in \Gamma_G(u): \ \ \dist(v) \leq \dist(u) - w_G(u,v)$$
% or, equivalently, if 
% $$\forall u \neq s: \ \min_{v \in \Gamma_G(u)} \dist(v) + w_G(v,u) \leq \dist(u).$$
% We furthermore say $\dist$ is perfectly tree-like if 
% $$\forall u \neq s: \ \min_{v \in \Gamma_G(u)} \dist(v) + w_G(v,u) = \dist(u).$$
% \end{definition}
% \fi



\subsection{Model: Minor-Aggregation for \pram}
\label{subsec:intro_minor_aggregation}

In this section we give a minimal-but-complete description of the \aggregate interface, which exposes to the user the following operations on a graph: (1) contract edges, thereby operating a minor, (2) each (super)node in the contracted graph can compute an aggregate (e.g., min, max, sum) of surrounding neighbors, and (3) add $\tilde{O}(1)$ arbitrarily-connected virtual nodes over the course of the algorithm. The goal is to design $\tO(1)$-round algorithms in this model. Such a \aggregate algorithm can be compiled to a near-optimal algorithm in both the parallel and distributed settings.

The full model, as defined in \cite{goranci2022universally,ghaffari2021universally}, is used in the distributed setting which requires specifying some low-level details we can leave out here. For a more in-depth discussion of \aggregate and its extensions to distributed models see \Cref{sec:computational-models}.

\textbf{Aggregations.} An \emph{aggregation operation} $\bigoplus$ is any associative function that combines two $\tilde{O}(1)$-bit inputs into one of equal size (e.g., sum or max). For multiple inputs $x_1, x_2, \ldots, x_k$, their \emph{aggregate} $\bigoplus_{i=1}^k x_i$ is defined by arbitrarily aggregating messages until one remains.

\begin{definition}[Minor-Aggregation model in \pram]\label{def:aggregation-congest-intro}
  We are given an undirected graph $G = (V, E)$. There is a single \pram processor and private memory associated with each node and each edge. Between-processor communication happens during synchronous rounds, and processors perform $\tilde{O}(1)$-work local computation between rounds. Each round consists of the following three steps (in that order).
  \begin{itemize}
  \item \textbf{Contraction step.} Each edge (associated processor) $e$ chooses a value $c_e = \{\bot, \top\}$. This defines a new \emph{minor network} $G' = (V', E')$ constructed as $G' = G / \{ e : c_e = \top \}$, i.e., by contracting all edges with $c_e = \top$ and self-loops removed. Vertices $V'$ of $G'$ are called supernodes, and we identify supernodes with the subset of nodes $V$ it consists of, i.e., if $s \in V'$ then $s \subseteq V$.

  \item \textbf{Consensus step.} Each individual node $v \in V$ chooses a $\tilde{O}(1)$-bit value $x_v$. For each supernode $s \in V'$ we define $y_s := \bigoplus_{v \in s} x_v$, where $\bigoplus$ is some aggregation operator. All nodes $v \in s$ learn $y_s$.

  \item \textbf{Aggregation step.} Each edge $e \in E'$ connecting supernodes $a \in V'$ and $b \in V'$ learns $y_a$ and $y_b$, and chooses two $\tilde{O}(1)$-bit values $z_{e, a}, z_{e, b}$ (i.e., one value for each endpoint). Finally, (every node of) each super $s \in V'$ learns the aggregate of its incident edges in $E'$, i.e., $\bigotimes_{e \in \text{incidentEdges(s)}} z_{e, s}$ where $\bigotimes$ is some aggregation operator.
  \end{itemize}
\end{definition}

\smallskip

\textbf{PRAM simulation.} Simulating contractions and aggregations is a well-known and simple primitive in \pram that can be performed in $\tilde{O}(1)$ time and $\tilde{O}(m)$ work (see e.g. \cref{thm:oracleSimulation}). 

We note that the following operations can be efficiently simulated.
\begin{itemize}
\item \textbf{Minors.} It is immediate from the model that any \aggregate algorithm can be run on a minor in a black-box manner.
\item \textbf{Node-disjoint scheduling.} Similarly, it is immediate that we can simultaneously run separate algorithms on node-disjoint and connected subgraphs of $G$.
\item \textbf{Virtual nodes.} Given a graph $G$, we can construct a \emph{virtual graph} by starting with a connected graph and repeatedly adding a \emph{virtual node} that is connected to an arbitrary set of neighbors. Due to the constraints in the distributed setting, we constrain the number of virtual nodes to $\tilde{O}(1)$. A \aggregate round on such graphs can be simulated in \pram with $\tilde{O}(m)$ work and $\tilde{O}(1)$ depth. For example, we frequently use this operation to connect a ``supersource'' node, enabling us to use our standard SSSP algorithm to implement a set-source-$S$ shortest path.
\end{itemize}

\textbf{Distributed storage and input.} Our \aggregate algorithms operate on objects that are \emph{``distributedly'' stored}, meaning that each processor has its own part of the object in private memory. Specifically, we store a \emph{node vector} $x \in \R^V$ by storing $x_v$ in node $v$. Similarly, edge vectors $x \in \R^{E}, x \in \R^{\vec{E}}, x\in \R^{\overleftrightarrow{E}}$ are distributed over edges. Subgraphs $H \subseteq G$ are specified by distributedly storing the characteristic vectors $\mathbb{1}_{V(H)} \in \R^{E(G)}$ and $\mathbb{1}_{E(H)} \in \R^{E(G)}$. Initially, the problem-specific input is assumed to be distributedly stored. For transshipment and SSSP, we assume the lengths (edge vector) and demands (node vector) are stored. At termination, the output is required to be stored.

\textbf{Oracles.} An oracle is a black-box function that takes a certain input (on the original graph) and produces a specified output. An algorithm with access to an oracle can, in each round, choose to perform a regular \aggregate round, or to call a single oracle (i.e., multiple oracle calls per round are forbidden). Some oracles we use only have an efficient \pram implementation, but no efficient \aggregate implementation.

%For example, \emph{partwise aggregation} oracle takes the private input and part ID on each node and outputs at each node the corresponding partwise aggregate.

\textbf{Ancestor and subtree sums.} The following operation is often useful. Given a (distributedly stored) tree $T$ and a root $r \in V(T)$, there is a deterministic $\tilde{O}(1)$-round \aggregate algorithm that computes for each node the ancestor and descendent sum (or a general aggregate) with respect to $T$ rooted at $v$ (see \Cref{lemma:ancestor-subtree-sum} for a fully formal version).


% Local Variables:
% TeX-master: "main"
% End:


==> Deterministic_SSSP/relatedWork.tex <==
\section{Further Related Work}
\label{sec:morerelatedwork}


We briefly mention few results out of a large body of works on SSSP and the related all pairs shortest paths (APSP) problem. 

While our paper focuses on the undirected variant of the problem, there is a long line of work on the directed variant. Many results on parallel algorithms mentioned in \cref{sec:intro} work for directed graphs. 
There is a long list of recent results in the \congest model on the directed shortest path problem \cite{GL18,FN18,CM20,CFR21,CLP21}. 


Finding a shortest path becomes much simpler if we can assume that it only has a small number of hops (edges). 
This motivates a successful line of work 
\cite{ullman1991high,cohen1994polylog,klein1997randomized,thorup2005approximate,thorup2006spanners,bernstein2009fully,henzinger2014decremental,Nan14,holzer2014approximation,miller2015improved,henzinger2016almost,EN16,abboud2018hierarchy,huang2019thorup} on the construction of so-called \emph{hopsets} -- small sets of edges that we can add to a graph to make the shortest paths use a small number of hops, while distorting the distances only by a small amount. 

The (approximate) SSSP problem is studied in many different models besides the parallel and the distributed one. 
To give some examples, it is studied in the (semi-) streaming model \cite{elkin2006efficient,feigenbaum2009graph,guruswami2016superlinear,henzinger2016almost,EN16}, the congested clique model \cite{Nan14,censor2019algebraic,le2016further,henzinger2016almost,censor2020fast}, Broadcast \congest model~\cite{BKKL17}, Hybrid model~\cite{AHKSS20,FHS20,kuhn2020computing,CLP21}, or the dynamic algorithms model \cite{shiloach1981line,henzinger2014decremental,henzinger2014sublinear}. 


%Indeed, known algorithms build on matrix multiplication or on transitive closure routines with $O(n^{3})$ work. 
%There is a line of work \cite{ullman1991high,klein1997randomized,spencer1997time,shi1999time} on randomized algorithms with different processor-time trade-offs but without much improvement on the cubic work bound for fast parallel algorithms. Cohen \cite{cohen1997using} gave a deterministic algorithm with similar trade-offs. 
%Another line of work \cite{galil1997all,alon1997exponent,zwick1998all} gave $(1+\eps)$-approximate all pairs shortest paths (APSP) algorithms with work equal to $\tO(n^{\omega})$, where $\omega < 2.37\dots$ is the fast matrix multiplication exponent~\cite{alman2021refined} . 

The related (directed) APSP problem was also considered in various distributed and parallel models \cite{galil1997all,alon1997exponent,zwick1998all,coppersmith1987matrix,alman2021refined,a1,censor2019algebraic,holzer2014approximation,le2016further,Elk17,huang2017distributed,agarwal2018deterministic,censor2020sparse,pontecorvi2018distributed,agarwal2019distributed,bernstein2019distributed,augustine2020shortest,agarwal2020faster,censor2020fast,dory2020exponentially,kuhn2020computing,censor2021sparsity}.

% Local Variables:
% TeX-master: "main"
% End:




==> Deterministic_SSSP/rounding.tex <==
\section{Transshipment Flow Rounding}
\label{sec:rounding}

\newcommand{\lrE}{\overleftrightarrow{E}}
\newcommand{\rH}{\overrightarrow{H}}


In this section, we prove the following theorem. Note that the returned solution is exact (i.e., has $\eps = 0$), even though an $(1+\eps)$-approximate solution would suffice. We remind the reader of the definitions of $\oRound_{0}$ and $\oEuler$ from \Cref{def:oracle_rounding,def:oracle_euler}.

\begin{theorem}[Rounding]
\label{thm:rounding}
Let $G$ be a weighted graph. The oracle $\oRound_{0}$ can be implemented in $\poly(\log n)$ \aggregate rounds and $\poly(\log n)$ oracle calls to $\oEuler$. 
\end{theorem}

The rest of the section is dedicated to the proof. Our algorithm is inspired by Cohen's rounding algorithm for integral flow~\cite{cohen1995approximateMaxFlow} in which one is given a fractional flow that satisfies integral demand constraints, and the algorithm constructs an integral flow of non-increased cost that satisfies the same demand. The algorithm uses bit-scaling, meaning that for $i = \log n, \ldots, 0$ (in decreasing order) it rounds the flow values to multiples of $2^{-i}$. The main observation is that, in the $i$-th step, the set of edges which are not multiples of $2^{-i}$ (but are multiples of $2^{-i-1}$ by the invariant), form a Eulerian graph (all nodes have even degrees). Such a graph can be decomposed into a collection of directed cycles, and on each cycle we either add or subtract $2^{-i-1}$. This does not impact the demand the flow satisfies, but makes the flow values multiples of $2^{-i}$, as requested. We extend this algorithm to round a fractional flow into a forest (or more precisely, a disjoint union of out-arborescences).

%\begin{theorem}
%Consider a graph $G=(V,E)$ with edge weights $\ell$, and consider a demand vector $b:V\to\mathbb R$ such that $b(v)\ge0$ for all $v\in V$ except for some $s\in V$ called the source. Let $f$ be a flow satisfying demand $b$ whose values $f(u,v)$ can be represented in binary using $O(\log n)$ bits before and after the decimal. There is a parallel algorithm that constructs in $\tilde{O}(m)$ work and $\tilde{O}(1)$ time a tree $T$ spanning all vertices $\{v:b(v)\ne0\}$ such that $\sum_{v:b(v)\ne0}b(v)d_T(s,v) \le \ell(f)$.
%\end{theorem}


For simplicity, we assume that each $b(v)$ is now an integer with absolute value $\textup{poly}(n)$. (This can be guaranteed by first multiplying each $f(u,v)$ by a large enough $\textup{poly}(n)$ so that each $f(u,v)$ and $b(v)$ is integral, and then computing the tree $T$ with this modified instance, which is still a satisfying tree for the original instance since both $\sum_{v:b(v)\ne0}b(v)d_T(s,v)$ and $\ell(f)$ are scaled by the same amount.)

Our algorithm proceeds in phases, from phase $i=0$ up to $\lceil\lg(-b(s))\rceil$. Initialize $f_0=f$; we maintain the invariant that each flow $f_i$ satisfies some demand $b_i$ whose entries are all integer multiples of $2^i$. 
In each phase $i$, our goal is to split $f_i$ into two flows $f_{i+1}$ and $\tilde f_i$ (i.e., $f_i=f_{i+1}+\tilde f_i$) such that (1) flow $\tilde f_i$ is supported on a collection of arc-disjoint paths with $f(u,v)=2^i$ for each arc $(u,v)$ on some path, and (2) all flow values in $f_{i+1}$ are integer multiples of $2^{i+1}$.
Since the initial $f_0$ is assumed to be integral, property~(2) means that we maintain the invariant that each flow $f_j$ has values that are integer multiples of $2^j$.

In each phase $i$, the algorithm does the following:
 \begin{itemize}
 \item Compute an out-arborescence $A_i$ rooted at $s$ supported by arcs $\{(u,v)\in\lrE:f_i(u,v)>0\}$ and spanning all vertices $v\in V:b_i(v)>0$. We later show in \Cref{lem:arbor} that this can be done in $O(\log n)$ rounds of \aggregate.
 \item Let $O_i=\{v\in V:b_i(v)\bmod2^{i+1}=2^i\}$ ($O_i$ for ``odd''). We construct a subgraph $B_i$ of $A_i$ by taking all arcs $(u,v)$ in $A_i$ where the subtree rooted at $v$ in $A_i$ contains an odd number of vertices in $O_i$.
 \item Define flow $\tilde f_i:\lrE\to\mathbb R_{\ge0}$ as $\tilde f_i(u,v)=2^i$ if $(u,v)$ is in $B_i$, and $\tilde f_i(u,v)=0$ otherwise.
 \item Construct a directed graph $H_i$ as follows: for each arc $(u,v)\in\lrE$ satisfying\linebreak $(f_i(u,v)-\tilde f_i(u,v))\bmod2^{i+1}=2^i$, add arc $(u,v)$ to $H_i$. We will prove that each vertex in $H$ has an even number of incident arcs. 
 \item Since the undirected version of $H$ is Eulerian, we call $\oEuler$ on the undirected $H$ to obtain an edge orientation where each vertex in $H$ has the same number of in-edges and out-edges. Define function $h_i:\lrE\to\mathbb R$ as $h_i(u,v)=2^i$ if the orientation of $(u,v)$ is $(u,v)$, and $h_i(u,v)=-2^i$ if it is $(v,u)$, and $h_i(u,v)=0$ for $(u,v)$ not in $H$.
 \item Define $f_{i+1}$ as either $f_i-\tilde f_i\pm h_i$, where we choose $+$ or $-$ depending on whichever minimizes $\ell(f_{i+1})$.
 \end{itemize}
Using $f_i$ and $B_i$, the algorithm now recovers a tree $T$ such that $\sum_{v\ne s}b(v)d_T(s,v)\le \ell(f)$ as follows. Initialize distance upper bounds $\tilde d(s)=0$ and $\tilde d(v)=\infty$ for all $v\ne s$, and initialize the parent function $p(v)=\bot$ for all $v\in V$. For $i$ in decreasing order, do the following:
 \begin{itemize}
 \item Partition $B_i$ into a (disjoint) set of maximal arborescences. For each such arborescence $A \subseteq B_i$ on vertices $U$ with root $r\in U$, set $\tilde d(u) \gets \min\{\tilde d(u),\tilde d(r)+d_{A}(r,u)\}$ for all $u\in U$ (in parallel). Also, for all $u\in U\setminus\{r\}$ whose value $\tilde d(u)$ was lowered, set $p(u)$ to the parent of $u$ in $A$. We note that the exact distances to the root of the arborescence can be computed in $\tilde{O}(1)$ rounds (e.g., via \Cref{lemma:ancestor-subtree-sum}).
 \end{itemize}

\subsection{Correctness}


\begin{lemma}\label{lem:structure}
The following properties are satisfied for each $i$:
 \begin{enumerate}
% \item Flow $\tilde f_i$ is supported on a collection of arc-disjoint paths with $f(u,v)=2^i$ for each arc $(u,v)$ on some path.
 \item $f_{i+1}+\tilde f_i$ satisfies demand vector $b_i$.
 \item All flow values in $f_{i+1}$ are integer multiples of $2^{i+1}$.
 \item For the demands $b_{i+1}$ satisfied by $f_{i+1}$, we have $b_{i+1}(v)\ge0$ for all $v\ne s$.
 \item The conditions of \Cref{lem:arbor} are satisfied on flow $f_i$, so that an arborescence $A_i$ rooted at $s$ is successfully found.% supported by arcs $\{(u,v)\in\lrE:f_i(u,v)>0\}$ spanning all vertices $v\in V:b_i(v)>0$.
 \item The flow $\tilde f_i$ satisfies $\tilde f_i(u,v)\le f_i(u,v)$ for all $(u,v)\in\lrE$.
 \item The flow $f_i-\tilde f_i$ satisfies a demand vector whose entries are multiples of $2^{i+1}$.
 \item The graph $H_i$ is Eulerian.
 \item We have $f_{i+1}(u,v)\ge0$ for all $(u,v)\in\lrE$ and $\ell(f_{i+1})+\ell(\tilde f_i)\le \ell(f_i)$.
 \end{enumerate}
\end{lemma}
\begin{proof}
We prove the properties together by induction on $i\ge0$, where we assume properties~(2)~and~(3) for $i-1$ if $i>0$ (and obtain them for free when $i=0$) and prove all nine properties for $i$.
 \begin{enumerate}
% \item[(1)] Property~(1) follows immediately by construction.
 \item[(4)] Property~(4) follows from property~(3) on $i-1$.% For simplicity, define $V^+=\{v\in V:b_i(v)>0\}$ and $\overrightarrow E^+=\{(u,v)\in\lrE:f_i(u,v)>0\}$. By property~(4) for $i-1$, only $b_i(s)$ is negative, so any decomposition of the flow $f_i$ into paths in $\overrightarrow E^+$ must consist of $s$--$v$ paths for each $v\in V^+$. Consider the graph $G'$ of the union of all such paths (which may not span all vertices in $V$). Since $s$ can reach all vertices in $G'$, the minimum cut between $s$ and any other vertex in $G'$ is at least $1$. By Edmonds' arborescence packing theorem, there is a spanning arborescence in $G'$, which is an arborescence in $\overrightarrow E^+$ spanning $V^+$. This completes property~(4).
 \item[(5)] We have $\tilde f_i(u,v)=2^i$ for all $(u,v)$ in $B_i$, which is contained in $A_i$, which is comprised of arcs $(u,v)\in \overrightarrow E^+$ with $f_i(u,v)>0$. By property~(2) on $i-1$, we also have $f_i(u,v)$ is a multiple of $2^i$, so $f_i(u,v)\ge2^i$. Property~(5) follows.
 \item[(6)] For each $v$, let $N_v$ denote the number of vertices in $O_i$ in the subtree rooted at $v$ in $A_i$. Let $C_v$ denote the children of $v$ in $A_i$. Then, the summation $N_v+\sum_{u\in C_v}N_u$ double-counts every vertex in $O_i$ in the subtree rooted at $v$, except possibly $v$. In other words, the summation is odd iff $v\in O_i$. Equivalently, $v\in O_i$ iff there are an odd number of odd terms in the summation, which by definition of $B_i$ means that $v$ is incident to an odd number of arcs in $B_i$. By construction of $\tilde f_i$, it follows that for the demand vector $\tilde b_i$ satisfied by $\tilde f_i$, we have $\tilde b_i(v)\equiv2^i\bmod2^{i+1}$ iff $v\in O_i$.

Therefore, if $v\in O_i$, then $b_i(v)-\tilde b_i(v)\equiv 2^i-2^i\equiv0\bmod2^{i+1}$. By property~(2) on $i-1$, the values of flow $f_i$ are all multiples of $2^i$, so for $v\notin O_i$, we have $b_i(v)\equiv0\bmod2^{i+1}$, which along with $\tilde b_i(v)=0\bmod2^{i+1}$ gives $b_i(v)-\tilde b_i(v)\equiv0\bmod2^{i+1}$, finishing property~(6).
 \item[(7)] By property~(6) proved above, $b_i(v)-\tilde b_i(v)\equiv0\bmod2^{i+1}$. We can write $b_i(v)-\tilde b_i(v)$ as 
\begin{align*}
 b_i(v)-\tilde b_i(v)&=\sum_{u:(u,v)\in\lrE}\big((f_i(u,v)-f_i(v,u))-(\tilde f_i(u,v)-\tilde f_i(v,u))\big) 
\\&= \sum_{u:(u,v)\in\lrE}\big( (f_i(u,v)-\tilde f_i(u,v))-(f_i(v,u)-\tilde f_i(v,u)) \big) .
\end{align*}
 By property~(2) on $i-1$ and by construction of $\tilde f_i$, all values $f_i(u,v)-\tilde f_i(u,v)$ are multiples of $2^i$. It follows that there are an even number of $(u,v)$ or $(v,u)$ satisfying $f_i(u,v)-\tilde f_i(u,v)\equiv2^i\bmod2^{i+1}$ or $f_i(u,v)-\tilde f_i(u,v)\equiv2^i\bmod2^{i+1}$ respectively. It follows that $H_i$ is Eulerian, concluding property~(7).
 \item[(8)] We first prove $f_{i+1}(u,v)\ge0$ for all $(u,v)\in\lrE$. Recall that $f_{i+1}=f_i-\tilde f_i\pm h_i$, so by property~(5), it suffices to only consider $(u,v)$ in $H$. By construction, we have $(f_i(u,v)-\tilde f_i(u,v))\bmod2^{i+1}=2^i$  for all arcs $(u,v)$ in $H$, and along with property~(5), this means that $f_i(u,v)-\tilde f_i(u,v)\ge2^i$. Adding or subtracting $h_i(u,v)$ can decrease the value by at most $2^i$, so $f_i(u,v)-\tilde f_i(u,v)\pm h_i(u,v)\ge0$.

Finally, $\ell(f_{i+1})+\ell(\tilde f_i)\le \ell(f_i)$ follows from the fact that $\frac12\big(\ell(f_i-\tilde f_i+h_i)+\ell(f_i-\tilde f_i-h_i)\big)=\ell(f_i-\tilde f_i)$ and that we take the one with smaller cost.
 \item[(2)] By property~(2) on $i-1$ and by construction of $\tilde f_i$, all values $f_i(u,v)-\tilde f_i(u,v)$ are multiples of $2^i$. If $(f_i(u,v)-\tilde f_i(u,v))\bmod2^{i+1}=2^i$, then arc $(u,v)$ is added to $H$, and $h_i(u,v)=\pm2^i$, so $f_{i+1}(u,v)\bmod2^{i+1}=0$. If $(f_i(u,v)-\tilde f_i(u,v))\bmod2^{i+1}=0$, then $(u,v)$ is not added to $H$, so $h_i(u,v)=0$ and $f_{i+1}(u,v)\bmod2^{i+1}=0$.
 \item[(3)] Let $\tilde b_i$ be the demand vector for $\tilde f_i$; we first show that $b_i-\tilde b_i\ge0$. By property~(2) and property~(3) on $i-1$, we have that $b_i(v)$ is a nonnegative multiple of $2^i$. Consider now flow $\tilde f_i$ that satisfies demand vector $\tilde b_i$. The only way for $\tilde b_i(v)>0$ is if the parent arc $(u,v)$ is in $B_i$ and no child arc is in $B_i$, in which case $\tilde b_i(v)=2^i$. By construction of $B_i$, this can only happen if $v\in O_i$, which gives $b_i(v)-\tilde b_i(v)\ge2^i-2^i\ge0$. For all other $v\ne s$, we have $b_i(v)-\tilde b_i(v)\ge b_i(v)\ge0$. It follows that $b_i-\tilde b_i\ge0$.

We next consider the addition of $h_i$. Since we orient arcs in $H$ so that each vertex has the same number of in-edges and out-edges, adding or subtracting $h_i$ to $f_i-\tilde f_i$ does not change the demand vector. This finishes property~(3), and this last observation also proves property~(1).
 \end{enumerate}
This concludes all the properties, and hence the proof.
\end{proof}


\begin{lemma}
$\sum_{v\ne s}b(v)\tilde d(v)\le \ell(f)$.
\end{lemma}
\begin{proof}
By \Cref{lem:structure}, we can apply induction on $i$ to obtain the following two properties:
 \begin{enumerate}
 \item[i.] $\sum_i\ell(\tilde f_i)\le \ell(f)$, which follows from property~(8), and
 \item[ii.] For all $i$, flow $\sum_{j\ge i}\tilde f_j$ satisfies demand vector $b_i$, which follows from property~(1) and the fact that each $f_j$ satisfies demand $b_j$.
 \end{enumerate}

Imagine performing the following single-commodity flow experiment. Begin with $-\infty$ commodity units on node $s$, and we tag each (integral) commodity unit with a value representing its ``distance traveled'' throughout the flows. In decreasing order of $i$, we execute flow $\tilde f_i$ by shifting commodity around (in integral amounts) according to the flow, and for each commodity unit shifted, we increase its ``distance traveled'' value by the distance shifted. Note that the total increase in value over all commodity units increases by exactly $\ell(\tilde f_i)$. Also, note that we are never deficient in commodity anywhere (outside of $s$), since our distribution of flow after iteration $i$ is exactly $\sum_{j\ge i}\tilde f_i$, which satisfies demand vector $b_j$ by property~(ii), and is therefore nonnegative at all $v\ne s$ by property~(3). Once we execute all flows $\tilde f_i$, each vertex $v\ne s$ has exactly $b(v)$ demand by property~(ii), and the total value of all commodity units is $\sum_i\ell(\tilde f_i)$, which is at most $\ell(f)$ by property~(i). 

It remains to show that the total ``distance traveled'' value of all commodity units is at least $\sum_{v\ne s}b(v)\tilde d(v)$. To do so, we claim that after executing any flow $\tilde f_i$, all units of flow at any $v\ne s$ have their value at least the current $\tilde d(v)$, which in turn is at least the final $\tilde d(v)$. This implies the lemma, since each $v\ne s$ ends up with exactly $b(v)$ units of flow after all flows $\tilde f_i$ are executed.

We now prove the claim by induction on decreasing $i$. Suppose that, right before executing flow $\tilde f_i$, a commodity unit at vertex $u$ had value $d_{\text{old}}$, and suppose that $\tilde d(u)=d_{\text{old}}$ at that time. If the unit travels to vertex $v$ in flow $\tilde f_i$, then its new value is $d_{\text{old}}+d_{A_i}(u,v)$, which is at least the new $\tilde d(v)\le d_{\text{old}}+d_{A_i}(u,v)$ by the way the algorithm updates $\tilde d(v)$.
\end{proof}




\begin{lemma}
For each $v\in V$, we have $d_T(s,v)\le\tilde d(v)$.
\end{lemma}
\begin{proof}
We induct on the distance $d_T(s,v)$ in increasing order. Given a vertex $v$, consider its parent $u$ in the tree $T$ (rooted at $s$), which satisfies $d_T(s,u)<d_T(s,v)$. At the time of updating $p(v)$ to $u$, we had $\tilde d(v)$ in some arborescence $A$ with root $r$, we had $\tilde d(v)=\tilde d(r)+d_A(r,v)=\tilde d(r)+d_A(r,u)+\ell(u,v)\ge \tilde d(u)+\ell(u,v)$ for the values of $\tilde d(u),\tilde d(v)$ at that time. The value $\tilde d(u)$ can only decrease over time, and on the other hand, the value $\tilde d(v)$ does not change since we assumed its final value. Therefore, $\tilde d(v)\ge\tilde d(u)+\ell(u,v)$ at the end. By induction, $d_T(s,u)\le\tilde d(u)$, and we obtain $\tilde d(v)\ge\tilde d(u)+\ell(u,v)\ge d_T(s,u)+\ell(u,v)=d_T(s,v)$, completing the induction.
\end{proof}



\begin{lemma}\label{lem:arbor}
Consider a flow $f$ on a network graph $G$ satisfying demands $b$ where $b(v)\ge0$ for all $v\ne s$ (for some source node $s$). Let $H$ be the directed graph with arcs $(u,v)$ whenever $f(u,v)>0$. Then, we can compute an arborescence of $H$ rooted at $s$ spanning all nodes $v$ with $b(v)>0$ in $O(\log n)$ \aggregate rounds.
\end{lemma}
\begin{proof}
The algorithm resembles Edmonds' arborescence algorithm, except adapted to span a subset of vertices. On each iteration, each vertex $v\ne s$ chooses an incoming neighbor $u_v$ if it exists. The algorithm contracts all connected components of the (undirected) graph consisting of all such edges $(u_v,v)$, and deletes any node $v$ without an incoming neighbor. The contracted component containing $s$ is named the new node $s$. The algorithm stops when there is a single node $s$. To construct the arborescence, the algorithm reverses the contractions in reverse chronological order, maintaining an arborescence of the current graph at each step. On each step, all contracted components are un-contracted. Edges in the arborescence of the contracted graph remain as edges in the arborescence of the un-contracted graph. This concludes the description of the algorithm, which clearly runs in $O(\log n)$ \aggregate rounds.

We will show that $(*)$ each contracted component that contains $s$ is always an arborescence, while each contracted component not containing $s$ is always a directed cycle. For the contracted component containing $s$, we add the edges of its arborescence to the new arborescence.  For each contracted component that is a directed cycle, we add all but one edge into the new arborescence. Aside from the proof of $(*)$, we can apply the standard analysis of Edmonds' algorithm to show that the algorithm constructs an arborescence rooted at $s$. We also need to show that all nodes $v\in V$ with $b(v)>0$ are spanned by the arborescence, which we show after $(*)$.

We now prove the statement $(*)$. The proof that the contracted component containing $s$ is an arborescence is also standard, and relies on the fact that we do not select an incoming neighbor into $s$. On the other hand, the proof that every other contracted component is a directed cycle is non-standard and relies on the specific construction of the graph $H$. Suppose for contradiction that such a component $C$ is not a directed cycle; then, there must be node $u$ in $C$ with no incoming neighbor but at least one outgoing neighbor. Let $S\subseteq V$ be the set of original vertices that eventually get contracted to $u$. Then, $S$ has no incoming neighbor in $H$ and at least one outgoing neighbor. By construction of $H$, this means that the flow $f$ flows out of $S$ on at least one arc, but never into $S$, so the net flow out of $S$ is positive. Since the flow satisfies demands $b$, it follows that $\sum_{v\in S}b(v)<0$. This contradicts the fact that $b(v)\ge0$ for all $v\in S$, since $S$ does not contain $s$.

Finally, we show that each node $v\in V$ with $b(v)>0$ is spanned by the arborescence. Suppose not; then, in some contracted graph, the node that $v$ got contracted to must have no incoming neighbors (after which that node is deleted). For this to happen, the set $S\subseteq V$ of original vertices that got contracted to that node must satisfy $\sum_{v\in S}b(v)\le0$. On the other hand, $b(v)>0$ and $b(u)\ge0$ for all $u\in S$ since $s\notin S$, a contradiction.
\end{proof}



% Local Variables:
% TeX-master: "main"
% End:


==> Deterministic_SSSP/sparse_cover.tex <==
%\section{Sparse Covers from Approximate Shortest Paths}

\section{Sparse Neighborhood Cover from Approximate Shortest Paths}
\label{sec:sparse-cover}

This section is dedicated to prove \cref{thm:sparse_cover}. Informally speaking, it states that we can construct a sparse neighborhood cover of covering radius $D/\poly\log(n)$ with $\poly(\log n)$ invocations to distance oracles $\oDist_{\eps,D'}$ for $\eps = 1/\poly\log(n)$ and  various $D' \leq D$. \\
The proof consists of three parts.
First, in \cref{sec:weak_clustering} we show how to compute a $D$-separated $\tilde{O}(D)$-weak-radius clustering (see below for the definition) that clusters a large fraction of the vertices (\cref{lem:weak_diam}). 
Second, in \cref{sec:strong_radius} we show how to compute a $D/\poly(\log n)$-separated $\tilde{O}(D)$-strong-radius clustering with $O(\log n)$ black-box invocations to the weak-radius clustering algorithm (\cref{lem:strongdiam}). 
Finally, we show how to compute a sparse neighborhood cover with covering radius $D / \poly(\log n)$ with $O(\log n)$ invocations of the strong-radius clustering algorithm (\cref{thm:sparse_cover}).

The weak- and strong- radius clustering algorithms are mostly straightforward generalizations of the $\congest$ algorithms from \cite{rozhon_ghaffari2019decomposition,chang_ghaffari2021strong_diameter} to a weighted setting with access to approximate distances. 

The only added difficulty is that due to the fact that we deal with approximate, and not exact, distances, some invariants from the original algorithms are now slowly deteriorating during the algorithm, and hence the analysis requires some more care.  

\paragraph{Definitions}

In this appendix, we slightly change and extend definitions of clusters and clusterings. 
Whenever we talk about a cluster (besides the statement of \cref{thm:sparse_cover} that uses the language of the rest of the paper), it is, formally, not just a set of nodes $C \subseteq V(G)$, but a pair $(C, T_C)$, where $C \subseteq V(G)$ and $T_C$ is a rooted tree. 
We have $C \subseteq V(T_C)$ and we think of $T_C$ as the \emph{Steiner tree} collecting the nodes of $C$. 
The \emph{radius} $R$ of a cluster $(C, T_C)$ is the radius of $T_C$. 
If $V(T_C) = C$, we talk about a \emph{strong-radius} cluster, otherwise we talk about a \emph{weak-radius} cluster. 
Sometimes, we still informally talk about ``a cluster $C$'' when the tree $T_C$ is clear from context.

Recall that a clustering $\fC = (C_j, T_{C_j})_{j \in J}$ is a collection of disjoint clusters. We say that $\fC$ is $D$-separated if for every $(C_i, T_{C_i}), (C_j, T_{C_j}) \in \fC, i \not= j,$ we have $\dist_G(C_i, C_j) \ge D$. 
 
 

\subsection{Weak-Radius Clustering}
\label{sec:weak_clustering}

\begin{lemma}[Deterministic Weak-Radius Clustering]
\label{lem:weak_diam}
Let $G$ be a weighted graph, $\Vrem \subseteq V(G)$ be a subset of its nodes, $D > 0$ and $\delta > 0$. We assume that each node of $G$ has a unique identifier from $[2^b]$ for $b=O(\log n)$. We define $\eps := \frac{1}{100b\log(n)}$. 

We can compute a $(1-\eps)^b D$-separated $O(D \log^3(n) \cdot 1/\delta)$-weak-radius clustering $\fC = (C_j, T_{C_j})_{j \in J}$ such that 
\begin{enumerate}
    \item $V(\fC) \subseteq \Vrem$,
    \item $ | \Vrem \setminus V(\fC) | \le \delta \cdot | \Vrem |$.
    \item We can implement any \aggregate operation on $\{C_j\}_{j \in J}$ or on $\{T_{C_j}\}_{j \in J}$ in $\poly\log(n)$ \aggregate rounds in $G$. 
    \item  Consider any $W \subseteq \Vrem$ and $(C,T_C) \in \fC$. 
    If $\dist_G(W, \Vrem \setminus W) > (1+\eps) D$, then we have the following. 
    Whenever we have $C \cap W \not = \emptyset$, then $C \subseteq W$ and for every $u \in V(T_C)$ we have $\dist_G(u, W) \le (1+\eps)D/2$. 
\end{enumerate}

The computation consists of $\poly\log(n)$ \aggregate rounds in $G$ and $\poly(\log n)$ calls to distance oracles $\oDist_{\eps, D}$ for various $D' \in [D/2, D]$.
\end{lemma}

The lemma is proven by a routine adaptation of the algorithm from \cite{rozhon_ghaffari2019decomposition}. 


\begin{proof}
The algorithm consists of $b$ phases and each phase consists of $O(\frac{1}{\delta} \cdot b \cdot \log( n )) = O(\log^2 (n) / \delta)$ steps. 
At the beginning, all nodes in $\Vrem$ are alive, that is, $\Valive = \Vrem$, but some nodes in $\Vrem$ stop being alive during the algorithm and then we call them dead. 
Throughout the course of the algorithm we maintain a partition of alive nodes into clusters. %We denote a cluster with the letter $C$. 
The Steiner tree $T_C$ of any such cluster $C$ can also contain any nodes from $V(G)$. 
At the very beginning, each node $u$ is a trivial cluster $(\{u\}, T_{\{u\}})$. 

Each cluster is assigned a unique identifier. In the beginning, the identifier of $\{u\}$ is simply defined as the identifier of $u$ and $C$ keeps that identifier, although during the algorithm $C$ can lose some nodes, including $u$. On the other hand, $T_C$ never loses nodes. 
We will maintain as an invariant that the radius of each $T_C$ grows only by $O(D)$ in each of the $\poly\log(n)$ many steps, and that we can implement \aggregate operations on each cluster $C$ in $\poly\log(n)$ \aggregate rounds, even though clusters may become disconnected. 

\paragraph{One Phase}
We now discuss the algorithm in greater detail. 
At the beginning of phase $i$, we mark all clusters such that the $i$-th bit in their identifier is $0$ as active and the rest of the clusters are marked as passive.

We now describe one step of the algorithm, in which active clusters potentially grow. Each active cluster is in one of two states. Either it is \emph{growing} or \emph{finished}. At the beginning of the phase, every active cluster is growing. 
Let $\Vactive \subseteq \Valive$ be the set of all nodes in active clusters. 

In each step of the $i$-th phase, we define $S$ as the set consisting of all the nodes in growing clusters and use the oracle $\oDist_{\eps,D\cdot (1-\eps)^i}$ with input $S$.
Note that we are allowed to use the oracle as $D \cdot (1-\eps)^b \ge D / 2$.  
The oracle outputs a forest $F$ with $S$ being the set of roots.
%Note that the root of each tree $T \subseteq \tilde{F}$ is in $S$. However, there can be a non-root node $s \in S \cap T$. For each such potential node $s$ we delete the edge from $s$ to its parent in $\tilde{F}$ from $\tilde{F}$ and make it a new root. This defines a new forest $F$ that has the property that it contains all nodes of $S$ as root nodes. Moreover, $F$ is clearly still retains the same distance guarantees as $\tilde{F}$. 



\paragraph{Growth of a cluster}
For each growing cluster $C$ consider all trees in $F$ such that their root is in $C$. We denote this forest as $F_C$ and think about is as a Steiner tree that collects all nodes ``proposing to join'' the cluster $C$ and which enables us to aggregate information about the proposing nodes. 
Every cluster $C$ computes $|F_C \cap (\Vrem \setminus \Vactive)|$. 
If $|F_C \cap (\Vrem \setminus \Vactive)| \ge \frac{\delta}{b} |C|$, the cluster $C$ grows. 
That is, all nodes in $F_C \cap (\Vrem \setminus \Vactive)$ join $C$.  These nodes leave their respective passive clusters.  This means that 
\begin{align*}
C_{new} := C \cup (F_C \cap (\Vrem \setminus \Vactive)).
\end{align*}

We now discuss how the Steiner tree $T_C$ is extended. 
Let $F'_C$ denote the rooted forest one obtains from $F_C$ by deleting all the nodes in $F_C$ whose subtree does not contain nodes of $C_{new}$. 
That is, $F'_C$ is a ``pruned'' version of the Steiner tree $F_C$ that does not contain nodes from $\Vrem$ that are not needed for aggregation. 

The vertex set of the new Steiner tree $T_{C_{new}}$ is $V(T_{C_{new}}) = V(T_C) \cup F'_C$. The edge set is $E(T_{C_{new}}) = E(T_C) \cup \{(u,v) \in E(F'_C) | u \not\in T_C \}$, where we use that each edge $e \in E(F'_C)$ knows its orientation from $u$ to $v$ in the direction of the root. That is, when combining the edge sets of the tree $T_C$ and the forest $F'_C$, we drop each edge of $F'_C$ that would result in some node having two parents. 

Otherwise, when $C$ decides not to grow, all nodes in $F_C \cap (\Vrem \setminus \Vactive)$ are removed from $\Valive$. 
In that case, $C$ finishes and stops growing in the current phase. 

This finishes the description of the algorithm, up to implementation details considered later. 

\begin{claim}
The total number of deleted nodes is at most $\delta \cdot   |\Vrem|$. 
\end{claim}
\begin{proof}
  We prove that in each phase we delete at most $\delta |\Vrem|/b$ nodes. The claim then follows. 
  Consider one phase of the algorithm. Let $C$ be some cluster and $n_C$ the total number of nodes contained in $C$ at the end of the phase. 
The cluster $C$ is responsible for deleting nodes of total weight at most $\delta n_C / b$. Hence, the total number of deleted nodes is upper bounded by $\sum_{C \text{ active in phase }i} \delta n_C /b \le \delta |\Vrem|/b$, as needed.  
\end{proof}

\begin{claim}
\label{cl:stop_growing}
In each phase, each cluster stops growing after $O(\log n \cdot b/\delta)$ steps. 
\end{claim}
\begin{proof}
For the sake of contradiction, assume there exists a cluster $C$ that was growing for all $t = O(\log  n  \cdot b/\delta)$ steps of a given phase. Then, $|C| \ge (1 + \delta/b)^t >  n  $, a contradiction. 
\end{proof}

\begin{claim}
After the algorithm terminates, for any two clusters $C_1 \neq C_2$ we have $\dist_G(C_1, C_2) \ge (1-\eps)^b D$. 
\end{claim}
\begin{proof}
%Let $\Vrem = V_{00\dots0} \sqcup V_{00\dots1} \sqcup \dots \sqcup V_{11\dots1}$ be the following split: each node $u \in V_b$, where $b$ is a bit string of length $i-1$, if it is in a cluster such that its first $i-1$ bits are $b$. 
We prove the following invariant by induction: After the $i$-th phase, if two clusters do not agree on their first $i$ bits, then their distance in $G$ is at least $(1-\eps)^i D$. The claim then follow by setting $i = b$. 
Suppose the invariant holds after the $(i-1)$-th phase (case $i=0$ is an easy special case). We show that this implies that the invariant also holds after the $i$-th phase. 



To do so, we first show the following property. After each step during the $i$-th phase, if two clusters do not agree on their first $i-1$ bits, then their distance in $G$ is at least $(1-\eps)^{i-1}D$.



Note that our induction hypothesis states that the property above holds at the beginning of the $i$-th phase. Hence, it remains to show that each step $j$ during phase $i$ preserves the property.

For this, it suffices to show that a node can only switch from one cluster to another cluster during the $j$-th step if the two clusters agree on their first $i-1$ bits.

To that end, consider some node $v$ and two clusters $C_1$ and $C_2$ before the $j$-th step. Assume that $v$ is contained in cluster $C_1$ before the $j$-th step and during the $j$-th step $v$ decides to join the cluster $C_2$.
It directly follows from the algorithm description that this can only happen if $\dist_G(C_2,v) \leq (1+\eps)(1-\eps)^i D < (1-\eps)^{i-1}D$.
In particular, $\dist_G(C_1,C_2) < (1-\eps)^{i-1}D$ and therefore the two clusters $C_1$ and $C_2$ agree on their first $i-1$ bits, as desired.

 

It remains to consider two clusters that agree on their first $i-1$ bits but disagree on their $i$-th bit.
Exactly one of those clusters, say $C$, is active during the $i$-th phase and by \cref{cl:stop_growing} we know that $C$ decides to stop growing at some point during the phase, by deleting all the nodes that proposed to join it in that step.
In particular, each alive node outside $C$ with a distance of at most $(1- \eps)^i D$ to $C$ either gets killed or decides to join an active cluster different from $C$. Since nodes in active clusters remain in the same active cluster until the end of the $i$-th phase, the distance of $C$ to any other cluster with a different $i$-th bit is at least $(1-\eps)^iD$ at the end of the $i$-th phase. 
This finishes the proof of the induction statement.


\end{proof}


\begin{claim}
For any cluster $C$, the radius of $T_C$ is $O(D \log^3(n)/\delta)$. 
\end{claim}
\begin{proof}
The radius of $T_C$ grows by $O((1+\eps)D)$ in each step. 
Each of the $b$ phases consists of $O(b /\delta \cdot \log n)$ steps. Hence, the radius of $T_C$ can be bounded by $O(b^2\log( n )D/\delta) = O(D \log^3(n) / \delta)$. 
\end{proof}

\begin{claim}
Consider any $W \subseteq \Vrem$ and $(C,T_C) \in \fC$. 
    If $\dist_G(W, \Vrem \setminus W) > (1+\eps) D$, then we have the following. 
    Whenever we have $C \cap W \not = \emptyset$, then $C \subseteq W$ and for any $u \in T_C$ we have $\dist_G(u, W) \le (1+\eps)D/2$. 
\end{claim}
\begin{proof}
Let $W \subseteq \Vrem$ be any set such that $\dist_G(W, \Vrem \setminus W) > (1+\eps) D$. A simple induction argument shows that any cluster $C$ that started as a node $u \in W$ will satisfy $C \subseteq W$ during the course of the algorithm and an analogous statement holds if we replace $W$ by $\Vrem \setminus W$. To show the second part, let $C' \subseteq W$ be some arbitrary cluster during the course of the algorithm. It suffices to show that for any node $u \in V(F'_{C'})$ in the pruned Steiner Tree it holds that $\dist_G(u,W) \leq (1+\eps)D/2$. As $u \in V(F'_{C'})$, there exists some node $v \in \Vrem$ that is contained in the subtree of $u$ in $F_{C'}$. Each node in $F_{C'}$ has a distance of at most $(1+\eps)D$ to its root.
As the root is contained in $W$, we have $\dist_G(W,v) \leq (1+\eps)D$. In particular, $v \notin \Vrem \setminus W$ but $v \in \Vrem$ and therefore $v \in W$.
Now, let $r$ be the root of $u$ in $F_{C'}$. As $v$ is an ancestor of $u$ in $F_{C'}$, we have

\begin{align*}
    \dist_{F_{C'}}(r,v)  = \dist_{F_{C'}}(r,u) + \dist_{F_{C'}}(u,v) \leq (1+\eps)D.
\end{align*}

In particular,

\begin{align*}
    \dist_G(u,W) \leq \dist_{F_{C'}}(u,\{r,v\}) \leq (1+\eps)D/2,
\end{align*}


as desired.
\end{proof}

\begin{claim}
\label{cl:weak_diam_aggregation}
During the construction, we can implement any \aggregate operation on clusters in $O(1/\delta \cdot \log^3(n))$ \aggregate rounds. 
\end{claim}
\begin{proof}
We will show how to implement any aggregate operation $\bigoplus$ on the clusters of some partial clustering $\fC$ that we have during the algorithm.  

Assume that each node $u$ is given some value $v_u$ and we wish to compute $\bigoplus_{u \in C} v_u$ for each $C \in \fC$. 
Let $F^1, F^2, \dots, F^k$ be the forests found by calls to $\oDist_{\eps, D'}$ so far and let $F'^1_C, F'^2_C, \dots, F'^k_C$, with $F'^i_C \subseteq F^i$, be the corresponding subforests that we used to grow $C$. 
We will run the following $k$ round algorithm. 
In the $i$-th round, for $0 \le i < k$, each tree $T \subseteq F'^{k-1}_C \subseteq F^{k-i}$ computes consensus of values of all nodes $u \in T \cap C$. 
That is, it computes $\bigoplus_{u \in T\cap C} v_u$. 
This can be done in one \aggregate round for all clusters $C$ in parallel, as each $T \subseteq F'^{k-i}_C$ is connected and the trees are mutually disjoint.  
Then, we remove the values of all nodes in $T \cap C$, except of the root $r$ of $T$ that takes the new value $v_r^{new} = \bigoplus_{u \in T\cap C} v_u$, that is, the result of the calculation. 
A straightforward induction argument shows that after $k$ rounds, the root $r_C$ of each cluster $C$ (that is, the node that defined $C$ at the beginning of the algorithm) knows the value of $\bigoplus_{u \in C} v_u$. 
Once the value of each cluster is computed, it can be broadcasted from $r_C$ back to all nodes in $C$. 
This is done analogously to the computation step, but the forests $F_1, F_2, \dots, F_k$ are now iterated over in the ascending order. 
\end{proof}

\begin{claim}
The algorithm can be implemented in $O(1/\delta^2 \cdot \log^6 n)$ \aggregate rounds and needs $O(1/\delta \cdot \log^3(n))$ calls to the oracle $\oDist_{\eps, D'}$ for $D' \in [D/2, D]$. 
\end{claim}
\begin{proof}
The algorithm has $O(\log n)$ phases and each consists of $O(1/\delta \cdot \log^2 n) $ steps. Let us now discuss the complexity of each step. 
In each step, the decision of each cluster to grow or not can be implemented with one call of the distance oracle $\oDist_{\eps, D'}$ and $O(1/\delta \cdot \log^3(n))$ \aggregate rounds, since the decision of each cluster to grow or not amounts to an aggregation on it and on $F_C$. 
After the decision of each cluster, we need to do additional bookkeeping. The only nontrivial part of it is pruning each forest $F_C$ into $F'_C$. To prune $F_C$, each node in it needs to know whether there are $\Vrem$ nodes in the subtree of it. This is a special case of the subtree sum problem that can be solved in $\poly\log(n)$ \aggregate rounds \cref{lemma:ancestor-subtree-sum}. 
Hence, the complexity of the algorithm is $1/\delta^2 \poly\log(n)$. 
The total number of invocations of $\oDist_{\eps, D'}$ is bounded by $O(1/\delta \cdot \log^3(n))$. 
\end{proof}

\end{proof}


\subsection{Strong-Radius Clustering}
\label{sec:strong_radius}

\begin{lemma}[Deterministic Strong-Radius Clustering]
\label{lem:strongdiam}
Let $G$ be a weighted graph, $\Vrem \subseteq V(G)$ and $D > 0$. We assume that each node of $G$ has a unique identifier from $[2^b]$ for $b=O(\log n)$ and set $\eps = \frac{1}{100b\log(n)}$. 

We can compute an $\eps D$-separated $O(D \log^4(n))$-strong-radius clustering $\fC_{out}$ such that $V(\fC_{out}) \subseteq \Vrem$ and $|V(\fC_{out})| \ge |\Vrem|/3$.

The computation consists of $\poly(\log n)$ \aggregate rounds in $G$ and $\poly(\log n)$ calls to distance oracles $\oDist_{\eps, D'}$ for various $D' \in [D , 10 D]$. 
\end{lemma}

The lemma is proven by an adaptation of the algorithm from \cite{chang_ghaffari2021strong_diameter}. 


\begin{proof}

  We compute the strong-radius clustering by the following algorithm. The algorithm has $k = O(\log n)$ phases and in the $i$-th phase we invoke the weak-radius clustering from \cref{lem:weak_diam} with parameters $\Vrem^i, D^i$ and $\delta^i = \delta = 1/(3k)$ to obtain an output clustering $\fC^i$.
  In each phase, we add new strong-radius clusters to an initially empty set $\fC_{out}$. 
    
    At the beginning, we set $\Vrem^1 = \Vrem$ and define $\fC^0 = \{ \Vrem \}$. 
    In the $i$-th phase of the algorithm we do the following. 
  \begin{enumerate}
      \item We invoke \cref{lem:weak_diam} with parameters $\Vrem^i, D^i = 10D \cdot (1-\eps)^{2ib}$ and $\delta^i$. The output is a $(1-\eps)^bD^i$-separated weak-radius clustering $\fC^i$. % with weak-radius $O(D^i \log^3 n \cdot 1/\delta) = O(D \cdot \log^4 n)$. %Moreover, each cluster $C \in \fC$ is accompanied with a strong-radius cluster $\overline{C} \supseteq C$ of radius $O(D \cdot \log^4 n)$. We have  $|\Vrem^i \setminus \bigcup_{C \in \fC^i} C| \le \delta |\Vrem^i| = |\Vrem^i|/(3k)$.
      \item For each cluster $C \in \fC^i$, there exists a (unique) cluster $\parent(C) \in \fC^{i-1}$ with $C \subseteq \parent(C)$ (\cref{cl:strong_laminar}). 
      If $|C| > |\parent(C))|/2$, then we add $(V(T_{C}), T_{C})$ to $\fC_{out}$. 
      \item 
      Let $C^i_1, C^i_2, \dots, C^i_\ell$ denote the clusters added to $\fC^{out}$ during the $i$-th phase. \\
      We set $\Vrem^{i+1} = \left( \bigcup_{C \in \fC^i} C \right)  \setminus (\bigcup_{j=1}^{\ell} \parent(C^i_j))$. 
      
     \end{enumerate} 
     At the very end we output the output set $\fC_{out}$. This finishes the description of the algorithm. 
     
     
     
     
  
\begin{claim}
\label{cl:strong_laminar}
For each cluster $C \in \fC^i$, there exists a (unique) cluster $\parent(C) \in \fC^{i-1}$ with $C \subseteq \parent(C)$ (\cref{cl:strong_laminar}). 
\end{claim}  
\begin{proof}
Consider an arbitrary cluster $C \in \fC^i$ and let $\parent(C)$ be any cluster in $\fC^{i-1}$ with $C \cap \parent(C) \neq \emptyset$. It suffices to show that $C \subseteq \parent(C)$.
Let $W = \parent(C)$. 
Note that $W \subseteq \Vrem^i$, since for each cluster $C' \in \fC^{i-1}$ either all nodes of $C'$ are in $\Vrem^i$ or no nodes are in $\Vrem^i$. 
Next, we have $\dist_G(W, \Vrem^i \setminus W) \ge (1-\eps)^b D^{i-1} > (1+\eps)D^i$, as the distance between any two clusters in $\fC^{i-1}$ is at least $(1-\eps)^bD^{i-1}$ and $D^i / D^{i-1} = (1-\eps)^{2b}$. 
Hence, the fourth property of \cref{lem:weak_diam} gives $C \subseteq \parent(C)$, as desired.
\end{proof}
  
\begin{claim}
\label{cl:strong_finish}
$\Vrem^k = \emptyset$. 
\end{claim}  
\begin{proof}
Let $C^0, C^1,\ldots, C^i$ be clusters such that $C^i \in \fC^i$ and $\parent(C^{j}) = C^{j -1}$ for $1 \le j \le i$. We have $|C^0| \leq n$ and $|C^{j}| \leq |C^{j -1 }|/2$. Hence, $|C^i| \leq n/2^{i-1}$.
Let $k = 3 + \lceil \log_2 n \rceil$. Then, $\fC^{k-1}$ cannot contain any clusters and therefore $\Vrem^k = \emptyset$. 
\end{proof}

\begin{claim}
\label{cl:strong_deleted}
$|V(\fC_{out})| \ge |\Vrem| / 3$. 
\end{claim}  
\begin{proof}
    \cref{cl:strong_finish} together with the algorithm description implies that for every node $u \in \Vrem$ at least one of the following holds.

    \begin{enumerate}
        \item $u \in  V(\fC_{out})$
        \item $u \in C$ and $C$ has a sibling $C'$ ($\parent(C) = \parent(C')$, $C \neq C'$) with $V(T_{C'}) \in \fC_{out}$ 
        \item $u \in \Vrem^i$ but the algorithm of \cref{lem:weak_diam} invoked in the $i$-th phase left $u$ unclustered 
    \end{enumerate}    
    
    There are at most $k \cdot \delta |\Vrem| = (1/3)|\Vrem|$ nodes that satisfy the third condition. 
    Moreover, as every cluster $C$ with $V(T_C) \in \fC^{out}$ satisfies $|C| \geq |\parent(C)|/2$, the total number of nodes that satisfy the first condition is at least as large as the total number of nodes that satisfy the second condition. Hence, $ |V(\fC_{out})| \geq (1/2)(2/3)|\Vrem|$, as desired.
\end{proof}

  
\begin{claim}
\label{cl:strong_padded}
For any two distinct clusters $C^{out}_1,C^{out}_2 \in \fC_{out}$, we have $\dist_G(C^{out}_1, C^{out}_2) \ge \eps D$. 
\end{claim}  
\begin{proof}
As $C^{out}_1,C^{out}_2 \in \fC_{out}$, there exists $i_1, i_2 \in [k]$ and two clusters $(C_1,T_{C_1}) \in \fC^{i_1}$ and $(C_2,T_{C_2}) \in \fC^{i_2}$ such that $C^{out}_1 = V(T_{C_1})$ and $C^{out}_2 = V(T_{C_2})$.
Without loss of generality $i_1 \le i_2$. 
We first compute a lower bound on the distance between $C_1 $ and $C_2$. 
Let $\hat{C}_1, \hat{C}_2 \in \fC^{i_1 - 1}$ such that $C_\ell \subseteq \hat{C}_\ell$ for $\ell \in [2]$. In particular, $\hat{C}_1 = \parent(C_1)$. 
We have $\hat{C}_1 \neq \hat{C}_2$. If $i_1 = i_2$, then $\hat{C}_1 \neq \hat{C}_2$ follows from the fact that $|C_\ell| > (1/2)| \hat{C}_\ell|$ for $\ell \in [2]$. If $i_1 < i_2$, then $\hat{C}_1 \neq \hat{C}_2$ follows from the fact that $\Vrem^{i_1 + 1} \cap \hat{C}_1 = \emptyset$ and $\Vrem^{i_2} \subseteq \Vrem^{i_1 + 1}$.
Hence,  

\begin{align*}
\dist_G(C_1,C_2)\geq \dist_G(\hat{C}_1, \hat{C}_2) \ge (1-\eps)^b D^{i_1 - 1}.    
\end{align*}


Moreover, with $W = \hat{C}_1$ we have $\dist_G(W,\Vrem^{i_1} \setminus W) \geq (1-\eps)^b D^{i_1 - 1} \geq (1+\eps)D^{i_1}$. This implies, as $C_1 \cap W \neq \emptyset$, that $\dist_G(u,W) \le (1+\eps)D^{i_1}/2$ for every $u \in V(T_{C_1}) = C^{out}_1$.
and, similarly, $\dist(T_{C^{i_2}}, \hat{C}^2) \le (1+\eps)D^{i_2}/2 \le (1+\eps)D^{i_1}/2$.
A similar argument shows that $\dist_G(u, \hat{C}_2) \leq (1+\eps)D^{i_2}/2$ for every $u \in V(T_{C_2})= C^{out}_2$.

Now, consider an arbitrary $v_1 \in C^{out}_1$ and $v_2 \in C^{out}_2$. We have 
\begin{align*}
\dist_G(v_1,v_2) &\geq 
\dist_G(\hat{C}_1, \hat{C}_2) - \dist_G(\hat{C}_1,v_1) - \dist_G(\hat{C}_2, v_2) \\
&\ge (1-\eps)^b D^{i_1 - 1} - 2(1+\eps)D^{i_1}/2\\
&= \left( (1-\eps)^b / (1-\eps)^{2b} - (1+\eps)\right) D^{i_1}
\ge 2\eps D^k \ge \eps D, 
\end{align*}
as needed. 
\end{proof}


To conclude the proof, note that each cluster $C \in \fC_{out}$ has strong-radius $O(D \log^3(n) \cdot 1/\delta) = O(D \log^4(n))$, clearly $V(\fC_{out}) \subseteq \Vrem$, the clustering is $\eps D$-separated by \cref{cl:strong_padded} and $|V(\fC_{out})| \ge |\Vrem|/3$ by \cref{cl:strong_deleted}. In each phase we call \cref{lem:weak_diam} once. In addition, each cluster needs to check whether it gets added to the output clustering by comparing its size to the size of its parent. If a cluster indeed gets added, it also needs to inform all the nodes in the parent cluster. This can be implemented in $O(1)$ aggregations on clusters that \cref{lem:weak_diam} outputted during the course of the algorithm. Hence, by the aggregation property in \cref{lem:weak_diam} the algorithm can be implemented in $\poly\log(n)$ \aggregate rounds and $\poly\log(n)$ calls to distance oracles $\oDist_{\eps, D'}$ for various $D' \in [D, 10D]$, as desired. 
\end{proof}

\subsection{Sparse Neighborhood Cover}
\label{sec:sparse_cover}

\begin{theorem}
\label{thm:sparse_cover}
Let $G$ be a weighted graph and $D \geq 0$.
Assume we have access to oracle $\oDist_{\eps,D'}$ for various $D' \in [\frac{D}{\log^7 n},D]$ and $\eps = \frac{1}{\log^3 n}$.
We can compute a sparse neighborhood cover with covering radius $\frac{D}{\log^7 n}$ such that each cluster $C$ in one of the clusterings comes with a rooted tree  $T_C$ of diameter at most $D$. The algorithm runs in $\poly(\log n)$ \aggregate rounds.
\end{theorem}
%\sparseCover*

\begin{proof}

Let $\Delta = \Theta(D / \log^4 n)$. 
Our algorithm consists of $t = 100 \lceil \log(n) \rceil$ rounds. Let $\Vrem^1 := V(G)$.
In the $i$-th round, we use the algorithm of \cref{lem:strongdiam} with $\Vrem^\Lref{lem:strongdiam} = \Vrem^i$ and ${D}^\Lref{lem:strongdiam} = \Delta$ to compute a $s = \Omega(\Delta/\log^2 n) = \Omega(D / \log^6 n)$-separated $\Theta(D)$-strong-radius clustering $\fC^i$ with $V(\fC^i) \subseteq \Vrem^i$ and $|V(\fC^i)| \geq |\Vrem^i|/3$. Moreover, we can choose the constant in the definition of $\Delta$ such that $\fC_i$ is $D/4$-strong-radius clustering. 
We then set $\Vrem^{i+1} = \Vrem^i \setminus V(\fC^i)$.

We now extend each cluster $(C,T_C) \in \fC^i$ to some new cluster $(\hat{C},T_{\hat{C}})$. This defines a new clustering $\hat{\fC}^i$. 
To do so, we first invoke the distance oracle $\oDist_{\eps,s/10}$ with input $V(\fC^i)$.
Let $F$ denote the rooted forest returned by the oracle.
For each $(C, T_C) \in \fC^i$, let $F_C \subseteq F$ be the forest which contains all trees in $F$ whose root is contained in $C$. We set $\hat{C} = C \cup V(F_C)$ and  define $T_{\hat{C}}$ as the rooted tree one obtains by adding the trees in $F_C$ to $T_C$, i.e, $V(T_{\hat{C}}) = V(F_C) \cup V(T_C)$ and $T_{\hat{C}}$ and $T_C$ have the same root. 
Clearly, any node in $T_{\hat{C}}$ has a distance of at most $D/4 + (1+\eps)(s/10) = D/2$ to the root. 
Moreover, as the clustering $\fC^i$ is $s$-separated, it follows that $\hat{\fC^i}$ is $\hat{s}$-separated with $\hat{s} := s/10 \leq s - 2(1+\eps)(s/10)$ and for any node $u$ with $\dist_G(u,C) \leq \hat{s}$ we have $u \in \hat{C}$.  
In particular, as $\Vrem^t = \emptyset$, for every node $u \in V(G)$ there exists some $i$ such that the ball of radius $\hat{s}$ around $u$ is fully contained in one of the clusters of $\hat{C}^i$.
Hence, $(\hat{\fC}^i)_{i \in [t]}$ is a sparse neighborhood cover with covering radius $\hat{s} \ge D/\log^7 n$ and each cluster $C$ of it comes with a rooted tree $T_C$ of diameter at most $2 \cdot (D/2) = D$. 

It directly follows from the guarantees of \cref{lem:strongdiam} that the computation consists of $\poly(\log n)$ \aggregate rounds in $G$ and $\poly(\log n)$ calls to distance oracles $\oDist_{\eps, D'}$ for $\eps := \frac{1}{100b \log(n)} \ge 1/\log^3 n$ and various $D' \in [D/\log^7 n, D]$.
\end{proof}






% Local Variables:
% TeX-master: "main"
% End:


==> TS-and-Boosting.tex <==


\section{Transshipment Boosting via Multiplicative Weights}\label{sec:boosting}

 % theorem 1.5
% Theorem 1.5. (Distributed oblivious routing evaluation). Let G = (V, E) be a weighted graph with weights in [1, n O(1) ]. There exists an exp(O(log n · log log n) 3/4 )-approximate ` 1 -oblivious routing R such that we can perform the following computations in exp(O(log n · log log n) 3/4 ) rounds of Minor-Aggregation. Given any distributedly stored node vector d ∈ R n and edge vector c ∈ R n , we can evaluate and distributedly store Rd ∈ R m and R T c ∈ R n


  % Let $R$ be an $\alpha$-approximate $\ell_1$-oblivious routing with respect to a transshipment instance on a weighted graph $G$. Suppose we can compute matrix-vector products with $R$ and $R^T$ in $M$ Minor-Aggregation rounds. Then we can compute and distributedly store a flow $f \in \R^m$ and a \emph{vector of potentials} $\phi$ in $\tilde{O}(\alpha^2\eps^{-2}M)$ rounds such that
  % \begin{enumerate}
  % \item $\norm{Wf}_1 \trleq (1+\eps)d^{\top} \phi \leq (1+\eps) \norm{d}_{\opt}$;
  % \item $\norm{Bf - d}_{\opt} \leq \eps \norm{d}_{\opt}$;
  % \item $\norm{W^{-1} B^T \phi}_\infty \le 1$.
  % \end{enumerate}


\begin{lemma}
\label{lem:transshipment_primal_dual}
Let $R \in \R^{V \times \vec{E}}$ be an $\alpha$-approximate $\ell_1$-oblivious routing on a weighted graph $H = (V, E)$ with weight vector $\ell \in \R^E$, let $b \in \R^V$ be a demand vector with $\sum_{v \in V} b_v = 0$, and let $0 < \eps < 1/2$. Suppose we can compute matrix-vector products with $R$ and $R^T$ in $M$ \aggregate rounds. Then, in $\eps^{-2}\poly(\alpha, M, \log n)$ \aggregate rounds, we can compute a flow $f \in \R^{\vec{E}}$ that satisfies the demand $b$, and a vector of potentials $\phi$ such that $\ell(f) \le (1+\eps)b^T\phi$.
\end{lemma}
\begin{proof}
  Lemma 6.1 of \cite{goranci2022universally} proves there exist a $\tilde{O}(\alpha^2 \eps^{-2} M)$ \aggregate round algorithm that computes a flow $f' \in \R^{\vec{E}}$ and potentials $\phi' \in \R^{V}$ satisfying (1) $\ell(f') \le (1 + \eps) b^T \phi \le (1 + \eps) \norm{b}_\opt$ , and (2) flow $f'$ satisfies a potentially different demand $b'$ with the guarantee $\norm{b - b'}_\opt \le \eps \norm{b}_\opt$ (i.e., that one can near-optimally route the difference). This nearly matches our required guarantees with the exception that we require our final flow $f$ to perfectly satisfy the guarantees.

  For future reference, we show that $\norm{b}_\opt \le (1 + 5 \eps) b^T \phi$. First, there exists a flow $f_2^*$ that satisfies $b'$ of $\ell(f_2^*) \le \norm{b'}_\opt \le \eps \norm{b}_\opt$. Since $f' + f_2^*$ satisfies $b$, we have that $\norm{b}_\opt \le \ell(f') + \ell(f_2^*) \le (1 + \eps) b^T \phi + \eps \norm{b}_\opt$. Therefore, $(1 - \eps) \norm{b}_\opt \le (1 + \eps) b^T \phi$, or $\norm{b}_\opt \le (1 + 5 \eps) b^T \phi$.

  To fix $f$, we can simply call the above procedure with an enhanced guarantee of $\eps' := \eps / \alpha$, guaranteeing $\norm{b - b'}_\opt \le \frac{\eps}{\alpha} \norm{b}_\opt$. Then, utilizing the $\alpha$-competitive oblivious routing $R$, we compute $f'' := R(b - b')$ which satisfies $\ell(f'') \le \alpha \norm{b - b'}_\opt \le \alpha \frac{\eps}{\alpha} \norm{b}_\opt = \eps \norm{b}_\opt$. Therefore, the flow $f' + f''$ (perfectly) satisfies $(b - b') + b' = b$ and has cost $\ell(f' + f'') \le \ell(f') + \ell(f'') \le (1 + \eps)b^T \phi + \eps \norm{b}_\opt \le (1 + \eps)b^T \phi + \eps (1 + 5 \eps) b^T \phi \le (1 + 5 \eps) b^T \phi$. Reducing $\eps$ by a factor of $5$ gives the final result.
\end{proof}


\begin{restatable}[Boosting + Rounding]{theorem}{boosting}
\label{theorem:boosting_rounding}
Let $R$ be an $\alpha$-approximate $\ell_1$-oblivious routing on a weighted graph $H$ and $s \in V(H)$ be arbitrary. For a given $\eps \in (0,1]$, one can compute:
\begin{itemize}
  \item A potential $\phi$ with $\phi(s) = 0$. 
  \item A tree $T$ rooted at $s$ such that for each $v \in V(H)$ we have that $\dist_T(v) \le (1 + \eps) \phi(v)$.    
  \end{itemize}
  The computation runs in $\tilde{O}(\poly(\alpha)\eps^{-2})$ \aggregate rounds in $H$, together with $\tilde{O}(\poly(\alpha)\eps^{-2})$ many computations of matrix-vector products with $R$ and $R^T$ and $\poly(\log n)$ oracle calls to $\oRound_{\eps / 2}$.
\end{restatable}
  The main ideas of the solution to this task were mostly presented as the Algorithm SSSPTree of \cite{haeuplerLi2018sssp}. We adapt the ideas from this and describe them here for completeness.
\begin{proof}

%  Initially, let $b \in \R^V$ be a demand with $b(s) \gets -(n-1)$ and $b(v) \gets 1$ for all $v \neq s$. 

First we present a procedure with $k = O(\log n)$ phases that in each phase constructs a tree-potential pair $\phi_i, T_i$ by invoking \cref{lem:transshipment_primal_dual}. 
During this procedure, we maintain a set of \emph{unhappy} nodes $V_i$. 
At the beginning, $V_i = V \setminus \{s\}$. 
A node $v \in V_i$ becomes happy in a phase $i$ if $d_{T_i}(s, v) \le (1+\eps)\phi_i(v)$. 
Let us moreover define $\zeta_i = \sum_{v \in V_i} \dist(s, v)$. 

We now describe the procedure in a greater detail and prove that $\zeta_i$ decreases by a constant factor every phase, hence after $ k = O(\log n)$ phases $\zeta_k  = 0$ and every node is happy. 
In each phase, we invoke \cref{lem:transshipment_primal_dual} with our $\ell_1$-oblivious routing $R$ and a demand $b(s) = -|V_i|$ and $b(v) = 1$ for all $v \in V_i$. 
 \Cref{lem:transshipment_primal_dual} returns a flow $f_i$ and a potential $\phi_i$ with $\ell(f_i) \le (1 + \frac{\eps}{10}) b^T \phi_i$; suppose that (by translation) $\phi_i(s) = 0$. 
 Using the rounding oracle $\oRound_{G, \eps/2}$ we round $f$ to a tree $T$ satisfying $\sum_{v, b(v) \neq 0} b(v) \dist_{T_i}(s, v) \le (1 + \frac{\eps}{2}) \ell(f_i)$. 
    Hence, have
  \begin{align}
  \label{eq:sss}
    \sum_{v \in V_i} \dist_{T_i}(s, v) 
    \le \left( 1 + \frac{\eps}{2}\right) \ell(f) 
    \le \left( 1 + \frac{\eps}{2} \right) \left( 1 + \frac{\eps}{10} \right) b^T \phi_i 
    \le \left( 1 + \frac{2}{3} \eps \right) \sum_{v \in V_i} \phi_i(v).  
  \end{align}
 
 %Note that the distances in $T$ are good on average, but not individually good. We use the following procedure to correct this issue.
Let $U_i \subseteq V_i$ be the set of nodes $v$ that become happy in phase $i$, that is, $v \in U_i$ if  $\dist_{T_i}(s, v) \le (1+\eps)\phi_i(v)$. 
  We can compute the root-to-$v$ distances in $T_i$ with the ancestor sum operation (\Cref{lemma:ancestor-subtree-sum}) in $\tilde{O}(1)$ \aggregate rounds. 
  Therefore, we can check for each node $v \in V_i$ whether $v \in U_i$ or not and define $V_{i+1} = V_i \setminus U_i$. 

  Since $\phi_i$ is a potential, we have $ \sum_{v\in U_i} \phi_i(v) \le \sum_{v \in U_i} \dist_{T_i}(s, v) $ and by definition $(1+\eps)\sum_{v\in V_i \setminus U_i} \phi_i(v) \le \sum_{v \in V_i \setminus U_i} \dist_{T_i}(s, v)$. 
  Together with above inequality we get
  \begin{align*}
      \sum_{v \in U_i} \phi_i(v) + \left( 1 +\eps \right)\sum_{v \in V_i \setminus U_i} \phi_i(v) \le \left( 1 + 2\eps/3 \right) \sum_{v \in V_i} \phi_i(v),
  \end{align*}
  hence
  \begin{align*}
   \eps \sum_{v \in V_i \setminus U_i} \phi_i(v) \le 2\eps/3 \sum_{v \in V_i} \phi_i(v) 
  \end{align*}
  or
  \begin{align}
  \label{eq:psss}
   \sum_{v \in U_i} \phi_i(v) \ge \sum_{v \in V_i} \phi_i(v)/3.  
  \end{align}
  
    Hence, we have 
    \begin{align*}
        \zeta_{i} - \zeta_{i+1}
        &= \sum_{v \in U_i} \dist(s, v)
        \ge \sum_{v \in U_i} \phi_i(v) && \text{$\phi_i$ is a potential} \\
        &\ge \sum_{v \in V_i} \phi_i(v)/3 &&  \text{Eq. \cref{eq:psss}}\\
        &\ge \sum_{v \in V_i} \dist_{T_i}(s, v)/4 &&  \text{Eq. \cref{eq:sss}}\\
        &\ge  \sum_{v \in V_i} \dist(s, v)/4
        = \zeta_i / 4 
    \end{align*}
  
Hence, after $k = O(\log n)$ phases $\zeta_k = 0$ and every node is happy. 

 Next, we use potentials $\phi_1, \ldots, \phi_k$ and trees $T_1, \ldots, T_k$ to construct a common potential $\phi$ and tree $T$ that we output. 
 First, we construct a common potential $\phi \in \R^V$ by $\phi(v) = \max_{i=1}^k \phi_i(v)$. 
 Note that $\phi$ is potential by \cref{fact:potential_min_max} and if $v$ got happy in the $i$-th phase, we have $d_{T_i}(s, v) \le (1+\eps)\phi(v)$. 

Second, we construct a common tree $T$ by letting each node maintain its $T$-\emph{parent} and a \emph{distance label} which is an upper bound on the distance to the root in $T$. First, direct all trees $T_i$ from the root to the leafs using \Cref{lemma:ancestor-subtree-sum}. 
Then, set $T := T_1$ (by copying the parent pointers) and initialize the distance label of $v$ with $\dist_{T_i}(s, v)$. Then, we process $T_2, T_3, \ldots, T_k$ one-by-one. Each node $v$ considers whether the distance label of the $T_i$-parent plus the weight of the $T_i$-parent-edge is smaller than the current distance label. If yes, its sets its parent pointer to its $T_i$-parent and updates the distance label. After processing all $T_i$, the parent pointers characterize the tree $T$. Furthermore, it is easy to show that the distance label for a node $v$ is upper bounded by $\min_{i=1}^k \dist_{T_i}(s, v)$, hence every node $v$ satisfies $\dist_{T}(s, v) \le (1+\eps)\phi(v)$. 
\end{proof}


==> abstract.tex <==
\begin{abstract}
\noindent This paper presents near-optimal deterministic parallel and distributed algorithms for computing $(1+\eps)$-approximate single-source shortest paths in any undirected weighted graph.
\medskip

\noindent On a high level, we deterministically reduce this and other shortest-path problems to $\tO(1)$ \footnote{We use $\tO$-notation to suppress polylogarthmic factors in the number of nodes $n$, e.g., $\tO(m) = m \log^{O(1)} n$. We use the term near-linear to mean $\tO(m)$.} Minor-Aggregations. 
A Minor-Aggregation computes an aggregate (e.g., max or sum) of node-values for every connected component of some subgraph.

\medskip


\noindent Our reduction immediately implies:
\begin{itemize}
    \item Optimal deterministic parallel (\pram) algorithms with $\tO(1)$ depth and near-linear work.
    \item Universally-optimal deterministic distributed (\congest) algorithms, whenever deterministic Minor-Aggregate algorithms exist. For example, an optimal $\tO(\hopDiameter{G})$-round deterministic \congest algorithm for excluded-minor networks.
\end{itemize}

\medskip

\noindent Several novel tools developed for the above results are interesting in their own right:

\begin{itemize}
    \item A local iterative approach for reducing shortest path computations ``up to distance $D$'' to computing low-diameter decompositions  ``up to distance $\frac{D}{2}$''. Compared to the recursive vertex-reduction approach of \cite{Li20}, our approach is simpler, suitable for distributed algorithms, and eliminates many derandomization barriers.
    \item A simple graph-based $\tO(1)$-competitive $\ell_1$-oblivious routing based on low-diameter decompositions that can be evaluated in near-linear work. The previous such routing~\cite{goranci2022universally} was $n^{o(1)}$-competitive and required $n^{o(1)}$ more work.   

    \item A deterministic algorithm to round any fractional single-source transshipment flow into an integral tree solution. 

    \item The first distributed algorithms for computing Eulerian orientations. 
\end{itemize}

\smallskip


\end{abstract}






==> algorithm-main.tex <==

\section{SSSP via Minor-Aggregations: A Local Iterative Reduction Cycle}
\label{sec:localiterative}



In \cref{sec:intro} and \cref{fig:main}, we gave an idealized and informal description of our algorithm.
The real set of reductions our algorithm is built on is not quite the perfect cycle from \cref{fig:main}, but instead it looks like \cref{fig:oracles}. 
In \cref{sec:key_definitions}, we give a formal definition for each part of this new ``cycle'' and explain how the parts of the new cycle correspond to parts in the old cycle. 
Once we have defined each part of the new cycle, each arrow in \cref{fig:oracles} corresponds to a formal statement.
These formal statements can be found in \cref{sec:implications_cycle}, along with informal explanations how the statements can be proven. \\
Finally, \cref{sec:main_theorems} contains statements of our main theorems together with simple proof sketches.
The formal proofs for all the results stated in \cref{sec:implications_cycle} and \cref{sec:main_theorems} can be found in \cref{sec:missingProofs}.


\begin{figure}[ht]
    \centering
    \includegraphics[width = \textwidth]{fig/oracles.eps}
    \caption{The figure illustrates a single iteration of our local iterative reduction cycle. At the beginning of the cycle, the algorithm has already computed a distance structure for every scale $D_j$ with $D_j < D_i$. After completion of the cycle, the algorithm has computed a distance structure for scale $D_i$, under the assumption that it has access to the rounding oracle $\oRound$ (or the \euler oracle $\oEuler$). \cref{lem:cycleone} states this result formally.
    Moreover, each arrow in the cycle corresponds to a formal statement of the following form: Given $A$ (and $B$), then one can efficiently (in $\tilde{O}(1)$ \aggregate rounds) compute $C$. }
    \label{fig:oracles}
\end{figure}

\subsection{Key Definitions and Oracles}
\label{sec:key_definitions}

The definition of the oblivious routing oracle $\oObliv_{D_i}$ relies on the definition of the graph $G_{S,D}$ and the definition of distance scales.

We start with the definition of the graph $G_{S,D}$.

\begin{definition}[Graph $G_{S,D}$]
Let $S \subseteq V$ and $D \in [\poly(n)]$. We construct the graph $G_{S,D}=(V \cup \{\vD,\sstar\}, E \cup \{\{\vD,u\} \mid u \in V\} \cup \{\{\sstar,u\} \mid u \in S\})$ by adding two additional nodes $\vD$ and $\sstar$ to $G$. The node $\vD$ is connected to each node in $V$ and the node $\sstar$ is connected to all the nodes in $S$, with all the new edges having a weight of $D$. Moreover, we denote with $G_S$ the unweighted graph one obtains by discarding the edge weights in the weighted graph $G_{S,D}$.
\end{definition}

Informally speaking, $G_{S,D}$ preserves distance information only up to distance $2D$. More formally, any shortest path between two nodes in $G$ remains a shortest path in $G_{S,D}$ if this path is of length at most $2D$. Shortest paths in $G$ longer than $2D$, on the other hand, are not preserved in $G_{S,D}$, since any two nodes in $G_{S,D}$ have a shortest path of length $2D$ via $\vD$.
Moreover, consider a shortest path tree from vertex $\sstar$ up to distance $2D$. If one removes $\sstar$ and $\vD$ from this tree, then the resulting forest is a shortest path forest in $G$ from set $S$ up to distance $D$. 

We next give the definition of distance scales, along with defining global parameters which are used throughout the paper.
\begin{definition}[Distance Scales]\label{def:distance_scales}
We set $\valSNC = \log^7(n)$, $\beta = 8\valSNC$ and $D_i = \beta^i$. 


A distance scale is a value contained in the set $\{D_i \colon i \in \mathbb{N}, D_i \leq n^2 \max_{e \in E} \ell(e)\}$.
In particular, if we denote with $i_{max}$ the largest integer $i$ for which $D_{i}$ is a distance scale, then $D_{i_{max}} \geq \diam(G)$.
\end{definition}

We are finally ready to formally define oracle $\oObliv_{D_i}$, the $\ell_1$-Oblivious Routing Oracle for scale $D_i$. It corresponds to computing an ``$\ell_1$-oblivious routing up to distance $D_i$'' in \cref{fig:main}.

\begin{restatable}[$\ell_1$-Oblivious Routing Oracle for scale $D_i$ --- $\oObliv_{D_i}$]{definition}{oblivousroutingoracle}
\label{def:oracle_oblivousrouting}
The $\ell_1$-Oblivious Routing Oracle for scale $D_i$, $\oObliv_{D_i}$, takes as input a set $S \subseteq V$ as well as a demand $b$ and a flow $f$ for $G_{S,D_i}$. It outputs $R_S b$ and $R_S^T f$ for a fixed $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing $R_S$ for $G_{S,D_i}$.
\end{restatable}

Next, we give the formal definition of the forest oracle $\oDist_{\eps,D}$.


\begin{restatable}[$(1+\eps)$-Approximate Forest for distance $D$ rooted at $S$ / Forest Oracle --- $\oDist_{\eps,D}$]{definition}{distanceoracle}\label{def:oracle_dist}
The forest oracle $\oDist_{\eps,D}$ takes as input a node set $S \subseteq V$.
The output is a $(1+\eps)$-approximate forest for distance $D$ rooted at $S$, which is a forest $F$ rooted at $S$ such that the following holds.
\begin{enumerate}
    \item For every $u \in V(G)$ with $\dist_G(S,u) \le D$ we have $u \in V(F)$.
    \item For every $u \in V(F)$, $\dist_F(S,u) \le (1+\eps)D$. 
\end{enumerate}
\end{restatable}

For a given distance scale $D_i$, having access to $\oDist_{\frac{1}{\log^3(n)},D}$ for every $D \in \left[ \frac{D_i}{\valSNC}, D_i\right]$ corresponds to ``$(1+\eps)$ set-shortest path up to distance $D_i$'' in \cref{fig:main}.


The notion of ``$(1+\eps)$ transshipment up to distance $D$'' in \cref{fig:main} does not have a direct correspondence in \cref{fig:oracles}.
However, the potential oracle $\oPot_{D_i}$ outputs a potential capturing a certain version of (dual) transshipment potentials. 
%We don't make this notion precise. \todo{V: rephrase}
The oracle $\oPot_{D_i}$ is defined as follows:

\begin{definition}[Potential for scale $D_i$ with respect to set $S$ / Potential Oracle --- $\oPot_{D_i}$] \label{def:potential}
The potential oracle $\oPot_{D_i}$ takes as input a node set $S \subseteq V$.
The output is a potential $\phi_{S, D_i} \in \R^{V(G_{S, D_i})}$ for scale $D_i$ with respect to $S$.
A potential for scale $D_i$ with respect to a set $S \subseteq V$ is a non-negative potential $\phi_{S,D_i}$ (satisfying the conditions given in \Cref{sec:preliminaries}) such that:
\begin{enumerate}
    \item $\forall v \in S:\ \phi_{S,D_i}(v) = 0$ and
    \item $\dist_G(v,S) \geq \frac{D_i}{\valSNC}$ implies $\phi_{S,D_i}(v) \geq 0.5\frac{D_i}{\valSNC}$.
\end{enumerate} 
\end{definition}


We next give the definition of a distance structure for scale $D_i$.
\begin{definition}[Distance Structure for scale $D_i$]
\label{def:distance_structure}
A distance-structure for scale $D_i$
consists of a sparse neighborhood cover with covering radius $\frac{D_i}{\valSNC}$. Moreover, each cluster $C$ in one of the clusterings comes with 
\begin{enumerate}
    \item a tree $T_C$ of diameter at most $D_i$ which spans $C$ and is rooted at some node $v_C \in C$. We refer to $v_C$ as the cluster center.
    \item A potential for scale $D_i$ with respect to $V \setminus C$ (known to nodes in $C$). \alert{we never defined what potentials with respect to a subset means.. also, with respect to which weighted graph is this? (I suppose $G_{D_i}$ or something.. but this is important to say?}
\end{enumerate}
\end{definition}

\alert{also, I think that the dist structure potentials are quite hard to parse for non-authors of this paper .. we should explain that this potentials with respect to the outside of the cluster actually means we want to know the distance to the boundary, but we are happy with an approximate distance that satisfies the potential smoothness properties or whatever.}

In \cref{fig:main}, ``distance structures up to distance $D$'' correspond to having a distance structure for every scale $D_j$ with $D_j \leq D$.

In \cref{sec:intro} we outlined the problem of rounding a transshipment flow, and that rounding can be deterministically reduced to solving $\tilde{O}(1)$ \euler problems. 
We now define the oracles for the two problems.

The rounding oracle is defined as follows. \alert{in sec 5 we actually give an implementation for a perfect $\eps = 0$ rounding oracle .. Christoph explained that this is to future-proof the proof as someone might come up with a (distributed) rounding faster algorithm in the future. However, without any explanation here this is extremely confusing (at least to me). Can we please add a explanation why we state it in this form.}

\begin{restatable}[Rounding Oracle --- $\oRound_{\eps}$]{definition}{roundingoracle}
\label{def:oracle_rounding}
The Rounding Oracle $\oRound_{\eps}$ takes as input a weighted graph $H$ with length function $\ell_H$ and a flow $f$ on $H$. The weighted graph $H$ needs to be a subgraph of some graph $H'$ that one can obtain from $G$ by adding up to $\tilde{O}(1)$ virtual nodes and adding edges of arbitrary nonnegative length incident to the virtual nodes. The flow $f$ needs to satisfy the following condition. Let $b$ be the demand that $f$ routes. Then, $b(v) \geq 0$ for all $v \in V(H)$ except for some $s \in V(H)$ called the source. 
The output is a rooted tree $T$ with root $s$ spanning all vertices of $H$ with non-zero demand such that $\sum_{v:b(v) \neq 0}b(v)\dist_T(s,v) \le (1+\eps')\ell_H(f)$ with $\eps' = \min \left( \eps,\frac{1}{20\log^3(n)\valSNC} \right)$. 
\end{restatable} 

Note that $\oRound_{\eps}$ takes as input a weighted graph that can have more vertices than $G$. This allows us to use $\oRound_{\eps}$ to round a transshipment flow defined on the graph $G_{S,D}$. 
Moreover, we sometimes just write $\oRound$, without a precision parameter $\eps$, which we define as $\oRound = \oRound_1 = \oRound_{\frac{1}{20\log^3(n)\valSNC}}$.

The \euler oracle is defined next. 

\begin{restatable}[\euler Oracle --- $\oEuler$]{definition}{euleroracle}
\label{def:oracle_euler}
The \euler oracle $\oEuler$ takes as input a Eulerian graph $H$. The graph $H$ has to be a subgraph of some graph $H'$ that one can obtain from $G$ by adding up to $\tilde{O}(1)$ virtual nodes and adding any edges incident to the virtual nodes.
The output is an orientation of the edges of $H$ such that the in-degree of every node is equal to its out-degree.
\end{restatable}







\subsection{Formal Statements Corresponding to \cref{fig:oracles}}
\label{sec:implications_cycle}

For the sake of this section, we say that we can solve a problem or compute a structure \emph{efficiently} if there exists a \aggregate algorithm for the task that runs in $\tilde{O}(1)$ rounds. 

In this subsection, we give one formal statement for each arrow in \cref{fig:oracles}, as promised at the beginning of \cref{sec:localiterative}.
Before that, we state a result which captures the main essence of our local iterative reduction cycle. 

\begin{restatable}[Main Lemma]{lemma}{cycleone}
\label{lem:cycleone}
Assume a distance structure for every scale $D_j$ smaller than scale $D_i$ and oracle $\oRound$ are given. A distance structure for scale $D_i$ can be efficiently computed.
\end{restatable}

\cref{lem:cycleone} is a simple corollary of the next four lemmas. The formal proof can be found in \cref{sec:missingProofs}.



\begin{restatable}{lemma}{cycletwo}
\label{lem:cycletwo}
Assume a distance structure for every scale $D_j$ smaller than scale $D_i$ is given. Then, $\oObliv_{D_i}$ can be efficiently computed. 
\end{restatable}
\cref{lem:cycletwo} follows from a simple adaption of our $\tO(1)$-competitive $\ell_1$-oblivious routing construction, explained in \cref{sec:l1-oblivious-routing}.

\begin{restatable}{lemma}{cyclethree}
\label{lem:cyclethree}
Assume oracle $\oRound$ and $\oObliv_{D_i}$ are given. Then, $\oPot_{D_i}$ and $\oDist_{\frac{1}{\log^3(n)},D}$ can be efficiently computed for every $D \in \left[ \frac{D_i}{\valSNC},D_i \right]$.
\end{restatable}
\cref{lem:cyclethree} follows mainly from previous work. More precisely, having access to a $\tO(1)$-competitive $\ell_1$-oblivious routing in $G_{S,D_i}$, we can compute the following two objects via boosting and rounding \cite{She17, BKKL17, Li20, goranci2022universally}. First, a $(1+\eps)$-SSSP-tree in $G_{S,D_i}$ rooted at $\sstar$. Second, an individually good $(1+\eps)$-approximate potential in $G_{S,D_i}$ for the single-source transshipment demand with source $\sstar$. 
For completeness, we give a summary of these steps in the proof of \cref{theorem:boosting_rounding}.

If one looks at what the aforementioned tree and potential in $G_{S,D_i}$ correspond to in the graph $G$, then one can relatively straightforwardly transform them to obtain a $\left(1+\frac{1}{\log^3 n}\right)$-approximate forest for $D$ rooted at $S$ and a potential for scale $D_i$ with respect to $S$, assuming $\eps = \frac{1}{\poly(\log n)}$ is sufficiently small.
The details of this transformation can be found in the proof of \cref{lem:cyclethree} in \cref{sec:missingProofs}.


\begin{restatable}{lemma}{cyclefour}
\label{lem:cyclefour}
Assume oracle $\oDist_{\frac{1}{\log^3(n)},D}$ is given for every $D \in \left[ \frac{D_i}{\valSNC},D_i \right]$. Then, a sparse neighborhood cover with covering radius $\frac{D_i}{\valSNC}$ together with a rooted spanning tree $T_C$ of diameter at most $D_i$ for every cluster $C$ in the cover can be computed efficiently.
\end{restatable}

\cref{lem:cyclefour} directly follows from \cite[Theorem C.4]{elkin2022decompositions}, which is proven by adapting the algorithms of \cite{rozhon_ghaffari2019decomposition,chang_ghaffari2021strong_diameter} for the closely-related network decomposition problem. 

%As a last step we want to use $\oPot$ and $\oDist$ to compute a distance structure for the next scale. For this we first use $\oDist$ to compute a sparse neighborhood cover and then use $\oPot$ and $\oDist$ to compute the distance information for each cluster, i.e., the tree and the potential. These two steps are formally given next:



\begin{restatable}{lemma}{cyclefive}
\label{lem:cyclefive}
Assume we are given an oracle $\oPot_{D_i}$ and a sparse neighborhood cover with covering radius $\frac{D_i}{\valSNC}$ together with a rooted spanning tree $T_C$ of diameter at most $D_i$ for every cluster $C$ in the cover. 
Then, a distance structure for scale $D_i$ can be computed efficiently.
\end{restatable}

Given a sparse neighborhood cover together with a tree for each cluster, it only remains to compute the potential for scale $D_i$ with respect to $V \setminus C$ for each cluster $C$ in the sparse neighborhood cover. 
One can compute the potentials for all the clusters in a given clustering $\fC$ simultaneously. The simplest approach for computing these potentials is to compute a single potential for scale $D_i$ with respect to all the nodes that are neighboring one of the clusters in $\fC$. This approach works as long as there does not exist a node that is both clustered and neighboring a different cluster. Even though this can indeed happen, there is a simple solution that solves this problem. The details can be found in the proof of \cref{lem:cyclefive} in \cref{sec:missingProofs}. 

\alert{this lemma is never proven, what is proven is a (differently stated and more precise) Theorem 5.1.. we should probably replace this lemma with that theorem.}
\begin{restatable}{lemma}{cycleeuler}
\label{lem:cycleeuler}
Assume the oracle $\oEuler$ is given. Then, $\oRound$ can be efficiently computed. 
\end{restatable}
The main ideas to prove this lemma were already discussed in the introduction.
The details can be found in \cref{sec:rounding}.

\subsection{Main Theorems}
\label{sec:main_theorems}

In this part, we state the main theorems of this paper. 

First of all, a simple induction proof on top of \cref{lem:cycleone} leads to the following result.

\begin{restatable}{lemma}{cyclesix}
\label{lem:cyclesix}
Assume oracle $\oRound$ is given. Then, a distance structure for every scale $D_i$ can be efficiently computed.
\end{restatable}

Note that for $i = 1$, \cref{lem:cycleone} states that given access to $\oRound$, one can efficiently compute a distance structure for scale $D_1$.
The complete induction proof can be found in \cref{sec:missingProofs}.


Given access to a distance structure for every scale $D_i$, the theorem below follows directly from our $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing scheme described in \cref{sec:l1-oblivious-routing}.

\begin{restatable}[Distance Structures give $\ell_1$-Oblivious Routing]{theorem}{cycleseven}
\label{theorem:cycleseven}
Assume a distance structure for every scale $D_i$ is given. Then, there exists a $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing $R$ for $G$ for which $R$ and $R^T$ can be efficiently evaluated.
\end{restatable}




As discussed in \Cref{sec:intro}, $\ell_1$-oblivious routing and rounding is sufficient to solve the $(1+\eps)$-SSSP tree and the $(1+\eps)$-transshipment problems~\cite{She17, BKKL17,Li20,goranci2022universally}.

\begin{restatable}[$\ell_1$-Oblivious Routing gives SSSP and transshipment]{theorem}{cycleeight}
\label{theorem:cycleeight}
Assume oracle $\oRound_{\eps/2}$ is given for some $\eps \in (0,1]$ and that there exists an efficient algorithm to evaluate $R$ and $R^T$ for some $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing $R$ for $G$. Then, the $(1+\eps)$-transshipment problem and the $(1+\eps)$-SSSP-tree problem in $G$ can be solved in $\tilde{O}(1/\eps^2)$ \aggregate rounds. 
\end{restatable}


Combining \cref{lem:cyclesix}, \cref{theorem:cycleseven} and \cref{theorem:cycleeight} results in the following theorem.

\begin{restatable}{theorem}{cyclenine}
\label{theorem:cyclenine}
Assume oracle $\oRound_{\eps/2}$ is given for some $\eps \in (0,1]$. The $(1+\eps)$-transshipment problem and the $(1+\eps)$-SSSP-tree problem in $G$ can be solved in $\tilde{O}(1/\eps^2)$ \aggregate rounds.
\end{restatable}

The theorem above together with the fact that $\oRound$ can be efficiently implemented given $\oEuler$ implies the following result.

\begin{restatable}{theorem}{cycleten}
\label{theorem:cycleten}
Assume oracle $\oEuler$ is given and let $\eps \in (0,1]$. The $(1+\eps)$-transshipment problem and the $(1+\eps)$-SSSP-tree problem in $G$ can be solved in $\tilde{O}(1/\eps^2)$ \aggregate rounds.
\end{restatable}

The \euler problem can be solved with near-linear work and polylogarithmic depth \cite{atallah_vishkin1984euler_pram}. Together with the theorem above and the fact that each $\aggregate$ round can be simulated with near-linear work and polylogarithmic depth, we obtain our main parallel result.

\mainparallel*

Moreover, our \congest algorithms for the \euler problem developed in \cref{sec:euler} together with general simulation results for the \congest model developed in prior work (see \cref{thm:compilation_pa_congest}), we obtain our main result in the \congest model.

\maindistributed*

We finish this section by stating the conditional results on universally-optimal SSSP and transshipment algorithms one can obtain from this work:


\begin{theorem} \label{lem:universalOptreduction1}
Suppose there exists a deterministic algorithm for partwise aggregation that runs in $\shortcutQuality{G} \cdot n^{o(1)}$ \congest rounds, then there exist deterministic $(1+\eps)$-SSSP and $(1+\eps)$-transshipment algorithms with a round complexity of $\shortcutQuality{G}) \cdot n^{o(1)}$, which is universally-optimal up to a $n^{o(1)}$-factor. 
\end{theorem}

We get even stronger conditional results if more efficient \congest algorithms for computing cycle covers as defined in \cite{parter_yogev2019cycle_decomp_near_linear,parter_yogev2019cycle_covers_minor_closed} are given. 

\begin{theorem}\label{lem:universalOptreduction2}
Suppose there exists a deterministic algorithm for partwise aggregation that runs in $\tO(\shortcutQuality{G})$ \congest rounds and a $(\tO(1),\tO(1))$ cycle cover algorithm for $\tO(1)$-diameter graphs which runs in $\tO(1)$ \congest rounds. Then, there exist deterministic $(1+\eps)$-SSSP and $(1+\eps)$-transshipment algorithms with a round complexity of $\tO(\shortcutQuality{G})$, which is universally-optimal up to polylogarithmic factors. 
\end{theorem}

While the polylogarithmically tight algorithmic results assumed in \Cref{lem:universalOptreduction2} seem out of reach of current techniques, our conditional results show that the problem-specific part towards universally optimal shortest path algorithms, even deterministic ones, are essentially fully understood through the techniques of this paper. 

\Cref{lem:universalOptreduction2} and \Cref{lem:universalOptreduction1} follow from \Cref{thm:main_distributed} in \cref{sec:missingProofs} which shows that to get the near-optimal round complexity of $\tO_{\eps}(\shortcutQuality{G})$ in \cref{thm:main_distributed}, it suffices to solve efficiently the Partwise-Aggregation problem (see \cref{sec:computational-models}) and implement efficiently the oracle $\oEuler$ which can be done by an efficient solution of the cycle cover problem (see \cref{sec:euler}). 




%\begin{remark}[Universally Optimal Algorithm?]
%We remark that the proof of \cref{thm:main_distributed} in \cref{sec:missingProofs} implies that to get the near-optimal round complexity of $\tO_{\eps}(\shortcutQuality{G})$ in \cref{thm:main_distributed}, it suffices to solve efficiently the Partwise-Aggregation problem (see \cref{sec:computational-models}) and implement efficiently the oracle $\oEuler$ which can be done by an efficient solution of the cycle cover problem (see \cref{sec:euler}). 
%\end{remark}






% Local Variables:
% TeX-master: "main"
% End:


==> euler.tex <==
\section{Distributed Algorithms for the Eulerian-Orientation Problem}
\label{sec:euler}

In this section, we show how to construct the \euler oracle $\oEuler$. 
Instead of talking about oracles, we talk about solving the \euler problem, in which we are asked to orient each edge such that each node has the same indegree and outdegree. 
The main result of the section is the following theorem. 

\begin{restatable}{theorem}{thmeuler}
\label{thm:euler_dist}
There are deterministic algorithms for the \euler problem (that is, implementing the oracle $\oEuler$) with the following round complexities. 
\begin{enumerate}
    \item $\tO(\hopDiameter{G})$ \congest rounds if $G$ comes from a fixed minor-free family. 
    \item $n^{o(1)}$ \congestPA rounds. 
    \item $\tO(\sqrt{n} + \hopDiameter{G})$ \congest rounds. 
\end{enumerate}
\end{restatable}


There is a simple deterministic parallel algorithm for the \euler problem with near-linear work and polylogarithmic depth \cite{atallah_vishkin1984euler_pram}. 
The algorithm starts by pairing up all edges at every node of $H$. This splits $E(H)$ into a set of closed walks. In the following $O(\log |E(H)|)$ rounds, edges of the same closed walk are collected and the whole walk is consistently oriented. 
This ensures the equal indegree and outdegree at each node of $H$. 

\begin{theorem}[\cite{atallah_vishkin1984euler_pram}]
\label{thm:euler_pram}
There is a deterministic $O(\log n)$ depth and $O(m \log n)$ work algorithm for the \euler problem on CRCW \pram.  
\end{theorem}

However, to the best of our knowledge there are no non-trivial distributed algorithms known for the Eulerian-Orientation problem. 
Here we provide a fast distributed algorithms using the Low Congestion Cycle Covers of \cite{parter_yogev2019cycle_covers_minor_closed,parter_yogev2019cycle_decomp_near_linear,hitron_parter2021adversarial_compilers}. 
First, we prove several preparatory lemmas in \cref{sec:eulerTechnical} and postpone the proof of \cref{thm:euler_dist} in \cref{sec:eulerMain}. 



\subsection{Technical Preparations}
\label{sec:eulerTechnical}

First, we prepare several necessary tools. We start by proving that if we contract degree two nodes in a graph, in the contracted graph we can simulate \congestPA rounds. 

\begin{lemma}
\label{lem:simulation_contraction}
Let $G$ be a graph and $G'$ be a graph we get by contracting every node of degree $2$ in $G$. 
Then we can simulate one \congestPA round in $G'$ in $O(1)$ \congestPA rounds in $G$. 

Moreover, if each edge $e \in E(G')$ is arbitrarily oriented, we can consistently orient the whole path in $G$ contracting to $e$ in that direction in $O(\log n)$ \congestPA rounds. 
\end{lemma}
\begin{proof}
To simulate one \congest round in $G'$, we first use one \congest round in $G$ to send the message along edges that remain the same in $G$ and $G'$. 
Moreover, for each path $u_1, u_2, \dots, u_k$ in $G$ that contracts to an edge $e$ in $G'$, we let $u_1$ send the message meant to $u_k$ to its neighbor $u_2$. 
The path $u_2, u_3, \dots, u_{k-1}$ is node-disjoint from all other contracted paths, hence the message to $u_k$ can be sent to $u_{k-1}$ with one call to the partwise aggregation oracle. In one final \congest round the message is delivered to $u_k$. 

The simulation of the partwise aggregation oracle in $G'$ is implemented analogously: each edge in $G'$ connecting two nodes of the same part is expanded to a full path. The new set of parts of $G$ is still node-disjoint. We then use the partwise aggregation oracle of $G$

The final claim is proven by building a tree of constant degree and radius $O(\log n)$ on top of each path, in $O(\log n)$ \congestPA rounds. 
The tree is then used to propagate an information about the orientation of the path to all nodes, in $O(\log n)$ \congestPA rounds. We omit details as they are standard and essentially the same as in the proof of \cref{euler:lem:sqrt}. 
\end{proof}

\paragraph{Dealing with virtual nodes}
Next, we discuss how to handle virtual nodes. See \cref{subsec:minor_aggregation} for the definitions related to virtual nodes. In what follows, we assume that the input graph $G$ may contain $\tO(1)$ virtual nodes and show how one can reduce this case to the case without any virtual nodes. 






\begin{lemma}[Variant of Lemma 4.3.2 in \cite{peleg2000distributed}]
\label{euler:lem:matching}
Let $T \subseteq G$ be a rooted tree of $G$ and $S$ a set of \emph{marked} nodes. 
Then, in $\tO(1)$ \congestPA rounds, we can output a set of paths $P= \{p_1, p_2, \dots, p_{\lfloor S/2 \rfloor}\}$ such that
\begin{enumerate}
    \item Each path $p \in P$ satisfies $p \subseteq T$. 
    \item All nodes of $S$, except of possibly one, are endpoints of exactly one $p \in P$. 
    \item Any two $p_1, p_2 \in P$ are edge-disjoint. 
    \item We can implement partwise aggregation on $P$ in $O(1)$ \congestPA rounds of $G$. 
\end{enumerate}

%Then, in $O(\hopDiameter{G})$ \congest rounds, we can output a matching $M = \{ \{s_1, t_1\}, \dots, \{s_{\lfloor S/2 \rfloor}, t_{\lfloor S/2 \rfloor}\} \}$, where for each $1 \le i \le \lfloor S/2 \rfloor$, $s_i, t_i \in S$. 

%Moreover, for each $\{s_i, t_i\}$, we return a subpath $P_i$ of $T$  with the following property. 
%Let $u_i$ be the node of $P_i$ closest to the root $r$ of $T$ and we write $P_i = P_i^1 \circ \{u_i\} \circ P_i^2$, that is, we write $P_i$ as a concatenation of a path from $s_i$ to a node below $u_i$, next a trivial path $\{u_i\}$, and a path from a node below $u_i$ to $t_i$. 
%Then, all sets $\{P_1^1, P_1^2, P_2^1, P_2^2, \dots, P_{\lfloor S/2 \rfloor}^1, P_{\lfloor S/2 \rfloor}^2\}$ are node-disjoint. 
\end{lemma}
\begin{proof}
We first describe how we build the set $P$ of paths. 
For each $u \in V(T)$, let $x_u = 1$ if $u\in S$ and $x_u = 0$ otherwise. We use \cref{lemma:ancestor-subtree-sum} to compute $s_u = \sum_{v \in T_u} x_v$ for every $u$, where $T_u$ is the subtree of $u$ in $T$. 
If $s_u$ is odd, $u$ will be connected in a path with its parent $\parent(u)$ (unless $u$ is the root) and sends this information to $\parent(u)$. Next, each node $u$ collects messages from all its children nodes to know which of them will be in the same path as $u$. The node $u$ arbitrarily pairs up these proposals into paths (for each such created path, $u$ is the node in it closest to the root). 
By construction, there is a leftover, unpaired, proposal if and only if $u$ itself proposed and $u \not\in S$ (unless $u$ is a root). 
In this case, the leftover unpaired child of $u$ is combined with $u$ in the same path. 
Otherwise, if $u\in S$ and children of $u$ are paired up, $u$ is the endpoint of a new path that continues to $\parent(u)$. 
This local algorithm defines the set of paths $P$. 
The only reason why $P$ not necessarily satisfies properties 1,2,3 from the lemma statement is that if $|S|$ is odd, $P$ contains an additional path from a vertex in $S$ to the root of $T$. Next, we describe how to implement any  partwise aggregation  on $P$ and this allows us to remove this additional path from $P$ so that it satisfies all three desired properties.  

To prove property 4, let $p_i \in P$ be any path and let us write $p_i = r_i, \dots, s_i^-, s_i, s_i^+, \dots, t_i$, where $s_i$ is the node on $p_i$ closest to the root of $T$. 
Consider any two paths $P_i,P_j$ and let $v \in P_i \cap P_j$. We know that the edge from $v$ to its parent can be present in at most one of the paths $P_i,P_j$ as they are edge-disjoint, hence $v \in \{s_i, s_j\}$. That is, if two paths $P_i, P_j$ intersect in a node, the node is the ``top'' node of one of them. 
Hence, to implement a  partwise aggregation on $P$, we compute the operation on the parts $\{\{r_i, \dots, s_i^-\}, \{s_i^+, \dots, t_i\}\}_{1 \le i \le {\lfloor S/2 \rfloor}}$ that are node-disjoint and use additional $O(1)$ \congest rounds to extend the operation to the set of full paths. 
\end{proof}

\begin{proposition}
\label{euler:prop:get_rid_of_virtual_edges}
Given an input $H$ to the \euler problem with $k = \tO(1)$ virtual nodes, there is a deterministic distributed algorithm that orients some subgraph $I \subseteq H$ such that 
\begin{enumerate}
    \item All edges incident to virtual nodes are in $I$. 
    \item Each node has the same indegree and outdegree in $I$. In particular, the residual graph $H \setminus I$ is still Eulerian. 
\end{enumerate}
The algorithm needs $\tO(1)$ \congestPA rounds. 
\end{proposition}

First, we sketch how to prove the above proposition if there is just one virtual node. 
We then proceed with the more difficult (but still routine) proof for multiple virtual nodes. 

To prove \cref{euler:prop:get_rid_of_virtual_edges} with $k = 1$, we start by finding any spanning forest $F$ of $H$ in $\tO(1)$ \congestPA rounds using the distributed MST algorithm \cite{kutten1998fast}. 
Next, we use \cref{euler:lem:matching} with $S$ being the neighborhood of the virtual node $u$. As the size of the neighbourhood of $u$ in any component of $F$ is even, we pair all of its nodes. 
Note that each constructed path closes a cycle together with the two appropriate virtual edges to $u$. We can use the fact that we can aggregate information on these paths (property 4 in \cref{euler:lem:matching}) to consistently orient the graph $I$ formed by these cycles, which proves the proposition in case $k = 1$. 
We now continue with the proof for $k = \tO(1)$. 

\begin{proof}
The first part of the algorithm consists of $k$ steps. 
During the $i$-th step we orient some of the virtual edges incident to $u_i$ as well as some non-virtual edges. We maintain a residual graph $H_i$ of not yet oriented edges at the beginning of the $i$-th phase. 

More precisely, at the beginning of the $i$-th phase we compute a spanning forest of $H_i[V(G)]$ (that is, we consider only the graph of non-virtual nodes and edges of $H_i$) by an MST algorithm. Next, in each connected component of $H_i[V(G)]$ we use, in parallel,  \cref{euler:lem:matching} to match nodes neighboring with $u_i$. At most one node is unmatched in each connected component of $H_i$. 
Each path $p$ in the set of matching paths closes a cycle together with the two virtual edges connecting the endpoints of $p$ with $u_i$. We can orient this cycle consistently in $\tO(1)$ \congestPA rounds using property (4) in \cref{euler:lem:matching}. This leaves us with a new residual graph $H_{i+1}$ such that $H_{i+1}[V(G)]$ has possibly more connected components but it still retains the property that each connected component of $H_{i+1}[V(G)]$ is incident to at most one edge from $u_i$. 
Hence, after $k$ phases, we are left with a residual graph $H' = H_{k+1}$ such that each connected component of $H'[V(G)]$ contains at most $k$ edges to virtual nodes. Moreover, the number of these incident virtual edges is even. 

In the second part of the algorithm, we use \cref{euler:lem:matching} on the spanning forest of $H'[V(G)]$ again, but this time every node incident to $\{u_1, \dots, u_k\}$ is in the set $S$. The lemma yields a set of edge-disjoint paths such that each path $p$ between two nodes $s$ and $t$, incident to $u_i$ and $u_j$, respectively, connects $u_i$ with $u_j$). 
For each such path, we replace the two virtual edges $\{u_i,s\}, \{u_j, t\}$ with a new virtual edge $\{u_i,u_j\}$, to create a new graph $H''$. After the replacement, there are no connections between the virtual and nonvirtual nodes, hence $H''$ satisfies that $H''[\{u_1, \dots, u_k\}]$ is an Eulerian graph. 
All nodes of $G$ now learn the graph $H''[\{u_1, \dots, u_k\}]$ in $O(k^2) = \tO(1)$ \congestPA rounds and all nodes of $G$ compute internally the same Eulerian orientation of it. 
Finally, we will uncontract each contracted edge $(u_i, u_j)$ of $H''[\{u_1, \dots, u_k\}]$ into the original path and orient the respective path $(u_i, s), p, (t, u_j)$ in the same direction as how the edge $(u_i, u_j)$ was oriented. 
More concretely, for every multi-edge $\{u_i, u_j\} \in E(H''[\{u_1\dots, u_k\}])$, we know two numbers $a_{ij}$ and $b_{ij}$ such that $a_{ij}$ paths contracted to an edge $\{u_i, u_j\}$ need to be oriented from $u_i$ to $u_j$ and $b_{ij}$ paths need to be oriented from $u_j$ to $u_i$. If each path $p$ retains a unique identifier, using binary search, in $\tO(1)$ \congestPA rounds we can decide that $a_{ij}$ paths connecting $u_i$ and $u_j$ with lower identifiers will be oriented from $u_i$ to $u_j$, and the rest in the opposite direction. 
Hence, in $\tO(1)$ \congestPA rounds, we can extend the Eulerian orientation of $H''[\{u_1, \dots, u_k\}]$ to an Eulerian orientation of a subgraph of $H'$ that contains all virtual edges, as needed. 
\end{proof}


\begin{comment}
\begin{lemma}
\label{lem:simulation_virtual}
Let $G$ be a graph and $H$ an Eulerian graph which is, up to a set of $k = \tO(1)$ virtual nodes $u_1, u_2, \dots, u_k$ a subgraph of $G$. 
Then, in $\tO(1)$ \aggregate rounds we can construct an Eulerian multigraph $H'$ which is a subset of $G$, up to multiplicities and up to a set of virtual edges $e_1, \dots, e_\ell$ such that
\begin{enumerate}
        \item One \congest or one \aggregate round on $G \cup H'$ can be implemented in one \congest plus $\tO(1)$ \aggregate rounds on $G$. 
        \item A solution of \euler with $H'$ can be lifted to a solution of \euler on $H$ in additional $\tO(1)$ \aggregate rounds on $G$. 
\end{enumerate}
\end{lemma}
\begin{proof}
For each virtual node $u$ we do the following. 
Let $T$ be the BFS tree in $G$ from some arbitrary non-virtual root node $r$. We use \cref{lem:matching_peleg} with the set $S$ being the set of nodes neighboring to $u$. 
Next, for each pair of nodes $s_i, t_i$, we add a virtual edge $\{s_i, t_i\}$ to $H$ instead of the two virtual edges $\{s_i, u\}, \{t_i, u\}$. 
We do the same for every virtual node. 
Each virtual node retains at most one edge connecting it to non-virtual nodes. 
We broadcast the set of all such edges to all the nodes in $O(\hopDiameter{G})$ rounds. 
Then, internally, each node computes a consistent orientation of a maximal set of cycles consisting of only virtual nodes. The remaining edges incident with virtual nodes form $\tO(1)$ paths that are then contracted to additional virtual edges. 
This process defines a graph $H'$ such that $V(H')$ contains no virtual nodes. 
Moreover, a solution to \euler on $H'$ can be lifted to a solution on $H$ in $\tO(\hopDiameter{G})$ additional \congest rounds. 

We start by proving item (1) from the statement. 
To implement one \congest round on $G \cup H'$, each virtual edge $\{s,t\}$ is replaced by the appropriate path $P = P^1 \circ \{u\} \circ P^2$. 
A message from $s$ to $t$ is sent in $2$ \aggregate and $2$ \congest rounds as follows: first $s$ sends it to the other endpoint of $P^1$, then it is passed to $u$ that passes it to the endpoint of $P^2$ that sends it to $t$. Since for given virtual node $u$ all appropriate paths $P$ are node-disjoint by \cref{lem:matching_peleg}, we can implement all sending along all virtual edges of $H'$ in $\tO(1)$ \congest plus \aggregate rounds, as needed. 

Additionally, one \aggregate round on $G \cup H'$ can be implemented in $\tO(1)$ \aggregate rounds on $G$, since for each virtual edge inside some connected component $C$, we can put its appropriate path in $T$ to $C$. Then, if we started with node-disjoint components $C_1, \dots, C_k$, after the replacement of each virtual edge by a path we have that each node is in $\tO(1)$ different components by item (3). 
\end{proof}
\end{comment}

\begin{comment}

\begin{definition}[Subdivided graph $\tG$]
Let $\tG$ be a graph such that $V(\tG) = \{ (u,e) | u \in e\}$. That is, the nodes of $\tG$ are the \emph{half-edges} in $G$. 
For each $e = \{u,v\} \in E(G)$, $\tG$ contains an edge between $(u,e)$ and $(v,e)$ and for every node $u \in V(G)$ such that $u$ is contained in edges $e_1, e_2, \dots, e_{\deg(u)}$, for every $1\le i < j \le \deg(u)$, $\tG$ contains an edge between $(u,e_i)$ and $(u,e_j)$. 
\end{definition}
Note that one round of communication in $\tG$ can be implemented in one communication round in $G$: each node $u \in V(G)$ will take care of all nodes $(u,e) \in V(\tG)$. 
Also, $\hopDiameter{G}(\tG) = O(\hopDiameter{G}(G))$. 
\end{comment}


\paragraph{Weaker Result} We now give an algorithm for the \euler problem with weaker than desired propeties. It will be used in the proof of \cref{thm:euler_dist}. 

\begin{lemma}
\label{euler:lem:sqrt}
There is a distributed algorithm that solves the \euler problem in $\tilde{O}(\sqrt{|E(G)|} + \hopDiameter{G})$ rounds. 
\end{lemma}
\begin{proof}
We assume the input Eulerian graph $H$ does not contain any virtual nodes, as we can deal with them using \cref{euler:prop:get_rid_of_virtual_edges} and \cref{thm:compilation_pa_congest} in $\tO(\sqrt{n} + \hopDiameter{G})$ \congest rounds. 
%First we deal with virtual nodes $u_1, u_2, \dots, u_k$, analogously to \cref{lem:simulation_virtual}. For each virtual node $u_i$, we find a collection $\fP_i$ of edge-disjoint paths of total length at most $n-1$, each of length at most $\hopDiameter{G}$, that pairs up non-virtual nodes incident to $u_i$. 
%We add all edges from $\fP_i, 1 \le i \le k$ to the graph $H$ and forget virtual nodes and edges incident to it. This creates a multigraph $H$ which is, up to multiplicities of edges which are bounded by $\tO(1)$, a subgraph of $G$. We will now solve the \euler problem in $H$, with the additional restriction that for each path $p \in \fP_i$, all of its edges need to be oriented consistently in one of two possible directions. Then it is easy to see how to extend the solution to a solution in $H$ in additional $\tO(\hopDiameter{G})$ \congest rounds. 

Each node $u$ arbitrarily pairs up the edges of $H$ incident to it -- note that their number is even. 
Starting in any edge, the pairing defines a closed walk containing the edge. We will next orient each such walk consistently, which solves the \euler problem. 

To orient the walks, each one first elects a leader in $O(\log n)$ steps as follows. At first, we interpret each edge as a path of length $1$. 
Next, we concatenate these paths using our pairing into progressively longer paths, until all paths of the walk are glued together. 
In particular, consider the incidence graph of our paths, induced by our edge pairing, which is always a set of disjoint cycles. 
In each step we use Linial's deterministic algorithm to compute a $(3, 4)$-ruling set \cite{linial92LOCAL}. 
That means we mark some of the paths such that the marked paths are of distance at least $3$ in the incidence graph, while every path is of distance at most $4$ to a marked path. Next, each unmarked path is joined with the closest marked path, to form a longer path. 
There are always at least $3$ and at most $5$ paths forming a longer path, unless the whole walk is connected in this step. 
Hence, in $O(\log n)$ steps, all paths are connected. Each step needs $O(\log^* n)$ \congest rounds of communication in the incidence graph. To simulate one round in the incidence graph, we need to implement sending messages in parallel from one endpoint of a path to the other endpoint. To do that, each path remembers its length. If it is at most $\sqrt{|E(H)|}$, then it sends the message from its endpoint to the other one along its edges. If it is more than $\sqrt{|E(H)|}$, it broadcasts the message to the whole graph using the edges of $G$. 
As there are at most $\sqrt{|E(H)|}$ such paths, it is a standard fact that, with correct implementation, in $O(\hopDiameter{H} + \sqrt{|E(H)|})$ rounds all broadcasts finish. 
Hence, in $\tO(\hopDiameter{H} + \sqrt{|E(H)|}) = \tO(\hopDiameter{G} + \sqrt{|E(G)|})$ rounds each walk can elect a leader. The leader chooses an arbitrary orientation and, similarly to the election, this orientation is messaged to smaller and smaller paths, until after additional $O(\log n)$ steps, each implemented in $\tO(\hopDiameter{G} +\sqrt{|E(G)|})$ rounds, each edge knows it. 

\begin{comment}
In particular, for each walk $e_1, e_2, \dots, e_k$, with $e_i = \{u_i, v_i\}$ and $v_i = u_{i+1}$ for each $1\le i \le k-1$, we consider the corresponding cycle $(e_1, u_1), (e_1, v_1), (e_2, u_2), (e_2, v_2), \dots, (e_k, u_k), (e_k, v_k)$ in $\tG$. Node that since the original walks are edge-disjoint, the cycles in $\tG$ are node-disjoint. 
Hence, in $O(1)$-aggregation round the nodes in the cycle $C$ can elect a leader and compute the number of nodes in $C$. 
After that, in additional $O(\log n)$ \aggregate rounds, we can gradually split $C$ into exponentially smaller node-disjoint paths, such that in step $i$ we have $O(2^i)$ paths of length $O(n/2^i)$. 
At the beginning, we arbitrarily choose one of the two possible orientation of the $C$ and whenever a path $p$ is split into two paths $p_1, p_2$, $p$ tells the border nodes of $p_1, p_2$ how their edges should be oriented. This way we orient consistently all edges of each $C$ in parallel, in $O(\log n)$ \aggregate rounds on $\tG$.  
We can use the trivial shortcuts on $\tG$ to implement this algorithm in $\tO(\sqrt{|V(\tG)|} + D_{\tG}) = \tO(\sqrt{m} + \hopDiameter{G})$ \congest rounds in $G$. 
\end{comment}

\end{proof}

\begin{remark}
The above result seems to imply that the \euler problem can be solved in $\tO(1)$ part-wise aggregations. 
However, in each step, the parts where aggregation happens are only edge-disjoint and not node-disjoint. 
\end{remark}



\paragraph{Cycle Covers}

The concept of cycle covers was introduced in the line of work \cite{parter_yogev2019cycle_covers_minor_closed,parter_yogev2019cycle_decomp_near_linear,hitron_parter2021adversarial_compilers,hitron2021broadcast} for the unrelated reason of making distributed computations more resilient to edge-faults introduced by a Byzantine adversary. 

\begin{definition}[$(d, c)$-cycle cover]
A $(d,c)$ cycle cover of $G$ is a collection of cycles $\fC = \{C_1, \dots, C_k\}$ in $G$ such that
\begin{enumerate}
    \item Each non-bridge edge of $G$ is in at least one $C \in \fC$ and at most $c$ different cycles. 
    \item Each cycle $C$ contains at most $d$ edges. 
\end{enumerate}
\end{definition}


\begin{lemma}[A variant of Theorem 11 in \cite{parter_yogev2019cycle_decomp_near_linear}, see also Fact 12 and Observation 13 in \cite{hitron_parter2021adversarial_compilers}]
\label{lem:general_cycle_cover}
For every graph $G$ and $0 < \eps < 1$ there is a deterministic \congest algorithm that computes a $(d,c)$ cycle cover $\fC$ with $d = 2^{O(1/\eps)}\hopDiameter{G}$ and $c = O(n^\eps)$ within $O (2^{O(1/\eps)} \cdot n^{O(\eps)} \cdot \hopDiameter{G})$ rounds.  
\end{lemma}
\begin{proof}
In \cite{parter_yogev2019cycle_decomp_near_linear}, the authors prove above theorem, but use a randomized algorithm. % with a better round complexity $\tilde{O} (2^{1/\eps} \cdot n^{\eps} \cdot \hopDiameter{G})$. 
Their algorithm uses randomness in two places. First, it uses a randomized routing through a set of paths with maximum dilation $d$ and total congestion of any edge bounded by $c$ in $\tO(c+d)$ \congest rounds. However, we can use a simple deterministic $\tO(cd)$ routing instead. 
Second, their algorithm uses a randomized Luby's algorithm \cite{luby86,alon86lubys_algorithm} to compute an MIS in a certain graph $\hat{G}$ in $O(\log n)$ rounds, where each round of communication in $\hat{G}$ can be implemented in $O(cd)$ rounds. Instead of Luby's algorithm, we can use the deterministic MIS algorithm from \cite{censor2017derandomizing,ghaffari_grunau_rozhon2020improved_network_decomposition} that works in $\tO(1)$ \congest rounds. 
\end{proof}


\paragraph{Excluded Minor Graph Families}
We will use the following results on the forbidden minor graph families. 

\begin{lemma}[Theorem 3 in \cite{parter_yogev2019cycle_covers_minor_closed}]
\label{lem:minor_closed_cycle_covers}
For every minor-closed, 2-connected graph $G$, in $\tilde{O}(\hopDiameter{G})$ rounds of the \congest model, one can construct an $(\tilde{O}(\hopDiameter{G}), \tilde{O}(1))$ cycle cover $\fC$ in $\tO(\hopDiameter{G})$ rounds.  
%For every minor-closed graph $G$, in $\tilde{O}(\hopDiameter{G})$ deterministic rounds of the \congest model, one can construct an $(\tilde{O}(OPT(G)), \tilde{O}(1))$ cycle cover $\fC$ in $\tO(OPT(G))$ \congest rounds. 
%Here, $OPT(G) = max_{e \in E(G)} min_{\text{cycle } C, e \in C} |C|$. 
\end{lemma}

\begin{comment}
\begin{corollary}
\end{corollary}
\begin{proof}
Consider any edge $e = \{u,v\} \in E(G)$ and start BFS from the set $\{u,v\}$. After at most $\hopDiameter{G}$ rounds this BFS covers the whole graph $G$ and constructs two BFS trees $T_u$ and $T_v$ rooted at $u$ and $v$, respectively. Due to 2-connectivity of $G$, there is an edge $f$ connecting the two trees and this edge closes a cycle containing $e$ of size $O(\hopDiameter{G})$. 
\end{proof}
\end{comment}

\subsection{The Eulerian Orientation Algorithm}
\label{sec:eulerMain}

Finally, we are ready to prove \cref{thm:euler_dist}. 

\begin{proof}
Let $H$ be the input Eulerian graph and assume there are no virtual nodes, as we can deal with them with \cref{euler:prop:get_rid_of_virtual_edges,thm:compilation_pa_congest}. 

We start with item (1), the proofs of other items will be similar. 
We will construct the Eulerian orientation in $t = \tO(1)$ steps. 
In the $i$-th step, we are given a residual Eulerian subgraph $H_i \subseteq H$ containing edges left to orient. 
We find a collection of edge-disjoint cycles $\fC$ containing at least $O(|E(H_i)| / \poly\log n)$ edges of $H_i$ in $\tO(\hopDiameter{G})$ \congest rounds and orient them consistently. %, such that the maximum size of each cycle is $s = \tO(\hopDiameter{G})$. 
%In the next $s$ \congest rounds, we consistently orient edges in each cycle in $\fC$ and 
Next, we discard oriented edges from $H_i$, creating a new residual Eulerian graph $H_{i+1}$ used in the next iteration. If $t = \tO(1)$ is chosen large enough, after $t$ rounds we have $|E(H_t)| = 0$ and we are done. 
It remains to describe how we find the set of edge-disjoint cycles $\fC$ which we do next.  


    We will work in a graph $H'_i$ that we get from $H_i$ by contracting all degree $2$ nodes and discarding isolated nodes. 
    When we work later with $H'_i$, we use \cref{lem:simulation_contraction} to reduce operations on $H'_i$ to operations on $H_i$ and \cref{thm:compilation_pa_congest} to reduce partwise aggregations on $H_i$ to $\tO(\hopDiameter{G})$ \congest operations on $H_i$. 
    Note that every node in $H'_i$ has degree at least $4$, as $H'_i$ is Eulerian and does not contain nodes of degree $0$ or $2$. 
    Hence, we have 
    \begin{align}
    \label{euler:eq:EV}
     |E(H'_i)| \ge 4|V(H'_i)|/2 = 2|V(H'_i)|.    
    \end{align}

    Next, we describe the algorithm. 
\begin{enumerate}
\newcommand{\bH}{\overline{H}}
\newcommand{\bC}{\overline{C}}
    \item Let $\bH_i$ be the graph that we get from $H'_i$ by subdividing each edge $e \in E(H'_i)$. That is, $V(\bH_i) = V(H'_i) \cup E(H'_i)$ and for $v \in V(H'_i), e \in E(H'_i)$ we have $\{v,e\} \in E(\bH_i)$ if $v \in e$.  
    We run the clustering algorithm for separated strong-diameter network decomposition from \cite{elkin2022decompositions} on $\bH_i$. 
    The algorithm discards at most $|E(\bH_i)|/10 = (|V(H'_i)| + |E(H'_i)|) / 10 $ nodes such that the undiscarded nodes form connected clusters $\bC_1, \bC_2, \dots, \bC_q$, each of strong radius $O(\log^2 n)$. 
    Moreover, for any two different clusters $\bC_i, \bC_j$ we have $d_{\bH_i}(\bC_i, \bC_j) \ge 3$. 
    The algorithm needs $\tO(1)$ \congest rounds of $\bH_i$, hence can be implemented in $\tO(1)$ \congest rounds of $H'_i$. 
    After building the clustering in $\bH_i$, for each $\bC \subseteq V(\bH_i)$ we define a cluster $C \subseteq V(H'_i)$ as follows: 
    For each node $e = \{u,v\} \in \bC \cap E(H'_i)$ we put both $u$ and $v$ to $C$. 
    This new clustering of nodes in $H'_i$ still consists of disjoint clusters due to the property $d_{\bH_i}(\bC_i, \bC_j) \ge 3$. Moreover, all clusters still have strong radius $O(\log^2 n)$ and the number of unclustered edges in $H'_i$ remains bounded by $(|V(H'_i)| + |E(H'_i)|) / 10$.   
    
    \item Each cluster runs the algorithm from \cref{lem:minor_closed_cycle_covers} to obtain its cycle cover $\fC$ such that each non-bridge edge is covered by $c = \tO(1)$ cycles of $\fC$ and each cycle of $\fC$ has size $d = \tO(D) = \tO(1)$. Note that total number of all bridges over all clusters is bounded by $|V(H'_i)|$. 
    \item Next, we implement the deterministic MIS algorithm of \cite{censor2017derandomizing} of round complexity $\tO(1)$ in the conflict graph of found cycles. In the conflict graph, each cycle $C \in \fC$ is connected with cycles of $\fC$ that share an edge with $C$. 
    One \congest round in the conflict graph can be implemented in $O(cd) = \tO(1)$ \congest rounds in $H'_i$, hence the overall round complexity of this step is $\tO(1)$ rounds in $H'_i$. 
    The found MIS is the set of cycles $\fC$ that we output. 
    

    \item Finally, we consistently orient the edges in the MIS in additional $d = \tO(1)$ \congest steps on $H'_i$. 
\end{enumerate}
    
    The whole algorithm uses $\tO(1)$ \congestPA steps in $H'_i$, hence using \cref{lem:simulation_contraction,thm:compilation_pa_congest}, we can make above steps run in $\tO(\hopDiameter{G})$ \congest rounds in $G$. 
    
    It remains to argue that the above algorithm orients at least $O(|E(H'_i)| / \poly\log(n))$ of $H'_i$. 
    The number of cycles in the conflict graph is at least the number of clustered non-bridge edges of $H'_i$, which is at least 
    \begin{align*}
     &|E(H'_i)| - (|V(H'_i)| + |E(H'_i)|) / 10 - |V(H')| \\
     & \ge \frac{9}{10} |E(H'_i)| - \frac{11}{10}|V(H'_i)|
     \ge |E(H'_i)| / 10. && \text{Equation \ref{euler:eq:EV}}
    \end{align*}

    On the other hand, the degree of each cycle $C$ in the conflict graph can be bounded by $cd = \tO(1)$, since each of $d$ edges of $C$ can intersect $c$ different cycles. 
    Hence, there are at least $|E(H'_i)| / (3cd)$ cycles in the MIS that cover at least $|E(H'_i)| / (3cd) = O(|E(H'_i)| / \poly\log(n))$ edges of $H'_i$ and the proof of item (1) is finished. 


To prove item (2), we simply use \cref{lem:general_cycle_cover} with $\eps = 1/\sqrt{\log n}$ instead of \cref{lem:minor_closed_cycle_covers}.
In each step we cover at least $|E(H'_i)|/2^{O(\sqrt{\log n})}$ edges and we set the number of steps $t$ to be of order $2^{O(\sqrt{\log n})} = n^{o(1)}$. 

To prove item (3), we adapt the above procedure so that by repeatedly orienting cycles, we orient all edges except at most $2n$ of them, in $n^{O(\eps)}$ \congest rounds for any constant $\eps > 0$. 
Then, we consider the $2n$ remaining edges forming a residual Eulerian subgraph and use \cref{euler:lem:sqrt} to orient them in $\tO(\sqrt{n} + \hopDiameter{G})$ time. It remains to adapt the above procedure to orient all but at most $2n$ edges in $n^{O(\eps)}$ rounds. 

We choose a sufficiently small constant $\eps  > 0$ and run the above procedure with the number of steps set to $t = n^{O(\eps)}$. Alternatively, we finish once the number of edges in $H_i$ drops below $2n$. 
During the procedure, we do not contract the degree $2$ nodes and instead of \cref{lem:minor_closed_cycle_covers} we use \cref{lem:general_cycle_cover} with our parameter $\eps$. 
An analysis analogous to the one above shows that, since we always have $|E(H_i)| \ge 2n$ (cf. Equation \ref{euler:eq:EV}), in each step of the process we orient at least $O(|E(H_i)| / n^{O(\eps)})$ edges. Hence, $t = n^{O(\eps)}$ steps are enough to finish. 
Moreover, one step can be implemented in $n^{O(\eps)}$ \congest rounds, without any need of partwise aggregations, implying the round complexity of $n^{O(\eps)} \cdot n^{O(\eps)} = n^{O(\eps)}$, which is less than $O(\sqrt{n})$ for small enough $\eps$, as needed. 
\end{proof}

% Local Variables:
% TeX-master: "main"
% End:

\begin{remark}
We believe, but do not prove, that any (randomized) algorithm for the  \euler problem on all graphs has to have round complexity $\tilde{\Omega}(\sqrt{n})$ for a graph of radius $\hopDiameter{G} = O(\log n)$. This can be seen by the following construction of the input graph $H$ and the network graph $G \supseteq H$. Let $H = \sqrt{n}C_{\sqrt{n}}$, that is, $H$ consists of $\sqrt{n}$ cycles $C_1, C_2,  \dots C_{\sqrt{n}}$, each of length $\sqrt{n}$. 
Let $V_0, V_1, \dots, V_{\sqrt{n}/2}$ be a partition of $V(H)$ defined as follows. $V_0$ is an arbitrary set of $\sqrt{n}$ nodes such that it contains exactly one node from each cycle $C_i$. 
Next, for $i > 0$ we define  $V_i$  as the set of nodes of distance $i$ from $V_0$. 
The network graph $G \supseteq H$ moreover contains the following additional nodes and edges. First, we build a binary tree on top of each $V_i$ (that is, $V_i$ are the leaves of the tree) and then an additional binary tree on top of the roots of these trees. This defines $G$. 
The graph $G$ contains $O(n)$ nodes and its diameter is $O(\log n)$. On the other hand, we believe one can mimic the well-known lower bound of \cite{sarma2012distributed} to prove that $\tilde{\Omega}({\sqrt{n}})$ rounds are needed to orient all cycles consistently.  
\end{remark}

==> introduction.tex <==
\section{Introduction}\label{sec:intro}

This paper gives essentially near-optimal\footnote{We refer to optimality up to polylogarithmic factors as \emph{near-optimality}, while \emph{almost-optimality} refers to optimality up to subpolynomial, i.e., $n^{o(1)}$, factors.} deterministic parallel algorithms for various $(1+\eps)$-approximate shortest-path-type problems in undirected weighted graphs. These problems include computing $(1+\eps)$-approximate shortest paths or shortest path trees from a single source (shortened to $(1+\eps)$-SSSP) and $(1 + \eps)$-approximate minimum transshipment (shortened to $(1+\eps)$-transshipment). Our algorithms run in polylogarithmic time and require near-linear work. This is optimal up to polylogarithmic factors. All prior parallel deterministic algorithms with polylogarithmic depth for $(1+\eps)$-SSSP required $n^{\Theta(1)}$ more work and, to our knowledge, no sub-quadratic work NC algorithm was known for $(1+\eps)$-transshipment. We also give deterministic distributed algorithms for the above problems, including the first non-trivial distributed deterministic $(1+\eps)$-transshipment algorithm. 

Computing a single-source shortest path is one of the most fundamental problems in combinatorial optimization. Already in 1956, Dijkstra \cite{dijkstra1959dijkstra} gave a simple deterministic $O(m \log n)$ time algorithm for computing an exact single-source shortest path tree in any directed graph. Parallel and distributed algorithms on the other hand have been subject of over three decades of extensive research \cite{ullman1991high,cohen1994polylog,klein1997randomized,spencer1997time,galil1997all,alon1997exponent,zwick1998all,shi1999time,Nan14,EN16,henzinger2016almost,BKKL17,Elk17,elkin2017linearsize,FN18,GL18,haeuplerLi2018sssp,elkin2019hopsets,EN19,henzinger2019deterministic,LPP19,CM20,elkinMatar2021detPRAMSSSP,goranci2022universally} with much remaining unknown. Much recent research has focused on $(1+\eps)$-approximate shortest paths in undirected graphs, the problem solved in this paper. We provide a detailed summary of this prior work next and describe related work on SSSP algorithms in other computational models or on other related problems, including all-pair-shortest-path and SSSP in directed graphs, in \Cref{sec:morerelatedwork}. We focus on randomized and deterministic parallel algorithms with polylogarithmic depth, i.e., RNC and NC algorithms. 

\paragraph{Parallel Algorithm.}
The \pram model of parallel computation was introduced in 1979. After a decade of intense study, Karp and Ramachandran noted in their influential 1989 survey on parallel algorithms~\cite{karp1989survey} that the ``transitive closure bottleneck'' for shortest-path-type problem required work ``far in excess of the time required to solve the problem sequentially''. Indeed, these algorithms build on matrix multiplication or on transitive closure routines and require $O(n^{3})$ work. A line of work \cite{ullman1991high,klein1997randomized,spencer1997time,cohen1997using,shi1999time} provided algorithms with different work-time trade-offs but without much improvement on the cubic work bound for fast parallel algorithms. 


% \begin{comment}
% Previous:

% Indeed, all algorithms build on matrix multiplication or transitive closure routines with $O(n^{3})$ work\alert{not sure what this sentence is supposed to say}. 
% Algorithms by  [UY91, KS97, Spe97, SS99] gave randomized algorithms with different processor-time tradeoffs but without much improvement on the cubic work bound for fast parallel algorithms. [Coh97] gave a deterministic algorithm with similar tradedoffs. [GM97, AGM97, Zwi98] gave algorithm with work equal to $\tO(m^{\omega})$, where $\omega < 2.37\ldots$ is the fast matrix multiplication exponent~\cite{}. 
% \end{comment}





In a major breakthrough, Cohen~\cite{cohen1994polylog} gave a randomized $(1 + \eps)$-SSSP algorithm based on hopsets with $\tO_\rho(1)$ time and $O(m^{1+\rho})$ work for any constant $\rho > 0$. Algorithms with slightly improved time-work tradoffs were given~\cite{elkin2017linearsize,elkin2019hopsets} but these algorithms still required a polynomial $m^{\rho}$ factor more work than Dijkstra's algorithm to parallelize shortest path computations to polylogarithmic parallel time. 
%On the other hand, using modern methods from continuous optimization \cite{She13,BKKL17,She17b}, recent algorithms 

This remained the state-of-the-art until 2020 when methods from continuous optimization developed by Sherman~\cite{She13,She17b} enabled further progress on shortest-path type problems. In particular, Sherman gave an $m \cdot n^{o(1)}$ sequential algorithm for the $(1+\eps)$-approximate minimum transshipment problem. \emph{Transshipment}, also known as uncapacitated min-cost flow, Wasserstein distance, or optimal transport, is the other major problem solved in this paper. The input to the transshipment problem on some weighted graph $G$ consists of a \emph{demand} $b$ which specifies for each node a positive or negative demand value with these values summing up to zero. The goal is to find a flow of minimum cost which sends flow from nodes with surplus to nodes with positive demands. Here the cost of routing a unit of flow over an edge is proportional to the weight/length of the edge. For example, an optimal transshipment flow for a demand with $b(s)=-1$ and $b(t)=1$ is simply a unit flow from $s$ to $t$ which decomposes into a distribution over shortest $(s,t)$-paths. We remark that transshipment is in many ways a powerful generalization of shortest-path problems, including computing SSSP (trees), with the exception that extracting trees or paths from a continuous transshipment flow often remains a hard problem itself which requires highly nontrivial rounding algorithms. While having an innocent feel to them, such rounding steps have a history of being inherently randomized and being algorithmic bottlenecks for shortest-path problems on several occasions. 

Sherman's almost-linear time transshipment algorithm did not imply anything new for SSSP at first, but it inspired two independent approaches by \cite{Li20} and Andoni, Stein, and Zhong \cite{AndoniSZ20} that led to near-optimal randomized parallel shortest path algorithms with polylogarithmic time and near-linear work. In particular, Li~\cite{Li20} improved several parts of Sherman's algorithm and combined it with the vertex-reduction framework that Peng~\cite{Pen16} had introduced to give the first near-linear time algorithm for $(1+\eps)$-maximum-flow. \cite{Li20} also adopts a randomized rounding algorithm of \cite{BKKL17} based on random walks to extract approximate shortest-path trees from transshipment flows. Overall, this results in randomized PRAM algorithms for both $(1+\eps)$-transshipment and $(1+\eps)$-SSSP with polylogarithmic time and near-linear work.
%We give a more detailed description of this in \alert{???}\Cref{???}.
Concurrently, Andoni, Stein, and Zhong \cite{AndoniSZ20} achieved the same result for $(1+\eps)$-transshipment by combining Sherman's framework with ideas from hop-sets. They also provide a randomized rounding based on random walks algorithm that can extract an $s$-$t$ shortest path. Later, this rounding was extended in Zhong's thesis~\cite{zhong2021new} to extract the full $(1+\eps)$-SSSP tree. 

It is remarkable that all parallel $(1+\eps)$-SSSP algorithms described above (with the exception of the super-quadratic work algorithms before Cohen's 25 year old breakthrough) crucially rely on randomization for efficiency. Indeed, the only modern deterministic parallel $(1+\eps)$-SSSP algorithm is a very recent derandomization of Cohen's algorithm by Elkin and Matar~\cite{elkinMatar2021detPRAMSSSP}. This algorithm suffers from the familiar $O(m^{1+\rho})$ work bound for a polylogarithmic time parallel algorithm. For the $(1+\eps)$-transshipment problem even less is known. Indeed we are not aware of any efficient deterministic parallel algorithm before this work and would expect that much larger polynomial work bounds would be required to achieve a deterministic algorithm with polylogarithmic parallel time.

In this paper, we give deterministic parallel algorithms for both the $(1 + \eps)$-SSSP and the $(1+\eps)$-transshipment problem in undirected weighted graphs. Both algorithms only require near-linear work and run in polylogarithmic time. This solves these two and various other shortest-path-type problems optimally, up to polylogarithmic factors. 

\begin{restatable}[Deterministic Parallel SSSP and Transshipment]{theorem}{mainparallel}
\label{thm:main_parallel}
There is a deterministic parallel algorithm that, given an undirected graph with nonnegative weights, computes a $(1+\eps)$-approximate single-source shortest path tree or a $(1+\eps)$-approximation to minimum transshipment in $\tO(m \cdot \eps^{-2})$ work and $\tO(1)$ time in the \pram model for any $\eps \in (0,1]$.
\end{restatable}

\paragraph{Distributed Algorithm.}
We also give new distributed $(1+\eps)$-SSSP and $(1+\eps)$-transshipment algorithms in the standard \congest model of distributed computing. 
For distributed algorithms a lower bound of $\Omega(\sqrt{n} + \Dhop)$ rounds is known for worst-case topologies~\cite{elkin2006unconditional,sarma2012distributed}, where $\Dhop$ is the unweighted (i.e., hop) diameter of the network. We refer to this as the \emph{existential lower bound} since it depends on the parameterization by $(n, \Dhop)$, as opposed to the later-discussed \emph{universal lower bound} which does not.

In his 2004 survey on distributed approximation, Elkin~\cite{elkin2004distributed} pointed to the distributed complexity of shortest paths approximations as one of two fundamental and wide-open problems in the area---as no non-trivial algorithms complementing the above lower bounds were known.

Since then, the $(1+\eps)$-SSSP problem is one of the most studiedonly give a brief summary here: Lenzen and Patt-Shamir gave an $\tO(n^{1/2 + \eps} + \Dhop)$-round $O(1 + \frac{\log 1/\eps}{\eps})$-SSSP algorithm \cite{lenzen2013fast} and a $(1+o(1))$-approximation in $\tO(n^{1/2}\cdot \Dhop^{1/4}+\Dhop)$ rounds was given by Nanongkai \cite{Nan14}. 
Building on Sherman's transshipment framework mentioned before, \cite{BKKL17} gave a randomized $\tO(\eps^{-3} \cdot (\sqrt n + \Dhop))$ algorithm.
The first algorithm improving over the $\Omega({\sqrt{n}})$ barrier was given in \cite{haeuplerLi2018sssp} with a running time of $\shortcutQuality{G} \cdot n^{o(1)}$ albeit with a bad $n^{o(1)}$-approximation. 
This was recently improved by \cite{goranci2022universally} to a $(1+\eps)$-approximation with the same round complexity. 
Using \cite{ghaffari_haeupler2021shortcuts_in_minor_closed}, this gives a $(1+\eps)$-approximation algorithm with round complexity $\Dhop \cdot n^{o(1)}$ for any excluded minor topology (e.g., planar graphs). 
All the above algorithms are randomized: The only deterministic distributed algorithm is the $(1 + o(1))$-SSSP algorithm of \cite{henzinger2019deterministic} with a $(n^{1/2+o(1)} + \Dhop^{1+o(1)})$ running time. For $(1+\eps)$-transshipment, the only known sublinear distributed algorithm is the randomized $\shortcutQuality{G} \cdot n^{o(1)}$-round algorithm of \cite{goranci2022universally}. No non-trivial  deterministic distributed $(1+\eps)$-transshipment algorithm (with sub-linear round complexity) was known prior to this work.

The distributed results of this paper include deterministic distributed algorithms for $(1+\eps)$-SSSP, its generalization $(1+\eps)$-\setssp (in which we are looking for distances from a subset of nodes), and  $(1+\eps)$-transshipment. Our results improve over the previous best running times of deterministic distributed algorithms for each of the above problems, both in the worst-case and for any excluded minor graph. Both the round and the message complexities (in $KT_0$, see \cite{peleg2000distributed} for the definition) of our algorithms are (existentially) optimal, up to $\poly\log n$ factors, in all cases. 
%The algorithm solves the more general version of the problem where the source of the shortest path computation is an arbitrary set of nodes. 

%as well as a universally optimal distributed algorithm if the topology is known. (this is actually not easily doable because we need fast deterministic routing, too. Technically one can achieve this using deterministic semi-oblivious routing but the local computations would be exponential time if one would want them to be deterministic. LOL

\begin{restatable}[Deterministic Distributed SSSP and Transshipment]{theorem}{maindistributed}
\label{thm:main_distributed}
There is a deterministic \congest algorithms that, given an undirected graph with non-negative weights, compute a $(1+\eps)$-approximate \setssp forest or a $(1+\eps)$-transshipment solution for any $\eps \in (0,1]$. Our algorithms have an optimal message complexity of $\tO (m) \cdot  \eps^{-2}$ and are guaranteed to terminate in at most 
\begin{enumerate}
    \item within at most $\tO(\sqrt{n} + \Dhop) \cdot \eps^{-2}$ rounds and
    \item within at most $\tO(\Dhop) \cdot  \eps^{-2}$ rounds if $G$ does not contain any $\tO(1)$-dense minor.
\end{enumerate}
%Here, $\Dhop$ is the hop diameter of $G$. 
\end{restatable}

%Our results are the first deterministic $(1+\eps)$-SSSP for excluded minor graphs and even improve the randomized complexity for these graphs. In terms of worst-case complexity, we improve the running time of the best deterministic algorithm of \cite{Nan14} to near-optimal, matching the time of the fastest randomized algorithm of \cite{BKKL17}.

\underline{Universal optimality.} Recently, the pervasive $\tilde{\Omega}(\Dhop + \sqrt{n})$ distributed lower bounds have been extended to a near-tight universal lower bound~\cite{haeupler2021universally} which shows that most optimization problems including all problems studied in this paper require $\tilde{\Omega}(\shortcutQuality{G})$ rounds on any communication graph $G$. Here $\shortcutQuality{G}$ is a natural graph parameter (we refer the interested reader to \cite{haeupler2021universally} for a formal definition). For experts interested in universally-optimal distributed algorithms we remark that the results of this paper imply strong conditional results. We state these results for the interested reader in \Cref{sec:main_theorems}. 



%In summary, this is the first deterministic distributed algorithm for excluded minor graph and simultaneously improves the running time to optimal up to polylog n factors compared to the best randomized algorithm. In terms of worst-case complexity this improved the running time of the best det algorithm of Nan to near optimal, matching the time of the near-optimal randomized algorithm of becker.



\subsection{Technical Overview}

\begin{figure}
    \centering
    \includegraphics[width = \textwidth]{fig/main.eps}
    \caption{This figure summarizes our approach with our contributions marked in red. It is known that a $\tO(1)$-competitive solution to $\ell_1$-oblivious routing can be boosted to a $(1+\eps)$-approximate transshipment which can then be rounded to yield a $(1+\eps)$-approximate SSSP tree. We close the circle of reductions by constructing certain distance structures from the approximate SSSP tree. Think of those distance structures as a family of clusterings on different scales, storing some additional distance information. One of our main technical contributions is the efficient construction of a $\tO(1)$-approximate oblivious routing from the distance structures, which closes the loop. \\
    This loop of reductions itself is not very useful as the complexity of the problems does not decrease. 
    We break this loop by our \emph{distance reduction} framework by showing one can construct distance structures ``up to distance $D$'' using distance structures ``up to distance $D /\poly\log n$. 
    %, we construct $\ell_1$-oblivious routing up to the larger distance $D$, which enables us to construct (in order) approximate transshipment, SSSP tree, and finally distance structures up to distance $D$. 
    %The notion of ``up to distance $D$'' is formalized by adding the virtual \emph{cheating node} connecting to all other nodes via an edge of length $D$. 
    After $O(\log n)$ iterations, we build up the desired solution to any of the four problems, in particular to approximate transshipment and set-SSSP. }
    \label{fig:main}
\end{figure}


While the results for SSSP and transshipment are important, the main impact of this paper will likely be the new tools and algorithmic ideas developed in this paper. We expect these ideas to be applicable beyond shortest path problems. Next, we give a brief summary of the most relevant parts and ideas of prior work which are needed to understand our work and put in proper context. We then give an informal high-level overview of our new algorithm and some of the new tools developed for it. A readable and more precise technical proof overview is given in \Cref{sec:localiterative}.

\subsubsection{Background and Prior Work}

{\bfseries Transshipment Boosting, $\ell_1$-Oblivious Routing, and Transshipment Flow Rounding} \\
All modern SSSP-algorithms, including ours, compute shortest paths via the transshipment problem (see text before \Cref{thm:main_parallel} for a definition). The key idea in this approach of Sherman~\cite{She13, She17b} is that even a rather bad $\alpha$-approximation algorithm for (dual) transshipment can be \emph{boosted} to a $(1+\eps)$-approximation. This is achieved via the multiplicative weights method (or equivalently: gradient descent) and requires only $\poly(\alpha, \eps^{-1}, \log n)$ invocations of the $\alpha$-approximation algorithm~\cite{She17b,BKKL17,zuzic2021simple}. A particularly convenient way of obtaining such a boostable $\alpha$-approximation is to design a linear matrix $R$ which maps any node-demand $b$ to an $\alpha$-approximate transshipment flow for $b$. Such a matrix is called an $\ell_1$-oblivious routing because linearity forces each node to route its demand obliviously, i.e., without knowledge of the demand on other nodes. As mentioned before, in order to obtain an actual $(1+\eps)$-SSSP tree from a transshipment flow most algorithms~\cite{Li20} are using an approach of \cite{becker2019low} which produces a $(1+\eps)$-SSSP tree after $O(\log n)$ adaptive applications of some rounding algorithm. All parts of this reduction except for the rounding algorithm are deterministic.

Putting all these pieces together proves that all one needs to obtain an efficient (deterministic) algorithm for both the  $(1+\eps)$-transshipment and the $(1+\eps)$-SSSP problem is a $\tO(1)$-competitive $\ell_1$-oblivious routing that can be evaluated efficiently and a (deterministic) rounding algorithm. Our algorithm uses these steps in a black-box fashion except that we need to replace the randomized rounding algorithm by a new deterministic transshipment flow rounding procedure. 

%our SSSP algorithm 

%The works that are most closely related to the algorithm presented here are the works of \cite{Li20,goranci2022universally}, which in turn build on multiplicative-weight boosting, pre-conditioning with $\ell_1$-routing, the vertex-reduction framework of Peng~\cite{Pen16}, and the Minor-Aggregations framework. We give a brief overview over the relevant parts of these prior works, some of which our algorithm utilizes in a black-box manner.

%{\bfseries SSSP via Transshipment, Multiplicative-Weight Boosting of Transshipment}\\
%Like all modern SSSP algorithms, we use the framework of Sherman~\cite{She13, She17b} which proceeds by reducing the problem to transshipment.
% This calls for solving a generalized continuous version of shortest paths---the transshipment problem (also called uncapacitated min-cost flow, Wasserstein distance, or optimal transport). The input to the problem is a weighted graph $G$ and a so-called \emph{demand vector} $b : V(G) \to \R$ satisfying $\sum_{v \in V(G)} b(v) = 0$. The goal is to find a flow of minimum cost that satisfies the demand $b$ (i.e., the inflow minus outflow at $v$ should equal $b(v)$).
%Transshipment clearly generalizes the $s$-$t$ shortest path problem since the min-cost solution satisfying the demand $b = \mathbb{1}_s - \mathbb{1}_t$ is the $s$-$t$ shortest path. Albeit more involved, transshipment also generalizes SSSP if one is given a rounding procedure which transforms the fractional flow to an integral one supported on a tree.

%The key feature exploited in all modern SSSP approaches is that an $\alpha$-approximation algorithm for (dual) transshipment can be \emph{boosted} to a $1+\eps$ approximation. This is achieved via gradient descent or, equivalently, the multiplicative weights method, using only $\poly(\alpha, \eps^{-1}, \log n)$ invocations of the $\alpha$-approximation algorithm~\cite{She17b,BKKL17,zuzic2021simple}. A particularly convenient way of obtaining an $\alpha$-approximate dual solution is to design a linear $\ell_1$-oblivious $\alpha$-competitive routing, described below. 


%In summary, it is sufficient to design any $\tO(1)$-competitive $\ell_1$-oblivious routing to near-optimally solve $(1+\eps)$-approximate transshipment, which can then be rounded to a solution for $(1+\eps)$-SSSP.

%{\bfseries Graph Based $\ell_1$-oblivious routing}\\
%Given a weighted graph $G$, the $\ell_1$-oblivious routing $R$ is a linear map (matrix) which maps a demand $b : V(G) \to \R$ to a flow $f := R b$ which is an approximately-optimal solution to the corresponding transshipment problem (satisfying demand $b$ on $G$). The routing has the adjective \emph{oblivious} since its linearity forces each node $v$ to route $v$'s demand without knowledge of the demand on other nodes. The goal in this paper is to design a deterministic routing that achieves a $\tO(1)$ approximation for all demands, while still allowing efficient evaluations.


%Othisne natural candidate for an $\ell_1$-oblivious routing would be to sample a probabilistic tree embedding of $G$ with $O(\log n)$-distance distortion and let each node route its demand to the root. This is a valid linear map and can be evaluated fast. Moreover, it is easy to see that the cost of the resulting flow is $O(\log n)$-competitive \emph{in expectation} with the optimal transshipment solution.

% The approximation is furthermore $O(\log n)$ in expectation if the demand is chosen independently from the randomness used to construct the map, which is provably best possible.

%Unfortunately, such a guarantee in expectation is not enough for the MW-boosting framework, as a valid $\alpha$-competitive routing needs to be competitive \emph{for all} demands. To boost the guarantee from an expected guarantee to a worst-case (for all) guarantee one can sample multiple linear maps as above and define $R$ to be the average. This can result in the desired deterministic approximation guarantee but only if linearly many samples are taken, leading to a quadratic time for construction and evaluation. There has thus been a consensus that such an approach cannot be made to work. 

\begin{comment}
All previous parallel approaches to construct a high-quality oblivious routing relied on first computing an $\ell_1$-embedding, which is a mapping from the nodes of a graph to vectors in $\ell_1$ such that the distances are approximately preserved, and then performing the routing in the (significantly simpler) $\ell_1$-space. This includes the approaches of Sherman~\cite{She17b}, Li~\cite{Li20}, Andoni, Stein, and Zhong~\cite{AndoniSZ20}, etc.
\end{comment}

% The drawback of this scheme is that the known $\ell_1$-embeddings are inherently randomized and that the routing and flow obtained are in the auxiliary (virtual) $\ell_1$-space. It is not clear how to obtain a flow in $G$ from this. Fortunately, merely a vector whose $\ell_1$-norm approximates the optimal transshipment flow cost is needed for the boosting framework.

%Instead, the $\ell_1$-oblivious routings of , are based on first computing an $\ell_1$-embedding and then performing an $\ell_1$-oblivious routing in this $\ell_1$-space, which is much easier. 

\begin{comment}
A very recent paper~\cite{goranci2022universally} showed that a simple graph-based $n^{o(1)}$-competitive $\ell_1$-oblivious routing could be directly defined on the network $G$ by using only a simple randomized graph decomposition primitive called \emph{low-diameter decomposition}. Unfortunately, many barriers prevent this approach from achieving a polylog-competitive routing even if one does not require deterministic algorithms. This paper builds upon their approach and develops the necessary tools and ideas to both yield polylog-competitiveness and deterministic guarantees of the routing.
\end{comment}

% $n^{o(1)}$ many low-diameter decompositions of exponentially increasing radii. Luckily, low-diameter decompositions (of super-low, $n^{o(1)}$, quality) can be computed in $n^{o(1)}$ minor aggregation steps using the algorithm of Haeupler and Li \cite{HL18}, which is basically following the simple pioneering approach of Alon et al.~\cite{alon1995graph}. The advantages of the approach of \cite{goranci2022universally} are that they work well with the \aggregate framework, that the routing matrix is simple, and directly maps to a flow in $G$ (rather than an auxiliary space). Unfortunately, this approach is fundamentally unable to achieve a $n^{o(1)}$-competitive routing even before attempting derandomization, even if one is given an oracle which constructs (optimal) $O(\log n)$-quality low-diameter decompositions. We develop many new tools in this paper in order to achieve this goal.


{\bfseries Vertex Reduction Framework}\\
Unfortunately, it is clear that $\ell_1$-oblivious routing cannot be done without having some approximate shortest path information. This chicken and egg problem is resolved via a clever vertex-reduction framework of Li~\cite{Li20}.  % first introduced by Peng~\cite{Pen16} for solving max-flow, i.e., the $\ell_\infty$ analog of SSSP / transshipment, and adapted to the transshipment setting by Li~\cite{Li20}. 
The vertex-reduction framework relies on a cyclic sequence of efficient problem reductions. For transshipment~\cite{Li20}, these problems are SSSP, transshipment, $\ell_1$-oblivious routing, and $\ell_1$-embedding. Specifically:
\begin{itemize}
\item To solve $(1+\eps)$-SSSP on $G$, it is sufficient to solve $(1+\eps)$-transshipment on $G$, 
\item for which it is sufficient to construct $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing on $G$ (via boosting),
\item for which it is sufficient to construct an $\tilde{O}(1)$-distortion $\ell_1$-embedding on $G$,
\item for which it is sufficient to solve $O(\log^2 n)$ instances of $\tilde{O}(1)$-SSSP on a sequence of graphs $G'_1, G'_2, \ldots, G'_{O(\log^2 n)}$, which are resolved recursively.
\end{itemize}
As stated, this simply reduced $(1+\eps)$-SSSP on $G$ to multiple $\tilde{O}(1)$-SSSP on graphs that are slightly larger than $G$, which isn't particularly helpful on its own. The key idea to transform this ``branching cycle'' into a branching spiral that terminates (fast) is to add a step into the cycle which applies ultrasparsification on $G'_i$, which is an operation that transforms a graph with $n$ nodes to a smaller graph with $\frac{n}{\gamma}$ nodes such that distances in the smaller graph $\tilde{O}(\gamma)$-approximate distances in the larger graph. Applying this step, we can reduce $(1 + \eps)$-SSSP on a graph with $n$ nodes to $O(\log^2 n)$ instances of $\tilde{O}(1)$-SSSPs on smaller graphs with $O\left(\frac{n}{\log^{100} n}\right)$ nodes. It is easy to see that the total size of all recursive calls falls exponentially on each subsequent level, hence the total parallel runtime is $\tilde{O}(1)$ and the total work $\tilde{O}(m)$ (since a single sequence of reductions requires $\tilde{O}(m)$ work).

%The issues with this approach is that (1) there are currently no known deterministic constructions of $\ell_1$-embeddings, and (2) the oblivious routing in the $\ell_1$-space is inherently hard to convert to a small number of minor aggregations (see below), leading to algorithms that are not appropriate for the distributed setting. \alert{mention somewher that this is performed on different graphs}

% Several of these reductions are losing polylogarithmic factors in approximation, but these turn into polylogarithmic increases in running time thanks to boosting. The key idea to transform this branching cycle into a branching spiral that terminates (fast) is to add a step into the cycle which applies ultrasparsification followed by vertex-sparsification. The two sparsification procedures used in this step replace the $n$-node graph $G$ by a graph $H$ with a $\frac{n}{\gamma}$ nodes for any polylogarithmic $\gamma$ while still approximating $G$ up to polylogarithmic factors. \todo{What does approximating mean in that context?}The loss in approximation is again removed with the boosting step. While a single SSSP on $G$ now still generates some $\beta = O(log^2 n)$ recursive SSSP calls, these SSSP calls are on \emph{on smaller graphs} with $\frac{n}{\gamma}$ nodes.

% The overall time complexity for these recursive calls satisfies the recurrence relation $T(n) = \beta T(n/\gamma) + \tO(n)$ which is easily seen to resolve to $T(n)=\tO(n)$ when $\gamma$ is chosen to be at least a constant factor larger than $\beta$.

% Figure 1 gives a slightly rearranged description of the algorithm of Li:

% $(1+eps)$-SSSP on G    



\iffalse

{\bfseries Vertex Reduction Framework}\\
The main problem with reducing $(1+\eps)$-SSSP to $\ell_1$-oblivious routing is that some non-trivial shortest path information is clearly necessary to route a flow $\tO(1)$-competitively. \cite{Li20} resolves this chicken and egg problem via the vertex-reduction framework of Peng~\cite{Pen16}. First a cyclic sequence of efficient problem reductions is established and then the cyclicity is broken up by introducing an ultra-sparsification and vertex reduction step. Overall one SSSP call on $G$ is reduced to $\tO(1)$ SSSP calls on smaller graphs $G_1, G_2, \ldots$ whose sizes sum up to at most $|G|/2$. Each $G_1$ is essentially a minor of $G$.


Starting with an SSSP algorithm Li produces uses $\tO(1)$ recursive calls to this SSSP algorithm to compute Bourgain's randomized $\tilde{O}(1)$-distortion $\ell_1$-embedding he then uses an ultra sparsification step to 

on $G$

Starting with the above mentioned reductions from SSSP via transshipment to $\ell_1$-oblivious routing Li add the following steps
\begin{itemize}
\item $\ell_1$-oblivious routing is reduced to 


To solve $(1+\eps)$-SSSP on $G$, it is sufficient to solve $(1+\eps)$-transshipment on $G$, 
\item for which it is sufficient to construct $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing on $G$ (via boosting),
\item for which it is sufficient to construct an $\tilde{O}(1)$-distortion $\ell_1$-embedding on $G$,
\item for which it is sufficient to solve $O(\log^2 n)$ instances of $\tilde{O}(1)$-SSSP on a sequence of graphs $G'_1, G'_2, \ldots, G'_{O(\log^2 n)}$, which are resolved recursively.
\end{itemize}


shows how to reduce t

, G'_{O(\log^2 n)}$

result in 



. For transshipment~\cite{Li20}, these problems are SSSP, transshipment, $\ell_1$-oblivious routing, and $\ell_1$-embedding. Specifically:
\begin{itemize}
\item To solve $(1+\eps)$-SSSP on $G$, it is sufficient to solve $(1+\eps)$-transshipment on $G$, 
\item for which it is sufficient to construct $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing on $G$ (via boosting),
\item for which it is sufficient to construct an $\tilde{O}(1)$-distortion $\ell_1$-embedding on $G$,
\item for which it is sufficient to solve $O(\log^2 n)$ instances of $\tilde{O}(1)$-SSSP on a sequence of graphs $G'_1, G'_2, \ldots, G'_{O(\log^2 n)}$, which are resolved recursively.
\end{itemize}


This chicken and egg problem is resolved via a clever vertex-reduction framework of Li~\cite{Li20}.

it is pretty clear 


\begin{comment}
All previous parallel approaches to construct a high-quality oblivious routing relied on first computing an $\ell_1$-embedding, which is a mapping from the nodes of a graph to vectors in $\ell_1$ such that the distances are approximately preserved, and then performing the routing in the (significantly simpler) $\ell_1$-space. This includes the approaches of Sherman~\cite{She17b}, Li~\cite{Li20}, Andoni, Stein, and Zhong~\cite{AndoniSZ20}, etc.
\end{comment}

t induces 


Unfortunately, it is clear that $\ell_1$-oblivious routing cannot be done without having some approximate shortest path information. This chicken and egg problem is resolved via a clever vertex-reduction framework of Li~\cite{Li20}.  % first introduced by Peng~\cite{Pen16} for solving max-flow, i.e., the $\ell_\infty$ analog of SSSP / transshipment, and adapted to the transshipment setting by Li~\cite{Li20}. 
The vertex-reduction framework relies on a cyclic sequence of efficient problem reductions. For transshipment~\cite{Li20}, these problems are SSSP, transshipment, $\ell_1$-oblivious routing, and $\ell_1$-embedding. Specifically:
\begin{itemize}
\item To solve $(1+\eps)$-SSSP on $G$, it is sufficient to solve $(1+\eps)$-transshipment on $G$, 
\item for which it is sufficient to construct $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing on $G$ (via boosting),
\item for which it is sufficient to construct an $\tilde{O}(1)$-distortion $\ell_1$-embedding on $G$,
\item for which it is sufficient to solve $O(\log^2 n)$ instances of $\tilde{O}(1)$-SSSP on a sequence of graphs $G'_1, G'_2, \ldots, G'_{O(\log^2 n)}$, which are resolved recursively.
\end{itemize}
As stated, this simply reduced $(1+\eps)$-SSSP on $G$ to multiple $\tilde{O}(1)$-SSSP on graphs that are slightly larger than $G$, which isn't particularly helpful on its own. The key idea to transform this ``branching cycle'' into a branching spiral that terminates (fast) is to add a step into the cycle which applies ultrasparsification on $G'_i$, which is an operation that transforms a graph with $n$ nodes to a smaller graph with $\frac{n}{\gamma}$ nodes such that distances in the smaller graph $\tilde{O}(\gamma)$-approximate distances in the larger graph. Applying this step, we can reduce $(1 + \eps)$-SSSP on a graph with $n$ nodes to $O(\log^2 n)$ instances of $\tilde{O}(1)$-SSSPs on smaller graphs with $O\left(\frac{n}{\log^{100} n}\right)$ nodes. It is easy to see that the total size of all recursive calls falls exponentially on each subsequent level, hence the total parallel runtime is $\tilde{O}(1)$ and the total work $\tilde{O}(m)$ (since a single sequence of reductions requires $\tilde{O}(m)$ work).

%The issues with this approach is that (1) there are currently no known deterministic constructions of $\ell_1$-embeddings, and (2) the oblivious routing in the $\ell_1$-space is inherently hard to convert to a small number of minor aggregations (see below), leading to algorithms that are not appropriate for the distributed setting. \alert{mention somewher that this is performed on different graphs}

% Several of these reductions are losing polylogarithmic factors in approximation, but these turn into polylogarithmic increases in running time thanks to boosting. The key idea to transform this branching cycle into a branching spiral that terminates (fast) is to add a step into the cycle which applies ultrasparsification followed by vertex-sparsification. The two sparsification procedures used in this step replace the $n$-node graph $G$ by a graph $H$ with a $\frac{n}{\gamma}$ nodes for any polylogarithmic $\gamma$ while still approximating $G$ up to polylogarithmic factors. \todo{What does approximating mean in that context?}The loss in approximation is again removed with the boosting step. While a single SSSP on $G$ now still generates some $\beta = O(log^2 n)$ recursive SSSP calls, these SSSP calls are on \emph{on smaller graphs} with $\frac{n}{\gamma}$ nodes.

% The overall time complexity for these recursive calls satisfies the recurrence relation $T(n) = \beta T(n/\gamma) + \tO(n)$ which is easily seen to resolve to $T(n)=\tO(n)$ when $\gamma$ is chosen to be at least a constant factor larger than $\beta$.

% Figure 1 gives a slightly rearranged description of the algorithm of Li:

% $(1+eps)$-SSSP on G    

% can be computed via log n calls to TS+randomized rounding which can all be answered using a single $\ell_1$-oblivious routing matrix of in G  (this is the boosting framework)

% $O(log^6 n)$-competitive $\ell_1$-oblivious routing matrix of G    

% using the two sparsification procedures the problem of finding an $\ell_1$-oblivious routing matrix of G can be reduced to finding an $\ell_1$-oblivious routing matrix for a graph H with $O(\frac{n}{100 log^2 n})$ nodes.

% $O(log^2 n)$-approx $\ell_1$-oblivious routing matrix of H

% Li showed that an $\ell_1$-oblivious routing can be computed using an $O(log^? n)$-distortion $\ell_1$-embedding of $H$. Such an $\ell_1$-embedding can be computed using Bourgains embedding which requires $\beta = O(log^2 n)$ calls to S-set-source shortest paths on $H$ for different vertext sets $S_1,S_2,\ldots,S_\beta$. These can be computed via single-source shortest path computations on the $\beta$ different graphs $H_i$ for $i \in [\beta]$, where $H_i$ is the graph $H$ plus one extra node $s$ connected to all nodes in $S_i$ via a short or zero length edges. 

% (1+eps)-SSSP on $H_1,H_2,\ldots,H_{\beta}$ with at most $\frac{n}{\gamma}$ nodes each
\fi

{\bfseries Minor Aggregates and the Low-Congestion Shortcuts Framework}\\
The low-congestion shortcuts framework was originally intended for designing simple and efficient \emph{distributed} graph algorithms and was developed over a long sequence of works~\cite{GH16,haeupler2016low,haeupler2016near,haeupler2018round,haeupler2018minor,ghaffari_haeupler2021shortcuts_in_minor_closed,haeupler2021universally,kogan2021low,ghaffari2021hop,GHR21}. However, this paper argues that the framework provides a natural language even for developing fast parallel algorithms. Indeed, we present our parallel SSSP algorithm using the framework and our hope is that this choice simplifies the exposition, even before considering the benefits of immediately obtaining distributed results.

We describe our algorithms in the recently introduced \aggregate model~\cite{goranci2022universally, ghaffari2021universally}, which offers an intuitive interface to the recent advancements in the low-congestion shortcut framework. In the \aggregate model, one can (1) contract edges, thereby operating a minor, (2) each (super)node in the contracted graph can compute an aggregate (e.g., min, max, sum) of surrounding neighbors, and (3) add $\tilde{O}(1)$ arbitrarily-connected virtual nodes over the course of the algorithm. The goal is to design $\tO(1)$-round algorithms in this model. Such a \aggregate algorithm can be compiled to a near-optimal algorithm in both the parallel and distributed settings.

% Note that computing a partwise aggregate is basically same as computing a node-wise aggregate in the minor in which each part is contracted. Any algorithm that uses some $k$ rounds of contractions and node-aggregation on the resulting minors thus directly translates into an algorithm with $\tilde{O}(k)$ partwise aggregations on $G$ (the different interfaces or partwise and minor aggregations account for the $\tilde{O}(1)$ overhead). Our goal is to design $\poly\log n$-round \aggregate algorithms, which immediately yield polylog-depth and near-linear-work parallel algorithms, and universally-optimal distributed algorithms. \Cref{sec:minoraggregatemodel} summarizes this model which we use throughout this paper.


\subsubsection{Our New Tools}

%Our first two tools are interesting beyond the problem of derandomization and we introduce them in a probabilistic language which is more intuitive. \alert{?!?!}

{\bfseries Near-Optimal Graph-Based $\ell_1$-oblivious routing}\\
The first key contribution of this paper is a new construction of graph-based $\ell_1$-oblivious routing with drastically improved guarantees from the so-called sparse neighborhood covers. A sparse neighborhood cover of distance scale $D$ is a collection of $O(\log n)$ clusterings (partitioning of the node set into disjoint \emph{clusters}) such that (1) each cluster has diameter at most $D$, and (2) each ball in $G$ of radius $D / (\log^{C} n)$ is fully contained in at least one cluster (for some fixed constant $C > 0$). Specifically, given sparse neighborhood covers for all $O(\log n)$ exponentially-increasing distance scales $\beta, \beta^2, \beta^3, \dots, \poly(n)$ for some $\beta = \tO(1)$ along with some extra distance information, we construct an $\tO(1)$-competitive $\ell_1$-oblivious routing. 
The algorithm greatly differs from all prior approaches, as all of them had inherent barriers preventing them from achieving deterministic near-optimality, which we describe below.

\underline{Derandomization issues:} Efficient constructions of an $\ell_1$-oblivious routing either use an $\ell_1$-embedding or so-called low-diameter decompositions; this is a clustering problem whose deterministic version is also known as a sparse neighborhood cover. 
Sparse neighborhood covers were introduced in the seminal work of \cite{awerbuch1990sparse} and applied with great success for many problems, including approximate shortest paths and other distance based problems \cite{cohen98pairwise_covers,bartal2021RamseyEmbeddings}. 

Since an efficient deterministic $\ell_1$-embedding is not known, we need a deterministic construction of sparse neighborhood covers.  
%The low-diameter decomposition, known to be efficiently constructable from approximate distances in the randomized world \cite{becker2019low}, is a probability distribution. 
Luckily, many of the ideas required to derandomize the computation of sparse neighborhood covers were developed very recently by a sequence of papers that derandomized the closely related network decomposition problem which is, essentially, an unweighted version of the sparse cover problem~\cite{rozhon_ghaffari2019decomposition,ghaffari_grunau_rozhon2020improved_network_decomposition,chang_ghaffari2021strong_diameter}.
In \cite{elkin2022decompositions}, these unweighted results were extended to an algorithm constructing sparse neighborhood cover for weighted graphs and this is the result that we use to solve the shortest path problem here. 
% It can be shown that all prior approaches based on low-diameter decompositions or sparse neighborhood covers are inherently unable to be polylog competitive. To this end, we crucially use several key ideas that depart from all prior constructions.

% \underline{Idea 1: Remembering where the flows came from.} Oblivious routing intuitively works by judiciously intermixing the demand, until eventually, all demand is routed to some single node (note that sending a negative demand along a directed edge corresponds to sending a positive demand over the reversed edge). This is a valid solution to the transshipment problem, albeit its competitiveness depends on the intermixing strategy. 
% However, all prior approaches have the property that flows/demands that are ever joined will not again split apart, but will be treated equally. 
% We, on the other hand, treat the flows differently based on their origin node, making the flows splittable even after being aggregated. This idea, along with the next one, allows us to convert the multiplicative losses to additive ones, helping us achieve polylog-competitive routing.

% \underline{Idea 2: Reduce the outflow of nodes close to the boundary.} All prior approaches work by choosing a clustering (from the sparse neighborhood cover or low-diameter decomposition) and then for each cluster $C \subseteq V(G)$ in the clustering they send all demand from $v \in C$ to the cluster center. On average, this operation both reduces the dispersion of the demand (we want the demand to be accumulated in a single node), and has an acceptable cost. However, in worst case, if a pair of close-together nodes $u, v$ are separated into different clusters (a low-probability event), the operation yields an unacceptably high cost for this pair. 
% Prior approaches address this issue by averaging the operation over a large number independently sampled clusters. On the other hand, we observe that if such a worst-case event happens, both nodes $u, v$ are extremely close to the cluster boundary. In motivates the following: a node close to the boundary only sends a small fraction of its demand to the cluster center.

% A quantitative version of these two ideas allow us to convert a sparse neighborhood cover for all distance scales to a $(\poly\log n)$-competitive oblivious routing matrix $R$ that can be efficiently evaluated using only minor-aggregations.


% Unfortunately, inherent barriers prevent low-diameter decomposition/sparse neighborhood cover-based approaches from achieving polylog-competitiveness 


%for all $O(\log n)$ exponentially-increasing distance scales. A sparse neighborhood cover of some distance scale $D$ is simply a .

%We develop this polylog-competitive $\ell_1$-oblivious routing by using (near-optimal) polylog-quality low-diameter decompositions (LDDs). A $\tilde{O}(1)$-quality low-diameter decomposition is a randomized partitioning of the nodes of $V$ into so-called \emph{clusters} of a specified radius $r$ such that two nodes $u, v$ are in different clusters with probability at most $\tilde{O}(1) \frac{\dist(u, v)}{r}$. Notably, we use a ``deterministic version'' of LDDs, namely sparse neighborhood covers; we mostly consider randomized approaches in this introductory discussion due to its relative simplicity. A randomized version of an LDD-based approach was considered in \cite{goranci2022universally}, but achieved only a $n^{o(1)}$-competitive routing. Moreover, many inherent barriers prevent an LDD-based approach from achieving polylog-competitiveness and we develop several new ideas described below to overcome them.

%For the purposes of this section, we pretend we have access to an oracle constructing polylog-quality LDDs (or sparse neighborhood covers). Note that this is also an important open problem which we solve concurrently using our local reduction framework described later.

%\underline{Idea 1: Remembering where the flows came from.}

%Oblivious routings generally work by taking a demand $b : V(G) \to R$ and judiciously intermixing it until, eventually, all demand is routed to some single node. This is a valid solution to the transshipment problem, albeit its competitiveness depends on the intermixing strategy. Note that sending a negative demand along a directed edge corresponds to sending a positive demand over the reversed edge.

% All current approaches to oblivious routing had the property that once two demand (i.e., flows) were merged in a single node during the intermixing, from this point on they were always routed together. Such strategies make the routing and the analysis simple: each intermixing step only depends on the demand vector given to it at the start, hence can be analyzed independently of other steps. For example, \cite{Li20} does a $\ell_1$-embedding based approach using $O(\log n)$ steps of intermixing, each blowing up the optimum by a multiplicative $(1 + 1 / \log n)$, yielding a polylog-competitive routing (in each step the current optimum is added to the solution). Similarly, \cite{goranci2022universally} does a LDD-based approach with $(\log n)^{1/4}$ steps of intermixing, each losing a $2^{\sqrt{\log n}}$ factor, hence yielding a $2^{(\log n)^{3/4}} = n^{o(1)}$-competitive routing. Unfortunately, all approaches that use LDDs and lose a polylog factor in each step (this is optimal) require at least $O(\frac{\log n}{\log \log n})$ steps, yielding only an (unusable) polynomially-competitive routing. This is a inherent barrier preventing LDDs-based approaches from being polylog-competitive.

% We overcome this barrier by remembering the origin of each flow. In other words, instead of simply remembering that, after an intermixing step, there is $b'_u$ flow at a node $u$, we remember that there is $b'_u(v)$ flow at $u$ that originated at node $v$. Therefore, each flow is treated differently based on its origin, making the flows splittable even after being aggregated at the same node. This idea, along with the next one, allows us to convert the multiplicative polylog-losses to additive ones, hence achieve a polylog-competitive routing.

% \underline{Idea 2: Reduce the outflow of nodes close to the boundary.}
% Consider the following natural intermixing step. Sample an LDD of (large) radius $r$, and send the entire demand of each node $v$ to the center of its cluster in the LDD. Let us examine how the demand $b := \mathbb{1}_u - \mathbb{1}_v$ supported on two nodes $u$ and $v$ at distance $\dist_G(u, v) = 1$ gets intermixed. If $u, v$ are in the same cluster, their demand gets merged and the new transshipment cost is $0$. On the other hand, if they end up in different clusters, the new transshipment cost grows by at most $+2r$, but this happens (by LDD properties) only with probability $\tilde{O}(1) \cdot \frac{1}{r}$. Therefore, in expectation the new transshipment cost grows by an (acceptable) polylog factor. However, in worst-case the cost grows by an (unacceptable) multiplicative $O(r)$, requiring the algorithm to average over $\tilde{O}(r)$ different LDDs until the blowup becomes acceptable. The key idea in the approach of is to gradually increase the radius \cite{goranci2022universally} by a $n^{o(1)}$ factor until a single cluster consumes the entire graph and the demand is consolidated in a single node. This gradual increase enables one to average only over $n^{o(1)}$ different LDD samples and achieve a worst-case guarantee, even when the radius is $\Omega(n)$.

% We, on the other hand, choose an approach that does not include a large number of repetitions to achieve worst-case guarantees. First, we note that if two very-close nodes $u$ and $v$ are not in the same cluster, then they are extremely close to the boundaries of their respective clusters. Our key idea is that nodes that are close to the boundary only send a small portion of their flow to the center of the LDD cluster. This allows us to repeat the LDD sampling until every node is far-away from the boundary in at least one sample, hence we repeat the sampling only $O(\log n)$ times.

% We now consider the intermixing strategy associated with a single LDD sample of radius $r$. Formally, let $b(u)$ the distance of $u$ to the boundary of $u$'s LDD cluster. The node $u$ will only send approximately $b(u) / r$ amount of flow to the center of the cluster (up to a polylog constant of proportionality which we ignore here). Therefore, since $\dist_G(u, v) = 1$, we know the difference in the flows sent by $u$ and $v$ to the some $r$-distant cluster center is at most $|b(u) - b(v)|/r \le 1/r$ (this is the amount we have to pay for), yielding a cost of at most $\tilde{O}(1)$ per LDD sample independent of the LDD radius. Of course, this only describes the routing in the first step. Later, as the radius of the LDD clusters increase, the flow that originated at $u$ (called $u$-associated flow) is already intermixed in various nodes, we generalize the strategy in the following way. Each node $w$ sends approximately $b(u) / r$-fraction of its incoming $u$-associated flow (from $w$) to the center of the LDD cluster \emph{containing the origin $u$} (note: $w$ is not considered here). Note that this idea crucially requires us to remember where the flow comes from. Again, it is easy to show that the cost per LDD is $\tilde{O}(1)$. After the LDD radius is exponentially increased for a logarithmic number of steps, the LDDs start consuming the entire graph and the entire demand is consolidated at a polylogarithmic cost, achieving a polylog-competitive routing (at least for $u, v$ at distance $1$, but also generally).

% \underline{Algorithmic remark.} 
% In addition to being extremely simple this new $\ell_1$-oblivious routing is also routing directly on the graph G and thus provides a linear $n \times m$ map $R$ which directly maps any node-demand to a $\tO(1)$-approximate transshipment flow in $G$. Moreover, the evaluations of this routing map $R$ can trivially be evaluated in near-linear time because it can be written as a product $R = A \times B$ of two sparse matrices $A$ and $B$. Here, $A$ maps each node to $\tO(1)$ paths and $B$ map each path to its edges, where each edge is used by at most $\tO(1)$ paths. These two sparse mappings can furthermore be directly read off in near-linear time if the $O(\log^2 n)$ LDDs and (approximate) distances of nodes to the LDD boundary are given.



% \alert{OLD}

% The first key contribution of this paper is a new graph-based $\ell_1$-oblivious routing with drastically improved guarantees. One way to look at this routing is following the idea of using probabilistic tree embeddings. For example, sampling $O(log n)$ hierarchical LDDs for each diameter $D_i = log^{2i} n$ with $i \in [\log n/2]$ one obtains $O(log^2 n)$ many Bartal-style probabilitstic tree embedding which are $O(log^3 n)$ approximate in expectation. Our $\ell_1$-oblivious routing can be seen as letting each node send its demand to the root of each of these $O(log^2 n)$ trees. Of course the well-known problem is that in each embedding every edge has a small probability of $\tO(1/n)$ that it is stretched by up to a factor of $n$ by a random embedding. However, for this a node has to be very close to the boundary of an LDD, indeed much closer than one should expect it to be for a random LDD. Furthermore, a node can immediately see in which of the tree embeddings such a potentially bad event happened. Lastly, since the probability for this is small most of the embeddings will be fine for every node. Intuitively speaking each node would like to only send demand in trees that are good for some chosen cut-off for goodness but this would result different nodes sending in different subset of trees. Instead our routing can be seen as defining a notion of goodness and simply sending in each tree demand proportional to its goodness. Our analysis shows that the closer any pair of nodes are the more related their goodness score is and that any loss in approximation of flows sent between them that are cause by differing goodness scores are proportional to the cost of the flow and thus do not decrease the approximation guarantee of the oblivious routing. On the other hand, this reweighting guarantees that any flow that is routed in an embedding between pairs that are highly overstretched is inversely proportional to this stretch due to a small goodness score and thus does not contributed much to the overall cost. 

% In addition to being extremely simple this new $\ell_1$-oblivious routing is also routing directly on the graph G and thus provides a linear $n \times m$ map $R$ which directly maps any node-demand to a $\tO(1)$-approximate transshipment flow in $G$. Moreover the evaluations of this routing map $R$ can trivially be evaluated in near-linear time because it can be written as a product $R = A \times B$ of two sparse matrices $A$ and $B$. Here, $A$ maps each node to $\tO(1)$ paths and $B$ map each path to its edges, where each edge is used by at most $\tO(1)$ paths. These two sparse mappings can furthermore be directly read of in near-linear time if the $O(log^2 n)$ LDDs and distances of nodes to the LDD boundary to compute the goodness scores are given.

% \textbf{Routing scheme.}

% \begin{itemize}

% \item For simplicity of exposition, we define a set of ``trivial clusters'' $\calS_0 := \bigcup_{v \in V(G\cheat_D)} \mathrm{TrivialCluster}(v)$, which contain exactly one node $v$ as its only member and its center (the padding is empty). Furthermore, let $c$ be the cheating node of $G\cheat_D$, and define $\calS_{L+1}$ to be a single cluster containing the entire $G\cheat_D$ in its core, with the cheating node as its center (and no padding). Note that the radius of this cluster is at most $D \le R_{L+1}$. This allows us to define $\calS := \bigcup_{\ell=0}^{L+1} \calS_\ell$ to be the set of clusters in our (extended) sparse neighborhood cover.
  
% \item We now describe a linear routing scheme on $G\cheat_D$ by describing the (unit) flow each node sends. A node $v$ sends a unit flow which we denote via $f(v) \in \mathbb{R}^{\vec{E}}$ and refer to it as the $v$-associated flow. The cheating node $c \in V(G\cheat_D)$ simply uses the trivial flow $f(c) = \vec{0}$, i.e., that leaves all of the demand in itself. For (non-cheating) nodes $v$, we specify $f(v)$ by specifying the amount of flow $f_{i, j}(v)$ that travels from the center of cluster $C_i \in \calS$ to another cluster center $C_j \in \calS$. Given $f_{i, j}(v)$ for all $C_i, C_j \in \calS$, we can convert the representation to $f(v)$ by choosing (an oriented) path $\Path_{i, j}$ between the centers (the path we specify later) and increasing the flow along each edge on the path by $f_{i, j}(v)$. Note that $\Path_{i, j}$ does not depend on $v$ (i.e., it is consistently chosen among different nodes).

%   \alert{did I handle the cheating node properly?}

% \item Consider a (non-cheating) node $v \in V(G)$. On a high-level, the $v$-associated flow first routes from $v$ (i.e., from $\calS_0$) to the centers of clusters $C \in \calS_1$ (i.e., on the first level), then to the centers of clusters $C \in \calS_2$ (on the second level), and so on until the centers of clusters $C \in \calS_\ell$. Finally, all available flow is routed from the centers of cluster in $\calS_\ell$ to the cheating node (i.e., the only cluster on level $L+1$).
  
% \item We now formally specify the $v$-associated flow. First, for each $\ell \in \{1, \ldots, L+1\}$, each cluster $C_i \in \calS_\ell$ that contains $v \in C_i$ computes a value $p_i(v)$ defined as the distance from $v$ to the closest node outside of $C_i$, divided by the radius of $C_i$. Furthermore, we define $w_\ell(v)$ as the sum of $p_i(v)$ over all clusters in $\calS_\ell$.
% \begin{align*}
%   p_i(v) :=   & \min\left( 1, \frac{\dist_G(v, V(G) \setminus C_i)}{R_\ell} \right) \\
%   w_\ell(v) := & \sum_{C_i \in \calS_\ell} p_i(v)
% \end{align*}

% The clusters $C_i$ that do not contain $v$ have $p_i(v) := 0$. In particular (this follows from the formula, but we make explicit for concreteness), on level $\ell=0$ we define $p_i(v) = 1$ when $C_i \in \calS_0$ is the trivial cluster containing $v$ and $p_i(v) = 0$ otherwise (hence $w_0(v) = 1$). On level $\ell = L+1$, we define $p_i(v) = 1$ if $C_i$ is the cluster containing all of $G\cheat_D$ (hence $w_{L+1}(v) = 1$).

% \item We now define $f_{ij}(v)$ to be the amount of flow we route from center of $C_i$ to the center of $C_j$ ($i, j$ range over the set of all clusters in the sparse neighborhood). Only flow from the previous level $\calS_{\ell}$ enters the next level $\calS_{\ell+1}$, hence $f_{ij} = 0$ unless $C_i \in \calS_\ell$ and $C_j \in \calS_{\ell+1}$. For each $\ell \in \{1, \ldots, L-1\}$ and each cluster $C_i \in \calS_\ell$, we split the flow entering the center of $C_i$ (from $\calS_{\ell-1}$) proportionally with respect to $p_j(v)$ and route the corresponding proportion to $C_j \in \calS_{\ell+1}$ (on the next level).
% \end{itemize}
 

{\bfseries Distance-reduction framework: Iterative and Locality-Friendly}\\
As we explained earlier, our new $\ell_1$-oblivious routing construction reduces the SSSP problem in $G$ to computing sparse neighborhood covers along with some extra distance information.
% Moreover, due to the reduction of outflow of nodes close to the boundary, each node is required to know (an approximate) distance to the boundary of its cluster.
Clearly, this requires our SSSP computation to compute some distance information, leading again to a chicken and egg problem. Unfortunately, directly applying the vertex-reduction framework is not compatible with our desire to obtain fast minor-aggregation (or distributed) algorithms. In particular, at the lowest level of the recursion, the vertex-reduction framework generates a polynomial number of constant-size SSSP problems, each of which essentially corresponds to a minor of $G$. While these problems can each be solved in constant time in the parallel setting, the fact that these minors can be arbitrarily overlapping and each correspond to large diameter subsets in $G$ means that polynomially many instead of the desired polylogarithmic number of minor aggregations are necessary.

This paper therefore designs a novel, completely different, and more locality-friendly complexity-reduction framework: \emph{distance reduction}. On a high-level, we show that obtaining ``sparse neighborhood covers up to distance scale $D$'' can be reduced to several ``shortest path computations up to distance $D$'' which are computable from ``sparse neighborhood covers up to distance $D/\poly\log n$'' (see \cref{fig:main}). 
This iterative and local nature of our distance-reduction framework directly translates into a small overall number of minor aggregations; this is in stark contrast to the inherently recursive vertex-reduction framework (which recurses on different graphs, requiring a recursive approach).
As a nice little extra, combining our distance-reduction framework with the new $\ell_1$-embedding makes for an algorithm that is (in our not exactly unbiased opinion) a good bit simpler than the previous algorithms of \cite{Li20,AndoniSZ20}. 
We note that this framework is more reminiscent of older approaches to hopset constructions~\cite{cohen1994polylog, EN16}. In these approaches, hopsets over longer paths which use at most $\ell / 2$ edges are used to bootstrap the construction of hopsets over paths using at most $\ell$ edges.

%Specifically, it removes not just the two sparsification procedures used for the vertex-reduction itself but also gets rid of other steps in the vertex-reduction framework that seem hard\todo{are they? the clustering approach to bourgain embedding needs distance only up to scale D} to derandomize, including Bourgain's $\ell_1$-embedding.

A key definition to formalize what exactly the ``up to distance $D$'' in our distance-reduction framework means is the following. We attach a virtual, so-called, \emph{cheating node} and connect it to all other nodes with an edge of length $D$. This new graph naturally preserves distance information ``up to distance $D$'' and the complexity of computing distances increases as $D$ increases.

%The formal definition of ``shortest path structures up to distance $D$'' in our framework can be found in \Cref{sec:bla} and corresponds to a family of $O(\log n)$ representative LDDs for each scale up to $D$ together with distance information for each node about their distance to the boundary to its cluster in each of the LDDs. This is exactly what is needed for our $\ell_1$-oblivious routings and we show that such a distance structure is sufficient to compute SSSP soluations in $G_{D,S}$ for any set $S$. 

% Figure 2 gives a summary of our iterative local complexity-reduction framework:

% A representative set of $O(log n)$  LDDs and their boundary distances in G for distance $D$

% can be computed using polylog n SSSP problems in $G_{D,S_i}$ for different sets $S_i$

% (1+eps)-SSSP on $G_{D,S}$ for polylogarithmically many $S$

% can be computed via log n calls to TS and a rounding procedure. Each TS problem on some $G_{D,S}$ can be answered using an $\ell_1$-oblivious routing matrix of for $G_{D,S}$  (this is the boosting framework)

% $O(log^6 n)$-approx $\ell_1$-oblivious routing matrix for graphs $G_{D,S}$ for polylogarithmically many $S$ 

% we show that a distance structure for distance $D/log^2 n$, i.e., sets of LDDs for distances in $G$ up to distance $D/log^2 n$ are sufficient to generate the $\ell_1$-oblivious routing matrix for $G_{D,S}$ for any $S$. 

% representative set of $O(log n)$  LDDs and their boundary distances in G for any distance $D_i = 2^{i}$ for integer $i$ with $D_i \leq D/2$


{\bfseries Derandomization: Deterministic Transshipment Flow Rounding via Eulerian Tours}\\
All previous transshipment approaches crucially use randomization. The most significant challenge we had to overcome in making our results deterministic stem from the following issue: The only problem that remains to be derandomized in this paper is \emph{rounding} a (fractional) transshipment solution to (a flow supported on) a tree, a crucial step in the distance-reduction framework. We prove the following theorem (only the parallel version is stated for simplicity). 

%The above two tools give a randomized reduction of the $(1+\eps)$-SSSP problem to polylogarithmically many minor aggregates. It remains to give a derandomization. Fortunately, our new framework has eliminated the $\ell_1$-embedding and the two sparsification steps. 
%We also do not need to develop any new ideas for computing sparse neighborhood covers deterministically but can use generalizations of the recent algorithms \cite{rozhon_ghaffari2019decomposition,ghaffari_grunau_rozhon2020improved_network_decomposition,chang_ghaffari2021strong_diameter} developed for unweighted graphs.% \todo{drop blurry ball growing citation somewhere \cite{becker2019low}}
%to weighted graph clusterings~\footnote{In this paper we only require a particularly simple variant of the clusterings given in \cite{} except that one needs some additional care to only use shortest paths computations in $G$ without any changes to its structure to preserve the iterative nature of our reduction framework. This is a special requirement which is not very natural outside the context of this paper and not easily addressed by the powerful general clustering method for weighted graphs given in \cite{}. For sake of clarity and completeness we therefore make this paper self-contained and provide the simplified clustering algorithm used in this paper in Appendix bla}. 

\begin{theorem}\label{thm:eulerrounding-intro}
There is a deterministic parallel algorithm which takes as an input any fractional transshipment flow $f$ satisfying some single-source transshipment demand $b$ in the graph $G$ and in near-linear work and polylogarithmic time outputs a flow $f'$ of equal or smaller cost which is supported on some tree in $G$.
\end{theorem}

While such a flow rounding seems an unlikely bottleneck for a deterministic SSSP algorithm, we remark that even for randomized algorithms a lot of complexity has come from this rounding step in the algorithms of \cite{Li20, AndoniSZ20, BKKL17}---all these approaches are based on random walks and are inherently randomized.

%Moreover, in the recent paper by Andoni, Stein, and Zhong~\cite{AndoniSZ20}, the lack of such a rounding procedure is the only reason why only $s$-$t$ shortest paths can be computed and not SSSP trees. However, this extension was later provided in Zhong's thesis~\cite{zhong2021new}.

Note that if the fractional flow $f$ is acyclic (has no \emph{directed} cycles), then there is a trivial randomized rounding which simply samples one outgoing edge for each node in $G$ through which flow is routed, choosing the probability of each edge proportional to the outflow in $f$. It is easy to see that retaining the edges that are in the connected component of the source truthfully samples a tree-supported flow from $f$. The complexity comes in once $f$ is not acyclic as the sampled edges can now create many connected components. This requires finding the cycles in these components, contracting the edges and again running a randomized out-edge sampling on the remaining graph. 

Deterministically none of the above works. Indeed, we are not aware of any simple(r) way of deterministically obtaining a tree-supported flow even if $f$ is acyclic. Our rounding procedure can be seen as a generalization of an algorithm of Cohen's rounding~\cite{cohen1995approximateMaxFlow}, which can be used to round any fractional transshipment flow to an integral flow by scaling flow values to only leave integral and half-integral flow values and then finding an Eulerian tour covering all half-integral edges. Pushing one half-unit of flow in the cheaper direction of this Eulerian tour makes all flow values fully integral and allows the scaling to be reduced. At the end of this procedure, all flow values are integral but this does not guarantee that the flow is supported on a tree. To eliminate any non-tree like parts of the flow we show how to keep the algorithm running and find further Eulerian tours until the flow becomes tree-supported. 

{\bfseries A Distributed Eulerian Tour Algorithm}\\
The problem of computing Eulerian Tours can be stated as follows. Given an undirected graph with all degrees even, direct the edges in such a way that the out-degree of every node equals the in-degree. Note that we do not require connectedness. While computing Eulerian tours is a well-known parallel primitive which can be efficiently computed in near-linear work and polylogarithmic time \cite{atallah_vishkin1984euler_pram}, there are, to our knowledge, no distributed algorithms known for this problem. 

Therefore, to also give \emph{distributed} SSSP algorithms in this paper we need to design efficient distributed Eulerian-tour algorithms that can then be used in the Eulerian-tour-based rounding procedure of \Cref{thm:eulerrounding-intro}.  We build the first algorithm computing such an Eulerian tour orientation by using algorithms from \cite{parter_yogev2019cycle_covers_minor_closed,parter_yogev2019cycle_decomp_near_linear} for low-congestion cycle covers. Interestingly, these low-congestion cycle covers were only developed for the completely unrelated purpose of making distributed computation resilient to Byzantine faults introduced by an adversary in a recent line of work \cite{parter_yogev2019cycle_covers_minor_closed,parter_yogev2019cycle_decomp_near_linear,hitron_parter2021adversarial_compilers,hitron2021broadcast}. 

\begin{theorem}[Informal]\label{thm:euler-intro}
There is a deterministic \congest algorithm which, given any Eulerian subgraph $H$ of the network $G$ as an input, computes an Eulerian tour orientation in $\tO(\sqrt{n} + \Dhop)$ rounds or $\tO(\Dhop)$ rounds if $G$ is an excluded-minor graph. %Here, $\Dhop$ is the hop diameter of $G$. % using sublinear number of \congest rounds and minor aggregates. 
%There also exists a deterministic \congest algorithm which computes an Eulerian tour orientation of any Eulearian subgraph of an $n$-node graph $G$ with hop diameter $D$ in $\tO(\sqrt{n} + D)$ rounds or $\tO(D)$ rounds if $G$ is an exluded-minor graph. 
\end{theorem}

The most general and fully formal statements of all results proven in this paper are given in \Cref{sec:main_theorems}.

% Local Variables:
% TeX-master: "main"
% End:



==> l1-Oblivious_Routing.tex <==
\section{$\ell_1$-Oblivious Routing with $\tilde{O}(1)$ Competitiveness and Evaluation Time via Sparse Neighborhood Covers}\label{sec:l1-oblivious-routing}

In this section, we prove our main result, an efficient $\ell_1$-oblivious routing in the distributed setting. We first give an overview of the new ideas required to overcome the barriers present in all previously known approaches, and then present a formal construction and proofs in \Cref{sec:routing-formal}.

\subsection{An Overview of New Ideas}\label{sec:routing-overview}

The first key contribution of this paper is a new graph-based $\ell_1$-oblivious routing with drastically improved guarantees. In order to simplify the discussion, in this overview we will explain the ideas from a randomized (low-diameter decomposition) perspective, rather than a deterministic (sparse neighborhood covers) one.

We develop this polylog-competitive $\ell_1$-oblivious routing by using (near-optimal) polylog-quality low-diameter decompositions (LDDs). A $\tilde{O}(1)$-quality low-diameter decomposition is a randomized partitioning of the nodes of $V$ into so-called \emph{clusters} of a specified radius $r$ such that two nodes $u, v$ are in different clusters with probability at most $\tilde{O}(1) \frac{\dist(u, v)}{r}$. Notably, we use a ``deterministic version'' of LDDs, namely sparse neighborhood covers; we mostly consider randomized approaches in this introductory discussion due to its relative simplicity. A randomized version of an LDD-based approach was considered in \cite{goranci2022universally}, but achieved only a $n^{o(1)}$-competitive routing. Moreover, many inherent barriers prevent an LDD-based approach from achieving polylog-competitiveness and we develop several new ideas described below to overcome them.

For the purposes of this section, we pretend we have access to an oracle constructing polylog-quality LDDs (or sparse neighborhood covers). Note that this is also an important open problem which we solve concurrently using our locality-friendly reduction framework from \cref{sec:localiterative}.

\underline{Idea 1: Remembering where the flows came from.}

Oblivious routings generally work by taking a demand $b : V(G) \to R$ and judiciously intermixing it until, eventually, all demand is routed to some single node. This is a valid solution to the transshipment problem, albeit its competitiveness depends on the intermixing strategy. Note that sending a negative demand along a directed edge corresponds to sending a positive demand over the reversed edge.

All current approaches to oblivious routing had the property that once two demand (i.e., flows) were merged in a single node during the intermixing, from this point on they were always routed together. Such strategies make the routing and the analysis simple: each intermixing step only depends on the demand vector given to it at the start, hence can be analyzed independently of other steps. For example, \cite{Li20} does a $\ell_1$-embedding based approach using $O(\log n)$ steps of intermixing, each blowing up the optimum by a multiplicative $(1 + 1 / \log n)$, yielding a polylog-competitive routing (in each step the current optimum is added to the solution). Similarly, \cite{goranci2022universally} does a LDD-based approach with $(\log n)^{1/4}$ steps of intermixing, each losing a $2^{\sqrt{\log n}}$ factor, hence yielding a $2^{(\log n)^{3/4}} = n^{o(1)}$-competitive routing. Unfortunately, all approaches that use LDDs and lose a polylog factor in each step (this is optimal) require at least $O(\frac{\log n}{\log \log n})$ steps, yielding only an (unusable) polynomially-competitive routing. This is a inherent barrier preventing LDDs-based approaches from being polylog-competitive.

We overcome this barrier by remembering the origin of each flow. In other words, instead of simply remembering that, after an intermixing step, there is $b'_u$ flow at a node $u$, we remember that there is $b'_u(v)$ flow at $u$ that originated at node $v$. Therefore, each flow is treated differently based on its origin, making the flows splittable even after being aggregated at the same node. This idea, along with the next one, allows us to convert the multiplicative polylog-losses to additive ones, hence achieve a polylog-competitive routing.

\underline{Idea 2: Reduce the outflow of nodes close to the boundary.}
Consider the following natural intermixing step. Sample an LDD of (large) radius $r$, and send the entire demand of each node $v$ to the center of its cluster in the LDD. Let us examine how the demand $b := \mathbb{1}_u - \mathbb{1}_v$ supported on two nodes $u$ and $v$ at distance $\dist_G(u, v) = 1$ gets intermixed. If $u, v$ are in the same cluster, their demand gets merged and the new transshipment cost is $0$. On the other hand, if they end up in different clusters, the new transshipment cost grows by at most $+2r$, but this happens (by LDD properties) only with probability $\tilde{O}(1) \cdot \frac{1}{r}$. Therefore, in expectation the new transshipment cost grows by an (acceptable) polylog factor. However, in worst-case the cost grows by an (unacceptable) multiplicative $O(r)$, requiring the algorithm to average over $\tilde{O}(r)$ different LDDs until the blowup becomes acceptable. The key idea in the approach of \cite{goranci2022universally} is to gradually increase the radius by an $n^{o(1)}$ factor until a single cluster consumes the entire graph and the demand is consolidated in a single node. This gradual increase enables one to average only over $n^{o(1)}$ different LDD samples and achieve a worst-case guarantee, even when the radius is $\Omega(n)$.

We, on the other hand, choose an approach that does not include a large number of repetitions to achieve worst-case guarantees. First, we note that if two very-close nodes $u$ and $v$ are not in the same cluster, then they are extremely close to the boundaries of their respective clusters. Our key idea is that nodes that are close to the boundary only send a small portion of their flow to the center of the LDD cluster. This allows us to repeat the LDD sampling until every node is far-away from the boundary in at least one sample, hence we repeat the sampling only $O(\log n)$ times.

We now consider the intermixing strategy associated with a single LDD sample of radius $r$. Formally, let $d(u)$ the distance of $u$ to the boundary of $u$'s LDD cluster. The node $u$ will only send approximately $d(u) / r$ amount of flow to the center of the cluster (up to a polylog constant of proportionality which we ignore here). Therefore, since $\dist_G(u, v) = 1$, we know the difference in the flows sent by $u$ and $v$ to the some $r$-distant cluster center is at most $|d(u) - d(v)|/r \le 1/r$ (this is the amount we have to pay for), yielding a cost of at most $\tilde{O}(1)$ per LDD sample independent of the LDD radius. Of course, this only describes the routing in the first step. Later, as the radius of the LDD clusters increase, the flow that originated at $u$ (called $u$-associated flow) is already intermixed in various nodes, we generalize the strategy in the following way. Each node $w$ sends approximately $d(u) / r$-fraction of its incoming $u$-associated flow (from $w$) to the center of the LDD cluster \emph{containing the origin $u$} (note: $w$ is not considered here). Note that this idea crucially requires us to remember where the flow comes from. Again, it is easy to show that the cost per LDD is $\tilde{O}(1)$. After the LDD radius is exponentially increased for a logarithmic number of steps, the LDDs start consuming the entire graph and the entire demand is consolidated at a polylogarithmic cost, achieving a polylog-competitive routing (at least for $u, v$ at distance $1$, but also generally).

\underline{Algorithmic remark.} 
In addition to being extremely simple this new $\ell_1$-oblivious routing is also routing directly on the graph G and thus provides a linear $n \times m$ map $R$ which directly maps any node-demand to a $\tO(1)$-approximate transshipment flow in $G$. Moreover, the evaluations of this routing map $R$ can trivially be evaluated in near-linear time because it can be written as a product $R = A \times B$ of two sparse matrices $A$ and $B$. Here, $A$ maps each node to $\tO(1)$ paths and $B$ map each path to its edges, where each edge is used by at most $\tO(1)$ paths. These two sparse mappings can furthermore be directly read off in near-linear time if the $O(\log^2 n)$ LDDs and (approximate) distances of nodes to the LDD boundary are given.

\subsection{Formal Construction of the Routing}\label{sec:routing-formal}




\begin{theorem}
\label{thm:oblivious_routing}
Let $G$ be a weighted graph. Assume a distance-structure for every scale $D_j, j < i$ is given.
Then, for a given set $S \subseteq V(G)$, there exists a $\textup{poly}(\log n)$-competitive $\ell_1$-oblivious routing $R$ for $G_{S,D_i}$ such that we can compute matrix-vector products with $R$ and $R^T$ in $\textup{poly}(\log n)$ \aggregate rounds in $G$. \\
Moreover, if $\beta^{i-1}/\valSNC$ is greater than the diameter of $G$, then there exists a $\textup{poly}(\log n)$-competitive $\ell_1$-oblivious routing $R$ for $G$ such that we can compute matrix-vector products with $R$ and $R^T$ in $\textup{poly}(\log n)$ \aggregate rounds in $G$.
\end{theorem}


\textbf{Extending the sparse covers to $G_{S,D_i}$.} For each $j<i$, consider the sparse neighborhood cover of $G$ from the distance-structure for distance $D_j$. Recall from \Cref{def:distance_structure} that it has covering radius $D_j/\valSNC$. Extend it to a sparse neighborhood cover of $G_{S,D_i}$ by letting $v_{D_i}$ and $s^*$ each be a singleton component, and name the new sparse neighborhood cover $\mathcal S_j$. We now claim that it still has covering radius $D_j/\valSNC$, this time on $G_{S,D_i}$. Since $D_j/\valSNC<D_i$, and since $v_{D_i}$ and $s^*$ have distance at least $D_i$ to all other nodes, the ball around any node $v\in V$ does not contain $v_{D_i}$ or $s^*$, so it is still fully contained in some cluster. The balls around $v_{D_i}$ and $s^*$ are simply the singleton sets $\{v_{D_i}\}$ and $\{s^*\}$, respectively, so they are also covered by their respective singleton clusters. It follows that the new sparse neighborhood cover has covering radius $D_i\ge D_i/\valSNC$. As for the potentials, we simply define $\tilde d_{\{v_{D_i}\}}(v_{D_i})=D_i$ and $\tilde d_{\{s^*\}}(s^*)=D_i$ for the clusters $\{v_{D_i}\}$ and $\{s^*\}$, respectively. These clearly satisfy \Cref{def:potential}.

Let $\mathcal S_i$ be the sparse neighborhood cover consisting of the entire graph $G_{S,D_i}$ as a single cluster $V'$, which has radius $2 D_i$ when centered at $v_{D_i}$. Let spanning tree of the cluster be the star centered at $v_{D_i}$ with leaves $V$, with $s^*$ attached to an arbitrary leaf node. We can trivially define $\tilde d_{V'}(v)=D_i$ for all $v\in V'$, which satisfies \Cref{def:potential} (where property~(1) is vacuously satisfied since there are no nodes outside the cluster).

\textbf{Notation.} For each clustering $\mathcal C$ in some sparse neighborhood cover $\mathcal S_j$, let $\tilde d_C$ be the corresponding distance label. For each cluster $C$ in some clustering, let $r_C$ be the cluster center, and let $T_C$ be the cluster spanning tree rooted at $r_C$ of radius at most $\alpha D_j$. Let $\gamma:=O(\log n)$ be an upper bound on the number of clusters in each clustering as guaranteed by Definition~\ref{def:distance_structure}. Furthermore, to avoid clutter, define $V':=V\cup\{v_{D_i},s^*\}$ as the vertices of $G_{S,D_i}$.

For each node $v\in V'$, integer $j<i$, and cluster $C$ containing $v$ that is in some clustering $\mathcal C\in\mathcal S_j$, define the value $p_{C}(v):=\max\{0,\tilde d_C(v)/D_j-0.25/\valSNC\}$, and for each $j<i$, define $w_j(v):=\sum_{C\in\mathcal C\in\mathcal S_j}p_{C}(v)$. 

\begin{lemma}\label{lem:w-lower-bound}
For all $j<i$, we have $w_\ell(v)\ge0.25/\valSNC$.
\end{lemma}
\begin{proof}
Since $\mathcal S_j$ is a sparse neighborhood cover of quality $\valSNC$, there exists a clustering $\mathcal C\in\mathcal S_j$ such that the ball around $v$ of radius $D_j/\valSNC$ is contained inside some cluster $C$ in $\mathcal C$. Equivalently, the distance of $v$ to a node outside $C$ is more than $D_j/\valSNC$. By property~(ii) of the definition of $\tilde d_C(v)$ (see Definition~\ref{def:distance_structure}), we have $\tilde d_C(v)\ge0.5D_j/\valSNC$. It follows that $w_j(v)\ge p_{C}(v)\ge\tilde d_C(v)/D_j-0.25/\valSNC\ge0.5/\valSNC-0.25/\valSNC=0.25/\valSNC$.
\end{proof}

We now describe the oblivious routing flow ``associated'' with each node $v\in V'$; the overall oblivious routing is simply the sum of the flows on each node $v$ multiplied by the demand at $v$.

The $v$-associated flow sends, for each $j<i$, and clusters $C\in\mathcal C\in\mathcal S_j$ and $C'\in \mathcal C'\in\mathcal S_{j+1}$ both containing $v$, a flow from the center $r_C$ to the center $r_{C'}$, and the amount of flow is $f_{C,C'}(v):=(p_{C}(v)/w_j(v))\cdot(p_{C'}(v)/w_{j+1}(v))$. (We do not yet specify the path from $r_C$ to $r_{C'}$ along which the flow is sent.) Over a single level $j$, the flow can be viewed as a ``product flow'' among all clusters $C$ in $\mathcal S_j$ and $C'$ in $\mathcal S_{j+1}$ containing $v$, weighted proportionally to $p_{C}(v)$ and $p_{C'}(v)$, respectively.

\begin{figure}
    \centering
    \includegraphics[width = .6\textwidth]{fig/routing.eps}
    \caption{Example of the first two levels of the oblivious routing under construction. The node $v$ is deep enough in two clusters $C_1, C_2$ in the sparse neighborhood cover $\mathcal{S}_1$ to send flow to their centers $r_{C_1}, r_{C_2}$. 
    There are two clusters $C'_1, C'_2$ in the cover $\mathcal{S}_2$ where $v$ is deep enough to send flow to their centers. The flow is sent from $r_{C_1}$ and $r_{C_2}$ and the amount of flow sent follows the product distribution $f_{C, C'}(v) \propto p_C(v) p_{C'}(v)$. Note that by \cref{obs:C-inside} we have $C_1 \cup C_2 \subseteq C'_1 \cap C'_2$. }
    \label{fig:routing}
\end{figure}

\begin{claim}\label{obs:flow-conservation}
For each $v\in V'\setminus\{v_{D_i}\}$, the $v$-associated flow sends $1$ unit of net flow out of $v$, $1$ unit of net flow into the virtual node $v_{D_i}$, and zero net flow into/out of any other node. The $v_{D_i}$-associated flow has zero net flow into/out of every node.
\end{claim}
\begin{proof}
Fix any node $v\in V'$. Since $\sum_{C\in\mathcal C\in\mathcal S_j}p_{C}(v)/w_j(v)=1$ for all $j$, it is easy to see that each node $v$ receives exactly $p_{C}(v)/w_j(v)$ total flow from level $j-1$ and sends exactly $p_{C}(v)/w_j(v)$ total flow to level $j+1$, which is a net flow of zero. This also means that for $j=1$, the node $v$ sends $1$ unit of flow out. Finally, since $\mathcal S_i$ has a single cluster with center $v_{D_i}$, all flow eventually coalesces at node $v_{D_i}$. This means that if $v\ne v_{D_i}$, then the flow sends $1$ unit out of $v$ and $1$ unit into $v_{D_i}$, and if $v=v_{D_i}$, then the two units of flow cancel, and the net flow is zero on every node.
\end{proof}

\begin{claim}\label{obs:C-inside}
We have $f_{C,C'}(v)\ne0$ only if $C\subseteq C'$.
\end{claim}
\begin{proof}
The claim is vacuous for $j=i-1$ since $\mathcal S_i$ has a single cluster of all the nodes, so assume that $j<i-1$. If $f_{C,C'}(v)\ne0$ then in particular, $p_{C'}(v)=\max\{0,\tilde d_{C'}(v)/D_{j+1}-0.25/\valSNC\}>0$, which implies that $\tilde d_{C'}(v)\ge 0.25D_{j+1}/\valSNC$. Since $\tilde d_{C'}$ is a potential with respect to $V'\setminus C'$, by properties~(1)~and~(2) of Definition~\ref{def:potential}, we have $\dist_G(v,V'\setminus C')\ge\tilde d_{C'}(v)\ge0.25D_{j+1}/\valSNC$. In other words, $v$ has distance at least $0.25D_{j+1}/\valSNC$ to the outside of cluster $C'$. Since $\valSNC\le\beta/8$ by construction, this distance is at least $2D_{j+1}/\beta=2D_j$. Since $C$ is a cluster of radius at most $D_j$, node $v$ has distance at most $2D_j$ to all of $C$, and it follows that $C\subseteq C'$. 
\end{proof}

The following lemma is key to bounding the competitive ratio of the oblivious routing algorithm.
\begin{lemma}\label{lem:flow-uv-diff}
Fix two nodes $u,v\in V'$. For every $j<i$ and two clusters $C\in\mathcal C\in\mathcal S_j$ and $C'\in\mathcal C'\in\mathcal S_{j+1}$, we have $|f_{C,C'}(u)-f_{C,C'}(v)|\le O(\gamma \valSNC d_G(u,v)/D_j)$.
\end{lemma}
\begin{proof}
Consider some $j<i$ and clusters $C\in\mathcal C\in\mathcal S_j$ and $C'\in \mathcal C'\in\mathcal S_{j+1}$.
To avoid clutter, let $d:=\dist_G(u,v)$ and $\delta:=\dist_G(u,v)/D_j$.
 The claim is trivial if $\delta\ge1/(\gamma \valSNC)$ since $f_{C,C'}(u),f_{C,C'}(v)\in[0,1]$ by construction. For the rest of the proof, assume that $\delta\le1/(\gamma \valSNC)$. It suffices to prove $f_{C,C'}(u)-f_{C,C'}(v)\le O(\gamma \valSNC d_G(u,v)/D_j)$ without the absolute value, since we can swap $u$ and $v$ to obtain the other direction.

By property~2(ii) of Definition~\ref{def:distance_structure}, both $|\tilde d_C(u)-\tilde d_C(v)|$ and $|\tilde d_{C'}(u)-\tilde d_{C'}(v)|$ are at most $d$, so both $|p_{C}(u)-p_{C}(v)|$ and $|p_{C'}(u)-p_{C'}(v)|$ are at most $d/D_j=\delta$. Since $w_j(v)=\sum_{C''\in\mathcal C''\in\mathcal S_j}p_{C''}(v)$ is the sum of at most $\gamma$ many terms, we have $|w_j(u)-w_j(v)|\le\gamma\delta$. Similarly, $|w_{j+1}(u)-w_{j+1}(v)| \le \gamma d/D_{j+1} \le \gamma d/D_j= \gamma\delta$. Therefore,
\begin{align*}
&f_{C,C'}(u)-f_{C,C'}(v)
\\&= \frac{p_{C}(v)}{w_j(v)}\cdot\frac{p_{C'}(v)}{w_{j+1}(v)} - \frac{p_{C}(u)}{w_j(u)}\cdot\frac{p_{C'}(u)}{w_{j+1}(u)}
\\&= \frac{p_{C}(v)p_{C'}(v)w_j(u)w_{j+1}(u) - p_{C}(u)p_{C'}(u)w_j(v)w_{j+1}(v)}{w_j(v)w_{j+1}(v)w_j(u)w_{j+1}(u)}
\\&\le \frac{p_{C}(v)p_{C'}(v)(w_j(v)+\gamma \delta)(w_{j+1}(v)+\gamma\delta) - (p_{C}(v)-\delta)(p_{C'}(v)-\delta)w_j(v)w_{j+1}(v)}{w_j(v)w_{j+1}(v)w_j(u)w_{j+1}(u)}
%\\&\le \frac{p_{C}(v)p_{C'}(v)(w_j(v)w_{j+1}(v)+\gamma\delta(w_j(v)+w_{j+1}(v))+(\gamma\delta)^2) - (p_{C}(v)-\delta)(p_{C'}(v)-\delta)w_j(v)w_{j+1}(v)}{w_j(v)w_{j+1}(v)w_j(u)w_{j+1}(u)}
.
\end{align*}
Expanding out the numerator and canceling out the $p_{C}(v)p_{C'}(v)w_j(v)w_{j+1}(v)$ terms, we obtain
\begin{align*}
&p_{C}(v)p_{C'}(v)(w_j(v)w_{j+1}(v)+\gamma\delta w_j(v)+\gamma\delta w_{j+1}(v)+(\gamma\delta)^2) 
\\&\quad-(p_{C}(v)p_{C'}(v)-\delta p_C(v)-\delta p_{C'}(v)+\delta^2)w_j(v)w_{j+1}(v) 
\\={}&  p_{C}(v)p_{C'}(v)(\gamma\delta w_j(v)+\gamma\delta w_{j+1}(v)+(\gamma\delta)^2) + (\delta p_C(v)+\delta p_{C'}(v)-\delta^2)w_j(v)w_{j+1}(v).
\end{align*}
Using that $p_{C}(v)\le w_j(v)$ and $p_{C'}(v)\le w_{j+1}(v)$, and ignoring the last $-\delta^2$ term, this is at most
\begin{align*}
&w_j(v)w_{j+1}(v)(\gamma\delta w_j(v)+\gamma\delta w_{j+1}(v)+(\gamma\delta)^2) + (\delta w_j(v)+\delta w_{j+1}(v))w_j(v)w_{j+1}(v) 
\\={}& w_j(v)w_{j+1}(v)((\gamma+1)\delta w_j(v)+(\gamma+1)\delta w_{j+1}(v)+(\gamma\delta)^2)
\end{align*}
Dividing by the denominator $w_j(v)w_{j+1}(v)w_j(u)w_{j+1}(u)$ and then using $|w_j(u)-w_j(v)|\le\gamma\delta$ and $|w_{j+1}(u)-w_{j+1}(v)|\le\gamma\delta$, we upper bound $f_{C,C'}(u)-f_{C,C'}(v)$ by
\begin{align*}
&\frac{(\gamma+1)\delta w_j(v)+(\gamma+1)\delta w_{j+1}(v)+(\gamma\delta)^2}{w_j(u)w_{j+1}(u)}
\\\le{}& \frac{(\gamma+1)\delta (w_j(u)+\gamma\delta)+(\gamma+1)\delta(w_{j+1}(u)+\gamma\delta)+(\gamma\delta)^2}{w_j(u)w_{j+1}(u)} \\\le{}& \frac{(\gamma+1)\delta w_j(u)+(\gamma+1)\delta w_{j+1}(u)+O(\gamma\delta)^2}{w_j(u)w_{j+1}(u)}
\\={}&\frac{(\gamma+1)\delta}{w_{j+1}(u)} + \frac{(\gamma+1)\delta}{w_j(u)} + \frac{O(\gamma\delta)^2}{w_j(u)w_{j+1}(u)}
.\end{align*}
Finally, using that $w_j(u),w_j(v)\ge0.25/\valSNC$ from \Cref{lem:w-lower-bound}, this is at most $O(\gamma \valSNC\delta+(\gamma \valSNC\delta)^2)$. Since $\delta\le1/(\gamma \valSNC)$, the linear term dominates, and we obtain the desired $f_{C,C'}(u)-f_{C,C'}(v)\le O(\gamma \valSNC\delta)$.
\end{proof}

\begin{lemma}\label{lem:competitive-ratio-final}
Assume that $\valSNC\le\beta/8$.
For any demand vector $b:\mathbb R^{V'}$ for the graph $G_{S,D_i}$, the summation
\begin{align*}
    \sum_{j<i}\sum_{\substack{C\in\mathcal C\in\mathcal S_j,\\C'\in\mathcal C'\in\mathcal S_{j+1}}}\bigg| \sum_{v\in V'}b(v)f_{C,C'}(v) \bigg|\cdot D_j
\end{align*}  is at most $i\gamma^3\valSNC$ times the optimal cost of a transshipment flow on $G_{S,D_i}$ satisfying demand $b$. 
\end{lemma}
\begin{proof}
Decompose the optimal transshipment flow into a collection $\mathcal P$ of paths. Fix a path with endpoints $u,v$ of flow value $F$, which contributes cost $F\cdot d_G(u,v)$ to the transshipment solution. For any $j<i$, there are at most $\gamma^2$ pairs $(\mathcal C,\mathcal C')$ with $\mathcal C\in\mathcal S_j$ and $\mathcal C'\in\mathcal S_{j+1}$, and for each $(\mathcal C,\mathcal C')$, there are at most two pairs $(C,C')$ with $C\in\mathcal C$ and $C'\in\mathcal C'$ for which either $f_{C,C'}(u)$ or $f_{C,C'}(v)$ is nonzero: these are the pairs $C,C'$ that either both contain $u$ or both contain $v$. So the total summation of $F\cdot |f_{C,C'}(u)-f_{C,C'}(v)|\cdot D_j$ from level $j$ is $O(\gamma^3\valSNC d_G(u,v))\cdot F$ by \Cref{lem:flow-uv-diff}. There are $i-1$ levels for a total of $O(i\gamma^3\valSNC d_G(u,v))\cdot F$, which we charge to the cost $F\cdot d_G(u,v)$ in the transshipment solution. It follows that $\sum_{u,v,F}\sum_{C,C'}F\cdot|f_{C,C'}(u)-f_{C,C'}(v)|\cdot D_j$ is at most $O(i\gamma^3\valSNC d_G(u,v))$ times the transshipment cost, so it remains to relate this summation to the desired $\sum_{C,C'}|\sum_{v\in V}b(v)f_{C,C'}(v)|\cdot D_j$.

 Summing over all paths in $\mathcal P$, we obtain 
\begin{align}
\sum_{u,v,F}\sum_{C,C'}F\cdot|f_{C,C'}(u)-f_{C,C'}(v)|\cdot D_j &\ge \sum_{C,C'}\left| \sum_{u,v,F}F\cdot(f_{C,C'}(u)-f_{C,C'}(v)) \right|\cdot D_j.\label{eq:comp-ratio}
\end{align}
Since the paths in $\mathcal P$ together form a transshipment solution that satisfies demand $b$, the sum of $F\cdot(\mathbbm1_u-\mathbbm1_v)$ over all paths in $\mathcal P$ (with endpoints $u,v$ and flow $F$) is exactly the demand vector $b$. That is, $\sum_{u,v,F}F\cdot(\mathbbm1_u-\mathbbm1_v)=b$ as vectors. Multiplying each vector coordinate $v$ by $f_{C,C'}(v)$ for any $C,C'$ and then summing over all coordinates, we obtain $\sum_{u,v,F}F\cdot(f_{C,C'}(u)-f_{C,C'}(v)) =\sum_{v\in V'}b(v)f_{C,C'}(v)$. It follows that the right-hand side of (\ref{eq:comp-ratio}) is exactly our desired expression $\sum_{C,C'}\left|\sum_{v\in V}b(v)f_{C,C'}(v)\right|\cdot D_j$, and we are done.
\end{proof}

In the next corollary, we replace $D_j$ in the summation with $D_{j+1}$, which is needed for our final analysis, and we also add an additional restriction $C\subseteq C'$.
\begin{corollary}\label{cor:competitive-ratio}
Assume that $\valSNC\le\beta/8$.
For any demand vector $b:V'\to\mathbb R$ for the graph $G_{S,D_i}$, the summation
\begin{align*}
    \sum_{j<i}\sum_{\substack{C\in\mathcal C\in\mathcal S_j,\\C'\in\mathcal C'\in\mathcal S_{j+1}\\{C\subseteq C'}}}\bigg| \sum_{v\in V'}b(v)f_{C,C'}(v) \bigg|\cdot D_{{j+1}}
\end{align*} 

at most $O(i\gamma^3\valSNC \beta)$ times the optimal cost of a transshipment flow on $G_{S,D_i}$ satisfying demand $b$.
\end{corollary}
\begin{proof}
We invoke \Cref{obs:C-inside}, which allows us to eliminate the restriction $C\subseteq C'$, since all other pairs $(C,C')$ satisfy $f_{(C,C')}(v)=0$ for all $v$.
The statement follows from \Cref{lem:competitive-ratio} and the fact that $D_{j+1}= D_j\cdot \beta$.
\end{proof}

We now define our oblivious routing matrix $R$. It is the product of two matrices $A\times B$, where $A\in\mathbb R^{\vec{E}\times P}$ and $B\in\mathbb R^{P\times(V')}$ where $P$ is the set of all pairs of clusters $C,C'\subseteq V'$ such that (1)~$C\subseteq C'$, and (2)~there exists $j<i$ such that $C$ is a cluster in some clustering $\mathcal C\in\mathcal S_j$ and $C'$ is a cluster in some clustering $\mathcal C'\in\mathcal S_{j+1}$.

We construct $B\in\mathbb R^{P\times V'}$ as $B_{(C,C'),v}=f_{(C,C')}(v)$ if clusters $C,C'$ both contain $v$, and $0$ otherwise. For $A\in\mathbb R^{\vec{E}\times P}$, consider two clusters $C,C'$. Since $C\subseteq C'$, we have in particular the center $r_C$ is in $C'$. Take the path from $r_C$ to $r_{C'}$ in the spanning tree $T_{C'}$ of $C'$. For each edge $(u,v)$ on the path, assign entry $A_{(u,v),(C,C')}=1$ if the path travels in the direction $u$ to $v$, and $-1$ otherwise. All other entries on column $(C,C')$ get assigned $0$.

\begin{lemma}\label{lem:competitive-ratio}
Assume that $\valSNC\le\beta/8$.
For any demand vector $b:\mathbb R^{V'}$ for the graph $G_{S,D_i}$, let $\textsf{\textup{opt}}(b)$ be the optimal cost of a transshipment flow on $G_{S,D_i}$ satisfying demand $b$. Then, $\textsf{\textup{opt}}(b)\le\left\lVert ABb\right\rVert_1\le i\gamma^3\valSNC \beta\textsf{\textup{opt}}(b)$.
\end{lemma}
\begin{proof}
We begin with the first inequality. Observe that by construction, for each $v\in V$ and $\mathbbm 1_v$ as the indicator vector of $v$, the vector $AB\mathbbm 1_v$ is the final flow distribution on nodes $V'$ of the $v$-associated flow. By \Cref{obs:flow-conservation}, this flow distribution is $\mathbbm 1_{v_{D_i}}$, i.e., all flow eventually ends up at $v_{D_i}$. Since $\sum_{v\in V'}b(v)=0$, the sum of the flows $AB\mathbbm 1_v$ over all $v\in V'$ routes all demands successfully. In other words, $AB\mathbbm 1_v$ is a valid transshipment flow on $G_{S,D_i}$ satisfying demand $b$, so its cost $\left\lVert ABb\right\rVert_1$ is at least $\textsf{opt}(b)$.

We now prove the second inequality. By construction of $B$, entry $(C,C')$ of $Bb$ is exactly $\sum_vb(v)f_{(C,C')}(v)$. Next, for the indicator vector $\mathbbm 1_{(C,C')}$, by construction of $A$, we have $\left\lVert A\mathbbm 1_{(C,C')}\right\rVert_1$ is exactly the length of the path from $r_C$ to $r_{C'}$ in the spanning tree $T_{C'}$ of $C'$, which is at most $\alpha D_j$ for the level $j$ whose $\mathcal S_j$ contains cluster $C'$. It follows that
\begin{align*}
\left\lVert ABb\right\rVert_1 &= \left\lVert A\times\sum_{(C,C')}\left(\sum_{v\in V}b(v)f_{C,C'}(v)\right)\mathbbm 1_{(C,C')}\right\rVert_1 
\\&\le \sum_{(C,C')}\left|\sum_{v\in V}b(v)f_{C,C'}(v)\right|\left\lVert A\mathbbm 1_{(C,C')}\right\rVert_1
\\&\le \sum_{\substack{(C,C')\\C'\in\mathcal C'\in\mathcal S_j}}\left|\sum_{v\in V}b(v)f_{C,C'}(v)\right|\alpha D_j.
\end{align*}
By \Cref{cor:competitive-ratio}, this is at most $\alpha\cdot O(i\gamma^3\valSNC \beta)\cdot\textsf{opt}(b)$.
\end{proof}

Finally, we discuss distributed implementations of multiplying by $R$ and $R^T$ for $R=AB$.

\begin{lemma}\label{lem:distributed-oblivious}
Suppose each node $v\in V$ knows $\tilde d_C(v)$ for all clusterings $C$ containing $v$. For any vector $b\in\mathbb R^V$ where each node $v$ knows $b(v)$, we can compute $Rb$ in $\textup{poly}(\gamma\log n)$ \aggregate rounds (on network $G$) so that each entry $(u,v)$ of $Rb$ is known by both $u$ and $v$. Also, for any vector $c\in\mathbb R^{\vec{E}}$ where each entry $c_{(u,v)}$ is known by $u$\ and $v$, we can compute $R^Tc$ in $\textup{poly}(\gamma\log n)$ \aggregate rounds (on network $G$) so that each node $v\in V$ learns entry $v$ of $R^Tc$.
\end{lemma}
\begin{proof}
We work on network $G_{S,D_i}$ instead, which can be simulated on network $G$ with a constant-factor blowup by \Cref{thm:simulating-virtual-nodes}.

To multiply $Rb$ for vector $b\in\mathbb R^V$, we first multiply $Bb$ as follows. For each $j<i$ and clusters $C\in\mathcal C\in\mathcal S_j$ and $C'\in\mathcal C'\in\mathcal S_{j+1}$ containing $v$, the node $v$ locally computes $f_{(C,C')}(v)$ using $\tilde d_C(v)$ and $\tilde d_{C'}(v)$. Then, for each level $j<i$ and each clustering $\mathcal C\in\mathcal S_j$, we perform a minor aggregation on each cluster $C\in\mathcal C$ to compute the sum $\sum_{v\in C}b(v)f_{(C,C')}(v)$ for all $C'$ (where $f_{(C,C')}(v)=0$ if $v\notin C'$). Here, we crucially use the fact that we only consider clusters $C'$ with $C\subseteq C'$, which is at most $\gamma$ many since there is at most one such cluster $C'$ in each clustering of $\mathcal S_{j+1}$. As a result of the aggregation, for each pair $(C,C')$, the center $r_C$ of $C$ knows entry $(C,C')$ in $Bb$. Finally, to compute $A(Bb)$, perform the following separately for each $j<i$ and each clustering $\mathcal C'\in\mathcal S_{j+1}$: for each cluster $C'\in\mathcal C'$ in parallel, take the spanning tree $T_{C'}$ rooted at $r_{C'}$ and for each $(C,C')$, initialize at node $r_C\in C'$ the value of entry $(C,C')$ in $Bb$, which is known by $r_C$. Call \Cref{lemma:ancestor-subtree-sum} to obtain all subtree sums, and for each node $v\in C'\setminus\{r_{C'}\}$ with parent $u$, the subtree sum at $v$ is exactly the contribution of the paths in cluster $C'$ to the total flow along edge $(u,v)$, possibly negated depending on the orientation of edge ($u,v)$. Each entry $(u,v)$ of $A(Bb)$ then becomes the sum of all such contributions over all $C'$ whose spanning tree $T_{C'}$ contains edge $(u,v)$,  This concludes multiplication by $R$.

To multiply $R^Tc$ for $c\in\mathbb R^{\vec{E}}$, we first multiply $A^Tc$ as follows. Perform the following separately for each $j<i$ and each clustering $\mathcal C'\in\mathcal S_{j+1}$: for each cluster $C'\in\mathcal C'$ in parallel, take the spanning tree $T_{C'}$ rooted at $r_{C'}$ and for each edge $(u,v)$ in $T_{C'}$, initialize the value of entry $(u,v)$ in $c$. Then, in $\textup{poly}(\log n)$ \aggregate rounds, we can compute, for each node $v\in C'$, the sum of all entries on the path from $r_{C'}$ to $v$ in $T_{C'}$ (\Cref{lemma:ancestor-subtree-sum}). In particular, for each pair $(C,C')$, this sum is entry $(C,C')$ of $A^Tc$, which node $r_C$ now knows. Finally, to compute $B^T(A^Tc)$, each cluster $C$ broadcasts entry $(C,C')$ of $A^Tc$ to all its nodes, which is again at most $\gamma$ many since we only consider clusters with $C\subseteq C'$. Each node $v$ can then locally compute $f_{(C,C')}(v)$ to learn its entry in $B^T(A^Tc)$.
\end{proof}

%We claim the bound $|P|\le(i-1)\gamma^2n$. For each $j<i$, there are at most $\gamma^2$ pairs $(\mathcal C,\mathcal C')$ with $\mathcal C\in\mathcal S_j$ and $\mathcal C'\in\mathcal S_{j+1}$, and for a given node $v\in V$, at most one cluster $C\in\mathcal C$ and $C'\in\mathcal C'$ can contain $v$, so at most $(i-1)\gamma^2$ many pairs of clusters $(C,C')\in P$ both contain $v$. Summing over all $v\in V$ gives the desired bound on $|P|$.

Together, \Cref{lem:competitive-ratio-final,lem:distributed-oblivious} conclude the first part of \Cref{thm:oblivious_routing}. 

For the last statement of the theorem, if $D_{i-1}/\valSNC$ is larger than the diameter of $G$, then we modify the sparse neighborhood covers as follows. For each $j<i$, remove the singleton clusters $\{v_{D_i}\}$ and $\{s^*\}$ from each clustering in $\mathcal S_j$ (and remove their potentials $\tilde d_{\{v_{D_i}\}}(v_{D_i})$ and $\tilde d_{\{s^*\}}(s^*)$). For the single clustering $V'$ in $\mathcal S_i$, replace it with a single cluster $V$ with an arbitrary spanning tree $T$ of $G$ with diameter at most $D_{i-1}$, which we show how to find later. Once again, we trivially define $\tilde d_V(v)=D_i$ for all $v\in V$. We construct the oblivious routing and matrices $A,B$ in the same way. By the same arguments, this is a $\poly(\log n)$-competitive $\ell_1$-oblivious routing matrix for $G$.

We now discuss how to compute the spanning tree $T$ of $G$ with diameter at most $D_{i-1}$. Since $\mathcal S_{i-1}$ is a sparse cover of covering radius $D_{i-1}/\valSNC$, there exists a clustering in $\mathcal S_{i-1}$ such that the ball of radius $D_{i-1}/\valSNC$ around any $v\in V$ is contained in some cluster $C$. Since $\beta^{i-1}/\valSNC$ is greater than the diameter of $G$, this cluster $C$ must contain all the vertices $V$. Therefore, the spanning tree $T_C$ of diameter at most $D_{i-1}$ is our desired spanning tree of $G$.

%The algorithm is iterative and takes $\gamma \valSNC\beta$ iterations, and maintains a tree $T$ of $G$ that eventually spans all vertices $V$ after all iterations. Initially, $T$ is the empty tree on a single arbitrary vertex $v_0\in V$. On each iteration, we select a clustering $\mathcal C$ of sparse neighborhood cover $\mathcal S_{i-1}$ and for each cluster $C$ with at least one vertex $v$ in $T$, we root the corresponding spanning tree $T_C$ of $C$ at $v$ and add to $T$ all edges in the rooted tree $T_C$ whose child endpoint was not a vertex in $T$. At the end of this iteration, $T$ is still a tree, and it contains all vertices in clusters $C$ that contained at least one vertex in $T$.

%Since each spanning tree $T_C$ has diameter at most $D_{i-1}$, the radius of $T_C$ (centered at $v_0$) grows additively by at most $D_{i-1}$ on each iteration, so over all $\gamma \valSNC\beta$ iterations, the final tree $T$ has radius at most $\gamma \valSNC\beta \cdot D_{i-1} = \gamma \valSNC D_i$, as promised. It remains to show that $T$ does in fact span $V$, which will depend on our choice of clustering $\mathcal C$ on each iteration, which we specify next.

%Over the $\gamma \valSNC\beta$ iterations, we select the clusterings $\mathcal C\in\mathcal S$ in a round-robin fashion: we order the clusterings arbitrarily as $\mathcal C_0,\ldots,\mathcal C_{\gamma-1}$ and on iteration $i$, we select clustering $C_{i\bmod\gamma}$. We show by induction on $k$ that at the end of the first $k\gamma$ iterations, all vertices of distance at most $k D_{i-1}/\valSNC$ from $v_0$ are spanned by $T$. After $\gamma \valSNC\beta$ iterations, this covers all vertices of distance at most $D_i$, which is all of $V$ since $D_i$ is greater than the diameter of $G$ by assumption.

%The claim is trivial for $k=0$, so assume that $k>0$. Let $v\in V$ be a vertex of distance at most $k D_{i-1}/\valSNC$ from $v_0$ not yet covered. Select a vertex $u$ with $\dist_G(u,v_0)\le(k-1) D_{i-1}/\valSNC$ and $\dist_G(v_0,v)\le D_{i-1}/\valSNC$, which by induction is spanned after $(k-1)\gamma$. Since $\mathcal S_{i-1}$ is a sparse cover of covering radius $D_{i-1}/\valSNC$, there exists a cluster $C$ in some clustering such that the ball of radius $D_{i-1}/\valSNC$ around $u$ is contained in $C$. In particular, $v\in C$. Since the round-robin algorithm visits cluster $C$ once on iterations $(k-1)\gamma+1$ through $k\gamma$, all vertices in $C$ are spanned by iteration $k\gamma$, which includes $v$, completing the induction.

%\alert{(Goran) .. not completely sure can we claim that the same routing works for G since the routing in $G_{S, bla}$ eventually aggregates everything in cheating node $v_{D_i}$ and this node does not exist in $G$. So if I understand everything correctly, when you talk about G you need to aggregate in some other node. This might be trivial, but it's probably wrong without talking how to adapt it. Jason: that's true... Seems like a lot of work to make the oblivious routing work without the cheating node, since I'd have to specify a spanning tree of diameter $D_i$ to use instead of the cheating node, and this isn't given to me. And our application doesn't need it since we just need the value of the routing. Could this part of the theorem statement just be removed? \color{blue} (Goran): I talked to Christoph, and he suggests doing the following. If you have a sparse cover where the distance scale is larger than the diameter of G, then at least one cluster preserves the entire graph, and you get the spanning tree along with it. Does that help? If you still feel it's a bit tediuos to prove it with this, we can probably removing it on the other end, but that will also take some work. (Jason): I wrote it up, wasn't too bad. Biggest part was just showing that I can construct the spanning tree since I'm given clusterings at smaller scales.}

This concludes our distributed $\ell_1$-oblivious routing algorithm. 

\paragraph{Remark.}

% Sparse matrices are particularly nice because vector-matrix products can trivially be computed in sparsity work and polylog n depths in \pram (once the matrix is computed). Unfortunately even for a path graph all known constructions (including our) do not yield a sparse $V \times E$ $l_1$-oblivious routing matrix. However as the next remark shows we easily can write our routing matrix $R$ as a product of two sparse $\tilde{O}(n) \times \tilde{O}(n)$ matrices. Vertex-matrix products for such a matrix product are similarly easy to evaluate. 

% Note that $|\mathcal P|=\tO(n)$ and that $B$ is a $n \times \tilde{O}(n)$ matrix with $\tilde{O}(n)$ non-zero entries. Indeed, $B_{(C,C'),v}\ne0$ only when $v\in C\cap C'$, and there are at most $O(\log^2n)$ clusters $C$ containing $v$, since there are $O(\log^2n)$ total clusterings $\mathcal C$ and each has at most one cluster containing $v$. On the other hand, the matrix $A$ as defined is not sparse since its construction is based on subtree sums, which are not sparse for unbalanced trees (like a path). 

% We remark that we can slightly modify the construction so that the oblivious routing matrix $R$ can indeed be written as a product of two \emph{\emph{sparse}} matrices. This gives an alternative, easy way to multiply vectors by $R$ and $R^T$ in near-linear time without resorting to subtree sums in the proof of \Cref{lem:distributed-oblivious}. (Since we do not require it for our distributed algorithm, we do not discuss how to construct the matrices in a distributed setting.)

% The additional idea is to represent subtree sums concisely by the standard trick of computing a DFS traversal of the spanning tree $T_{C'}$ and then building a segment tree on top of the linear ordering of nodes. Recall from the proof of \Cref{lem:distributed-oblivious} that to multiply matrices $A$ and $Bb$, we take, for each cluster $C'$, the spanning tree $T_{C'}$ rooted at $r_{C'}$, and for each relevant cluster $C$, we initialize at node $r_C\in C'$ the value of entry $(C,C')$ in $Bb$. For each edge $(u,v)$ in $T_{C'}$, the contribution of cluster $C'$ to entry $(u,v)$ in the product $A\times Bb$ then becomes a subtree sum on this tree. We can represent all subtree sums concisely as follows: take a DFS traversal of $T_{C'}$ so that each subtree consists of consecutive nodes in the traversal order, and build a segment tree on top of the linear ordering of $C'$, which is a collection of $O(|C'|\log|C'|)$ segments such that (1)~each subtree of $T_{C'}$ consists of consecutive nodes in the linear ordering, (2)~each set of consecutive nodes in the ordering is a disjoint union of $O(\log|C'|)$ of these segments, and (3)~each node appears in $O(\log|C'|)$ many segments. Now, instead of taking matrix $B$ in the matrix product of $R$, we instead build a matrix $B'$ whose rows represent these segments (over all clusters $C'$). Namely, for a given cluster $C'$, for each segment of nodes $Q\subseteq C'$, we add a row of $B'$ whose value is the sum of all rows $(C,C')$ of $B$ satisfying $r_C\in Q$. This gives us $O(|C'|\log|C'|)$ new rows for cluster $C'$. To bound the sparsity of these rows, note that each nonzero entry in some $(C,C')$ can only make $O(\log|C'|)$ entries nonzero in the new rows, since only $O(\log|C'|)$ many segments can contain node $r_C$. It follows that the number of nonzero entries of the $O(|C'|\log|C'|)$ new rows is at most $O(\log|C'|)$ times the number of nonzero entries of entries $(C,C')$ in $B$. Since $B$ has $\tO(m)$ entries, it follows that $B'$ does as well.

% We now construct matrix $A'$ to sum up the segments accordingly. Namely, for a row $(u,v)$ and cluster $C'$, instead of assigning value $\pm1$ at columns $(C,C')$ whose node $r_C$ is in the subtree, we instead assign $\pm1$ to the segments comprising this subtree. This is at most $O(\log|C'|)$ nonzero entries for each $(C,C')$, and there are $O(\log n)$ clusters $C'$ containing edge $(u,v)$ on each of the $i$ levels, so each row $(u,v)$ has at most $\poly(\log n)$ nonzero entries. Thus, $A'$ has $\tO(m)$ nonzero entries.



% \alert{End here. Below is a sketch of the same argument, except Bernhard uses heavy-light decomposition, which I feel is more complicated than my subtree-sum approach.}
Sparse matrices are particularly nice because vector-matrix products can trivially be computed in sparsity work and polylog n depths in \pram (once the matrix is computed). Unfortunately even for a path graph there cannot exist a sparse $\vec{E} \times V$ $l_1$-oblivious routing matrix.\footnote{Here is a simple argument that the oblivious routing matrix $R$ must have $\Omega(n^2)$ nonzero entries. Let the vertices of the path be $v_1,\ldots,v_n$ in that order, and assume for simplicity that $n$ is even. For each $i$ from $1$ to $n/2$, consider the demand $\mathbb{1}_{v_i} - \mathbb{1}_{v_{i+n/2}}$. Clearly, the optimal routing routes $1$ flow along each edge from $v_i$ to $v_{i+n/2}$, but note that \emph{any} feasible routing must route nonzero flow along those edges. This means that $R(\mathbb{1}_{v_i} - \mathbb{1}_{v_{i+n/2}})$ has $\Omega(n)$ nonzero entries, which implies that columns $v_i$ and $v_{i+n/2}$ in $R$ together have $\Omega(n)$ nonzero entries. Summed over all $i$, this is $\Omega(n^2)$ nonzero entries in $R$.} However as the next remark shows we easily can write our routing matrix $R$ as a product of two sparse $\tilde{O}(n) \times \tilde{O}(n)$ matrices. Vertex-matrix products for such a matrix product are similarly easy to evaluate. 

Note that $|P|=O(n\log^2 n)$ and that $B$ is a $\tilde{O}(n) \times n$ with $\tilde{O}(n)$ non-zero entries - at most $O(\log^2 n)$ per node. Indeed each node has its demand routed through only $O(\log^2 n)$ clusters-centers, namely the ones it is contained in, which is at most one for each of the $O(\log^2 n)$ clusterings. The matrix $A$ as defined above is not sparse as most paths between cluster centers can be $O(n)$ long. However we can decompose these paths in such a way that $A$ can be written as a product of two sparse matrices. For this note that for the paths from smaller clusters to larger clusters all come from the spanning tree $T_C$ of this clustering. Decompose this spanning tree into a set of polylog n many paths by first doing a heavy-light decomposition of the tree and then taking each of the resulting paths and for every power of two $2^j$ cutting it into segments by cutting the path at any node which is a multiple of $2^j$ (starting from any end). For a clustering do this for all spanning trees of all clusters simultaneously. This results in $O(n \log n)$ paths per clustering and $O(n \log^3 n)$ paths overall. Call the set of these paths $P'$. Note that any path between the cluster centers of two clusters $C,C'$ with $C \subset C'$ along the spanning tree $T_{C'}$ can be written as a concatenation of $O(\log n)$ paths from $P'$. Moreover each edge is used by at most $O(\log^3 n)$ paths in $P'$ since it is a union of $O(\log^2 n)$ disjoint set of paths and there are at most $O(\log n)$ intervals per paths that contain an edge $e$. Overall, we can write the matrix $A$ as a product of a sparse $\vec{E} \times P'$ matrix $A_1$ with $O(\log^2 n)$ one entries per edge (indeed there is only a $m' = O(n \log^2 n)$ size subset of edges, namely the union of the spanning trees for each clustering, which are used by the routing at all, all other edges never carry any flow) and a $P' \times P$ matrix $A_2$ which assigns each cluster center pair to at most $O(\log n)$ paths in $P'$. This writes $R=A_1 A_2 B$ as the product of three sparse matrices. Moreover, since every node is mapped to at most $O(\log^3 n)$ cluster pairs by $B$ and each cluster pair is mapped to at most $O(\log n)$ paths from $P'$ the matrix-product of $A_2 B$ is sparse and assigns each node to $O(\log^4 n)$ paths in $P'$. In total this writes $R$ as a product of a $m' \times O(n \log^3 n)$ matrix with is $O(\log^2 n)$-row sparse and a $O(n \log^3 n) \times n$ matrix which is $O(\log^4 n)$-column sparse. Given the distance structures and their trees the heavy-light decomposition can be computed in $\tilde{O}(1)$ \aggregate rounds \Cref{lemma:ancestor-subtree-sum} and therefore also in PRAM.


%%% OLD STUFF
\iffalse

\oblivious*
\todo{Please change the language so that it fits the theorem above}
\textbf{Setting.} Let $G$ be the underlying graph and let $D > 0$. We are given sparse neighborhood covers $\calS_1, \calS_2, \ldots, \calS_L$ of $G$ where $\calS_\ell$ has radius $R_\ell := R^\ell$ for some $R := O(\log^5 n)$, quality $\valSNC := O(\log^4 n)$, and are each composed of $\gamma = \tilde{O}(1)$ clusterings. The number of levels $L = \tilde{O}(1)$ is such that $R_{L+1} \ge D$. We define the \textbf{cheating graph} $G\cheat_D$ as $G$ adjoined with an special \textbf{cheating node} $c$ that is connected to each node $v \in V(G)$ with a distance of $D$.

\textbf{Assumptions (to be removed).}
\begin{itemize}
\item We assume exact distances and exact computation of $p_i$'s.
\item We don't discuss algorithmic issues.
\end{itemize}


\textbf{Routing scheme.}

\begin{itemize}

\item For simplicity of exposition, we define a set of ``trivial clusters'' $\calS_0 := \bigcup_{v \in V(G\cheat_D)} \mathrm{TrivialCluster}(v)$, which contain exactly one node $v$ as its only member and its center (the padding is empty). Furthermore, let $c$ be the cheating node of $G\cheat_D$, and define $\calS_{L+1}$ to be a single cluster containing the entire $G\cheat_D$ in its core, with the cheating node as its center (and no padding). Note that the radius of this cluster is at most $D \le R_{L+1}$. This allows us to define $\calS := \bigcup_{\ell=0}^{L+1} \calS_\ell$ to be the set of clusters in our (extended) sparse neighborhood cover.
  
\item We now describe a linear routing scheme on $G\cheat_D$ by describing the (unit) flow each node sends. A node $v$ sends a unit flow which we denote via $f(v) \in \mathbb{R}^{\vec{E}}$ and refer to it as the $v$-associated flow. The cheating node $c \in V(G\cheat_D)$ simply uses the trivial flow $f(c) = \vec{0}$, i.e., that leaves all of the demand in itself. For (non-cheating) nodes $v$, we specify $f(v)$ by specifying the amount of flow $f_{i, j}(v)$ that travels from the center of cluster $C_i \in \calS$ to another cluster center $C_j \in \calS$. Given $f_{i, j}(v)$ for all $C_i, C_j \in \calS$, we can convert the representation to $f(v)$ by choosing (an oriented) path $\Path_{i, j}$ between the centers (the path we specify later) and increasing the flow along each edge on the path by $f_{i, j}(v)$. Note that $\Path_{i, j}$ does not depend on $v$ (i.e., it is consistently chosen among different nodes).

  \alert{did I handle the cheating node properly?}

\item Consider a (non-cheating) node $v \in V(G)$. On a high-level, the $v$-associated flow first routes from $v$ (i.e., from $\calS_0$) to the centers of clusters $C \in \calS_1$ (i.e., on the first level), then to the centers of clusters $C \in \calS_2$ (on the second level), and so on until the centers of clusters $C \in \calS_\ell$. Finally, all available flow is routed from the centers of cluster in $\calS_\ell$ to the cheating node (i.e., the only cluster on level $L+1$).
  
\item We now formally specify the $v$-associated flow. First, for each $\ell \in \{1, \ldots, L+1\}$, each cluster $C_i \in \calS_\ell$ that contains $v \in C_i$ computes a value $p_i(v)$ defined as the distance from $v$ to the closest node outside of $C_i$, divided by the radius of $C_i$. Furthermore, we define $w_\ell(v)$ as the sum of $p_i(v)$ over all clusters in $\calS_\ell$.
\begin{align*}
  p_i(v) :=   & \min\left( 1, \frac{\dist_G(v, V(G) \setminus C_i)}{R_\ell} \right) \\
  w_\ell(v) := & \sum_{C_i \in \calS_\ell} p_i(v)
\end{align*}

The clusters $C_i$ that do not contain $v$ have $p_i(v) := 0$. In particular (this follows from the formula, but we make explicit for concreteness), on level $\ell=0$ we define $p_i(v) = 1$ when $C_i \in \calS_0$ is the trivial cluster containing $v$ and $p_i(v) = 0$ otherwise (hence $w_0(v) = 1$). On level $\ell = L+1$, we define $p_i(v) = 1$ if $C_i$ is the cluster containing all of $G\cheat_D$ (hence $w_{L+1}(v) = 1$).

\item We now define $f_{ij}(v)$ to be the amount of flow we route from center of $C_i$ to the center of $C_j$ ($i, j$ range over the set of all clusters in the sparse neighborhood). Only flow from the previous level $\calS_{\ell}$ enters the next level $\calS_{\ell+1}$, hence $f_{ij} = 0$ unless $C_i \in \calS_\ell$ and $C_j \in \calS_{\ell+1}$. For each $\ell \in \{1, \ldots, L-1\}$ and each cluster $C_i \in \calS_\ell$, we split the flow entering the center of $C_i$ (from $\calS_{\ell-1}$) proportionally with respect to $p_j(v)$ and route the corresponding proportion to $C_j \in \calS_{\ell+1}$ (on the next level).

\begin{lemma}\label{lemma:flow-entering-cluster}
  The total amount of $v$-associated flow entering (the center of) $C_i \in \calS_\ell$ is $\frac{p_i(v)}{w_\ell(v)}$, for all $\ell$ (i.e., $\ell \in \{0, \ldots, L+1\}$).
\end{lemma}
\begin{proof}
  Let $C_x \in \calS_{\ell-1}$ be a cluster on the previous level. From $C_x$ to $C_i$ we route a flow proportional to $p_i(v)$, hence we route a $\frac{p_i(v)}{w_{\ell}}$-fraction of $C_x$'s flow due to $w_\ell(v)$ be the normalizing factor (i.e., $\sum_{C_i \in \calS_{\ell}} \frac{p_i(v)}{w_{\ell}} = 1$). Note that this fraction does not depend on $x$, hence we route the same fraction of flow for each $C_x \in \calS_{\ell-1}$. Since the total amount of flow entering all (centers of) clusters on the previous level is $1$, we conclude that the amount of flow entering (the center of) $C_i$ is $\frac{p_i(v)}{w_{\ell}}$. Finally, we note that for $\ell = L+1$ and cheating node $c$, by definition the entire unit flow enters $c$. This agrees with the formula since $p_c(v) = w_{L+1}(v) = 1$, hence $1 = \frac{p_c(v)}{w_{L+1}(v)}$.
\end{proof}

\alert{CHECK IF EVERYTHING FITS WITHIN OUT EXTENDED DEFINITION OF CLUSTERS AND WHATNOT .. from this point on!}

\begin{lemma}
  The total amount of $v$-associated flow routed between (the center of) $C_i \in \calS_\ell$ and (the center of) $C_j \in \calS_{\ell+1}$ is $f_{ij}(v) = \frac{p_i(v)}{w_\ell(v)} \cdot \frac{p_j(v)}{w_{\ell+1}(v)}$, for all $\ell$ (i.e., $\ell \in \{1, \ldots, L\}$).
\end{lemma}
\begin{proof}
  We know that from $C_i$ to $C_j$ we route a flow proportional to $p_j(v)$, hence we route a $\frac{p_j(v)}{w_{\ell+1}}$-fraction of $C_i$'s flow since $\sum_{C_j \in \calS_{\ell+1}} \frac{p_j(v)}{w_{\ell+1}} = 1$. Combining it with the amount of flow entering $C_i \in \calS_\ell$ being $\frac{p_i(v)}{w_\ell(v)}$ (\Cref{lemma:flow-entering-cluster}), we get that $f_{ij}(v) = \frac{p_i(v)}{w_\ell(v)} \cdot \frac{p_j(v)}{w_{\ell+1}(v)}$, as needed.
\end{proof}

Finally, we specify the paths $\Path_{i, j}$ along which we route the flow between the centers $c_i$ of $C_i \in \calS_{\ell}$ and center $c_j$ of $C_j \in \calS_{\ell+1}$ (for all $\ell \in \{0, \ldots, L\}$). Assuming that $f_{i, j}(v) > 0$ (otherwise we need not specify the paths), We simply define $\Path_{i, j}$ to be an arbitrary path between $c_i$ and $c_j$ of length (distance) at most $\tilde{O}(R_\ell)$. This must exist since if $f_{i, j}(v) > 0$ we have that the core of both $C_i$ and $C_j$ contains $v$, hence their radii bounds tell us that $\dist_G(c_i, c_j) \le \dist_G(c_i, v) + \dist_G(v, c_j) \le R_\ell + R_{\ell+1} \le 2 \cdot R \cdot R_\ell = \tilde{O}(R_\ell)$.

\textbf{Misc calculations.}


\begin{lemma}\label{lemma:magnitude-properties-p-w}
  We have that for all $\ell$ (i.e., $\ell \in \{0, \ldots, L+1\}$:
  \begin{align*}
    %p_i(v) \le 1 \text{ \alert{is this even true?}}\\
    w_\ell(v) \ge 1/\valSNC \\
    %w_\ell(v) \le \gamma \text{ \alert{is this even true?}} \\
  \end{align*}
\end{lemma}
\begin{proof}
  For $\ell = 0$ or $\ell = L+1$ the claim is immediate from the definition. Otherwise, since $\calS_\ell$ is a sparse neighborhood cover of radius $R_\ell$ and quality $\valSNC$, the ball around $v$ of radius $R_\ell / \valSNC$ is contained in the core of some cluster $C_i \in \calS_{\ell}$. Therefore, $w_\ell(v) \ge p_i(v) = \dist_G(v, V(G) \setminus C_i) / R_\ell \ge (R_\ell / \valSNC) / (R_\ell) \ge 1/\valSNC$.
\end{proof}

\begin{lemma}
  Fix two nodes $u, v$ and let $d := \dist_G(u, v)$. For every $\ell$ (i.e., $\ell \in \{0, \ldots, L+1\}$) and each cluster $i \in \calS_\ell$ we have that:
  \begin{align} 
    p_i(u) - p_i(v) \le \frac{d}{R_\ell} \\
    | \{ i : p_i(v) \neq 0 \} | \le \gamma \label{eq:p-support-size} \\
    w_\ell(u) - w_\ell(v) \le 2 \gamma \cdot \frac{d}{R_\ell} = \tilde{O}(\frac{d}{R_\ell}) \\
    w_\ell(u) \le w_\ell(v) \cdot ( 1 + 2 \gamma \valSNC \frac{d}{R_\ell} ) = w_\ell(v) \cdot (1 + \tilde{O}(\frac{d}{R_\ell}) )
  \end{align}
\end{lemma}
\begin{proof}
  \begin{itemize}
  \item By triangle inequality, we have that: $p_i(u) \le \frac{\dist_G(u, V(G) \setminus C_i)}{R_\ell} \le \frac{\dist_G(u, v) + \dist_G(v, V(G) \setminus C_i)}{R_\ell} \le \frac{d}{R_\ell} + p_i(v)$.

  \item The support size $| \{ i : p_i(v) \neq 0 \} | \le \gamma$ since in each clustering only one cluster can contain $v$, and only that cluster (within the clustering) can have $p_i(v) \neq 0$.

  \item Due to the support size, we have that $w_\ell(v) - w_\ell(u) \le \sum_{C_i \in \calS_\ell} p_i(v) - p_i(v) \le 2 \gamma \frac{d}{R_\ell}$ as the difference is $0$ whenever $p_i(v) = p_i(u) = 0$.

  \item $w_\ell(u) = w_\ell(v) \cdot \frac{w_\ell(u)}{w_\ell(v)} \le w_\ell(v) \cdot \frac{w_\ell(v) + 2 \gamma d/R_\ell}{w_\ell(v)} \le w_\ell(v) \cdot (1 + 2 \gamma \valSNC \frac{d}{R_\ell}) = (1 + \tilde{O}(\frac{d}{R_\ell})) \cdot w_\ell(v)$ ... in the last inequality we used $w_\ell(v) \ge 1/\valSNC$ from \Cref{lemma:magnitude-properties-p-w}.
  \end{itemize}
\end{proof}


\begin{lemma}
  Fix two nodes $u, v$ and let $d := \dist_G(u, v)$. For every $\ell$ (i.e., $\ell \in \{0, \ldots, L\}$) and each two clusters $i \in S_\ell, j \in S_{\ell+1}$ we have that:
  \begin{align}
    R_\ell \cdot [ f_{i, j}(u) - f_{i, j}(v) ] \le \tilde{O}(d) ???
  \end{align}
\end{lemma}
\begin{proof}
  First, we note that the claim is trivial if $d \ge R_\ell$ since $0 \le f_{i, j} \le 1$, giving us that $| R_\ell \cdot [ f_{i,j}(u) - f_{i, j}(v) | \le 2 d = O(d)$. In the following, we assume that $d \le R_\ell$. To simplify calculations, we replace $\delta := d/R_\ell$ (note that $\delta \le 1$).
  \begin{align*}      
    f_{i,j}(u) - f_{i, j}(v) & = \frac{p_i(v)}{w_\ell(v)} \cdot \frac{p_j(v)}{ w_{\ell+1}(v) } - \frac{p_i(u)}{w_\ell(u)} \cdot \frac{p_j(u)}{w_{\ell+1}(u)} \\
                             & = ( w_{\ell}(u) w_{\ell+1}(u) )^{-1} \cdot \left[ [1 + \tilde{O}(\delta)]^2 \cdot p_i(v) p_j(v) - p_i(u) p_j(u) \right] \\
                             & \le \valSNC^2 \cdot \left[ [1 + \tilde{O}(\delta)] \cdot p_i(v) p_j(v) - p_i(u) p_j(u) \right]
  \end{align*}
  \begin{align*}
    (1 + \tilde{O}(\delta)) p_i(v) p_j(v) - p_i(u) p_j(v) & \le (1 + \tilde{O}(\delta)) (p_i(u) + \delta) (p_j(u) + \delta) - p_i(u) p_j(v) \\
                                                          & = \tilde{O}(\delta) p_i(u) p_j(u) + \tilde{O}(\delta) + \tilde{O}(\delta)^2 \\
                                                          & \le \tilde{O}(\delta)
  \end{align*}
  Combining, we get that $f_{i,j}(u) - f_{i, j}(v) \le \valSNC^2 \cdot \tilde{O}(\delta) = \tilde{O}(d / R_\ell)$. Finally, we have that $R_\ell \cdot [ f_{i, j}(u) - f_{i, j}(v) ] \le R_\ell \cdot \tilde{O}(d / R_\ell) = \tilde{O}(d)$, as required.

\end{proof}

\end{itemize}


\textbf{Cost analysis.}

\begin{lemma}
  It is sufficient to prove it for every pair of nodes $u, v$ that they are $\alpha$-approximate. \alert{write this out}
\end{lemma}
\begin{proof}
  BLA
\end{proof}


Fix two nodes $u, v$ and let $d := \dist_G(u, v)$. Let $w_G(\Path_{i, j})$ be the length of $\Path_{i, j}$. Calculation of the total cost between $u, v$:
\begin{align*}
  \sum_{C_i, C_j \in \calS} w_G(\Path_{i, j}) \cdot | f_{i, j}(v) - f_{i, j}(u) | & \le \sum_{\ell=0}^{L} \sum_{C_i \in \calS_\ell} \sum_{C_j \in \calS_{\ell+1}} w_G(\Path_{i, j}) \cdot | f_{i, j}(v) - f_{i, j}(u) | \\
                                                                                  & \le \sum_{\ell=0}^{L} \sum_{C_i \in \calS_\ell} \sum_{C_j \in \calS_{\ell+1}} \tilde{O}(R_\ell) \cdot | f_{i, j}(v) - f_{i, j}(u) | \\
                                                                                  & \le \sum_{\ell=0}^{L} \sum_{C_i \in \calS_\ell} \sum_{C_j \in \calS_{\ell+1}} \1{f_{i, j}(u) \neq 0 \lor f_{i, j}(v) \neq 0} \cdot \tilde{O}(d)  \\
                                                                                  & \le (L+1) \cdot 2\gamma \tilde{O}(d) = \tilde{O}(d) \\
\end{align*}


%%% END OLD STUFF
\fi


% Local Variables:
% TeX-master: "main"
% End:





==> minor-aggregation-model.tex <==
\section{Computational Models: Minor-Aggregation, \congest, \pram}\label{sec:computational-models}

In this section we give a description of various models we use throughout this paper.

\subsection{\congest model}

First, we define the standard distributed model of computation called \congest. Any algorithm defined in the \aggregate model efficiently compiles down to \congest.

\begin{definition}[\congest]
  We are given an undirected graph $G = (V, E)$ called the ``communication network''. The vertices of $G$ are called nodes and they are independent computational units (i.e., have their own processor and private memory). Communication between nodes occurs in synchronous rounds. In each round, each pair of nodes adjacent in $G$ exchange $O(\log n)$ bits. Nodes perform arbitrary local computation between rounds. Initially, nodes wake up at the same time and only know their unique $O(\log n)$-bit ID.
\end{definition}

\subsection{Partwise Aggregation, Low-Congestion Shortcut Framework, and the \congestPA model}
We start by giving some background on partwise aggregation (PA) and the low-congestion shortcut framework before defining the \congestPA model.

\textbf{Partwise aggregation (PA)} is a high-level primitive that frequently arises while designing distributed (and parallel) algorithms. A partwise aggregation task is specified by giving each node a \emph{private value}, choosing a simple aggregation function such as min, max, or sum, and specifying a collection of connected and node-disjoint subsets $P_1, P_2, \ldots \subseteq V$. To solve partwise aggregation, all nodes $v$ are required to output the aggregate of all private values of the nodes in $v$'s part. Note that PA is immediately solvable in parallel using near-linear work and polylogarithmic depth. 

While extremely simple, the utility of PA stems from the fact that many important graph problems (e.g., MST, SSSP, min-cut, etc.) can be reduced to a small (polylogarithmic or $n^{o(1)}$) number of partwise aggregation instances. Therefore, any reduction to $\poly\log n$ many PA instances directly gives near-optimal parallel algorithms.

\textbf{The low-congestion shortcuts framework} was first introduced in \cite{GH16} and developed over a long sequence of works~\cite{GH16,haeupler2016low,haeupler2016near,haeupler2018round,haeupler2018minor,ghaffari_haeupler2021shortcuts_in_minor_closed,haeupler2021universally,kogan2021low,ghaffari2021hop,GHR21}. %that recently culminated in the design of universally-optimal distributed algorithms.
The framework defines a natural graph parameter called $\shortcutQuality{G}$ which assigns a number to each undirected and unweighted graph $G$. The framework then shows that shortcut quality is \emph{THE} parameter that characterizes the distributed complexity for a large class of seemingly unrelated graph problems. In particular: any distributed \congest algorithm for MST, (approximate) min-cuts, connectivity, max-flow, partwise aggregation~\cite{haeupler2021universally}, and SDD or Laplacian system solving~\cite{forster2020minor,anagnostides2021accelerated} requires \emph{at least} $\shortcutQuality{G}$ rounds on a network $G$ (up to polylogarithmic factors), even if only a non-trivial approximation is required and randomization is allowed. In more details, on a fixed graph $G$ the adversary can always force any correct algorithm to require $\tilde{\Omega}(\shortcutQuality{G})$ rounds if the adversary is allowed to choose the input (e.g., edge weights).
%We remark that this lower bound holds when 

On the other hand, the framework complements the above lower bound with an efficient distributed implementation of partwise aggregation. The ultimate goal would be to show that PA can be solved in (deterministic) $\tilde{O}(\shortcutQuality{G})$ \congest rounds, which would be near-optimal and would yield unconditional universally near-optimal algorithms for all of the above problems. However, we currently only achieve such a result under some conditions about the graph topology $G$. For example, such a result can be achieved in excluded-minor graphs where \cite{haeupler2016low} and \cite{haeupler2018minor} show that PA can be solved in $\tilde{O}(\shortcutQuality{G}) = \tilde{O}(\hopDiameter{G})$ rounds. Moreover, very recent work on hop-bounded oblivious routings and hop-bounded expander decomposition~\cite{ghaffari2021hop,GHR21} shows that PA can be solved in randomized $n^{o(1)}$ \congest rounds whenever $\shortcutQuality{G} \le n^{o(1)}$.

With the knowledge that PA can be efficiently implemented, we define the \congestPA  model which is simply \congest with access to a PA oracle.
\begin{definition}[\congestPA model]
  The \congestPA model naturally extends the \congest model. However, in each round we can choose to either perform a standard \congest round, or we can call the PA oracle. For the latter, each node chooses a private input at the start and learns the partwise aggregate at the end of the round.
\end{definition}

Per the above discussion, we can implement the PA oracle with the following constraints.
\begin{theorem}\label{thm:congestpa-simulation}
  A $\tau$-round \congestPA algorithm can be simulated in $\tilde{O}(\tau \cdot \tau_{PA})$ rounds of \congest, where $\tau_{PA}$ is the number of rounds in which one can solve any partwise aggregation instance on $G$. The following bounds have been proven for $\tau_{PA}$:
  \begin{itemize}
  \item For all graphs $G$, there is a deterministic algorithm with $\tau_{PA} \le \tilde{O}(\hopDiameter{G} + \sqrt{n})$.~\cite{GH16}
  \item If $G$ is minor-free, there is a deterministic algorithm with $\tau_{PA} \le \tilde{O}(\hopDiameter{G})$ (the hidden constants depend on the family).~\cite{ghaffari_haeupler2021shortcuts_in_minor_closed}
  \item If the nodes of $G$ know the topology in advance, there is a randomized algorithm with $\tau_{PA} \le \tilde{O}(\shortcutQuality{G})$.~\cite{haeupler2021universally}
  \item If $\shortcutQuality{G} \le n^{o(1)}$, there is a randomized algorithm with $\tau_{PA} \le n^{o(1)}$.~\cite{GHR21}
  \end{itemize}
\end{theorem}

\subsection{Minor-Aggregation Model}
\label{subsec:minor_aggregation}

In this section we define the \aggregate model, defined in \cite{goranci2022universally} and \cite{ghaffari2021universally}, an expressive model which provides an easy-to-use interface to the most recent advancements in the low-congestion framework. Specifically, the \aggregate model leverages partwise aggregation to implement fast aggregation operations on minors of the communication network $G$. The connection between minor aggregations and partwise aggregations is straightforward: computing a partwise aggregate is basically the same as computing a node-wise aggregate in the minor in which each part is contracted.

We first define a notion of aggregations and then formally specify the Distributed \aggregate model.

\begin{definition}[Aggregation operator]
  An aggregation operator $\bigoplus$ takes two $B$-bit inputs $m_1, m_2$ for some $B = \tilde{O}(1)$, and combines them into a new $B$-bit output $m_1 \bigoplus m_2$. Furthermore, given $k$ inputs $m_1, \ldots, m_k$, their $\bigoplus$-aggregate $\bigoplus_{i=1}^k m_i$ is the result from arbitrarily aggregating some two inputs until a single one remains.
\end{definition}

Note that for a commutative and associative operator (e.g., sum or max), the value $\bigoplus_{i=1}^n m_i$ is unique.
However, we gain flexibility by allowing for arbitrary operators where the output might depend on the execution sequence. 

\begin{definition}[Distributed Minor-Aggregation model]\label{def:aggregation-congest}
  We are given an undirected graph $G = (V, E)$. Both nodes and edges are separate computational units (i.e., have their own processor and private memory). Communication occurs in synchronous rounds and nodes/edges perform $\tilde{O}(1)$-work local computation between rounds. Initially, nodes wake up at the same time and only know their unique $\tilde{O}(1)$-bit ID, while edges know the IDs of their endpoints. Each round consists of the following three steps (in that order).
  \begin{itemize}    
  \item \textbf{Contraction step.} Each edge $e$ chooses a value $c_e = \{\bot, \top\}$. This defines a new \emph{minor network} $G' = (V', E')$ constructed as $G' = G / \{ e : c_e = \top \}$, i.e., by contracting all edges with $c_e = \top$ and self-loops removed. Vertices $V'$ of $G'$ are called supernodes, and we identify supernodes with the subset of nodes $V$ it consists of, i.e., if $s \in V'$ then $s \subseteq V$.

  \item \textbf{Consensus step.} Each individual node $v \in V$ chooses a $\tilde{O}(1)$-bit value $x_v$. For each supernode $s \in V'$ we define $y_s := \bigoplus_{v \in s} x_v$, where $\bigoplus$ is some predefined aggregation operator. All nodes $v \in s$ learn $y_s$.

  \item \textbf{Aggregation step.} Each edge $e \in E'$ connecting supernodes $a \in V'$ and $b \in V'$ learns $y_a$ and $y_b$, and chooses two $\tilde{O}(1)$-bit values $z_{e, a}, z_{e, b}$ (i.e., one value for each endpoint). Finally, (every node of) each super $s \in V'$ learns the aggregate of its incident edges in $E'$, i.e., $\bigotimes_{e \in \text{incidentEdges(s)}} z_{e, s}$ where $\bigotimes$ is some predefined aggregation operator.
  \end{itemize}
\end{definition}

\textbf{Distributed storage and inputs.} Our \aggregate algorithm operates on objects that are \emph{``distributedly'' stored}, meaning that each processor has its own part of the object in private memory. Specifically, we store a \emph{node vector} $x \in \R^V$ by storing $x_v$ in node $v$. Similarly, edge vectors $x \in \R^{E}, x \in \R^{\vec{E}}, x\in \R^{\overleftrightarrow{E}}$ are distributed over edges. Subgraphs $H \subseteq G$ are specified by distributedly storing the characteristic vectors $\mathbb{1}_{V(H)} \in \R^{E(G)}$ and $\mathbb{1}_{E(H)} \in \R^{E(G)}$. Initially, the problem-specific input is assumed to be distributedly stored. For transshipment and SSSP, we assume the lengths (edge vector) and demands (node vector) are stored. At termination, the output is required to be distributedly stored.

\textbf{Minors.} Algorithms designed in this model can take advantage of several high-level primitives typically unavailable in other distributed models (due to the power of being able to solve PA). Notably, any algorithm can be run on any minor in a black-box manner. For example, this allows extremely simple descriptions of contraction-based algorithms such as Boruvka's MST algorithm.

\begin{corollary}\label{corollary:computation-on-minors}
  Any $\tau$-round \aggregate algorithm on a minor $G' = G / F$ of $G = (V, E)$ can be simulated via a $\tau$-round \aggregate algorithm on $G$. Initially, each edge $e \in E$ needs to know whether $e \in F$ or not. Upon termination, each node in $G$ learns all the information that the supernode it was contained in learned.
\end{corollary}

\textbf{Node-disjoint scheduling.} It is immediate, but useful to note, that we can can simultaneously run algorithms on node-disjoint subsets.
\begin{corollary}\label{lemma:node-disjoint-scheduling}
  Let $G$ be an undirected graph. Given any $\tau$-round \aggregate algorithms $A_1, \ldots, A_k$ running on node-disjoint and connected subgraphs (of $G$) $H_1, H_2, \ldots, H_k$, we can run $A_1, \ldots, A_k$ simultaneously within a $\tau$-round \aggregate algorithm $A$ that runs on $G$.
\end{corollary}

\textbf{Ancestor and subtree sums.} The following operation, proven in \cite{ghaffari2021universally}, is often useful.
\begin{lemma}[Ancestor and subtree sums]\label{lemma:ancestor-subtree-sum}
  Let $F$ be a forest (each edge $e$ knows whether $e \in E(F)$ or not) and suppose that each connected component has a unique root (each node knows whether it is the root). Suppose each node $v$ has an $\tilde{O}(1)$-bit private input $x_v$. There is a deterministic $\tilde{O}(1)$-round Minor-Aggregation algorithm that computes for each node $v$ the values values $p_v := \bigoplus_{\ell \in A(v)} x_w$ and $s_v := \bigoplus_{\ell \in D(v)} x_w$, where $A(v)$ and $D(v)$ are the set of ancestors and descendants of $v$ of $F$ with respect to the root, where $\bigoplus$ is some pre-defined aggregation operator.
\end{lemma}

\textbf{Simulation in \congest and \pram.} It is immediately clear that any \aggregate algorithm can be turned into a fast \pram algorithm. However, the power of the \aggregate framework comes from the possibility of compiling it to an efficient distributed (i.e., \congest) algorithm, assuming the partwise aggregation oracle can be solved efficiently---which is provided by the low-congestion shortcut framework (under some conditions). This is formalized in the following theorem.

\begin{theorem}\label{thm:compilation_pa_congest}
  Let $A$ be any (deterministic) $\tau$-round \aggregate algorithm on $G$ with $n := |V(G)|$ and $m := |E(G)|$. In \pram, we can deterministically simulate $A$ with $\tilde{O}(m \cdot \tau)$ work and $\tilde{O}(\tau)$ depth. Furthermore, in the distributed setting, we can simulate $A$ in $\tilde{O}(\tau)$ \congestPA rounds.
\end{theorem}
\begin{proof}
  The \pram part of the theorem is immediate. The randomized \congestPA simulation is proven in \cite{goranci2022universally}, albeit without explicitly defining the \congestPA model. The deterministic \congestPA simulation is proven in \cite{ghaffari2021universally}, albeit also without explicitly defining the \congestPA model.
\end{proof}


\subsection{Virtual Nodes in the \aggregate Model}

Another useful high-level primitive is adding $\tilde{O}(1)$ arbitrarily-connected virtual nodes to the communication network $G$ and running an arbitrary \aggregate algorithm in a black-box manner on the new graph while only incurring a $\tilde{O}(1)$ slowdown. Note that such an operation is completely inadmissible in other models of distributed computing like \congest~\cite{peleg2000distributed} where nodes are allowed to send/receive arbitrary (i.e., non-aggregate) information to/from each one of their neighbors separately, as this would allow efficiently communicating the entire network topology to a single node and solving the problem locally. On the other hand, virtual-node addition can be efficiently simulated in the \aggregate model due to the ``aggregate''-nature of communication. For example, we use this operation to connect a ``supersource'' node, enabling us to use our standard SSSP algorithm to implement a set-source-$S$ shortest path.

Given a graph $G$, we can construct a \emph{virtual graph} by repeatedly adding a \emph{virtual node} and connecting it to an arbitrary set of neighbors. This is formalized in the following definition.
\begin{definition}
  A virtual graph $G\virt$ extending a connected graph $G = (V, E)$, is a graph whose node set can be partitioned into $V$ and a set of so-called \emph{virtual nodes} $V\virt$, i.e., $V(G\virt) = V \sqcup V\virt$. Furthermore, the edge set $E(G\virt)$ can be partitioned into $E$ and a set of so-called \emph{virtual edges} $E\virt$ with the property that every virtual edge is adjacent to at least one virtual node. We say $G\virt$ has at most $\beta$ virtual nodes if $|V\virt| \le \beta$.
\end{definition}

\textbf{Distributed storage of virtual graphs.} In order to ``construct'' a virtual graph, one needs to be able to distributedly store it; unfortunately, this requires specifying some low-level storage details. A virtual graph $G\virt$ is distributedly stored in $G$ in the following way. A virtual edge connecting a non-virtual $u$ and a virtual $v$ is only stored in $u$ (other nodes do not need to know about its existence). A virtual edge between two virtual nodes is required to be known by all nodes. All nodes know about all virtual nodes.

% \begin{definition}[Virtual node addition]\label{def:virtual-node-addition}
%   Adding a virtual node to a graph $G = (V, E)$ corresponds to changing $G$ into $G\virt = (V \cup \{\mathrm{virt}\}, E \cup \bigcup_{v \in \Gamma\virt} \{ \mathrm{virt}, v\})$, where $\mathrm{virt}$ is a new ``virtual'' node, and $\Gamma\virt \subseteq V$ are the set of neighbors of $\mathrm{virt}$. Edges adjacent to virtual nodes are called ``virtual edges''.
% \end{definition}

\textbf{Simulations on virtual graphs.} We can add $\beta$ many virtual (arbitrarily interconnected) nodes to any graph $G$ and still simulate any Minor-Aggregation algorithm on the virtual graph with a $O(\beta + 1)$ blowup in the number of rounds. We say a node/edge $a$ simulates a virtual node/edge $v$ if $a$'s private memory contains all data of $v$'s private memory in the virtual graph (i.e., $a$ knows what $v$ is outputting in each round, and learns everything $v$ receives). The following simulation result formalizes this (proven in \cite{ghaffari2021universally}).
\begin{theorem}\label{thm:simulating-virtual-nodes}
  Suppose $A\virt$ is a $\tau$-round Minor-Aggregation algorithm on a virtual graph $G\virt(\beta)$ that extends $G$ and has at most $\beta$ virtual nodes. Any such $A\virt$ can be simulated in $G$ with a $\tau \cdot O(\beta + 1)$-round Minor-Aggregation algorithm.
  Upon termination, each non-virtual node $v \in V(G)$ learns all information learned by $v$ and all virtual nodes in $A\virt$.

  Each virtual node is simulated by all (non-virtual) nodes. Similarly, the virtual edges connecting two virtual nodes are simulated by all nodes, while the edges connecting a virtual and a non-virtual node are simulated by the non-virtual node.
\end{theorem}

Suppose we are given a \aggregate algorithm on a graph with virtual nodes. We can simulate the algorithm in \congest by first applying \Cref{thm:simulating-virtual-nodes}, thereby obtaining a (non-virtual) \aggregate algorithm. Then, we can use the general simulation results \Cref{thm:compilation_pa_congest,thm:oracleSimulation} to obtain a \congest algorithm.

\subsection{Oracles in the \congest and Minor-Aggregation Model}

An oracle is a black-box function that takes a certain input (on the original graph) and produces a specified output. A \aggregate/\congest algorithm with access to an oracle can, in each round, choose to perform a regular \aggregate/\congest round, or to make a single oracle call (i.e., multiple oracle calls per round are forbidden). For example, \congestPA is simply the \congest model with access to the PA oracle. 
The reason why oracles are useful are results like the following fact that follows from \cref{thm:compilation_pa_congest}. 

\begin{fact}[Oracle simulation]
  \label{thm:oracleSimulation}
  Suppose $A$ is a $\tau$-round \aggregate algorithm with access to oracles $\fO^1, \ldots, \fO^k$. The following simulation results hold:
  \begin{enumerate}
  \item Suppose each oracle $\fO^i$ call can be simulated in \pram in at most $\tau_{work}$ work and $\tau_{time}$ time. Then $A$ can be simulated with a \pram algorithm in total work $\tilde{O}(\tau \cdot (\tau_{work} + m))$ and total time $\tilde{O}(\tau \cdot (\tau_{time} + 1))$.

  \item Suppose each oracle $\fO^i$ call can be simulated in \congestPA in at most $\tau_{oracle}$ rounds. Then $A$ can be simulated with a \congestPA algorithm in at most $\tilde{O}(\tau \cdot (\tau_{oracle} + 1))$ rounds.
  
  \item Suppose each oracle $\fO^i$ call can be simulated in \congest in at most $\tau_{oracle}$ rounds. Then $A$ can be simulated with a \congest algorithm in at most $\tilde{O}(\tau \cdot (\tau_{oracle} + \sqrt{n} + \hopDiameter{G} ))$ rounds. 
  
    \item Suppose each oracle $\fO^i$ call can be simulated in \congest in at most $\tau_{oracle}$ rounds on a fixed minor-free family. 
    Then $A$ can be simulated with a \congest algorithm in at most $\tilde{O}(\tau \cdot (\tau_{oracle} + \hopDiameter{G} ))$ rounds. 
  \end{enumerate}
\end{fact}


\begin{comment}
For the distributed setting, we can combine the fact above with the \congestPA simulation result (\Cref{thm:congestpa-simulation}) to obtain the following result.
\begin{corollary}\label{corollary:minor-oracle-to-congest}
  Suppose $A$ is a $\tau$-round \aggregate algorithm with access to oracles $\fO^1, \ldots, \fO^k$ that can all be implemented in at most $\tau_{oracle}$ \congestPA rounds. Then $A$ can be simulated in $\tilde{O}(\tau \cdot \tau_{PA})$ \congest rounds, where the bounds from \Cref{thm:congestpa-simulation} apply. In particular, on excluded-minor graphs, $A$ can be simulated in $\tilde{O}(\tau \cdot \hopDiameter{G})$ \congest rounds.
\end{corollary}
\end{comment}
% Local Variables:
% TeX-master: "main"
% End:



==> missingproofsgeneralresults.tex <==
\section{Missing Proofs of \cref{sec:localiterative}}
\label{sec:missingProofs}
\cycleone*

\begin{proof}
Combining \cref{lem:cycletwo} and \cref{lem:cyclethree} implies that $\oPot_{D_i}$ and $\oDist_{\eps,D}$ can be efficiently computed for every $D \in \left[\frac{D_i}{\valSNC},D_i \right]$ and every $\eps = \frac{1}{\tilde{O}(1)}$.
Being able to efficiently compute $\oDist_{\eps,D}$ for every $D \in \left[\frac{D_i}{\valSNC},D_i\right]$ and every $\eps = \frac{1}{\tilde{O}(1)}$  together with \cref{lem:cyclefour} implies that we can efficiently compute a sparse neighborhood cover with covering radius $\frac{D_i}{\valSNC}$ together with a rooted spanning tree $T_C$ of diameter at most $D_i$ for every cluster $C$ in the cover.
Moreover, once we have computed such a sparse neighborhood cover, \cref{lem:cyclefive} together with the fact that we can efficiently compute $\oPot_{D_i}$ implies that we can efficiently compute a distance structure for the scale $D_i$, as desired.
\end{proof}

\cycletwo*

\begin{proof}
Directly follows from the first part of \cref{thm:oblivious_routing}.
\end{proof}


\cyclethree*

\begin{proof}

Consider an arbitrary $D \in \left[\frac{D_i}{\valSNC},D_i \right]$ and $S  \subseteq V$. 
We show how to answer both $\oDist_{\frac{1}{\log^3(n)},D}(S)$ and $\oPot_{D_i}(S)$.

In case $S = \emptyset$, we can answer $\oDist_{\frac{1}{\log^3(n)},D}(S)$ by returning an empty forest and $\oPot_{D_i}(S)$ by setting $\phi_{S,D_i}(v) = D_i$ for every $v \in V$.
Hence, it remains to consider the case $S \neq \emptyset$.


When $S$ is the first input given to $\oObliv_{D_i}$, then $\oObliv_{D_i}$ implements matrix-vector products with some fixed matrix. We denote this matrix by $R_S$.
%For a moment, assume that our actual input graph is $G_{S,D_i}$ instead of $G$.
We invoke \cref{theorem:boosting_rounding} with $R = R_S$, $H = G_{S,D_i}$, $\eps = \frac{1}{10\log^3(n)\valSNC}$ and $s = \sstar$ to get an algorithm running in $\tilde{O}(1)$ \aggregate rounds when given access to the rounding oracle $\oRound_{\eps/2} = \oRound$ and an oracle which performs matrix-vector products with $R_S$ and $R_S^T$.

The output of the algorithm consists of two parts.
First, a potential $\phi$ for $G_{S,D_i}$ with $\phi(\sstar) = 0$. \\
Second, a tree $T \subseteq G_{S,D_i}$ rooted at $\sstar$ such that for each $v \in V(G_{S,D_i})$ we have $\dist_T(\sstar, v) \leq (1+\eps) \phi(v)$.

We can efficiently simulate this algorithm in $G$, viewing $G_{S,D_i}$ as a virtual graph with two virtual nodes that extend $G$.
Indeed, \cref{thm:simulating-virtual-nodes} implies that each \aggregate round in $G_{S,D_i}$ can be simulated with $O(1)$ \aggregate rounds in $G$. Moreover, we can use the oracle $\oObliv_{D_i}$ to compute the $\tilde{O}(1)$ matrix-vector products with $R_S$ and $R_S^T$. Finally, we can directly simulate the oracle $\oRound$ for the virtual graph $G_{S,D_i}$ with the oracle $\oRound$ for the actual graph $G$, as the set of valid input graphs for both oracles are the same.

Next, we show that $T$ can be used to efficiently answer $\oDist_{\frac{1}{\log^3(n)},D}(S)$ and $\phi$ can be used to efficiently answer $\oPot_{D_i}(S)$.

\paragraph{Implementing the Forest Oracle}

We answer $\oDist_{\frac{1}{\log^3(n)},D}(S)$ by returning the rooted forest $F$ with 

\begin{enumerate}
    \item $V(F) = \{v \in V \colon \dist_T(\sstar, v) \leq (1+\eps)(D_i + D)\}$,
    \item each node $v \in V(F) \cap S$ is a root in $F$, and
    \item each node $v \in V(F) \setminus S$ has the same parent in $F$ and $T$.
\end{enumerate}

Note that $F$ is only well-defined if for each node $v \in V(F) \setminus S$, the parent of $v$ in $T$, which we denote by $p_v$, is actually a vertex in $F$.
We first verify that $p_v \in V$, which is equivalent to $p_v \notin \{\sstar, v_D\}$. Clearly, $p_v \neq s^*$, as there is no edge in $G_{S,D_i}$ between $s^*$ and a node in $V \setminus S$.
For the sake of contradiction, assume that $p_v = v_D$. Then, 
\begin{align*}\dist_T(\sstar,v) = \dist_T(\sstar, v_D) + \dist_T(v_D,v) \geq 2D_i + D_i> (1+\eps)(D_i + D),
\end{align*}
which is a contradiction with $\dist_T(\sstar,v) \leq (1+\eps)(D_i + D)$, which follows from $v \in V(F)$.
Hence, $p_v \in V$ and as $\dist_G(\sstar,p_v) \leq \dist_G(\sstar,v)\leq (1+\eps)(D_i + D)$, we can conclude that $p_v \in V(F)$.

Next, we show that each node $v \in V$ with $\dist_G(S,v) \leq D$ is contained in $V(F)$. 
This is indeed the case as 
\begin{align*}\dist_T(\sstar,v) \leq (1+\eps)\dist_{G_{S,D_i}}(\sstar,v) \leq (1+\eps)(D_i + D).
\end{align*}

In particular, each node in $S$ is contained in $V(F)$ and therefore $F$ is a forest rooted at $S$. 
It therefore remains to verify that for each node $v \in V(F)$, $\dist_F(S,v) \leq (1+\frac{1}{\log^3(n)})D$.
To that end, consider the unique path between $\sstar$ and $v$ in the tree $T$. This path contains at least one vertex in $S$. Let $s$ be the last vertex in $S$ on that path. From the previous discussion, it follows that $\dist_F(s,v) = \dist_T(s,v)$, as the unique path between $s$ and $v$ in $T$ is fully  contained in $F$. We therefore have,

\begin{align*}
    &\dist_F(S,v) \leq \dist_T(s,v) \leq \dist_T(\sstar,v) - D_i \\
    &\leq (1+\eps)(D_i + D) - D_i\leq D + 2\eps D_i\leq \left( 1+\frac{1}{\log^3(n)} \right) D,
\end{align*}

where the last inequality follows from $D \geq \frac{D_i}{\valSNC}$ and $\eps \leq \frac{1}{2\log^3(n)\valSNC}$.




\paragraph{Implementing the Potential Oracle}
We answer $\oPot_{D_i}(S)$ by setting for each $v \in V$
$$\phi_{S,D_i}(v) = \max(\phi(v) - D_i,0).$$

As $\phi_{S,D_i}$ can be written as a maximum of two potentials, $\phi_{S,D_i}$ is a valid (non-negative) potential according to \cref{fact:potential_min_max}. It therefore remains to verify the two conditions stated in \cref{def:potential}. We first verify the first condition. Consider am arbitrary vertex $v \in S$. We have

\begin{align*}\phi(v) \leq \phi(\sstar) + |\phi(v) - \phi(\sstar)| \leq 0 + \ell_{G_{S,D_i}}(s^*,v) \le D_i
\end{align*}

and therefore $\phi_{S,D_i}(v) = 0$.



To verify the second condition, consider an arbitrary $v \in V$ with $\dist_G(v,S) \geq \frac{D_i}{\valSNC}$. We have



\begin{align*}\phi_{S,D_i}(v) \geq \phi(v) - D_i \geq \frac{\dist_T(\sstar, v)}{1+\eps} - D_i \geq \frac{D_i + \dist_G(v,S)}{1+\eps} - D_i \geq \frac{D_i/\valSNC - \eps D_i}{1+\eps} \geq 0.5\frac{D_i}{\valSNC},
\end{align*}


where the last equality follows from $\eps \leq \frac{1}{10 \valSNC}$. 
\end{proof}



\cyclefour*

\begin{proof}
Directly follows from \cref{thm:sparse_cover} with $D = D_i$.
\end{proof}

\cyclefive*

\begin{proof}
Given the sparse neighborhood cover together with the trees, the only missing piece for the distance structure for the scale $D_i$ is a potential for the scale $D_i$ with respect to $V \setminus C$ for every cluster $C$ in one of the clusterings (which only needs to be known to the nodes inside $C$).

Let $\fC$ be one of the clusterings in the sparse neighborhood cover.  
We show how to simultaneously compute for each cluster $C \in \fC$ a potential for scale $D_i$. 

For each node $v$, let $id(v)$ denote the unique $O(\log n)$-bit identifier of $v$.
We assign each cluster $C \in \fC$ an identifier by concatenating the identifier of its cluster center $id(v_C)$ with the bit-wise negation of $id(v_C)$.
We call the resulting $b$-bit identifier $id(C)$.
For $j \in [b]$, we say that a cluster is active in round $j$ if the $j$-th bit of its identifier is $1$.
Note that for two distinct clusters $C_1,C_2 \in \fC$, there exists at least one round in which $C_1$ is active and $C_2$ is inactive.
We denote with $V_{active,j} \subseteq V$ the set of vertices that are contained in a cluster that is active in round $j$.
In round $j$, we use oracle $\oPot_{D_i}$ with input $V \setminus V_{active,j}$ to compute a potential $\phi_j$ for scale $D_i$ with respect to $V \setminus V_{active,j}$.

For each cluster $C \in \fC$ and $v \in V$, we set $\phi_{V \setminus C, D_i}(v) = \min_{\text{$j \colon$ $C$ is active in round $j$}} \phi_j(v)$.

We show that $\phi_{V \setminus C,D_i}$ is a potential for scale $D_i$ with respect to $V \setminus C$.

First, $\phi_{V \setminus C, D_i}$ is the minimum of non-negative potentials and therefore a non-negative potential itself according to \cref{fact:potential_min_max}.
It therefore remains to verify that $\phi_{V \setminus C, D_i}$ satisfies the two conditions of \cref{def:potential}. To verify the first condition, consider an arbitrary $v \in V \setminus C$. We have to show that $\phi_{V \setminus C, D_i}(v) = 0$. There exists some round $j$ in which $C$ is active and $v$ is not contained in an active cluster. For this $j$, $\phi_j(v) = 0$ and therefore $\phi_{V \setminus C, D_i}(v) = 0$, as desired.


It remains to check the second condition. To that end, consider an arbitrary $v \in V$ with $\dist_G(v,V \setminus C) \geq \frac{D_i}{\valSNC}$.
We need to show that this implies $\phi_{V \setminus C,D_i}(v) \geq 0.5\frac{D_i}{\valSNC}$.
Consider an arbitrary round $j$ in which $C$ is active.
As $\dist_G(v,V \setminus C) \geq \frac{D_i}{\valSNC}$, we have $\dist_G(v,V \setminus V_{active,j}) \geq \frac{D_i}{\valSNC}$ which in turn implies $\phi_j(v) \geq 0.5\frac{D_i}{\valSNC}$.
Hence, $\phi_{V \setminus C,D_i}(v) \geq 0.5\frac{D_i}{\valSNC}$.

The result now follows by iterating over all of the $O(\log n)$ clusterings in the sparse neighborhood cover.
\end{proof}

\cycleeuler*
\begin{proof}
Directly follows from \cref{thm:rounding}. 
\end{proof}


\cyclesix*

\begin{proof}
We prove by induction on $i$ that a distance structure for every scale $D_j$ with $j \leq i$ can be computed in $i \cdot \tilde{O}(1)$ \aggregate rounds.
The base case $i = 1$ directly follows from \cref{lem:cycleone}.
Now, consider an arbitrary $i > 1$ (such that $D_i$ is a scale) and assume that the claim above holds for $i-1$. Hence, we can compute a distance structure for every scale $D_j$ with $j \leq i - 1$ in $(i-1)\tilde{O}(1)$ \aggregate rounds.
Now, applying \cref{lem:cycleone} with the scale $D_i$ implies that in $\tilde{O}(1)$ additional \aggregate rounds we can compute a distance structure for the scale $D_i$, which finishes the induction step.
This finishes the proof, as there are only $O(\log n)$ different scales.
\end{proof}


\cycleseven*

\begin{proof}
Directly follows from the second part of \cref{thm:oblivious_routing}.
\end{proof}

\cycleeight*

\begin{proof}
First, \cref{lem:transshipment_primal_dual} implies that the $(1+\eps)$-transshipment problem can be solved in $\tO(1/\eps^2)$ \aggregate rounds.
Second, the tree returned by the algorithm of \cref{theorem:boosting_rounding} is a $(1+\eps)$-SSSP-tree and the algorithm runs in $\tO(1/\eps^2)$ \aggregate rounds, as each of the $\tilde{O}(1)$ matrix-vector products with $R$ and $R^T$ can be computed in $\tO(1)$ \aggregate rounds.
\end{proof} 

\cyclenine*

\begin{proof}
\cref{lem:cyclesix} states that a distance structure for every scale $D_i$ can be efficiently computed (as $\oRound$ can be implemented with $\oRound_{\eps/2}$).
Together with \cref{theorem:cycleseven}, this implies that there exists an $\tilde{O}(1)$-competitive $\ell_1$-oblivious routing $R$ for $G$ for which $R$ and $R^T$ can be efficiently evaluated.
Combining this with \cref{theorem:cycleeight}, we can conclude that the $(1+\eps)$-transshipment problem and the $(1+\eps)$-SSSP-tree problem in $G$ can be efficiently solved.
\end{proof}

\cycleten*

\begin{proof}
Directly follows from \cref{theorem:cyclenine} together with \cref{lem:cycleeuler}. 
\end{proof}

\mainparallel*

\begin{proof}
\cref{thm:euler_pram} states that there exists a \pram algorithm with near-linear work and $\tO(1)$ depth that implements $\oEuler$. The result now follows by \cref{theorem:cycleten}. 
\end{proof}

\maindistributed*

\begin{proof}
\cref{thm:euler_dist} states that the oracle $\oEuler$ can be implemented with the desired round complexity. The result for the single source shortest path then follows from \cref{theorem:cycleten,thm:oracleSimulation}. 
To extend it to the shortest forest from the set $S$ problem, we add a virtual node $s$ to our graph and connect it to nodes of $S$ via edges of weight $0$ (technically, we do not allow zero weights, but we can choose the weight to be negligible to all other weights). Then, we use the fact that, by definition, the oracle $\oEuler$ supports virtual nodes and, by \cref{thm:simulating-virtual-nodes} we can simulate virtual nodes in the \aggregate model. 
\end{proof}


==> preamble.tex <==
\usepackage{fullpage}
\usepackage{parskip}

\usepackage{amsthm,amsmath,amssymb,booktabs,xcolor,graphicx}
\usepackage{thm-restate}
\usepackage{bbm}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{appendix}
\usepackage{enumerate}
\usepackage{mathbbol}
\usepackage[numbers]{natbib}
\usepackage{comment}
\usepackage[shortlabels]{enumitem}

\usepackage[margin=1in]{geometry}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

%\usepackage[textsize=small,backgroundcolor=orange!20]{todonotes}
\usepackage[disable]{todonotes}
\usepackage[hidelinks]{hyperref}
\usepackage{url}
\usepackage{etoolbox}
\usepackage{appendix}
\usepackage{xspace}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
% \usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage[labelfont=bf]{caption}
\usepackage[noabbrev,capitalize]{cleveref}
\crefname{equation}{}{} %remove ``Equation''    
\newcommand{\creflastconjunction}{, and\nobreakspace} %Oxford comma
\AtBeginEnvironment{appendices}{\crefalias{section}{appendix}} %appendices

\usepackage[color,final]{showkeys} %add in 'final' into parameter to remove showkeys
\renewcommand\showkeyslabelformat[1]{\scalebox{.8}{\normalfont\footnotesize\ttfamily#1}\hspace{-.5em}}
% showkeys font
\colorlet{refkey}{orange!20}
\colorlet{labelkey}{blue!30}

% ------   Theorem Styles -------
\numberwithin{equation}{section}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{algo}[theorem]{Algorithm}
\crefname{claim}{Claim}{Claims}

\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem*{question*}{Question}
\newtheorem{fact}[theorem]{Fact}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{question}[theorem]{Question}
\newtheorem*{definition*}{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{setup}[theorem]{Setup}
\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\newtheorem*{notation}{Notation}
\newcommand{\assign}{\leftarrow}

%\newcommand{\alert}[1]{{\color{orange}#1}}
\newcommand{\alert}[1]{}
\renewcommand{\tilde}{\widetilde}

% ----- Delimiters ----
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\snorm}[1]{\lVert#1\rVert}
\newcommand{\ang}[1]{\left\langle #1 \right\rangle}
\newcommand{\sang}[1]{\langle #1 \rangle}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\sqb}[1]{\left[ #1 \right]}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\setcond}[2]{\left\{ #1 \;\middle\vert\; #2 \right\}}
\newcommand{\cond}[2]{\left( #1 \;\middle\vert\; #2 \right)}
\newcommand{\sqcond}[2]{\left[ #1 \;\middle\vert\; #2 \right]}
\newcommand{\one}{\mathbbm{1}}
\newcommand{\otilde}{\widetilde{O}}
\newcommand{\poly}{\mathrm{poly}}

\newcommand{\fC}{\mathcal{C}}
\newcommand{\mb}{\mathbb}
\newcommand{\potential}{\phi}
\newcommand{\mbf}{\mathbf}
\newcommand{\mbm}{\mathbbm}
\newcommand{\mc}{\mathcal}
\newcommand{\mf}{\mathfrak}
\newcommand{\mr}{\mathrm}
\newcommand{\ol}{\overline}
\newcommand{\on}{\operatorname}
\newcommand{\wh}{\widehat}
\newcommand{\wt}{\widetilde}
\newcommand{\edit}[1]{{\color{red}#1}}
\renewcommand{\l}{\langle}
\renewcommand{\r}{\rangle}
\newcommand{\RFin}[1]{2^{\mb{RP}^#1}_{\on{fin}}}
\newcommand{\g}{\nabla}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\argmin}{\mathrm{argmin}}
\newcommand{\eps}{\varepsilon}
\newcommand{\etal}{\textit{et~al.}}
\newcommand{\Tr}{\mathrm{Tr}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\ls}{\lesssim}
\newcommand{\pe}{\preceq}
\newcommand{\se}{\succeq}
\newcommand{\op}{\mathrm{op}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calS}{\mathcal{S}}
%\newcommand{\dist}{\mathrm{dist}}
\newcommand{\diam}{\textrm{diam}}
\newcommand{\parent}{\textrm{par}}
\renewcommand{\d}{d}
\newcommand{\Dpad}{D_\textrm{pad}}
\newcommand{\fO}{\mathcal{O}}
\newcommand{\setssp}{set-source shortest path\xspace}
\newcommand{\tO}{\tilde{O}}
\newcommand{\tG}{\tilde{G}}
\newcommand{\fP}{\mathcal{P}}
\newcommand{\polylog}{\mathrm{polylog\ }}
\newcommand{\btodo}[1]{{\bfseries ToDo: #1}\\}
\newcommand{\congest}{\ensuremath{\mathsf{CONGEST}}\xspace}
\newcommand{\congestPA}{\ensuremath{\mathsf{CONGEST}^{PA}}\xspace}
\newcommand{\aggregate}{\ensuremath{\mathsf{Minor}}\text{-}\ensuremath{\mathsf{Aggregation}}\xspace}
\newcommand{\pram}{\ensuremath{\mathsf{PRAM}}\xspace}
\newcommand{\euler}{\ensuremath{\textsc{Eulerian-}\textsc{Orientation}}\xspace}
\newcommand{\1}[1]{\mathbb{1}[#1]}
\newcommand{\cheat}{\ensuremath{^{\mathrm{cheat}}}\xspace}
\newcommand{\Path}{\mathrm{Path}}

\newcommand{\oEuler}{\fO^{Euler}}
\newcommand{\oRound}{\fO^{Round}}
\newcommand{\oDist}{\fO^{Forest}}
\newcommand{\oForest}{\fO^{Forest}}
\newcommand{\oPot}{\fO^{Pot}}
\newcommand{\oObliv}{\fO^{Obliv}}

\newcommand{\Dhop}{\hopDiameter{G}}
\newcommand{\sstar}{s^*}
\newcommand{\vD}{v_D}
\newcommand{\Lref}[1]{{\text{L\ref{#1}}}}
\newcommand{\Tref}[1]{{\text{T\ref{#1}}}}
\newcommand{\Pref}[1]{{\text{P\ref{#1}}}}
\newcommand{\Coref}[1]{{\text{C\ref{#1}}}}

\newcommand{\defeq}{\stackrel{\mathrm{\scriptscriptstyle def}}{=}}
\newcommand{\opt}{\mathrm{OPT}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\cost}{{\mathrm{cost}}}
\newcommand{\shortcutQuality}[1]{\mathrm{Shortcut}\-\mathrm{Quality}(#1)}
\newcommand{\hopDiameter}[1]{\mathrm{Hop}\-\mathrm{Diam}(#1)}
\newcommand{\diameter}{\mathrm{HopDiameter}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\virt}{\ensuremath{_{\mathrm{virt}}}\xspace}

\newcommand{\bnote}[1]{{\bfseries B: #1}}
\newcommand{\todob}[1]{}   %these are markers for my todo list

\newcommand{\core}{\mathrm{core}}
\newcommand{\pad}{\mathrm{pad}}
\newcommand{\Vrem}{V_\textrm{remaining}}
\newcommand{\Valive}{V_\textrm{alive}}
\newcommand{\Vdead}{V_\textrm{dead}}
\newcommand{\Vactive}{V_{\text{active}}}
\newcommand{\PA}{\ensuremath{^{\mathrm{PA}}}\xspace}

\newcommand{\valSNC}{\tau}

\newcommand{\minorplusvirtual}{\textrm{Class}}


% Local Variables:
% TeX-master: "main"
% End:



==> preliminaries.tex <==

\section{Preliminaries and Terminology}\label{sec:preliminaries}

In this section, we first review some basic terminology related to graphs, clusterings, shortest paths and (transhipment) flows. Afterwards, we describe the computational models we use in this paper.

\paragraph{Graphs.} 
For a graph $G$ we use $V(G), E(G)$ to denote its node set and edge set, respectively. The set of neighbors of a node $v$ is denoted with $\Gamma_G(v) \subseteq V$.
An eulerian graph is a graph with $|\Gamma_G(v)|$ being even for every $v \in V(G)$.
It is often convenient to direct $E$ consistently. For simplicity and without loss of generality, we assume that $V = \{v_1, v_2, \ldots, v_{n}\}$ and define $\vec{E} = \{ (v_i,v_j) \mid (v_i, v_j) \in E, i < j\}$. We identify $E$ and $\vec{E}$ by the obvious bijection. We chose this orientation for simplicity and concreteness: arbitrarily changing the orientations does not influence the results (if done consistently). We also introduce the notation $\overleftrightarrow{E}$ which includes each edge of $\{u, v\} \in E$ in both directions: $(u, v) \in \overleftrightarrow{E}$ and $(v, u) \in \overleftrightarrow{E}$. 


A weighted graph $G$ is an undirected graph, together with a function $\ell_G : E \rightarrow \{1, \ldots, n^{O(1)}\}$ that assigns a polynomially-bounded non-negative weight to each edge in $E$. We sometimes use just $\ell$ if $G$ is clear from context. This weight function induces a distance function $\dist_G(u, v)$ on $G$. For two sets of nodes $A,B \subseteq V(G)$ we define $\dist_G(U,W) = \min_{u \in U, w \in W} \dist_G(u, w)$ and sometimes write $\dist_G(U, w)$ for $\dist_G(U, \{w\})$. 
A ball $B_G(u, r)$ of radius $r$ around a node $u$ is a set of nodes $v$ such that $\dist_G(u, v) \le r$. The diameter of a weighted graph $G$ is defineed as $\diam(G) = \max_{u,v} \dist_G(u,v)$ and its hop diameter $\hopDiameter{G}$ is the longest unweighted shortest path (i.e., in terms of hops and not weight). 

\paragraph{Clusters and Clusterings.}
A \emph{cluster} $C$ is a set of nodes $C \subseteq V(G)$. 
A \emph{clustering} $\fC$ is a collection of disjoint clusters.
Finally, a \emph{sparse neighborhood cover} of a graph $G$ with \emph{covering radius} $R$ is a collection of $\gamma := O(\log n)$ \footnote{Sometimes we use $\log(\cdot)$ outside the $O$-notation, in which case it stands for $\log_2(\cdot)$. \alert{is this even used anywhere?} } clusterings $\fC_1, \dots, \fC_\gamma$ such that for each node $v \in V(G)$ there exists some $i \in \{1,\ldots,\gamma\}$ and some $C \in \fC_i$ with $B(v, R) \subseteq C$. 


%\paragraph{Smooth Functions}

%We say that a function $\phi: V(G) \rightarrow [n^{O(1)}]$ is \emph{smooth} if it satisfies that for any two nodes $u, v$ we have $\phi(u) - \phi(v) \le \dist_G(u, v)$. Equivalently, we can require that for any edge $\{u, v\}$ we have $\phi(u) - \phi(v) \le \ell(\{u,v\})$. 

%\begin{fact}
%\label{fact:smoothMinMaxSum}
%Let $\phi_1, \phi_2, \dots, \phi_k$ be smooth.  
%Then $\sum_{i = 1}^k \phi_i/k,\, \min_{i = 1}^k \phi_i,\, \max_{i  = 1}^k \phi_i$ is smooth. 
%\end{fact}

\paragraph{Flows, Transshipment, and SSSP.}
Given a graph $G=(V,E)$, a flow is either a function $f:\overleftrightarrow{E}\to\mathbb R_{\ge0}$ (that is identified with a vector $\R_{\ge 0}^{\overleftrightarrow{R}}$ by the obvious identification), or a function $f : \vec{E} \to \R$ (identified with $\R^{\vec{E}}$). We often use one or the other flow notation for convenience. Given $f \in \overleftrightarrow{E}$, we can covert it to $f' \in \vec{E}$ by letting $(f')_{(u, v)} := f(u, v) - f(v, u)$ and, similarly, in the other direction $f_{(u, v)} := \1{(u, v) \in \vec{E}} f'_{(u, v)} - \1{(v, u) \in \vec{E}} f'_{(v, u)}$. A \emph{demand} $b$ is simply a function $b : V \to \mathbb{R}$ (or equivalently $\R^V$) satisfying $\sum_{v \in V} b_v = 0$. We say a flow $f \in \R^{\overleftrightarrow{E}}$ \emph{satisfies} a demand $b \in \R^V$ if for all $v \in V$, we have $\sum_{u:(u,v)\in\overleftrightarrow{E}}(f(u,v)-f(v,u))=b(v)$. Given edge weights $\ell \in \R^{E}$, the \emph{transshipment cost} of the flow is $\ell(f) := \sum_{(u,v)\in\overleftrightarrow E}\ell(\{u,v\})f(u,v)$.

Furthermore, we say that a function $\phi: V(G) \rightarrow \mathbb{R}$ (a vector in $\mathbb{R}^{V(G)}$) is a \emph{potential} if $|\phi(u) - \phi(v)| \le \dist_G(u, v)$ for all $u,v \in V$. Equivalently, we can require that for every edge $\{u, v\}$ we have $|\phi(u) - \phi(v)| \le \ell(\{u,v\})$. We note the following useful fact about potentials.
\begin{fact}
\label{fact:potential_min_max}
If $\phi_1, \phi_2, \ldots, \phi_k$ are potentials, then $\phi_{min}$ and $\phi_{max}$ are also potentials. Here, $\phi_{min}(v) = \min_{i \in [k]} \phi_i(v)$ and
$\phi_{max}(v) = \max_{i \in [k]} \phi_i(v)$ for all $v\in V$.
\end{fact}

This now allows us to formally define (approximate) transshipment and SSSP.
\begin{definition}[Transshipment]
  Given a (connected) graph $G = (V, E)$ with lengths $\ell \in \R^E$ and a demand $b \in \R^V$, the transshipment problem asks us to find (1) a flow $f \in \R^{\vec{E}}$, and (2) a potential $\potential \in \R^V$ that minimize/maximize their respective program in the following primal-dual formulation:
  \begin{align*} % \label{eq:transshipmentLP}
    \min~ \ell(f) : \text{$f$ is a flow satisfying $b$}, && \max~ b^{\top} \potential : \text{$\potential$ is a potential}. %\label{eq:transshipmentDualLP}
  \end{align*}
  For $\alpha \ge 1$, a solution $(f, \potential)$ is $\alpha$-approximate if both $f$ and $\potential$ are feasible ($f$ satisfies $b$, $\potential$ is a potential), and $\ell(f) \le \alpha \cdot b^{\top} \potential$. Note that a $1$-approximate solution is optimal.
\end{definition}
\begin{definition}[SSSP and \setssp] 
  Suppose we are given a (connected) graph $G = (V, E)$ with lengths $\ell \in \R^E$. Given a \emph{set-source} $S \subseteq V$, the $\alpha$-approximate \setssp problem asks us to compute a forest $F$ spanning $G$ such that $\dist_F(S, u) \le \alpha \cdot \dist_G(S, u)$ for each node $v \in V$. The problem is called $\alpha$-approximate SSSP when $S = \{ s \}$. The singleton node $s \in S$ is called the \emph{source}.
\end{definition}

% A \emph{demand} is a $b \in \R^{V}$. We say a demand is \emph{proper} if $\one^T b=0$. A \emph{flow} is a vector $f \in \R^{\vec{E}}$. A flow $f$ \emph{routes} demand $b$ if $Bf = b$. It is easy to see only proper demands are routed by flows. The cost $\ell(f)$ of a flow $f$ is $\norm{Lf}_1$.
% %
% For a weighted graph $G$ and a given proper demand $b$ the \emph{transshipment problem} asks to find a flow $f_d^*$ of minimum cost among flows that route $b$. When the underlying graph is clear from the context, we let $\norm{b}_\opt := \ell(f_d^*)$ denote the cost of the optimal flow for routing demand $b$. For any $\alpha \geq 1$, we say a flow $f$ is $\alpha$-\emph{approximate} if $\ell(f) \leq \alpha \cdot \norm{b}_\opt$ (such a flow does not necessarily need to route $b$).
% %
% n the vector $\phi \in \R^{V}$ are generally referred to as vertex \emph{potentials}.
 
% \todo{merge with description below}

\paragraph{$\ell_1$-Oblivious Routing.}
Let $G = (V, E)$ be a fixed graph with weights $\ell \in \R_{\ge 0}^{E}$. For a demand $b \in \R^V$ with $\sum_{v \in V} b_v = 0$ we define $\norm{b}_\opt := \ell(f_b^*)$ to be the cost of the minimum-cost flow that satisfies the demand $b$. Then, the $\ell_1$-oblivious routing is defined as follows.

%For any $k$ and $\alpha > 1$, Sherman~\cite{She17b} defined an $\alpha$-approximate (linear) $\ell_1$-preconditioner for a weighted graph $G$ as a $k \times n$ matrix $P$, such that, for any proper demand $d$ it holds that $$\norm{d}_\opt \le \norm{P d}_1 \le \alpha \norm{d}_\opt.$$ Any such $\alpha$-preconditioner which can be computed in $T$ rounds can be used to give a $\tilde{O}(\eps^{-2} \alpha^2 T)$ algorithm for transshipment~\cite{She17}. We are constructing a strictly stronger object that is required to output a flow that routes any demand with $\alpha$-approximate cost.

\begin{definition}[$\ell_1$-oblivious routing]
  For a graph $G=(V,E)$, a matrix $R \in \R^{\vec{E} \times V}$ is called a (linear) $\ell_1$-oblivious routing if for any demand $b \in \R^V$ with $\sum_{v \in V} b_v = 0$ the flow $f := R b \in \R^{\vec{E}}$ satisfies the demand $b$. Furthermore, an $\ell_1$-oblivious routing $R$ is $\alpha$-competitive if for all demands $b \in \R^V$ with $\sum_{v \in V} b_v = 0$ we have that the cost of the flow $f_{R,b}:=Rb$ is at most $\alpha \norm{b}_\opt$, i.e., $\ell(f_{R,b}) \leq \alpha \cdot \norm{b}_\opt$.
\end{definition}



% \iffalse
% We still don't know what the right way and definition to talk about smoth distances. We thus won't use any such terminology here and simply stick to the standard language of approximate shortest path trees and transshipment potentials.

% \subsection{Smooth Distance Function}

% For a given subset $S \subseteq V$ of \emph{source nodes} we say a function $\dist_S : V\times V \rightarrow [n^{O(1)}]$ is a valid distance (upper bound) function if $\dist_S(s)=0$ for every node $s \in S$ and if for every node $u \in V$ it holds that $\dist_S(u) \geq d_G(S,u)$. \alert{(G) what is dist(s) .. it's a 2-ary function?}
% Throughout the paper we assume (for now) that there is a single source, i.e., $|S|=1$, but all results and notions straightforwardly carry over to larger $S$.  \alert{(G) so the definitions don't carry over or are we talking about the general problem of solving SSSP? why not just write out the definitions?} 
% We also usually assume that $s$ is always the designated source node and in that case largely omit $S = \{s\}$ from subscripts of $\dist$.

% \begin{definition}[strongly-approximate $\alpha$-approximate SSSP distance]
% A valid distance function $\dist$ for a graph $G$ and source node $s$ is strongly $\alpha$-approximate for some $\alpha \geq 1$ if $$\forall u,v: \ \ |\dist(u) - \dist(v)| \leq \alpha \cdot d_G(u,v).$$
% \end{definition}
% \begin{definition}[(perfectly) tree-like distance functions]
% Let $\dist$ be a valid distance on $G$. We say $\dist$ is tree-like if $$\forall u \neq s: \ \exists v \in \Gamma_G(u): \ \ \dist(v) \leq \dist(u) - w_G(u,v)$$
% or, equivalently, if 
% $$\forall u \neq s: \ \min_{v \in \Gamma_G(u)} \dist(v) + w_G(v,u) \leq \dist(u).$$
% We furthermore say $\dist$ is perfectly tree-like if 
% $$\forall u \neq s: \ \min_{v \in \Gamma_G(u)} \dist(v) + w_G(v,u) = \dist(u).$$
% \end{definition}
% \fi



\subsection{Model: Minor-Aggregation for \pram}
\label{subsec:intro_minor_aggregation}

In this section we give a minimal-but-complete description of the \aggregate interface, which exposes to the user the following operations on a graph: (1) contract edges, thereby operating a minor, (2) each (super)node in the contracted graph can compute an aggregate (e.g., min, max, sum) of surrounding neighbors, and (3) add $\tilde{O}(1)$ arbitrarily-connected virtual nodes over the course of the algorithm. The goal is to design $\tO(1)$-round algorithms in this model. Such a \aggregate algorithm can be compiled to a near-optimal algorithm in both the parallel and distributed settings.

The full model, as defined in \cite{goranci2022universally,ghaffari2021universally}, is used in the distributed setting which requires specifying some low-level details we can leave out here. For a more in-depth discussion of \aggregate and its extensions to distributed models see \Cref{sec:computational-models}.

\textbf{Aggregations.} An \emph{aggregation operation} $\bigoplus$ is any associative function that combines two $\tilde{O}(1)$-bit inputs into one of equal size (e.g., sum or max). For multiple inputs $x_1, x_2, \ldots, x_k$, their \emph{aggregate} $\bigoplus_{i=1}^k x_i$ is defined by arbitrarily aggregating messages until one remains.

\begin{definition}[Minor-Aggregation model in \pram]\label{def:aggregation-congest-intro}
  We are given an undirected graph $G = (V, E)$. There is a single \pram processor and private memory associated with each node and each edge. Between-processor communication happens during synchronous rounds, and processors perform $\tilde{O}(1)$-work local computation between rounds. Each round consists of the following three steps (in that order).
  \begin{itemize}
  \item \textbf{Contraction step.} Each edge (associated processor) $e$ chooses a value $c_e = \{\bot, \top\}$. This defines a new \emph{minor network} $G' = (V', E')$ constructed as $G' = G / \{ e : c_e = \top \}$, i.e., by contracting all edges with $c_e = \top$ and self-loops removed. Vertices $V'$ of $G'$ are called supernodes, and we identify supernodes with the subset of nodes $V$ it consists of, i.e., if $s \in V'$ then $s \subseteq V$.

  \item \textbf{Consensus step.} Each individual node $v \in V$ chooses a $\tilde{O}(1)$-bit value $x_v$. For each supernode $s \in V'$ we define $y_s := \bigoplus_{v \in s} x_v$, where $\bigoplus$ is some aggregation operator. All nodes $v \in s$ learn $y_s$.

  \item \textbf{Aggregation step.} Each edge $e \in E'$ connecting supernodes $a \in V'$ and $b \in V'$ learns $y_a$ and $y_b$, and chooses two $\tilde{O}(1)$-bit values $z_{e, a}, z_{e, b}$ (i.e., one value for each endpoint). Finally, (every node of) each super $s \in V'$ learns the aggregate of its incident edges in $E'$, i.e., $\bigotimes_{e \in \text{incidentEdges(s)}} z_{e, s}$ where $\bigotimes$ is some aggregation operator.
  \end{itemize}
\end{definition}

\smallskip

\textbf{PRAM simulation.} Simulating contractions and aggregations is a well-known and simple primitive in \pram that can be performed in $\tilde{O}(1)$ time and $\tilde{O}(m)$ work (see e.g. \cref{thm:oracleSimulation}). 

We note that the following operations can be efficiently simulated.
\begin{itemize}
\item \textbf{Minors.} It is immediate from the model that any \aggregate algorithm can be run on a minor in a black-box manner.
\item \textbf{Node-disjoint scheduling.} Similarly, it is immediate that we can simultaneously run separate algorithms on node-disjoint and connected subgraphs of $G$.
\item \textbf{Virtual nodes.} Given a graph $G$, we can construct a \emph{virtual graph} by starting with a connected graph and repeatedly adding a \emph{virtual node} that is connected to an arbitrary set of neighbors. Due to the constraints in the distributed setting, we constrain the number of virtual nodes to $\tilde{O}(1)$. A \aggregate round on such graphs can be simulated in \pram with $\tilde{O}(m)$ work and $\tilde{O}(1)$ depth. For example, we frequently use this operation to connect a ``supersource'' node, enabling us to use our standard SSSP algorithm to implement a set-source-$S$ shortest path.
\end{itemize}

\textbf{Distributed storage and input.} Our \aggregate algorithms operate on objects that are \emph{``distributedly'' stored}, meaning that each processor has its own part of the object in private memory. Specifically, we store a \emph{node vector} $x \in \R^V$ by storing $x_v$ in node $v$. Similarly, edge vectors $x \in \R^{E}, x \in \R^{\vec{E}}, x\in \R^{\overleftrightarrow{E}}$ are distributed over edges. Subgraphs $H \subseteq G$ are specified by distributedly storing the characteristic vectors $\mathbb{1}_{V(H)} \in \R^{E(G)}$ and $\mathbb{1}_{E(H)} \in \R^{E(G)}$. Initially, the problem-specific input is assumed to be distributedly stored. For transshipment and SSSP, we assume the lengths (edge vector) and demands (node vector) are stored. At termination, the output is required to be stored.

\textbf{Oracles.} An oracle is a black-box function that takes a certain input (on the original graph) and produces a specified output. An algorithm with access to an oracle can, in each round, choose to perform a regular \aggregate round, or to call a single oracle (i.e., multiple oracle calls per round are forbidden). Some oracles we use only have an efficient \pram implementation, but no efficient \aggregate implementation.

%For example, \emph{partwise aggregation} oracle takes the private input and part ID on each node and outputs at each node the corresponding partwise aggregate.

\textbf{Ancestor and subtree sums.} The following operation is often useful. Given a (distributedly stored) tree $T$ and a root $r \in V(T)$, there is a deterministic $\tilde{O}(1)$-round \aggregate algorithm that computes for each node the ancestor and descendent sum (or a general aggregate) with respect to $T$ rooted at $v$ (see \Cref{lemma:ancestor-subtree-sum} for a fully formal version).


% Local Variables:
% TeX-master: "main"
% End:


==> relatedWork.tex <==
\section{Further Related Work}
\label{sec:morerelatedwork}


We briefly mention few results out of a large body of works on SSSP and the related all pairs shortest paths (APSP) problem. 

While our paper focuses on the undirected variant of the problem, there is a long line of work on the directed variant. Many results on parallel algorithms mentioned in \cref{sec:intro} work for directed graphs. 
There is a long list of recent results in the \congest model on the directed shortest path problem \cite{GL18,FN18,CM20,CFR21,CLP21}. 


Finding a shortest path becomes much simpler if we can assume that it only has a small number of hops (edges). 
This motivates a successful line of work 
\cite{ullman1991high,cohen1994polylog,klein1997randomized,thorup2005approximate,thorup2006spanners,bernstein2009fully,henzinger2014decremental,Nan14,holzer2014approximation,miller2015improved,henzinger2016almost,EN16,abboud2018hierarchy,huang2019thorup} on the construction of so-called \emph{hopsets} -- small sets of edges that we can add to a graph to make the shortest paths use a small number of hops, while distorting the distances only by a small amount. 

The (approximate) SSSP problem is studied in many different models besides the parallel and the distributed one. 
To give some examples, it is studied in the (semi-) streaming model \cite{elkin2006efficient,feigenbaum2009graph,guruswami2016superlinear,henzinger2016almost,EN16}, the congested clique model \cite{Nan14,censor2019algebraic,le2016further,henzinger2016almost,censor2020fast}, Broadcast \congest model~\cite{BKKL17}, Hybrid model~\cite{AHKSS20,FHS20,kuhn2020computing,CLP21}, or the dynamic algorithms model \cite{shiloach1981line,henzinger2014decremental,henzinger2014sublinear}. 


%Indeed, known algorithms build on matrix multiplication or on transitive closure routines with $O(n^{3})$ work. 
%There is a line of work \cite{ullman1991high,klein1997randomized,spencer1997time,shi1999time} on randomized algorithms with different processor-time trade-offs but without much improvement on the cubic work bound for fast parallel algorithms. Cohen \cite{cohen1997using} gave a deterministic algorithm with similar trade-offs. 
%Another line of work \cite{galil1997all,alon1997exponent,zwick1998all} gave $(1+\eps)$-approximate all pairs shortest paths (APSP) algorithms with work equal to $\tO(n^{\omega})$, where $\omega < 2.37\dots$ is the fast matrix multiplication exponent~\cite{alman2021refined} . 

The related (directed) APSP problem was also considered in various distributed and parallel models \cite{galil1997all,alon1997exponent,zwick1998all,coppersmith1987matrix,alman2021refined,a1,censor2019algebraic,holzer2014approximation,le2016further,Elk17,huang2017distributed,agarwal2018deterministic,censor2020sparse,pontecorvi2018distributed,agarwal2019distributed,bernstein2019distributed,augustine2020shortest,agarwal2020faster,censor2020fast,dory2020exponentially,kuhn2020computing,censor2021sparsity}.

% Local Variables:
% TeX-master: "main"
% End:




==> rounding.tex <==
\section{Transshipment Flow Rounding}
\label{sec:rounding}

\newcommand{\lrE}{\overleftrightarrow{E}}
\newcommand{\rH}{\overrightarrow{H}}


In this section, we prove the following theorem. Note that the returned solution is exact (i.e., has $\eps = 0$), even though an $(1+\eps)$-approximate solution would suffice. We remind the reader of the definitions of $\oRound_{0}$ and $\oEuler$ from \Cref{def:oracle_rounding,def:oracle_euler}.

\begin{theorem}[Rounding]
\label{thm:rounding}
Let $G$ be a weighted graph. The oracle $\oRound_{0}$ can be implemented in $\poly(\log n)$ \aggregate rounds and $\poly(\log n)$ oracle calls to $\oEuler$. 
\end{theorem}

The rest of the section is dedicated to the proof. Our algorithm is inspired by Cohen's rounding algorithm for integral flow~\cite{cohen1995approximateMaxFlow} in which one is given a fractional flow that satisfies integral demand constraints, and the algorithm constructs an integral flow of non-increased cost that satisfies the same demand. The algorithm uses bit-scaling, meaning that for $i = \log n, \ldots, 0$ (in decreasing order) it rounds the flow values to multiples of $2^{-i}$. The main observation is that, in the $i$-th step, the set of edges which are not multiples of $2^{-i}$ (but are multiples of $2^{-i-1}$ by the invariant), form a Eulerian graph (all nodes have even degrees). Such a graph can be decomposed into a collection of directed cycles, and on each cycle we either add or subtract $2^{-i-1}$. This does not impact the demand the flow satisfies, but makes the flow values multiples of $2^{-i}$, as requested. We extend this algorithm to round a fractional flow into a forest (or more precisely, a disjoint union of out-arborescences).

%\begin{theorem}
%Consider a graph $G=(V,E)$ with edge weights $\ell$, and consider a demand vector $b:V\to\mathbb R$ such that $b(v)\ge0$ for all $v\in V$ except for some $s\in V$ called the source. Let $f$ be a flow satisfying demand $b$ whose values $f(u,v)$ can be represented in binary using $O(\log n)$ bits before and after the decimal. There is a parallel algorithm that constructs in $\tilde{O}(m)$ work and $\tilde{O}(1)$ time a tree $T$ spanning all vertices $\{v:b(v)\ne0\}$ such that $\sum_{v:b(v)\ne0}b(v)d_T(s,v) \le \ell(f)$.
%\end{theorem}


For simplicity, we assume that each $b(v)$ is now an integer with absolute value $\textup{poly}(n)$. (This can be guaranteed by first multiplying each $f(u,v)$ by a large enough $\textup{poly}(n)$ so that each $f(u,v)$ and $b(v)$ is integral, and then computing the tree $T$ with this modified instance, which is still a satisfying tree for the original instance since both $\sum_{v:b(v)\ne0}b(v)d_T(s,v)$ and $\ell(f)$ are scaled by the same amount.)

Our algorithm proceeds in phases, from phase $i=0$ up to $\lceil\lg(-b(s))\rceil$. Initialize $f_0=f$; we maintain the invariant that each flow $f_i$ satisfies some demand $b_i$ whose entries are all integer multiples of $2^i$. 
In each phase $i$, our goal is to split $f_i$ into two flows $f_{i+1}$ and $\tilde f_i$ (i.e., $f_i=f_{i+1}+\tilde f_i$) such that (1) flow $\tilde f_i$ is supported on a collection of arc-disjoint paths with $f(u,v)=2^i$ for each arc $(u,v)$ on some path, and (2) all flow values in $f_{i+1}$ are integer multiples of $2^{i+1}$.
Since the initial $f_0$ is assumed to be integral, property~(2) means that we maintain the invariant that each flow $f_j$ has values that are integer multiples of $2^j$.

In each phase $i$, the algorithm does the following:
 \begin{itemize}
 \item Compute an out-arborescence $A_i$ rooted at $s$ supported by arcs $\{(u,v)\in\lrE:f_i(u,v)>0\}$ and spanning all vertices $v\in V:b_i(v)>0$. We later show in \Cref{lem:arbor} that this can be done in $O(\log n)$ rounds of \aggregate.
 \item Let $O_i=\{v\in V:b_i(v)\bmod2^{i+1}=2^i\}$ ($O_i$ for ``odd''). We construct a subgraph $B_i$ of $A_i$ by taking all arcs $(u,v)$ in $A_i$ where the subtree rooted at $v$ in $A_i$ contains an odd number of vertices in $O_i$.
 \item Define flow $\tilde f_i:\lrE\to\mathbb R_{\ge0}$ as $\tilde f_i(u,v)=2^i$ if $(u,v)$ is in $B_i$, and $\tilde f_i(u,v)=0$ otherwise.
 \item Construct a directed graph $H_i$ as follows: for each arc $(u,v)\in\lrE$ satisfying\linebreak $(f_i(u,v)-\tilde f_i(u,v))\bmod2^{i+1}=2^i$, add arc $(u,v)$ to $H_i$. We will prove that each vertex in $H$ has an even number of incident arcs. 
 \item Since the undirected version of $H$ is Eulerian, we call $\oEuler$ on the undirected $H$ to obtain an edge orientation where each vertex in $H$ has the same number of in-edges and out-edges. Define function $h_i:\lrE\to\mathbb R$ as $h_i(u,v)=2^i$ if the orientation of $(u,v)$ is $(u,v)$, and $h_i(u,v)=-2^i$ if it is $(v,u)$, and $h_i(u,v)=0$ for $(u,v)$ not in $H$.
 \item Define $f_{i+1}$ as either $f_i-\tilde f_i\pm h_i$, where we choose $+$ or $-$ depending on whichever minimizes $\ell(f_{i+1})$.
 \end{itemize}
Using $f_i$ and $B_i$, the algorithm now recovers a tree $T$ such that $\sum_{v\ne s}b(v)d_T(s,v)\le \ell(f)$ as follows. Initialize distance upper bounds $\tilde d(s)=0$ and $\tilde d(v)=\infty$ for all $v\ne s$, and initialize the parent function $p(v)=\bot$ for all $v\in V$. For $i$ in decreasing order, do the following:
 \begin{itemize}
 \item Partition $B_i$ into a (disjoint) set of maximal arborescences. For each such arborescence $A \subseteq B_i$ on vertices $U$ with root $r\in U$, set $\tilde d(u) \gets \min\{\tilde d(u),\tilde d(r)+d_{A}(r,u)\}$ for all $u\in U$ (in parallel). Also, for all $u\in U\setminus\{r\}$ whose value $\tilde d(u)$ was lowered, set $p(u)$ to the parent of $u$ in $A$. We note that the exact distances to the root of the arborescence can be computed in $\tilde{O}(1)$ rounds (e.g., via \Cref{lemma:ancestor-subtree-sum}).
 \end{itemize}

\subsection{Correctness}


\begin{lemma}\label{lem:structure}
The following properties are satisfied for each $i$:
 \begin{enumerate}
% \item Flow $\tilde f_i$ is supported on a collection of arc-disjoint paths with $f(u,v)=2^i$ for each arc $(u,v)$ on some path.
 \item $f_{i+1}+\tilde f_i$ satisfies demand vector $b_i$.
 \item All flow values in $f_{i+1}$ are integer multiples of $2^{i+1}$.
 \item For the demands $b_{i+1}$ satisfied by $f_{i+1}$, we have $b_{i+1}(v)\ge0$ for all $v\ne s$.
 \item The conditions of \Cref{lem:arbor} are satisfied on flow $f_i$, so that an arborescence $A_i$ rooted at $s$ is successfully found.% supported by arcs $\{(u,v)\in\lrE:f_i(u,v)>0\}$ spanning all vertices $v\in V:b_i(v)>0$.
 \item The flow $\tilde f_i$ satisfies $\tilde f_i(u,v)\le f_i(u,v)$ for all $(u,v)\in\lrE$.
 \item The flow $f_i-\tilde f_i$ satisfies a demand vector whose entries are multiples of $2^{i+1}$.
 \item The graph $H_i$ is Eulerian.
 \item We have $f_{i+1}(u,v)\ge0$ for all $(u,v)\in\lrE$ and $\ell(f_{i+1})+\ell(\tilde f_i)\le \ell(f_i)$.
 \end{enumerate}
\end{lemma}
\begin{proof}
We prove the properties together by induction on $i\ge0$, where we assume properties~(2)~and~(3) for $i-1$ if $i>0$ (and obtain them for free when $i=0$) and prove all nine properties for $i$.
 \begin{enumerate}
% \item[(1)] Property~(1) follows immediately by construction.
 \item[(4)] Property~(4) follows from property~(3) on $i-1$.% For simplicity, define $V^+=\{v\in V:b_i(v)>0\}$ and $\overrightarrow E^+=\{(u,v)\in\lrE:f_i(u,v)>0\}$. By property~(4) for $i-1$, only $b_i(s)$ is negative, so any decomposition of the flow $f_i$ into paths in $\overrightarrow E^+$ must consist of $s$--$v$ paths for each $v\in V^+$. Consider the graph $G'$ of the union of all such paths (which may not span all vertices in $V$). Since $s$ can reach all vertices in $G'$, the minimum cut between $s$ and any other vertex in $G'$ is at least $1$. By Edmonds' arborescence packing theorem, there is a spanning arborescence in $G'$, which is an arborescence in $\overrightarrow E^+$ spanning $V^+$. This completes property~(4).
 \item[(5)] We have $\tilde f_i(u,v)=2^i$ for all $(u,v)$ in $B_i$, which is contained in $A_i$, which is comprised of arcs $(u,v)\in \overrightarrow E^+$ with $f_i(u,v)>0$. By property~(2) on $i-1$, we also have $f_i(u,v)$ is a multiple of $2^i$, so $f_i(u,v)\ge2^i$. Property~(5) follows.
 \item[(6)] For each $v$, let $N_v$ denote the number of vertices in $O_i$ in the subtree rooted at $v$ in $A_i$. Let $C_v$ denote the children of $v$ in $A_i$. Then, the summation $N_v+\sum_{u\in C_v}N_u$ double-counts every vertex in $O_i$ in the subtree rooted at $v$, except possibly $v$. In other words, the summation is odd iff $v\in O_i$. Equivalently, $v\in O_i$ iff there are an odd number of odd terms in the summation, which by definition of $B_i$ means that $v$ is incident to an odd number of arcs in $B_i$. By construction of $\tilde f_i$, it follows that for the demand vector $\tilde b_i$ satisfied by $\tilde f_i$, we have $\tilde b_i(v)\equiv2^i\bmod2^{i+1}$ iff $v\in O_i$.

Therefore, if $v\in O_i$, then $b_i(v)-\tilde b_i(v)\equiv 2^i-2^i\equiv0\bmod2^{i+1}$. By property~(2) on $i-1$, the values of flow $f_i$ are all multiples of $2^i$, so for $v\notin O_i$, we have $b_i(v)\equiv0\bmod2^{i+1}$, which along with $\tilde b_i(v)=0\bmod2^{i+1}$ gives $b_i(v)-\tilde b_i(v)\equiv0\bmod2^{i+1}$, finishing property~(6).
 \item[(7)] By property~(6) proved above, $b_i(v)-\tilde b_i(v)\equiv0\bmod2^{i+1}$. We can write $b_i(v)-\tilde b_i(v)$ as 
\begin{align*}
 b_i(v)-\tilde b_i(v)&=\sum_{u:(u,v)\in\lrE}\big((f_i(u,v)-f_i(v,u))-(\tilde f_i(u,v)-\tilde f_i(v,u))\big) 
\\&= \sum_{u:(u,v)\in\lrE}\big( (f_i(u,v)-\tilde f_i(u,v))-(f_i(v,u)-\tilde f_i(v,u)) \big) .
\end{align*}
 By property~(2) on $i-1$ and by construction of $\tilde f_i$, all values $f_i(u,v)-\tilde f_i(u,v)$ are multiples of $2^i$. It follows that there are an even number of $(u,v)$ or $(v,u)$ satisfying $f_i(u,v)-\tilde f_i(u,v)\equiv2^i\bmod2^{i+1}$ or $f_i(u,v)-\tilde f_i(u,v)\equiv2^i\bmod2^{i+1}$ respectively. It follows that $H_i$ is Eulerian, concluding property~(7).
 \item[(8)] We first prove $f_{i+1}(u,v)\ge0$ for all $(u,v)\in\lrE$. Recall that $f_{i+1}=f_i-\tilde f_i\pm h_i$, so by property~(5), it suffices to only consider $(u,v)$ in $H$. By construction, we have $(f_i(u,v)-\tilde f_i(u,v))\bmod2^{i+1}=2^i$  for all arcs $(u,v)$ in $H$, and along with property~(5), this means that $f_i(u,v)-\tilde f_i(u,v)\ge2^i$. Adding or subtracting $h_i(u,v)$ can decrease the value by at most $2^i$, so $f_i(u,v)-\tilde f_i(u,v)\pm h_i(u,v)\ge0$.

Finally, $\ell(f_{i+1})+\ell(\tilde f_i)\le \ell(f_i)$ follows from the fact that $\frac12\big(\ell(f_i-\tilde f_i+h_i)+\ell(f_i-\tilde f_i-h_i)\big)=\ell(f_i-\tilde f_i)$ and that we take the one with smaller cost.
 \item[(2)] By property~(2) on $i-1$ and by construction of $\tilde f_i$, all values $f_i(u,v)-\tilde f_i(u,v)$ are multiples of $2^i$. If $(f_i(u,v)-\tilde f_i(u,v))\bmod2^{i+1}=2^i$, then arc $(u,v)$ is added to $H$, and $h_i(u,v)=\pm2^i$, so $f_{i+1}(u,v)\bmod2^{i+1}=0$. If $(f_i(u,v)-\tilde f_i(u,v))\bmod2^{i+1}=0$, then $(u,v)$ is not added to $H$, so $h_i(u,v)=0$ and $f_{i+1}(u,v)\bmod2^{i+1}=0$.
 \item[(3)] Let $\tilde b_i$ be the demand vector for $\tilde f_i$; we first show that $b_i-\tilde b_i\ge0$. By property~(2) and property~(3) on $i-1$, we have that $b_i(v)$ is a nonnegative multiple of $2^i$. Consider now flow $\tilde f_i$ that satisfies demand vector $\tilde b_i$. The only way for $\tilde b_i(v)>0$ is if the parent arc $(u,v)$ is in $B_i$ and no child arc is in $B_i$, in which case $\tilde b_i(v)=2^i$. By construction of $B_i$, this can only happen if $v\in O_i$, which gives $b_i(v)-\tilde b_i(v)\ge2^i-2^i\ge0$. For all other $v\ne s$, we have $b_i(v)-\tilde b_i(v)\ge b_i(v)\ge0$. It follows that $b_i-\tilde b_i\ge0$.

We next consider the addition of $h_i$. Since we orient arcs in $H$ so that each vertex has the same number of in-edges and out-edges, adding or subtracting $h_i$ to $f_i-\tilde f_i$ does not change the demand vector. This finishes property~(3), and this last observation also proves property~(1).
 \end{enumerate}
This concludes all the properties, and hence the proof.
\end{proof}


\begin{lemma}
$\sum_{v\ne s}b(v)\tilde d(v)\le \ell(f)$.
\end{lemma}
\begin{proof}
By \Cref{lem:structure}, we can apply induction on $i$ to obtain the following two properties:
 \begin{enumerate}
 \item[i.] $\sum_i\ell(\tilde f_i)\le \ell(f)$, which follows from property~(8), and
 \item[ii.] For all $i$, flow $\sum_{j\ge i}\tilde f_j$ satisfies demand vector $b_i$, which follows from property~(1) and the fact that each $f_j$ satisfies demand $b_j$.
 \end{enumerate}

Imagine performing the following single-commodity flow experiment. Begin with $-\infty$ commodity units on node $s$, and we tag each (integral) commodity unit with a value representing its ``distance traveled'' throughout the flows. In decreasing order of $i$, we execute flow $\tilde f_i$ by shifting commodity around (in integral amounts) according to the flow, and for each commodity unit shifted, we increase its ``distance traveled'' value by the distance shifted. Note that the total increase in value over all commodity units increases by exactly $\ell(\tilde f_i)$. Also, note that we are never deficient in commodity anywhere (outside of $s$), since our distribution of flow after iteration $i$ is exactly $\sum_{j\ge i}\tilde f_i$, which satisfies demand vector $b_j$ by property~(ii), and is therefore nonnegative at all $v\ne s$ by property~(3). Once we execute all flows $\tilde f_i$, each vertex $v\ne s$ has exactly $b(v)$ demand by property~(ii), and the total value of all commodity units is $\sum_i\ell(\tilde f_i)$, which is at most $\ell(f)$ by property~(i). 

It remains to show that the total ``distance traveled'' value of all commodity units is at least $\sum_{v\ne s}b(v)\tilde d(v)$. To do so, we claim that after executing any flow $\tilde f_i$, all units of flow at any $v\ne s$ have their value at least the current $\tilde d(v)$, which in turn is at least the final $\tilde d(v)$. This implies the lemma, since each $v\ne s$ ends up with exactly $b(v)$ units of flow after all flows $\tilde f_i$ are executed.

We now prove the claim by induction on decreasing $i$. Suppose that, right before executing flow $\tilde f_i$, a commodity unit at vertex $u$ had value $d_{\text{old}}$, and suppose that $\tilde d(u)=d_{\text{old}}$ at that time. If the unit travels to vertex $v$ in flow $\tilde f_i$, then its new value is $d_{\text{old}}+d_{A_i}(u,v)$, which is at least the new $\tilde d(v)\le d_{\text{old}}+d_{A_i}(u,v)$ by the way the algorithm updates $\tilde d(v)$.
\end{proof}




\begin{lemma}
For each $v\in V$, we have $d_T(s,v)\le\tilde d(v)$.
\end{lemma}
\begin{proof}
We induct on the distance $d_T(s,v)$ in increasing order. Given a vertex $v$, consider its parent $u$ in the tree $T$ (rooted at $s$), which satisfies $d_T(s,u)<d_T(s,v)$. At the time of updating $p(v)$ to $u$, we had $\tilde d(v)$ in some arborescence $A$ with root $r$, we had $\tilde d(v)=\tilde d(r)+d_A(r,v)=\tilde d(r)+d_A(r,u)+\ell(u,v)\ge \tilde d(u)+\ell(u,v)$ for the values of $\tilde d(u),\tilde d(v)$ at that time. The value $\tilde d(u)$ can only decrease over time, and on the other hand, the value $\tilde d(v)$ does not change since we assumed its final value. Therefore, $\tilde d(v)\ge\tilde d(u)+\ell(u,v)$ at the end. By induction, $d_T(s,u)\le\tilde d(u)$, and we obtain $\tilde d(v)\ge\tilde d(u)+\ell(u,v)\ge d_T(s,u)+\ell(u,v)=d_T(s,v)$, completing the induction.
\end{proof}



\begin{lemma}\label{lem:arbor}
Consider a flow $f$ on a network graph $G$ satisfying demands $b$ where $b(v)\ge0$ for all $v\ne s$ (for some source node $s$). Let $H$ be the directed graph with arcs $(u,v)$ whenever $f(u,v)>0$. Then, we can compute an arborescence of $H$ rooted at $s$ spanning all nodes $v$ with $b(v)>0$ in $O(\log n)$ \aggregate rounds.
\end{lemma}
\begin{proof}
The algorithm resembles Edmonds' arborescence algorithm, except adapted to span a subset of vertices. On each iteration, each vertex $v\ne s$ chooses an incoming neighbor $u_v$ if it exists. The algorithm contracts all connected components of the (undirected) graph consisting of all such edges $(u_v,v)$, and deletes any node $v$ without an incoming neighbor. The contracted component containing $s$ is named the new node $s$. The algorithm stops when there is a single node $s$. To construct the arborescence, the algorithm reverses the contractions in reverse chronological order, maintaining an arborescence of the current graph at each step. On each step, all contracted components are un-contracted. Edges in the arborescence of the contracted graph remain as edges in the arborescence of the un-contracted graph. This concludes the description of the algorithm, which clearly runs in $O(\log n)$ \aggregate rounds.

We will show that $(*)$ each contracted component that contains $s$ is always an arborescence, while each contracted component not containing $s$ is always a directed cycle. For the contracted component containing $s$, we add the edges of its arborescence to the new arborescence.  For each contracted component that is a directed cycle, we add all but one edge into the new arborescence. Aside from the proof of $(*)$, we can apply the standard analysis of Edmonds' algorithm to show that the algorithm constructs an arborescence rooted at $s$. We also need to show that all nodes $v\in V$ with $b(v)>0$ are spanned by the arborescence, which we show after $(*)$.

We now prove the statement $(*)$. The proof that the contracted component containing $s$ is an arborescence is also standard, and relies on the fact that we do not select an incoming neighbor into $s$. On the other hand, the proof that every other contracted component is a directed cycle is non-standard and relies on the specific construction of the graph $H$. Suppose for contradiction that such a component $C$ is not a directed cycle; then, there must be node $u$ in $C$ with no incoming neighbor but at least one outgoing neighbor. Let $S\subseteq V$ be the set of original vertices that eventually get contracted to $u$. Then, $S$ has no incoming neighbor in $H$ and at least one outgoing neighbor. By construction of $H$, this means that the flow $f$ flows out of $S$ on at least one arc, but never into $S$, so the net flow out of $S$ is positive. Since the flow satisfies demands $b$, it follows that $\sum_{v\in S}b(v)<0$. This contradicts the fact that $b(v)\ge0$ for all $v\in S$, since $S$ does not contain $s$.

Finally, we show that each node $v\in V$ with $b(v)>0$ is spanned by the arborescence. Suppose not; then, in some contracted graph, the node that $v$ got contracted to must have no incoming neighbors (after which that node is deleted). For this to happen, the set $S\subseteq V$ of original vertices that got contracted to that node must satisfy $\sum_{v\in S}b(v)\le0$. On the other hand, $b(v)>0$ and $b(u)\ge0$ for all $u\in S$ since $s\notin S$, a contradiction.
\end{proof}



% Local Variables:
% TeX-master: "main"
% End:


==> sparse_cover.tex <==
%\section{Sparse Covers from Approximate Shortest Paths}

\section{Sparse Neighborhood Cover from Approximate Shortest Paths}
\label{sec:sparse-cover}

This section is dedicated to prove \cref{thm:sparse_cover}. Informally speaking, it states that we can construct a sparse neighborhood cover of covering radius $D/\poly\log(n)$ with $\poly(\log n)$ invocations to distance oracles $\oDist_{\eps,D'}$ for $\eps = 1/\poly\log(n)$ and  various $D' \leq D$. \\
The proof consists of three parts.
First, in \cref{sec:weak_clustering} we show how to compute a $D$-separated $\tilde{O}(D)$-weak-radius clustering (see below for the definition) that clusters a large fraction of the vertices (\cref{lem:weak_diam}). 
Second, in \cref{sec:strong_radius} we show how to compute a $D/\poly(\log n)$-separated $\tilde{O}(D)$-strong-radius clustering with $O(\log n)$ black-box invocations to the weak-radius clustering algorithm (\cref{lem:strongdiam}). 
Finally, we show how to compute a sparse neighborhood cover with covering radius $D / \poly(\log n)$ with $O(\log n)$ invocations of the strong-radius clustering algorithm (\cref{thm:sparse_cover}).

The weak- and strong- radius clustering algorithms are mostly straightforward generalizations of the $\congest$ algorithms from \cite{rozhon_ghaffari2019decomposition,chang_ghaffari2021strong_diameter} to a weighted setting with access to approximate distances. 

The only added difficulty is that due to the fact that we deal with approximate, and not exact, distances, some invariants from the original algorithms are now slowly deteriorating during the algorithm, and hence the analysis requires some more care.  

\paragraph{Definitions}

In this appendix, we slightly change and extend definitions of clusters and clusterings. 
Whenever we talk about a cluster (besides the statement of \cref{thm:sparse_cover} that uses the language of the rest of the paper), it is, formally, not just a set of nodes $C \subseteq V(G)$, but a pair $(C, T_C)$, where $C \subseteq V(G)$ and $T_C$ is a rooted tree. 
We have $C \subseteq V(T_C)$ and we think of $T_C$ as the \emph{Steiner tree} collecting the nodes of $C$. 
The \emph{radius} $R$ of a cluster $(C, T_C)$ is the radius of $T_C$. 
If $V(T_C) = C$, we talk about a \emph{strong-radius} cluster, otherwise we talk about a \emph{weak-radius} cluster. 
Sometimes, we still informally talk about ``a cluster $C$'' when the tree $T_C$ is clear from context.

Recall that a clustering $\fC = (C_j, T_{C_j})_{j \in J}$ is a collection of disjoint clusters. We say that $\fC$ is $D$-separated if for every $(C_i, T_{C_i}), (C_j, T_{C_j}) \in \fC, i \not= j,$ we have $\dist_G(C_i, C_j) \ge D$. 
 
 

\subsection{Weak-Radius Clustering}
\label{sec:weak_clustering}

\begin{lemma}[Deterministic Weak-Radius Clustering]
\label{lem:weak_diam}
Let $G$ be a weighted graph, $\Vrem \subseteq V(G)$ be a subset of its nodes, $D > 0$ and $\delta > 0$. We assume that each node of $G$ has a unique identifier from $[2^b]$ for $b=O(\log n)$. We define $\eps := \frac{1}{100b\log(n)}$. 

We can compute a $(1-\eps)^b D$-separated $O(D \log^3(n) \cdot 1/\delta)$-weak-radius clustering $\fC = (C_j, T_{C_j})_{j \in J}$ such that 
\begin{enumerate}
    \item $V(\fC) \subseteq \Vrem$,
    \item $ | \Vrem \setminus V(\fC) | \le \delta \cdot | \Vrem |$.
    \item We can implement any \aggregate operation on $\{C_j\}_{j \in J}$ or on $\{T_{C_j}\}_{j \in J}$ in $\poly\log(n)$ \aggregate rounds in $G$. 
    \item  Consider any $W \subseteq \Vrem$ and $(C,T_C) \in \fC$. 
    If $\dist_G(W, \Vrem \setminus W) > (1+\eps) D$, then we have the following. 
    Whenever we have $C \cap W \not = \emptyset$, then $C \subseteq W$ and for every $u \in V(T_C)$ we have $\dist_G(u, W) \le (1+\eps)D/2$. 
\end{enumerate}

The computation consists of $\poly\log(n)$ \aggregate rounds in $G$ and $\poly(\log n)$ calls to distance oracles $\oDist_{\eps, D}$ for various $D' \in [D/2, D]$.
\end{lemma}

The lemma is proven by a routine adaptation of the algorithm from \cite{rozhon_ghaffari2019decomposition}. 


\begin{proof}
The algorithm consists of $b$ phases and each phase consists of $O(\frac{1}{\delta} \cdot b \cdot \log( n )) = O(\log^2 (n) / \delta)$ steps. 
At the beginning, all nodes in $\Vrem$ are alive, that is, $\Valive = \Vrem$, but some nodes in $\Vrem$ stop being alive during the algorithm and then we call them dead. 
Throughout the course of the algorithm we maintain a partition of alive nodes into clusters. %We denote a cluster with the letter $C$. 
The Steiner tree $T_C$ of any such cluster $C$ can also contain any nodes from $V(G)$. 
At the very beginning, each node $u$ is a trivial cluster $(\{u\}, T_{\{u\}})$. 

Each cluster is assigned a unique identifier. In the beginning, the identifier of $\{u\}$ is simply defined as the identifier of $u$ and $C$ keeps that identifier, although during the algorithm $C$ can lose some nodes, including $u$. On the other hand, $T_C$ never loses nodes. 
We will maintain as an invariant that the radius of each $T_C$ grows only by $O(D)$ in each of the $\poly\log(n)$ many steps, and that we can implement \aggregate operations on each cluster $C$ in $\poly\log(n)$ \aggregate rounds, even though clusters may become disconnected. 

\paragraph{One Phase}
We now discuss the algorithm in greater detail. 
At the beginning of phase $i$, we mark all clusters such that the $i$-th bit in their identifier is $0$ as active and the rest of the clusters are marked as passive.

We now describe one step of the algorithm, in which active clusters potentially grow. Each active cluster is in one of two states. Either it is \emph{growing} or \emph{finished}. At the beginning of the phase, every active cluster is growing. 
Let $\Vactive \subseteq \Valive$ be the set of all nodes in active clusters. 

In each step of the $i$-th phase, we define $S$ as the set consisting of all the nodes in growing clusters and use the oracle $\oDist_{\eps,D\cdot (1-\eps)^i}$ with input $S$.
Note that we are allowed to use the oracle as $D \cdot (1-\eps)^b \ge D / 2$.  
The oracle outputs a forest $F$ with $S$ being the set of roots.
%Note that the root of each tree $T \subseteq \tilde{F}$ is in $S$. However, there can be a non-root node $s \in S \cap T$. For each such potential node $s$ we delete the edge from $s$ to its parent in $\tilde{F}$ from $\tilde{F}$ and make it a new root. This defines a new forest $F$ that has the property that it contains all nodes of $S$ as root nodes. Moreover, $F$ is clearly still retains the same distance guarantees as $\tilde{F}$. 



\paragraph{Growth of a cluster}
For each growing cluster $C$ consider all trees in $F$ such that their root is in $C$. We denote this forest as $F_C$ and think about is as a Steiner tree that collects all nodes ``proposing to join'' the cluster $C$ and which enables us to aggregate information about the proposing nodes. 
Every cluster $C$ computes $|F_C \cap (\Vrem \setminus \Vactive)|$. 
If $|F_C \cap (\Vrem \setminus \Vactive)| \ge \frac{\delta}{b} |C|$, the cluster $C$ grows. 
That is, all nodes in $F_C \cap (\Vrem \setminus \Vactive)$ join $C$.  These nodes leave their respective passive clusters.  This means that 
\begin{align*}
C_{new} := C \cup (F_C \cap (\Vrem \setminus \Vactive)).
\end{align*}

We now discuss how the Steiner tree $T_C$ is extended. 
Let $F'_C$ denote the rooted forest one obtains from $F_C$ by deleting all the nodes in $F_C$ whose subtree does not contain nodes of $C_{new}$. 
That is, $F'_C$ is a ``pruned'' version of the Steiner tree $F_C$ that does not contain nodes from $\Vrem$ that are not needed for aggregation. 

The vertex set of the new Steiner tree $T_{C_{new}}$ is $V(T_{C_{new}}) = V(T_C) \cup F'_C$. The edge set is $E(T_{C_{new}}) = E(T_C) \cup \{(u,v) \in E(F'_C) | u \not\in T_C \}$, where we use that each edge $e \in E(F'_C)$ knows its orientation from $u$ to $v$ in the direction of the root. That is, when combining the edge sets of the tree $T_C$ and the forest $F'_C$, we drop each edge of $F'_C$ that would result in some node having two parents. 

Otherwise, when $C$ decides not to grow, all nodes in $F_C \cap (\Vrem \setminus \Vactive)$ are removed from $\Valive$. 
In that case, $C$ finishes and stops growing in the current phase. 

This finishes the description of the algorithm, up to implementation details considered later. 

\begin{claim}
The total number of deleted nodes is at most $\delta \cdot   |\Vrem|$. 
\end{claim}
\begin{proof}
  We prove that in each phase we delete at most $\delta |\Vrem|/b$ nodes. The claim then follows. 
  Consider one phase of the algorithm. Let $C$ be some cluster and $n_C$ the total number of nodes contained in $C$ at the end of the phase. 
The cluster $C$ is responsible for deleting nodes of total weight at most $\delta n_C / b$. Hence, the total number of deleted nodes is upper bounded by $\sum_{C \text{ active in phase }i} \delta n_C /b \le \delta |\Vrem|/b$, as needed.  
\end{proof}

\begin{claim}
\label{cl:stop_growing}
In each phase, each cluster stops growing after $O(\log n \cdot b/\delta)$ steps. 
\end{claim}
\begin{proof}
For the sake of contradiction, assume there exists a cluster $C$ that was growing for all $t = O(\log  n  \cdot b/\delta)$ steps of a given phase. Then, $|C| \ge (1 + \delta/b)^t >  n  $, a contradiction. 
\end{proof}

\begin{claim}
After the algorithm terminates, for any two clusters $C_1 \neq C_2$ we have $\dist_G(C_1, C_2) \ge (1-\eps)^b D$. 
\end{claim}
\begin{proof}
%Let $\Vrem = V_{00\dots0} \sqcup V_{00\dots1} \sqcup \dots \sqcup V_{11\dots1}$ be the following split: each node $u \in V_b$, where $b$ is a bit string of length $i-1$, if it is in a cluster such that its first $i-1$ bits are $b$. 
We prove the following invariant by induction: After the $i$-th phase, if two clusters do not agree on their first $i$ bits, then their distance in $G$ is at least $(1-\eps)^i D$. The claim then follow by setting $i = b$. 
Suppose the invariant holds after the $(i-1)$-th phase (case $i=0$ is an easy special case). We show that this implies that the invariant also holds after the $i$-th phase. 



To do so, we first show the following property. After each step during the $i$-th phase, if two clusters do not agree on their first $i-1$ bits, then their distance in $G$ is at least $(1-\eps)^{i-1}D$.



Note that our induction hypothesis states that the property above holds at the beginning of the $i$-th phase. Hence, it remains to show that each step $j$ during phase $i$ preserves the property.

For this, it suffices to show that a node can only switch from one cluster to another cluster during the $j$-th step if the two clusters agree on their first $i-1$ bits.

To that end, consider some node $v$ and two clusters $C_1$ and $C_2$ before the $j$-th step. Assume that $v$ is contained in cluster $C_1$ before the $j$-th step and during the $j$-th step $v$ decides to join the cluster $C_2$.
It directly follows from the algorithm description that this can only happen if $\dist_G(C_2,v) \leq (1+\eps)(1-\eps)^i D < (1-\eps)^{i-1}D$.
In particular, $\dist_G(C_1,C_2) < (1-\eps)^{i-1}D$ and therefore the two clusters $C_1$ and $C_2$ agree on their first $i-1$ bits, as desired.

 

It remains to consider two clusters that agree on their first $i-1$ bits but disagree on their $i$-th bit.
Exactly one of those clusters, say $C$, is active during the $i$-th phase and by \cref{cl:stop_growing} we know that $C$ decides to stop growing at some point during the phase, by deleting all the nodes that proposed to join it in that step.
In particular, each alive node outside $C$ with a distance of at most $(1- \eps)^i D$ to $C$ either gets killed or decides to join an active cluster different from $C$. Since nodes in active clusters remain in the same active cluster until the end of the $i$-th phase, the distance of $C$ to any other cluster with a different $i$-th bit is at least $(1-\eps)^iD$ at the end of the $i$-th phase. 
This finishes the proof of the induction statement.


\end{proof}


\begin{claim}
For any cluster $C$, the radius of $T_C$ is $O(D \log^3(n)/\delta)$. 
\end{claim}
\begin{proof}
The radius of $T_C$ grows by $O((1+\eps)D)$ in each step. 
Each of the $b$ phases consists of $O(b /\delta \cdot \log n)$ steps. Hence, the radius of $T_C$ can be bounded by $O(b^2\log( n )D/\delta) = O(D \log^3(n) / \delta)$. 
\end{proof}

\begin{claim}
Consider any $W \subseteq \Vrem$ and $(C,T_C) \in \fC$. 
    If $\dist_G(W, \Vrem \setminus W) > (1+\eps) D$, then we have the following. 
    Whenever we have $C \cap W \not = \emptyset$, then $C \subseteq W$ and for any $u \in T_C$ we have $\dist_G(u, W) \le (1+\eps)D/2$. 
\end{claim}
\begin{proof}
Let $W \subseteq \Vrem$ be any set such that $\dist_G(W, \Vrem \setminus W) > (1+\eps) D$. A simple induction argument shows that any cluster $C$ that started as a node $u \in W$ will satisfy $C \subseteq W$ during the course of the algorithm and an analogous statement holds if we replace $W$ by $\Vrem \setminus W$. To show the second part, let $C' \subseteq W$ be some arbitrary cluster during the course of the algorithm. It suffices to show that for any node $u \in V(F'_{C'})$ in the pruned Steiner Tree it holds that $\dist_G(u,W) \leq (1+\eps)D/2$. As $u \in V(F'_{C'})$, there exists some node $v \in \Vrem$ that is contained in the subtree of $u$ in $F_{C'}$. Each node in $F_{C'}$ has a distance of at most $(1+\eps)D$ to its root.
As the root is contained in $W$, we have $\dist_G(W,v) \leq (1+\eps)D$. In particular, $v \notin \Vrem \setminus W$ but $v \in \Vrem$ and therefore $v \in W$.
Now, let $r$ be the root of $u$ in $F_{C'}$. As $v$ is an ancestor of $u$ in $F_{C'}$, we have

\begin{align*}
    \dist_{F_{C'}}(r,v)  = \dist_{F_{C'}}(r,u) + \dist_{F_{C'}}(u,v) \leq (1+\eps)D.
\end{align*}

In particular,

\begin{align*}
    \dist_G(u,W) \leq \dist_{F_{C'}}(u,\{r,v\}) \leq (1+\eps)D/2,
\end{align*}


as desired.
\end{proof}

\begin{claim}
\label{cl:weak_diam_aggregation}
During the construction, we can implement any \aggregate operation on clusters in $O(1/\delta \cdot \log^3(n))$ \aggregate rounds. 
\end{claim}
\begin{proof}
We will show how to implement any aggregate operation $\bigoplus$ on the clusters of some partial clustering $\fC$ that we have during the algorithm.  

Assume that each node $u$ is given some value $v_u$ and we wish to compute $\bigoplus_{u \in C} v_u$ for each $C \in \fC$. 
Let $F^1, F^2, \dots, F^k$ be the forests found by calls to $\oDist_{\eps, D'}$ so far and let $F'^1_C, F'^2_C, \dots, F'^k_C$, with $F'^i_C \subseteq F^i$, be the corresponding subforests that we used to grow $C$. 
We will run the following $k$ round algorithm. 
In the $i$-th round, for $0 \le i < k$, each tree $T \subseteq F'^{k-1}_C \subseteq F^{k-i}$ computes consensus of values of all nodes $u \in T \cap C$. 
That is, it computes $\bigoplus_{u \in T\cap C} v_u$. 
This can be done in one \aggregate round for all clusters $C$ in parallel, as each $T \subseteq F'^{k-i}_C$ is connected and the trees are mutually disjoint.  
Then, we remove the values of all nodes in $T \cap C$, except of the root $r$ of $T$ that takes the new value $v_r^{new} = \bigoplus_{u \in T\cap C} v_u$, that is, the result of the calculation. 
A straightforward induction argument shows that after $k$ rounds, the root $r_C$ of each cluster $C$ (that is, the node that defined $C$ at the beginning of the algorithm) knows the value of $\bigoplus_{u \in C} v_u$. 
Once the value of each cluster is computed, it can be broadcasted from $r_C$ back to all nodes in $C$. 
This is done analogously to the computation step, but the forests $F_1, F_2, \dots, F_k$ are now iterated over in the ascending order. 
\end{proof}

\begin{claim}
The algorithm can be implemented in $O(1/\delta^2 \cdot \log^6 n)$ \aggregate rounds and needs $O(1/\delta \cdot \log^3(n))$ calls to the oracle $\oDist_{\eps, D'}$ for $D' \in [D/2, D]$. 
\end{claim}
\begin{proof}
The algorithm has $O(\log n)$ phases and each consists of $O(1/\delta \cdot \log^2 n) $ steps. Let us now discuss the complexity of each step. 
In each step, the decision of each cluster to grow or not can be implemented with one call of the distance oracle $\oDist_{\eps, D'}$ and $O(1/\delta \cdot \log^3(n))$ \aggregate rounds, since the decision of each cluster to grow or not amounts to an aggregation on it and on $F_C$. 
After the decision of each cluster, we need to do additional bookkeeping. The only nontrivial part of it is pruning each forest $F_C$ into $F'_C$. To prune $F_C$, each node in it needs to know whether there are $\Vrem$ nodes in the subtree of it. This is a special case of the subtree sum problem that can be solved in $\poly\log(n)$ \aggregate rounds \cref{lemma:ancestor-subtree-sum}. 
Hence, the complexity of the algorithm is $1/\delta^2 \poly\log(n)$. 
The total number of invocations of $\oDist_{\eps, D'}$ is bounded by $O(1/\delta \cdot \log^3(n))$. 
\end{proof}

\end{proof}


\subsection{Strong-Radius Clustering}
\label{sec:strong_radius}

\begin{lemma}[Deterministic Strong-Radius Clustering]
\label{lem:strongdiam}
Let $G$ be a weighted graph, $\Vrem \subseteq V(G)$ and $D > 0$. We assume that each node of $G$ has a unique identifier from $[2^b]$ for $b=O(\log n)$ and set $\eps = \frac{1}{100b\log(n)}$. 

We can compute an $\eps D$-separated $O(D \log^4(n))$-strong-radius clustering $\fC_{out}$ such that $V(\fC_{out}) \subseteq \Vrem$ and $|V(\fC_{out})| \ge |\Vrem|/3$.

The computation consists of $\poly(\log n)$ \aggregate rounds in $G$ and $\poly(\log n)$ calls to distance oracles $\oDist_{\eps, D'}$ for various $D' \in [D , 10 D]$. 
\end{lemma}

The lemma is proven by an adaptation of the algorithm from \cite{chang_ghaffari2021strong_diameter}. 


\begin{proof}

  We compute the strong-radius clustering by the following algorithm. The algorithm has $k = O(\log n)$ phases and in the $i$-th phase we invoke the weak-radius clustering from \cref{lem:weak_diam} with parameters $\Vrem^i, D^i$ and $\delta^i = \delta = 1/(3k)$ to obtain an output clustering $\fC^i$.
  In each phase, we add new strong-radius clusters to an initially empty set $\fC_{out}$. 
    
    At the beginning, we set $\Vrem^1 = \Vrem$ and define $\fC^0 = \{ \Vrem \}$. 
    In the $i$-th phase of the algorithm we do the following. 
  \begin{enumerate}
      \item We invoke \cref{lem:weak_diam} with parameters $\Vrem^i, D^i = 10D \cdot (1-\eps)^{2ib}$ and $\delta^i$. The output is a $(1-\eps)^bD^i$-separated weak-radius clustering $\fC^i$. % with weak-radius $O(D^i \log^3 n \cdot 1/\delta) = O(D \cdot \log^4 n)$. %Moreover, each cluster $C \in \fC$ is accompanied with a strong-radius cluster $\overline{C} \supseteq C$ of radius $O(D \cdot \log^4 n)$. We have  $|\Vrem^i \setminus \bigcup_{C \in \fC^i} C| \le \delta |\Vrem^i| = |\Vrem^i|/(3k)$.
      \item For each cluster $C \in \fC^i$, there exists a (unique) cluster $\parent(C) \in \fC^{i-1}$ with $C \subseteq \parent(C)$ (\cref{cl:strong_laminar}). 
      If $|C| > |\parent(C))|/2$, then we add $(V(T_{C}), T_{C})$ to $\fC_{out}$. 
      \item 
      Let $C^i_1, C^i_2, \dots, C^i_\ell$ denote the clusters added to $\fC^{out}$ during the $i$-th phase. \\
      We set $\Vrem^{i+1} = \left( \bigcup_{C \in \fC^i} C \right)  \setminus (\bigcup_{j=1}^{\ell} \parent(C^i_j))$. 
      
     \end{enumerate} 
     At the very end we output the output set $\fC_{out}$. This finishes the description of the algorithm. 
     
     
     
     
  
\begin{claim}
\label{cl:strong_laminar}
For each cluster $C \in \fC^i$, there exists a (unique) cluster $\parent(C) \in \fC^{i-1}$ with $C \subseteq \parent(C)$ (\cref{cl:strong_laminar}). 
\end{claim}  
\begin{proof}
Consider an arbitrary cluster $C \in \fC^i$ and let $\parent(C)$ be any cluster in $\fC^{i-1}$ with $C \cap \parent(C) \neq \emptyset$. It suffices to show that $C \subseteq \parent(C)$.
Let $W = \parent(C)$. 
Note that $W \subseteq \Vrem^i$, since for each cluster $C' \in \fC^{i-1}$ either all nodes of $C'$ are in $\Vrem^i$ or no nodes are in $\Vrem^i$. 
Next, we have $\dist_G(W, \Vrem^i \setminus W) \ge (1-\eps)^b D^{i-1} > (1+\eps)D^i$, as the distance between any two clusters in $\fC^{i-1}$ is at least $(1-\eps)^bD^{i-1}$ and $D^i / D^{i-1} = (1-\eps)^{2b}$. 
Hence, the fourth property of \cref{lem:weak_diam} gives $C \subseteq \parent(C)$, as desired.
\end{proof}
  
\begin{claim}
\label{cl:strong_finish}
$\Vrem^k = \emptyset$. 
\end{claim}  
\begin{proof}
Let $C^0, C^1,\ldots, C^i$ be clusters such that $C^i \in \fC^i$ and $\parent(C^{j}) = C^{j -1}$ for $1 \le j \le i$. We have $|C^0| \leq n$ and $|C^{j}| \leq |C^{j -1 }|/2$. Hence, $|C^i| \leq n/2^{i-1}$.
Let $k = 3 + \lceil \log_2 n \rceil$. Then, $\fC^{k-1}$ cannot contain any clusters and therefore $\Vrem^k = \emptyset$. 
\end{proof}

\begin{claim}
\label{cl:strong_deleted}
$|V(\fC_{out})| \ge |\Vrem| / 3$. 
\end{claim}  
\begin{proof}
    \cref{cl:strong_finish} together with the algorithm description implies that for every node $u \in \Vrem$ at least one of the following holds.

    \begin{enumerate}
        \item $u \in  V(\fC_{out})$
        \item $u \in C$ and $C$ has a sibling $C'$ ($\parent(C) = \parent(C')$, $C \neq C'$) with $V(T_{C'}) \in \fC_{out}$ 
        \item $u \in \Vrem^i$ but the algorithm of \cref{lem:weak_diam} invoked in the $i$-th phase left $u$ unclustered 
    \end{enumerate}    
    
    There are at most $k \cdot \delta |\Vrem| = (1/3)|\Vrem|$ nodes that satisfy the third condition. 
    Moreover, as every cluster $C$ with $V(T_C) \in \fC^{out}$ satisfies $|C| \geq |\parent(C)|/2$, the total number of nodes that satisfy the first condition is at least as large as the total number of nodes that satisfy the second condition. Hence, $ |V(\fC_{out})| \geq (1/2)(2/3)|\Vrem|$, as desired.
\end{proof}

  
\begin{claim}
\label{cl:strong_padded}
For any two distinct clusters $C^{out}_1,C^{out}_2 \in \fC_{out}$, we have $\dist_G(C^{out}_1, C^{out}_2) \ge \eps D$. 
\end{claim}  
\begin{proof}
As $C^{out}_1,C^{out}_2 \in \fC_{out}$, there exists $i_1, i_2 \in [k]$ and two clusters $(C_1,T_{C_1}) \in \fC^{i_1}$ and $(C_2,T_{C_2}) \in \fC^{i_2}$ such that $C^{out}_1 = V(T_{C_1})$ and $C^{out}_2 = V(T_{C_2})$.
Without loss of generality $i_1 \le i_2$. 
We first compute a lower bound on the distance between $C_1 $ and $C_2$. 
Let $\hat{C}_1, \hat{C}_2 \in \fC^{i_1 - 1}$ such that $C_\ell \subseteq \hat{C}_\ell$ for $\ell \in [2]$. In particular, $\hat{C}_1 = \parent(C_1)$. 
We have $\hat{C}_1 \neq \hat{C}_2$. If $i_1 = i_2$, then $\hat{C}_1 \neq \hat{C}_2$ follows from the fact that $|C_\ell| > (1/2)| \hat{C}_\ell|$ for $\ell \in [2]$. If $i_1 < i_2$, then $\hat{C}_1 \neq \hat{C}_2$ follows from the fact that $\Vrem^{i_1 + 1} \cap \hat{C}_1 = \emptyset$ and $\Vrem^{i_2} \subseteq \Vrem^{i_1 + 1}$.
Hence,  

\begin{align*}
\dist_G(C_1,C_2)\geq \dist_G(\hat{C}_1, \hat{C}_2) \ge (1-\eps)^b D^{i_1 - 1}.    
\end{align*}


Moreover, with $W = \hat{C}_1$ we have $\dist_G(W,\Vrem^{i_1} \setminus W) \geq (1-\eps)^b D^{i_1 - 1} \geq (1+\eps)D^{i_1}$. This implies, as $C_1 \cap W \neq \emptyset$, that $\dist_G(u,W) \le (1+\eps)D^{i_1}/2$ for every $u \in V(T_{C_1}) = C^{out}_1$.
and, similarly, $\dist(T_{C^{i_2}}, \hat{C}^2) \le (1+\eps)D^{i_2}/2 \le (1+\eps)D^{i_1}/2$.
A similar argument shows that $\dist_G(u, \hat{C}_2) \leq (1+\eps)D^{i_2}/2$ for every $u \in V(T_{C_2})= C^{out}_2$.

Now, consider an arbitrary $v_1 \in C^{out}_1$ and $v_2 \in C^{out}_2$. We have 
\begin{align*}
\dist_G(v_1,v_2) &\geq 
\dist_G(\hat{C}_1, \hat{C}_2) - \dist_G(\hat{C}_1,v_1) - \dist_G(\hat{C}_2, v_2) \\
&\ge (1-\eps)^b D^{i_1 - 1} - 2(1+\eps)D^{i_1}/2\\
&= \left( (1-\eps)^b / (1-\eps)^{2b} - (1+\eps)\right) D^{i_1}
\ge 2\eps D^k \ge \eps D, 
\end{align*}
as needed. 
\end{proof}


To conclude the proof, note that each cluster $C \in \fC_{out}$ has strong-radius $O(D \log^3(n) \cdot 1/\delta) = O(D \log^4(n))$, clearly $V(\fC_{out}) \subseteq \Vrem$, the clustering is $\eps D$-separated by \cref{cl:strong_padded} and $|V(\fC_{out})| \ge |\Vrem|/3$ by \cref{cl:strong_deleted}. In each phase we call \cref{lem:weak_diam} once. In addition, each cluster needs to check whether it gets added to the output clustering by comparing its size to the size of its parent. If a cluster indeed gets added, it also needs to inform all the nodes in the parent cluster. This can be implemented in $O(1)$ aggregations on clusters that \cref{lem:weak_diam} outputted during the course of the algorithm. Hence, by the aggregation property in \cref{lem:weak_diam} the algorithm can be implemented in $\poly\log(n)$ \aggregate rounds and $\poly\log(n)$ calls to distance oracles $\oDist_{\eps, D'}$ for various $D' \in [D, 10D]$, as desired. 
\end{proof}

\subsection{Sparse Neighborhood Cover}
\label{sec:sparse_cover}

\begin{theorem}
\label{thm:sparse_cover}
Let $G$ be a weighted graph and $D \geq 0$.
Assume we have access to oracle $\oDist_{\eps,D'}$ for various $D' \in [\frac{D}{\log^7 n},D]$ and $\eps = \frac{1}{\log^3 n}$.
We can compute a sparse neighborhood cover with covering radius $\frac{D}{\log^7 n}$ such that each cluster $C$ in one of the clusterings comes with a rooted tree  $T_C$ of diameter at most $D$. The algorithm runs in $\poly(\log n)$ \aggregate rounds.
\end{theorem}
%\sparseCover*

\begin{proof}

Let $\Delta = \Theta(D / \log^4 n)$. 
Our algorithm consists of $t = 100 \lceil \log(n) \rceil$ rounds. Let $\Vrem^1 := V(G)$.
In the $i$-th round, we use the algorithm of \cref{lem:strongdiam} with $\Vrem^\Lref{lem:strongdiam} = \Vrem^i$ and ${D}^\Lref{lem:strongdiam} = \Delta$ to compute a $s = \Omega(\Delta/\log^2 n) = \Omega(D / \log^6 n)$-separated $\Theta(D)$-strong-radius clustering $\fC^i$ with $V(\fC^i) \subseteq \Vrem^i$ and $|V(\fC^i)| \geq |\Vrem^i|/3$. Moreover, we can choose the constant in the definition of $\Delta$ such that $\fC_i$ is $D/4$-strong-radius clustering. 
We then set $\Vrem^{i+1} = \Vrem^i \setminus V(\fC^i)$.

We now extend each cluster $(C,T_C) \in \fC^i$ to some new cluster $(\hat{C},T_{\hat{C}})$. This defines a new clustering $\hat{\fC}^i$. 
To do so, we first invoke the distance oracle $\oDist_{\eps,s/10}$ with input $V(\fC^i)$.
Let $F$ denote the rooted forest returned by the oracle.
For each $(C, T_C) \in \fC^i$, let $F_C \subseteq F$ be the forest which contains all trees in $F$ whose root is contained in $C$. We set $\hat{C} = C \cup V(F_C)$ and  define $T_{\hat{C}}$ as the rooted tree one obtains by adding the trees in $F_C$ to $T_C$, i.e, $V(T_{\hat{C}}) = V(F_C) \cup V(T_C)$ and $T_{\hat{C}}$ and $T_C$ have the same root. 
Clearly, any node in $T_{\hat{C}}$ has a distance of at most $D/4 + (1+\eps)(s/10) = D/2$ to the root. 
Moreover, as the clustering $\fC^i$ is $s$-separated, it follows that $\hat{\fC^i}$ is $\hat{s}$-separated with $\hat{s} := s/10 \leq s - 2(1+\eps)(s/10)$ and for any node $u$ with $\dist_G(u,C) \leq \hat{s}$ we have $u \in \hat{C}$.  
In particular, as $\Vrem^t = \emptyset$, for every node $u \in V(G)$ there exists some $i$ such that the ball of radius $\hat{s}$ around $u$ is fully contained in one of the clusters of $\hat{C}^i$.
Hence, $(\hat{\fC}^i)_{i \in [t]}$ is a sparse neighborhood cover with covering radius $\hat{s} \ge D/\log^7 n$ and each cluster $C$ of it comes with a rooted tree $T_C$ of diameter at most $2 \cdot (D/2) = D$. 

It directly follows from the guarantees of \cref{lem:strongdiam} that the computation consists of $\poly(\log n)$ \aggregate rounds in $G$ and $\poly(\log n)$ calls to distance oracles $\oDist_{\eps, D'}$ for $\eps := \frac{1}{100b \log(n)} \ge 1/\log^3 n$ and various $D' \in [D/\log^7 n, D]$.
\end{proof}






% Local Variables:
% TeX-master: "main"
% End:

